Diagram of Representations of Universal Algebras

Theory of representations of universal algebra is a natural development of the theory of universal algebra. In the book, I considered representation of universal algebra, diagram of representations and examples of representation. Morphism of the representation is the map that conserve the structure of the representation. Exploring of morphisms of the representation leads to the concepts of generating set and basis of representation.

==> Abstract.1908.04418.English.tex <==
%auto-ignore
\begin{abstract}
Theory of representations of universal algebra
is a natural development of the theory of universal algebra.
In the book, I considered representation of universal algebra,
diagram of representations and examples of representation.
Morphism of the representation is the map that conserve
the structure of the representation.
Exploring of morphisms of the representation leads to the concepts 
of generating set and basis of representation.
\end{abstract}


==> Abstract.1908.04418.Russian.tex <==
%auto-ignore
\begin{abstract}
Теория представлений универсальной алгебры
является естественным развитием теории универсальной алгебры.
В книге рассмотрены представление универсальной алгебры,
диаграммы представлений и примеры представления.
Морфизм представления - это отображение, сохраняющее
структуру представления.
Изучение морфизмов представлений ведёт к понятиям
множества образующих и базиса представления.
\end{abstract}


==> Algebra.Representation.Russian.tex <==
%auto-ignore
\input{Algebra.Representation.Eq}

\chapter{Представление универсальной алгебры}
\labelChapter{Representation of Algebra}

\section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\begin{definition}
\labelDefinition{representation of algebra} 
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
$A_1$ или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
\qed
\end{definition}

Диаграмма
\ShowEq{consider representation of Omega algebra}
означает, что мы рассматриваем представление $\Omega_1$\Hyph алгебры $A_1$.
Отображение $f(a)$ является образом
\ShowEq{a in A1}.
Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

Существует несколько способов описать представление.
Мы можем указать отображение $f$, имея в виду что область определения -
это $\Omega_1$\Hyph алгебра $A_1$ и область значений - это $\Omega_1$\Hyph алгебра
\ShowEq{End O2}{A_2}.
Либо мы можем указать $\Omega_1$\Hyph алгебру $A_1$
и $\Omega_2$\Hyph алгебру $A_2$, имея в виду что нам известна структура
отображения $f$.\,\footnote{
Например, мы рассматриваем векторное пространство $V$ над полем $D$
(раздел \RefSection{Vector Space}).
}

\begin{definition}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnote{
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
Смотри также теорему
\RefTheorem{effective representation of multiplicative Omega-group}.
}
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}f{A_1}{A_2}
эффективно тогда и только тогда, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что\,\footnote{
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}f{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a_1\ne e$
существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{fam ne m}
}
}
\ShowEq{faa ne fba}
\end{theorem}
\begin{proof}
Пусть представление $f$ эффективно и
\EqParm{a ne b}{=.}
Если для любого
\ShowEq{a in A}2{}
верно равенство
\ShowEq{faa=fba}
то
\DrawEq[{a_1}{b_1}]{fa=fb}{}
Это противоречит утверждению, что представление $f$ эффективно.

Пусть из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что
\ShowEq{faa ne fba}
Следовательно, из утверждения
\ShowEq{a1 ne b1}
следует, что
\ShowEq{fa ne fb}
Согласно определению
\RefDefinition{effective representation of algebra},
представление $f$ эффективно.
\end{proof}

\ShowDefinition{free representation of algebra}

\begin{theorem}
\labelTheorem{free representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},
если из утверждения
\DrawEq[{a_1}{b_1}]{fa=fb}-
следует, что
\ShowEq{a=b}.
\end{theorem}

\begin{proof}
Утверждение
\DrawEq[{a_1}{b_1}]{fa=fb}-
верно тогда и только тогда, когда
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2.
\end{proof}

\begin{theorem}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{theorem}
\begin{proof}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является свободным представлением.
Пусть
\ShowEq{ab in A1}
Согласно определению
\RefDefinition{free representation of algebra},
из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что
\ShowEq{a=b}.
Следовательно, если
\EqParm{a ne b}{=c}
то существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{faa ne fba}
Согласно теореме
\RefTheorem{representation is effective},
представление $f$ эффективно.
\end{proof}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{definition}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnote{
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}
если для любых
\EqParm{ab in A}{A=2,=z}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\labelTheorem{Representation is single transitive iff}
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{single transitive representation generates algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{b in A2, o in O1}
Для любых $A_2$\Hyph чисел
\ShowEq{b1n}
существуют $A_1$\Hyph числа
\ShowEq{a1n}an{}
такие, что
\ShowEq{b=fa 1n}
Мы определим операцию $\omega$ на множестве $A_2$ равенством
\ShowEq{b1no=a1nob}
Мы также требуем, что выбор $A_2$\Hyph числа $b$ не зависит от операции $\omega$.
\end{proof}

\begin{theorem}
%\labelTheorem{single transitive representation generates algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
эффективное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть
\ShowEq{o in O12}
Тогда
\ShowEq{a1nob=a1nbo}
\end{theorem}

\section{Морфизм представлений универсальной алгебры}

\begin{theorem}
Пусть $A_1$ и $B_1$ - $\Omega_1$\Hyph алгебры.
Представление $\Omega_1$\Hyph алгебры $B_1$
\ShowEq{B1->*A2}
и гомоморфизм $\Omega_1$\Hyph алгебры
\ShowEq{A1->B1}
определяют представление $f$ $\Omega_1$\Hyph алгебры $A_1$
\ShowEq{AB1->*A2}
\end{theorem}
\begin{proof}
Отображение $f$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2},
так как отображение $g$ является гомоморфизмом $\Omega_1$\Hyph алгебры $B_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}.
\end{proof}

Мы будем также пользоваться диаграммой
\ShowEq{A1B1->*A2}
вместо диаграммы
\EqRef{AB1->*A2}.

Если мы изучаем представление $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебрах $A_2$ и $B_2$, то нас интересуют отображения
$A_2\rightarrow B_2$, сохраняющие структуру представления.

\ShowDefinition{morphism of representations of universal algebra}

\begin{remark}
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем кортеж отображений
\ShowEq{map r12}r{}
мы будем также называть отображением
и пользоваться записью
\ShowEq{f:A->B}rfg
Пусть
\ShowEq{a=a12}
- кортеж $A$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{r(a)12}
для образа кортежа $A$\Hyph чисел
при морфизме представлений $r$.
\qed
\end{remark}

\begin{definition}
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Tuple of maps is morphism of representations iff}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{definition}
\end{theorem}
\begin{proof}
Для произвольного $m\in A_2$ равенство
\EqRef{morphism of representations of universal algebra, definition, 2}
имеет вид
\eqRef{morphism of representations of universal algebra, 2m}{definition}.
\end{proof}

\begin{remark}
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B_1$, пользуясь буквой по образцу $b\in B_1$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
\qed
\end{remark}

\begin{remark}
\labelRemark{morphism of representations of universal algebra}
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{definition}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{definition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{definition}.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{morphism of representations and algebra}
Рассмотрим представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ 
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$.
Морфизм
\ShowEq{r12:A->B}rAB
представлений из $f$ в $g$
удовлетворяет соотношению
\ShowEq{morphism of representations of universal algebra, 1}
для произвольной операции
\ShowEq{omega in Omega1(n)}
\end{theorem}
\begin{proof}
Так как $f$ - гомоморфизм, мы имеем
\ShowEq{morphism of representations of universal algebra, 2}
Из \EqRef{morphism of representations of universal algebra, definition, 2} и
\EqRef{morphism of representations of universal algebra, 2} следует
\ShowEq{morphism of representations of universal algebra, 3}
Так как $r_1$ - гомоморфизм, из
\EqRef{morphism of representations of universal algebra, 3} следует
\ShowEq{morphism of representations of universal algebra, 4}
Так как $g$ - гомоморфизм, из
\EqRef{morphism of representations of universal algebra, 4} следует
\EqRef{morphism of representations of universal algebra, 1}.
\end{proof}

\begin{theorem}
\labelTheorem{morphism of representations and homomorphism of algebra}
Пусть отображение
\ShowEq{r12:A->B}rAB
является морфизмом из представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ в представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$.
Если представление $f$ эффективно, то отображение
\ShowEq{*R:*A2->*B2}
определённое равенством
\ShowEq{morphism of representations, star morphism}
является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как представление $f$ эффективно, то для выбранного преобразования
$\BlueText{f(a)}$ выбор элемента $a$ определён однозначно.
Следовательно, преобразование $\RedText{g(r_1(a))}$
в равенстве \EqRef{morphism of representations, star morphism}
определено корректно.

Так как $f$ - гомоморфизм, мы имеем
\ShowEq{morphism of representations, star morphism, 2}
Из \EqRef{morphism of representations, star morphism} и
\EqRef{morphism of representations, star morphism, 2} следует
\ShowEq{morphism of representations, star morphism, 3}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations, star morphism, 3} следует
\ShowEq{morphism of representations, star morphism, 4}
Так как $g$ - гомоморфизм,
\ShowEq{morphism of representations, star morphism, 5}
следует из
\EqRef{morphism of representations, star morphism, 4}.
Следовательно, отображение $r^*_2$ является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{proof}

\begin{theorem}
\labelTheorem{morphism of representations of universal algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
однотранзитивное представление $\Omega_1$\Hyph алгебры $A_1$ и
\ShowEq{f:A->*B}g{B_1}{B_2}
однотранзитивное представление $\Omega_1$\Hyph алгебры $B_1$.
Если отображение
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
является гомоморфизмом $\Omega_1$\Hyph алгебры,
то существует морфизм
представлений из $f$ в $g$
\ShowEq{r12:A->B}rAB
\end{theorem}
\begin{proof}
Выберем гомоморфизм $r_1$.
Выберем элемент $m\in A_2$
и элемент $n\in B_2$. 
Чтобы построить отображение $r_2$, рассмотрим следующую диаграмму
\DrawEq{morphism of representations of universal algebra, 2m 1}{}
Из коммутативности диаграммы $(1)$ следует
\DrawEq{morphism of representations of universal algebra, 2m}{}
Для произвольного $m'\in A_2$ однозначно определён
\ShowEq{a in A1}{}
такой, что
\ShowEq{m'=.m}
Следовательно, мы построили отображении $r_2$,
которое удовлетворяет равенству
\EqRef{morphism of representations of universal algebra, definition, 2}.
\end{proof}

\begin{theorem}
\labelTheorem{unique morphism of representations of universal algebra}
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа
\ShowEq{n=r2(m)}
заданного элемента $m\in A_2$.
\end{theorem}
\begin{proof}
Из доказательства теоремы
\RefTheorem{morphism of representations of universal algebra}
следует, что выбор гомоморфизма $r_1$ и элементов
$m\in A_2$, $n\in B_2$ однозначно определяет отображение $r_2$.
\end{proof}

\begin{theorem}
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно,
то для любого эндоморфизма
\ShowEq{r in End A1}
существует морфизм
представления $f$
\ShowEq{r12:A->B}rAA
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\ShowEq{morphism representation rR diagram}
Утверждение теоремы является следствием теоремы
\RefTheorem{morphism of representations of universal algebra}.
\end{proof}

\section{Теорема о разложении морфизмов расслоений}

\begin{theorem}
\labelTheorem{product of morphisms of representations of F algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$,
\ShowEq{f:A->*B}h{C_1}{C_2}
представление $\Omega_1$\Hyph алгебры $C_1$.
Пусть определены морфизмы представлений $\Omega_1$\Hyph алгебры
\ShowEq{r12:A->B}pAB
\ShowEq{r12:A->B}qBC
Тогда определён морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{r12:A->B}rAC
где
\ShowEq{r=q*p}
Мы будем называть морфизм
\ShowEq{map r12}r{}
представлений из $f$ в $h$
\AddIndex{произведением морфизмов
\ShowEq{map r12}p{}
и
\ShowEq{map r12}q{}
представлений универсальной алгебры}
{product of morphisms of representations of universal algebra}.
\end{theorem}
\begin{proof}
Мы можем представить утверждение теоремы,
пользуясь диаграммой
\ShowEq{product of morphisms of representations of F algebra}
Отображение $r_1$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру $C$.
Нам надо показать, что отображение
\ShowEq{map r12}r{}
удовлетворяет
\EqRef{morphism of representations of universal algebra, definition, 2}:
\ShowEq{product of morphisms of representations of F algebra, 1}
\end{proof}

\begin{definition}
\labelDefinition{transformation coordinated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}
следует
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{transformation correlated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование
\EqParm{f in End A2}{=c}
согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве
\EqParm{End A2/S}{S=S,=.}
\end{theorem}
\begin{proof}
Пусть $h=\mathrm{nat}\ S$. Если
\ShowEq{m1 m2 modS},
то $h(m_1)=h(m_2)$. Поскольку
\EqParm{f in End A2}{=z}
согласованно с эквивалентностью $S$,
то $h(f(m_1))=h(f(m_2))$. Это позволяет определить
преобразование $F$ согласно правилу
\ShowEq{morphism of representations and equivalence, 0}

Пусть $\omega$ - n\Hyph арная операция $\Omega_1$\Hyph алгебры.
Пусть
\ShowEq{f1n in End A2}
и
\ShowEq{morphism of representations and equivalence}
Согласно условию теоремы, преобразование
\ShowEq{morphism of representations and equivalence, 1}
согласованно с эквивалентностью $S$.
Следовательно, из условия
\ShowEq{m1 m2 modS}
и определения
\RefDefinition{transformation coordinated with equivalence}
следует
\ShowEq{morphism of representations and equivalence, 2}
Следовательно, мы можем определить операцию $\omega$ на множестве
\EqParm{End A2/S}{S=S,=z}
по правилу
\ShowEq{morphism of representations and equivalence, 3}
Из определения
\EqRef{morphism of representations and equivalence, 0}
и равенства
\EqRef{morphism of representations and equivalence, 2}
следует, что мы корректно определили
операцию $\omega$ на множестве
\EqParm{End A2/S}{S=S,=.}
\end{proof}

\begin{definition}
\labelDefinition{isomorphism of repesentations of Omega algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}rAB
морфизм представлений из $f$ в $g$ такой, что
$r_1$ - изоморфизм $\Omega_1$\Hyph алгебры и $r_2$
- изоморфизм $\Omega_2$\Hyph алгебры.
Тогда отображение
\ShowEq{map r12}r{}
называется
\AddIndex{изоморфизмом представлений}
{isomorphism of repesentations of Omega algebra}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{decompositions of morphism of representations}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\begin{proof}
Утверждения
\ShowEq{decompositions of morphism of representations, diagram ref}
являются следствием теоремы
\RefTheorem{first isomorphism theorem}.
Следовательно, диаграммы $(1)$ и $(2)$ коммутативны.

Мы начнём с диаграммы $(4)$.

Пусть
\ShowEq{m1=m2 ker t2}
Следовательно,
\ShowEq{morphism of representations of algebra, (4), 1}
Если
\ShowEq{a1=a2 ker t1}
то
\ShowEq{morphism of representations of algebra, (4), 2}
Следовательно,
\ShowEq{p1(a1)=p1(a2)}
Так как отображение
\ShowEq{map r,R}{t_1}{t_2}{}
- морфизм представлений, то
\ShowEq{morphism of representations of algebra, (4), 3 4}
Из \EqRef{morphism of representations of algebra, (4), 1},
\EqRef{morphism of representations of algebra, (4), 2},
\EqRef{morphism of representations of algebra, (4), 3},
\EqRef{morphism of representations of algebra, (4), 4}
следует
\ShowEq{morphism of representations of algebra, (4), 5}
Из \EqRef{morphism of representations of algebra, (4), 5}
следует
\ShowEq{morphism of representations of algebra, (4), 6}
и, следовательно,
\ShowEq{morphism of representations of algebra, (4), 7}
Из \EqRef{morphism of representations of algebra, (4), 7}
следует, что отображение
\ShowEq{morphism of representations of algebra, (4), 8}
определено корректно и является преобразованием множества
\EqParm{A2/ker}{I=2,=.}

Из равенства
\EqRef{morphism of representations of algebra, (4), 6}
(в случае $a_1=a_2$) следует, что, для любого $a$, преобразование
согласованно с эквивалентностью $\mathrm{ker}\,t_2$.
Из теоремы
\RefTheorem{transformation correlated with equivalence} следует,
что на множестве
\EqParm{End A2/S}{S=ker,=.}
определена структура $\Omega_1$\Hyph алгебры.
Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{transformation correlated with equivalence, 1}
пространства
\EqParm{A2/ker}{I=2,=.}
Мы положим
\ShowEq{morphism of representations of algebra, (4), 9}
Следовательно, отображение $F$ является представлением
$\Omega_1$\Hyph алгебры
\EqParm{A2/ker}{I=1,=.}

Согласно теореме
\RefTheorem{Tuple of maps is morphism of representations iff},
утверждение
\RefItem{(p12) is morphism of representations}
является следствием
\EqRef{morphism of representations of algebra, (4), 8}.

Рассмотрим диаграмму $(5)$.

\begin{lemma}
\labelLemma{(q12) is morphism of representations}
{\it
Отображение
\ShowEq{map r12}q{}
является морфизмом представлений $F$ и $G$.
}
\end{lemma}

{\sc Доказательство.}
Так как $q_2$ - биекция, то мы можем отождествить элементы множества
\EqParm{A2/ker}{I=2,=z}
и множества $t_2(A_2)$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 1}
Мы можем записать преобразование $F(\RedText{p_1(a)})$
множества
\EqParm{A2/ker}{I=2,=z}
в виде
\ShowEq{morphism of representations of algebra, (5), 2}
Так как $T$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3}
множества $RA_2$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3}
зависит от
\ShowEq{p(a) in A1/ker}
Так как $q_1$ - биекция, то мы можем отождествить элементы множества
\EqParm{A2/ker}{I=1,=z}
и множества $t_1(A_1)$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 6}
Следовательно, мы определили отображение
\ShowEq{G:tA1->tA2}
согласно равенству
\ShowEq{morphism of representations of algebra, (5), 4}

Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{morphism of representations of algebra, (5), 7}
множества $t_2(A_2)$. Мы положим
\ShowEq{morphism of representations of algebra, (5), 5}
Согласно \EqRef{morphism of representations of algebra, (5), 4}
операция $\omega$ корректно определена на множестве
\ShowEq{End tA2}
Следовательно, отображение $G$ является представлением
$\Omega_1$\Hyph алгебры.

Согласно теореме
\RefTheorem{Tuple of maps is morphism of representations iff},
лемма
является следствием
\EqRef{morphism of representations of algebra, (5), 4}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{(q1-1,q2-1) is morphism of representations}
{\it
Отображение
\ShowEq{map r,R}{q_1^{-1}}{q_2^{-1}}{}
является морфизмом представлений $G$ и $F$.
}
\end{lemma}

{\sc Доказательство.}
Так как $q_2$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 1}
следует
\ShowEq{morphism of representations of algebra, (5), 1a}
Мы можем записать преобразование $G(\RedText{t_1(a)})$
множества $t_2(A_2)$ в виде
\ShowEq{morphism of representations of algebra, (5), 2a}
Так как $q_2$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3a}
множества
\EqParm{A2/ker}{I=2,=.}
Преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
зависит от $\RedText{t_1(a)}\in t_1(A_1)$.
Так как $q_1$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 6}
следует
\ShowEq{morphism of representations of algebra, (5), 6a}
Так как по построению диаграмма $(5)$ коммутативна, то преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
совпадает с преобразованием
\EqRef{morphism of representations of algebra, (5), 2}.
Равенство
\EqRef{morphism of representations of algebra, (5), 5}
можно записать в виде
\ShowEq{morphism of representations of algebra, (5), 5a}
Согласно теореме
\RefTheorem{Tuple of maps is morphism of representations iff},
лемма
является следствием
\EqRef{morphism of representations of algebra, (5), 4},
\EqRef{morphism of representations of algebra, (5), 1a},
\EqRef{morphism of representations of algebra, (5), 6a}.
\hfill\(\odot\)

Утверждение
\RefItem{(q12) is isomorphism of representations}
является следствием определения
\RefDefinition{isomorphism of repesentations of Omega algebra}
и лемм
\RefLemma{(q12) is morphism of representations}
и
\RefLemma{(q1-1,q2-1) is morphism of representations}.

Диаграмма $(6)$ является самым простым случаем в нашем доказательстве.
Поскольку отображение $r_2$ является вложением и диаграмма $(2)$
коммутативна, мы можем отождествить $n\in B_2$ и $\BlueText{t_2(m)}$,
если $n\in\textrm{Im}t_2$. Аналогично, мы можем отождествить
соответствующие преобразования.
\ShowEq{morphism of representations of algebra, (6), 1}
Следовательно,
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
(утверждение
\RefItem{(r12) is morphism of representations}).

Для доказательства утверждения
\RefItem{exists decompositions of morphism of representations}
осталось показать, что определённое
в процессе доказательства представление $g'$ совпадает
с представлением $g$, а операции над преобразованиями совпадают
с соответствующими операциями на
\ShowEq{End O2}{B_2}.
\ShowEq{morphism of representations of algebra, (6), 2}
\end{proof}

\section{Приведенный морфизм представлений}

Из теоремы \RefTheorem{decompositions of morphism of representations}
следует, что мы можем свести задачу изучения морфизма представлений
$\Omega_1$\Hyph алгебры
к случаю, описываемому диаграммой
\ShowEq{morphism of representations of algebra, reduce, 1}

\begin{theorem}
\labelTheorem{morphism of representations of algebra, reduce}
Диаграмма \EqRef{morphism of representations of algebra, reduce, 1}
может быть дополнена представлением $F_1$
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре
\EqParm{A2/ker}{I=2,=z}
так, что диаграмма
\ShowEq{morphism of representations of algebra, reduce, 2}
коммутативна. При этом множество преобразований представления $F$ и
множество преобразований представления $F_1$ совпадают.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно положить
\ShowEq{F1(a)=F(p1(a))}
Так как отображение $p_1$ - сюрьекция, то $\mathrm{Im}F_1=\mathrm{Im}F$.
Так как $p_1$ и $F$ - гомоморфизмы $\Omega_1$\Hyph алгебры, то $F_1$
- также гомоморфизм $\Omega_1$\Hyph алгебры.
\end{proof}

Теорема \RefTheorem{morphism of representations of algebra, reduce}
завершает цикл теорем, посвящённых структуре морфизма представлений
$\Omega_1$\Hyph алгебры.
Из этих теорем следует, что мы можем упростить задачу
изучения морфизма представлений
$\Omega_1$\Hyph алгебры и ограничиться морфизмом представлений вида
\ShowEq{id:A1->A1 A2->B2}

\ShowDefinition{reduced morphism of representations}

\begin{theorem}
\labelTheorem{map is reduced morphism of representations iff}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
является приведенным морфизмом представлений тогда и только тогда, когда
\DrawEq{reduced morphism representation =}{definition}
\end{theorem}

\begin{proof}
Равенство
\eqRef{reduced morphism representation =}{definition}
следует из равенства
\EqRef{morphism of representations of universal algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{reduced morphism of representations and homomorphism of algebra}
Пусть отображение
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
является приведенным морфизмом из представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ в представление
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$.
Если представление $f$ эффективно, то отображение
\ShowEq{*R:*A2->*B2}
определённое равенством
\ShowEq{reduced morphism of representations, star morphism}
является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{morphism of representations and homomorphism of algebra},
если мы положим
$h=id$.
\end{proof}

\begin{theorem}
\labelTheorem{reduced morphism of representations of universal algebra}
Пусть представления
\ShowEq{f:A->*B}f{A_1}{A_2}
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивны.
Существует приведенный морфизм
представлений из $f$ в $g$
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
\end{theorem}
\begin{proof}
Выберем элемент $m\in A_2$
и элемент $n\in B_2$. 
Чтобы построить отображение $r_2$, рассмотрим следующую диаграмму
\ShowEq{reduced morphism representation H, diagram}
Из коммутативности диаграммы $(1)$ следует
\DrawEq{reduced morphism representation =}{}
Для произвольного $m'\in A_2$ однозначно определён
\ShowEq{a in A1}{}
такой, что
\ShowEq{m'=.m}
Следовательно, мы построили отображении $r_2$,
которое удовлетворяет равенству
\EqRef{morphism of representations of universal algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{unique reduced morphism of representations of universal algebra}
Пусть представления
\ShowEq{f:A->*B}f{A_1}{A_2}
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивны.
Приведенный морфизм представлений из $f$ в $g$
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
определён однозначно
с точностью до выбора образа $n=r_2(m)\in B_2$
заданного элемента $m\in A_2$.
\end{theorem}
\begin{proof}
Из доказательства теоремы
\RefTheorem{reduced morphism of representations of universal algebra}
следует, что выбор элементов
$m\in A_2$, $n\in B_2$ однозначно определяет отображение $r_2$.
\end{proof}

\begin{theorem}
\labelTheorem{morphisms representations, B B/N}
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Пусть $N$ - такая конгруэнция\,\footnote{Смотри
определение конгруэнции на с. \citeBib{Cohn: Universal Algebra}-71.}
на $\Omega_2$\Hyph алгебре $B$, что любое преобразование
\ShowEq{h in End B}
согласованно с конгруэнцией $N$.
Существует представление
\ShowEq{representation B/N}
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $B/N$
и отображение
\ShowEq{morphisms representations, B B/N}
является приведенным морфизмом представления $f$
в представление $f_1$
\ShowEq{morphisms representations, B B/N 1}
\end{theorem}
\begin{proof}
Любой элемент множества $B/N$ мы можем представить в виде $j(a)$, $a\in B$.

Согласно теореме
\citeBib{Cohn: Universal Algebra}-II.3.5, мы можем определить
единственную структуру $\Omega_2$\Hyph алгебры на множестве $B/N$.
Если $\omega\in\Omega_2(p)$,
то мы определим операцию $\omega$ на множестве $B/N$
согласно равенству (3) на странице \citeBib{Cohn: Universal Algebra}-73
\ShowEq{omega B/N}

Также как в доказательстве теоремы
\RefTheorem{decompositions of morphism of representations},
мы можем определить представление
\ShowEq{representation B/N}
с помощью равенства
\ShowEq{representation B/N 1}
Равенство
\EqRef{representation B/N 1}
можно представить с помощью диаграммы
\ShowEq{representation B/N 2}
Пусть $\omega\in\Omega_2(p)$.
Так как отображения $f(a)$ и $j$
являются гомоморфизмами $\Omega_2$\Hyph алгебры, то
\ShowEq{representation B/N 3}
Из равенства \EqRef{representation B/N 3}
следует, что
отображение $f_1(a)$ является гомоморфизмом $\Omega_2$\Hyph алгебры.
Из равенства
\EqRef{representation B/N 1},
согласно определению
\ShowEq{ref reduced morphism of representations}
следует, что отображение $j$ является приведенным морфизмом представления $f$
в представление $f_1$.
\end{proof}

\begin{theorem}
\labelTheorem{morphism representations and kernel equivalence}
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Пусть $N$ - такая конгруэнция
на $\Omega_2$\Hyph алгебре $B$, что любое преобразование
\ShowEq{h in End B}
согласованно с конгруэнцией $N$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные морфизмы представлений\,\footnote{Утверждение леммы аналогично утверждению 
на странице \citeBib{Serge Lang}-94.}
\ShowEq{morphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
представления $\Omega_1$\Hyph алгебры $A$.
Мы определим морфизм $R_1\rightarrow R_2$
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{morphisms category, diagram}
Приведенный морфизм $\mathrm{nat}\,N$ представления $f$
в представление $f_1$
(теорема \RefTheorem{morphisms representations, B B/N})
является универсально отталкивающим в категории $\mathcal A$.\,\footnote{Определение
универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.}
\end{theorem}
\begin{proof}
Существование и единственность отображения $h$,
для которого коммутативна диаграмма
\ShowEq{morphisms category, universal, diagram}
следует из теоремы
\RefTheorem{maps and kernel equivalence}.
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{morphisms category, h}

Пусть $\omega\in\Omega_2(p)$.
Так как отображения $R$ и $j$ являются гомоморфизмами $\Omega_2$\Hyph
алгебры, то
\ShowEq{morphisms category, h 1}
Из равенства
\EqRef{morphisms category, h 1}
следует, что отображение $h$ является гомоморфизмом $\Omega_2$\Hyph алгебры.

Так как отображение $R$ является приведенным морфизмом представления $f$
в представление $g$, то верно равенство
\ShowEq{morphism representations f g}
Из равенства
\EqRef{morphisms category, h}
следует
\ShowEq{morphism representations f1 g 1}
Из равенств
\EqRef{morphism representations f g},
\EqRef{morphism representations f1 g 1}
следует
\ShowEq{morphism representations f1 g 2}
Из равенств
\EqRef{morphisms category, h},
\EqRef{morphism representations f1 g 2}
следует
\ShowEq{morphism representations f1 g 3}
Из равенств
\EqRef{representation B/N 1},
\EqRef{morphism representations f1 g 3}
следует
\ShowEq{morphism representations f1 g 4}
Из равенства
\EqRef{morphism representations f1 g 4}
следует, что отображение $h$ является приведенным морфизмом
представления $f_1$ в представление $g$.
\end{proof}

\section{Автоморфизм представления универсальной алгебры}

\begin{definition}
\labelDefinition{endomorphism of representation of F algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Приведенный морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{R:A2->A2}
такой, что $r_2$ - эндоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{эндоморфизмом представления}
{endomorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно,
то для любых
\ShowEq{a2.in A2}
существует единственный эндоморфизм
\ShowEq{R:A2->A2}
представления $f$
такой, что
\ShowEq{Ra21=a22}
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\ShowEq{endomorphism representation r2 diagram}
Существование эндоморфизма является следствием теоремы
\RefTheorem{morphism of representations of universal algebra}.
Единственность эндоморфизма для заданных $p$, $q\in A_2$
является следствием теоремы
\RefTheorem{unique morphism of representations of universal algebra},
когда $r_1=\id$.
\end{proof}

\begin{theorem}
\labelTheorem{Endomorphisms of representation form semigroup}
Эндоморфизмы представления $f$ порождают полугруппу.
\end{theorem}
\begin{proof}
Из теоремы
\RefTheorem{product of morphisms of representations of F algebra}
следует, что произведение эндоморфизмов
\ShowEq{map r,R}{id}{p_2},
\ShowEq{map r,R}{id}{r_2}{}
представления $f$
является эндоморфизмом
\ShowEq{map r,R}{id}{p_2\circ r_2}{}
представления $f$.
\end{proof}

\begin{definition}
\labelDefinition{automorphism of representation of F algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{R:A2->A2}
такой, что $r_2$ - автоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{автоморфизмом представления}
{automorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{group of automorphisms of representation}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество автоморфизмов представления $f$ порождает
\AddIndex{группу}{group of automorphisms of representation}
\ShowEq{group of automorphisms of representation}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{automorphisms R P}
- автоморфизмы представления $f$.
Согласно определению
\RefDefinition{automorphism of representation of F algebra},
отображения
\ShowEq{automorphisms R P}
являются автоморфизмами
$\Omega_2$\Hyph алгебры $A_2$.
Согласно теореме II.3.2,
(\citeBib{Cohn: Universal Algebra}, c. 60),
отображение $r_2\circ p_2$
является автоморфизмом
$\Omega_2$\Hyph алгебры $A_2$.
Из теоремы
\RefTheorem{product of morphisms of representations of F algebra}
и определения
\RefDefinition{automorphism of representation of F algebra}
следует, что произведение автоморфизмов
$r_2\circ p_2$ представления $f$ является автоморфизмом представления $f$.

Пусть
\ShowEq{automorphisms R P Q}
- автоморфизмы представления $f$.
Из цепочки равенств
\ShowEq{associativity of product of automorphisms of representation}
следует ассоциативность произведения для отображений\,\footnote{
При доказательстве ассоциативности произведения
я следую примеру полугруппы
из \citeBib{Kurosh: General Algebra}, с. 20, 21.}
\ShowEq{automorphisms R P Q}.

Пусть $r_2$ - автоморфизм представления $f$.
Согласно определению
\RefDefinition{automorphism of representation of F algebra}
отображение $r_2$
является автоморфизмом
$\Omega_2$\Hyph алгебры $A_2$.
Следовательно, отображение $r_2^{-1}$
является автоморфизмом
$\Omega_2$\Hyph алгебры $A_2$.
Для автоморфизма $r_2$ представления справедливо равенство
\eqRef{morphism of representations of universal algebra, 2m}{definition}.
Положим
\ShowEq{m'=r2(m)}
Так как $r_2$ - автоморфизм $\Omega_2$\Hyph алгебры,
то
\ShowEq{m=r-2(m')}
и равенство
\eqRef{morphism of representations of universal algebra, 2m}{definition}
можно записать в виде
\ShowEq{morphism of representations of universal algebra, definition, 2m-1}
Так как отображение $r_2$
является автоморфизмом
$\Omega_2$\Hyph алгебры $A_2$,
то из равенства
\EqRef{morphism of representations of universal algebra, definition, 2m-1}
следует
\ShowEq{morphism of representations of universal algebra, definition, 2m-1, 1}
Равенство
\EqRef{morphism of representations of universal algebra, definition, 2m-1, 1}
соответствует равенству
\eqRef{morphism of representations of universal algebra, 2m}{definition}
для отображения $r_2^{-1}$.
Следовательно, отображение $r_2^{-1}$ является автоморфизмом
представления $f$.
\end{proof}


==> Basis.Diagram.Russian.tex <==
%auto-ignore
\input{Basis.Diagram.Eq}

\chapter{Базис диаграммы представлений универсальной алгебры}
\labelChapter{Basis of Diagram of Representations of Universal Algebra}

\section{Множество образующих диаграммы представлений}

Мы строим базис диаграммы представлений
по той же схеме, что мы построили базис представления
в секции \RefSection{Basis of representation}.

\begin{definition}
Пусть $(f,A)$ -
диаграмма представлений.
Кортеж множеств
\ShowEq{tuple of sets 1 n}N
называется
\AddIndex{кортежем стабильных множеств диаграммы представлений}
{tuple of stable sets of diagram of representations}
$(f,A)$,
если
\ShowEq{tuple of sets 1 n, ij}
для любых
\ShowEq{tuple of sets 1 n, ai}
при условии, что существует представление $f_{ij}$.
Мы также будем говорить, что кортеж множеств
\ShowEq{tuple of sets 1 n}N
стабилен относительно диаграммы представлений
$(f,A)$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{diagram of subrepresentations}
Пусть
$(f,A)$
- диаграмма представлений.
Пусть множество $N_{(i)}\subset A_{(i)}$ является
подалгеброй $\Omega_{(i)}$\Hyph алгебры $A_{(i)}$, \Kb[i]1.
Пусть кортеж множеств
\ShowEq{tuple of sets 1 n}N
стабилен относительно диаграммы представлений
$(f,A)$.
Тогда существует диаграмма представлений
\ShowEq{diagram of subrepresentations}
такая, что
\ShowEq{representation of algebra A in tuple N 2 n, 1}
Диаграмма представлений
\EqRef{diagram of subrepresentations}
называется
\AddIndex{подпредставлением}{subrepresentation}
диаграммы представлений $(f,A)$.
\end{theorem}
\begin{proof}
Пусть $\omega$ - $m$\Hyph арная операция
$\Omega_i$\Hyph алгебры $A_i$, $i=1$, ..., $n$.
Тогда для любых
\ShowEq{diagram of subrepresentations, a i}i
и любого $a_j\in N_j$
\ShowEq{diagram of subrepresentations, a i omega}
Пусть $\omega$ - $m$\Hyph арная операция
$\Omega_j$\Hyph алгебры $A_j$, $j=1$, ..., $n$.
Тогда для любых
\ShowEq{diagram of subrepresentations, a i}j
и любого $a_i\in N_i$
\ShowEq{diagram of subrepresentations, a j omega}
Утверждение теоремы доказано.
\end{proof}

Из теоремы
\RefTheorem{diagram of subrepresentations}
следует, что если диаграммы представлений
\EqRef{diagram of subrepresentations}
являются диаграммой подпредставлений диаграммы представлений
$(f,A)$,
то отображение
\ShowEq{diagram of subrepresentations, n}
является морфизмом диаграм представлений.

\begin{theorem}%
Множество\,\footnote{Эта теорема
аналогична определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94)}
\ShowEq{lattice of subdiagrams, diagram of representations}
всех диаграм подпредставлений диаграмы представлений
$(f,A)$
порождает
систему замыканий на диаграме представлений $(f,A)$
и, следовательно, является полной структурой.
\end{theorem}
\begin{proof}
Пусть для данного $\lambda\in\Lambda$,
\ShowEq{tuple of lambda sets 1 n}
кортеж множеств,
стабильных относительно диаграммы представлений
$(f,A)$.
Операцию пересечения на множестве $\mathcal B[f,A]$
мы определим согласно правилу
\ShowEq{set of subrepresentations, intersection, diagram}
$\cap K_{\lambda,(i)}$ - подалгебра
$\Omega_{(i)}$\Hyph алгебры $A_{(i)}$.
Пусть
\ShowEq{aj in cap Kj}
Для любого $\lambda\in\Lambda$ и для любого
\ShowEq{set of subrepresentations, intersection, i, 1}
Следовательно,
\ShowEq{set of subrepresentations, intersection, i, 2}
Следовательно, операция пересечения
диаграмм подпредставлений определена корректно.
\end{proof}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Если
\ShowEq{tuple of sets 1 n}X
кортеж множеств, то
\ShowEq{tuple of generating sets of diagram of representations, 1}
является пересечением всех кортежей
\ShowEq{tuple of sets 1 n}K
стабильных относительно диаграммы представлений $(f,A)$
и таких, что для \Kb[i]1,
$K_{(i)}$ - подалгебра $\Omega_{(i)}$\Hyph алгебры $A_{(i)}$,
содержащая $X_{(i)}$.

\begin{theorem}%
\labelTheorem{structure of subrepresentations in diagram of representations}
Пусть\,\footnote{
Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, стр. 94.}
$(f,A)$ - диаграмма представлений.
Пусть
\ShowEq{tuple of sets 1 n}X
Для каждого значения $(i)$, \Kb[i]1,
определим подмножества $X_{(i)k}\subset A_{(i)}$ индукцией по $k$.
\ShowEq{structure of subrepresentations in representation, 2}
Для каждого значения $(i)$ положим
\ShowEq{structure of subrepresentations in representation, 3}
Тогда
\ShowEq{structure of subrepresentations in representation, 4}
\end{theorem}
\begin{proof}
Для каждого значения $(i)$ доказательство теоремы
совпадает с доказательством теоремы
\RefTheorem{structure of subrepresentations}.
%\RefRemark{diagram of representations}
%Небольшое отличие есть лишь в доказательстве утверждения
%\RefItem{ax in Xk+1 i}.
\ifx\texFuture\Defined
Так как для определения устойчивого подмножества
$\Omega_i$\Hyph алгебры $A_i$
нас интересует только некоторое устойчивое подмножество
$\Omega_{i-1}$\Hyph алгебры $A_{i-1}$,
мы должны сперва найти устойчивое  подмножество
$\Omega_{i-1}$\Hyph алгебры $A_{i-1}$ прежде, чем
мы найдём устойчивое  подмножество в $\Omega_i$\Hyph алгебре $A_i$.
\fi
\end{proof}

\ShowEq{subrepresentation generated by tuple of sets}
называется
\AddIndex{подпредставлением}{subrepresentation}
диаграммы представлений $(f,A)$,
порождённым кортежем множеств $X$,
а $X$ -
\AddIndex{множеством образующих}{generating set}
диаграммы представлений J[f,X].
В частности, множество образующих
диаграммы представлений $(f,A)$
будет такой кортеж
\ShowEq{tuple of sets 1 n}X
что
$J[f,X]=A$.

Из теоремы
\RefTheorem{structure of subrepresentations in diagram of representations}
следует следующее определение.

\begin{definition}
\labelDefinition{words of element, diagram of representations}
Пусть
\ShowEq{tuple of sets 1 n}X
кортеж множеств.
Для любого кортежа $A$\Hyph чисел
\ShowEq{tuple of A numbers}
существует
\AddIndex{кортеж $\Omega$\Hyph слов}{tuple of Omega words}
\ShowEq{tuple of Omega words}
определённых согласно следующему правилу.
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{ai in Xi()}
то $a_{(i)}$ - $\Omega_{(i)}$\Hyph слово
\ShowEq{words of element, diagram of representations, ai}
\item Если
\ShowEq{a(i)1p}
- $\Omega_{(i)}$\Hyph слова, \Kb[i]1, и
$\omega\in\Omega_{(i)}(p)$, то
\ShowEq{a(i)1p omega}
- $\Omega_{(i)}$\Hyph слово.
\labelItem{words of element, diagram of representations, omega i}
\item Пусть $a_i=a_{(i)}$ - $\Omega_{(i)}$\Hyph слово,
$a_j=a_{(j)}$ - $\Omega_{(j)}$\Hyph слово.
Пусть существует представление $f_{ij}$.
Тогда $f_{ij}(a_i)(a_j)$
- $\Omega_{(j)}$\Hyph слово.
\labelItem{words of element, diagram of representations, a i j}
\end{enumerate}
Обозначим
\ShowEq{set of tuples of Omega words}
\AddIndex{множество кортежей $\Omega$\Hyph слов}{set of tuples of Omega words}
диаграммы представлений J[f,X].
\qed
\end{definition}

Мы рассматриваем кортеж $A$\Hyph чисел
в определении
\RefDefinition{words of element, diagram of representations},
так как нам нужен алгоритм формирования
кортежа $\Omega$\Hyph слов.
Однако при решении конкретных задач
нам может понадобиться только некоторое подмножество кортежа $A$\Hyph чисел.
Например, в аффинном пространстве
мы можем рассматривать либо множество точек,
либо множество векторов.

Выбор $\Omega_{(i)}$\Hyph слова относительно множества образующих $X$ неоднозначен.
Поэтому, если $\Omega_{(i)}$\Hyph число имеет различные
$\Omega_{(i)}$\Hyph слова, то мы, чтобы их отличать, будем пользоваться индексами:
\ShowEq{w w1 w2[fXm] ()}

\begin{definition}
\labelDefinition{tuple of equivalences on the set of Omega-words}
Множество образующих $X$ диаграммы представлений $(f,A)$
порождает кортеж отношений эквивалентности
\ShowEq{rho fX()=}
на множестве кортежей $\Omega$\Hyph слов.
\qed
\end{definition}

Согласно определению
\RefDefinition{tuple of equivalences on the set of Omega-words},
два $\Omega_{(i)}$\Hyph слова относительно
множества образующих $X$ диаграммы представлений $(f,A)$
эквивалентны тогда и только тогда, когда
они соответствуют одному и тому же $A_{(i)}$\Hyph числу.
Когда мы будем записывать равенство
двух $\Omega_{(i)}$\Hyph слов относительно
множества образующих $X$ диаграммы представлений $(f,A)$,
мы будем иметь в виду, что это равенство верно
с точностью до отношения эквивалентности
\ShowEq{rho fX()}

Мы будем пользоваться записью
\ShowEq{morphism image, diagram of representations}
для образа кортежа элементов
\ShowEq{a=(a(i))}a{}
при морфизме диаграммы представлений.

\begin{theorem}
\labelTheorem{map of words of diagram of representations}
Пусть $X$ - множество образующих диаграммы представлений $(f,A)$.
Пусть $Y$ - множество образующих диаграммы представлений $(g,B)$.
Морфизм $r$ диаграммы представлений
$(f,A)$
порождает отображение $\Omega$\Hyph слов
\ShowEq{map of words of diagram of representations}
такое, что для любого
\ShowEq{(i),(1...n)}
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of coordinates of diagram of representations, a in X, 1}
то
\ShowEq{map of words of diagram of representations, a in X}
\item Если
\ShowEq{map of words of diagram of representations, omega, 1}
то для операции
$\omega\in\Omega_{(i)}(p)$ справедливо
\ShowEq{map of words of diagram of representations, omega}
\item Если
\ShowEq{map of words of diagram of representations, am, 1}
то
\ShowEq{map of words of diagram of representations, am}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждения
\RefItem{map of words of diagram of representations, a in X},
\RefItem{map of words of diagram of representations, omega}
справедливы в силу определения морфизма $r$.
Утверждение
\RefItem{map of words of diagram of representations, am}
следует из равенства
\EqRef{morphism of diagram of representations, levels k k+1}.
\end{proof}

\begin{remark}
\labelRemark{coordinates of diagram of representations}
Пусть $r$ - морфизм диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$.
Пусть
\ShowEq{map of words of diagram of representations 1}
Теорема
\RefTheorem{map of words of diagram of representations}
утверждает, что
\ShowEq{map of words of diagram of representations 2}
Теорема
\RefTheorem{map of words of diagram of representations}
также утверждает, что
кортеж $\Omega$\Hyph слов, представляющий $a$ относительно $X$, и
кортеж $\Omega$\Hyph слов, представляющий $a'$ относительно $Y$,
формируются согласно одному и тому же алгоритму.
Это позволяет рассматривать кортеж $\Omega$\Hyph слов $w[g,Y,a']$
как кортеж отображений
\ShowEq{coordinates of element relative to generating set}{(k)}a
\ShowEq{tuple of coordinates relative to generating set}{,a}
\DrawEq[{(k)}a]{coordinates of representation 3 fg}{diagram}

Если $f=g$, то вместо отображения
\eqRef{coordinates of representation 3 fg}{diagram}
мы будем рассматривать отображение
\ShowEq{coordinates of diagram of representation 3}
такое, что, если для некоторого морфизма $r$ 
\ShowEq{coordinates of diagram of representations 4}
то
\ShowEq{coordinates of diagram of representations 5}

Отображение
$\ShowSymbol{coordinates relative to set}{}$
называется
\AddIndex{координатами $A_{(k)}$\Hyph числа $a_{(k)}$}{coordinates relative to set}
относительно кортежа множеств $X$.
Аналогично, мы можем рассмотреть координаты множества
\ShowEq{subset of representation}{(k)}
относительно множества $X$
\ShowEq{subset of coordinates of representation}{(k)}a
Обозначим
\ShowEq{tuple of coordinates relative to generating set}{}%
\ShowEq{coordinate set of representation}{(k)}a
\AddIndex{множество координат представления $J[f,X]$}
{coordinate set of representation}.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{set of coordinates, diagram of representations, omega}
На множестве координат $W_{(k)}[f,X]$ определена структура $\Omega_{(k)}$\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть $\omega\in\Omega_{(k)}(n)$. Тогда для любых
\ShowEq{set of coordinates, 1k, omega}
положим
\ShowEq{set of coordinates, k, omega}
Согласно замечанию
\RefRemark{coordinates of diagram of representations},
из равенства
\EqRef{set of coordinates, k, omega}
следует
\ShowEq{set of coordinates, 2k, omega}
Согласно правилу
\RefItem{words of element, diagram of representations, omega i},
из равенства
\EqRef{set of coordinates, 2k, omega}
следует
\ShowEq{set of coordinates, 3k, omega}
Из равенства
\EqRef{set of coordinates, 3k, omega}
следует
корректность определения
\EqRef{set of coordinates, k, omega}
операции $\omega$
на множестве координат $W_{(k)}[f,X]$.
\end{proof}

\begin{theorem}
\labelTheorem{set of coordinates, diagram of representations, am}
Если определено предсталение $f_{jk}$
$\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$,
то определено представление $F_{jk}$
$\Omega_j$\Hyph алгебры $W_j[f,X]$
в $\Omega_k$\Hyph алгебре $W_k[f,X]$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{set of coordinates, 1 j}j.
Тогда для любого
\ShowEq{set of coordinates, 1 j}k,
положим
\ShowEq{set of coordinates, am k}
Согласно замечанию
\RefRemark{coordinates of diagram of representations},
из равенства
\EqRef{set of coordinates, am k}
следует
\ShowEq{set of coordinates, 2, am k}
Согласно правилу
\RefItem{words of element, diagram of representations, a i j},
из равенства
\EqRef{set of coordinates, 2, am k}
следует
\ShowEq{set of coordinates, 3, am k}
Из равенства
\EqRef{set of coordinates, 3, am k}
следует корректность определения
\EqRef{set of coordinates, am k}
представления $\Omega_j$\Hyph алгебры $W_j[f,X]$
в $\Omega_k$\Hyph алгебре $W_k[f,X]$.
\end{proof}

\begin{sloppypar}
\begin{corollary}
\labelCorollary{set of coordinates, diagram of representations, am}
Кортеж $\Omega$\Hyph алгебр
\ShowEq{W=(W1n)}
и множество представлений $F$
порождает диаграмму представлений
\ShowEq{(F,W[])}FfX.
\qed
\end{corollary}
\end{sloppypar}

\begin{theorem}
\labelTheorem{map of words of diagram of representations, 1}
Пусть
$(f,A)$, $(g,B)$
- диаграммы представлений.
Для заданных множеств
\ShowEq{map of coordinates of diagram of representations, Xk}
рассмотрим кортеж отображений
\ShowEq{map of coordinates of diagram of representations, R}
таких, что для любого
\ShowEq{(k)=1n}
отображение
\ShowEq{map of coordinates of diagram of representations, Rk}
согласовано со структурой диаграммы представлений,
т. е.
\ShowEq{map of words of diagram of representations; omega}
\ShowEq{map of words of diagram of representations, morphism}
Рассмотрим кортеж отображений $\Omega$\Hyph слов
\ShowEq{map of words of diagram of representations, W}
удовлетворяющее условиям
\RefItem{map of words of diagram of representations, a in X},
\RefItem{map of words of diagram of representations, omega},
\RefItem{map of words of diagram of representations, am},
и такое, что
\ShowEq{map of words of diagram of representations, W in X}
Для каждого $(k)$,
\ShowEq{(k)=1n}
существует гомоморфизм $\Omega_{(k)}$\Hyph алгебры
\ShowEq{map of coordinates of diagram of representations, r}
определённый правилом
\ShowEq{morphism based on map of words of diagram of representations}
Кортеж гомоморфизмов
\ShowEq{A=A(1n)1n}r
является морфизмом диаграмм представлнений
$J[f,X]$ и $J[g,Y]$.
\end{theorem}
\begin{proof}
Для любого
\ShowEq{(k)=1n}
рассмотрим отображение
\ShowEq{f:A->B}{r_{(k)}}{A_{(k)}}{B_{(k)}}

\begin{lemma}
\labelLemma{maps rk and Rk coinside on the set Xk}
{\it
Для любого
\ShowEq{(k)=1n}
на множестве $X_{(k)}$ отображения $r_{(k)}$ и $R_{(k)}$ совпадают,
и отображение $r_{(k)}$ согласовано со структурой $\Omega_{(k)}$\Hyph алгебры.
}
\end{lemma}

{\sc Доказательство.}
Если
\ShowEq{map of words of diagram of representations, w(a)=a}
то $a_{(k)}\in X_{(k)}$.
Согласно условию
\RefItem{map of words of diagram of representations, a in X},
равенство
\ShowEq{map of words of diagram of representations, r(a)=R(a)}
является следствием равенств
\EqRef{morphism based on map of words of diagram of representations},
\EqRef{map of words of diagram of representations, w(a)=a}.
Лемма является следствием равенства
\EqRef{map of words of diagram of representations, r(a)=R(a)}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{map rk is homomorphism}
Пусть $\omega\in\Omega_{(k)}(p)$.
\ShowEq{map of words of diagram of representations, omega 2}
\end{lemma}

{\sc Доказательство.}
Мы будем доказывать лемму индукцией по сложности
$\Omega_{(k)}$\Hyph слова.

Если
\ShowEq{map of words of diagram of representations, omega 1}
то равенство
\EqRef{map of words of diagram of representations, omega 2}
является следствием утверждения
\EqRef{map of words of diagram of representations; omega}.

Пусть предположение индукции верно для
\ShowEq{map of words of diagram of representations, r(a), omega, 1}
Пусть
\ShowEq{map of words of diagram of representations, r(a), omega, 2}
Согласно предположению индукции,
равенство
\ShowEq{map of words of diagram of representations, r(a), omega, 2a}
является следствием равенств
\EqRef{morphism based on map of words of diagram of representations},
\EqRef{map of words of diagram of representations, r(a), omega, 2}.
Если
\ShowEq{map of words of diagram of representations, r(a), omega, 3}
то согласно условию
\RefItem{words of element, diagram of representations, omega i},
\ShowEq{map of words of diagram of representations, r(a), omega, 4}
Согласно условию
\RefItem{map of words of diagram of representations, omega},
равенство
\ShowEq{map of words of diagram of representations, r(a), omega, 5}
является следствием равенств
\EqRef{morphism based on map of words of diagram of representations},
\EqRef{map of words of diagram of representations, r(a), omega, 3},
\EqRef{map of words of diagram of representations, r(a), omega, 2a}.
Равенство
\EqRef{map of words of diagram of representations, omega 2}
является следствием равенства
\EqRef{map of words of diagram of representations, r(a), omega, 5}.
\hfill\(\odot\)

Согласно лемме
\RefLemma{maps rk and Rk coinside on the set Xk},
отображения $r_{(k)}$ и $R_{(k)}$ совпадают на множестве $X_{(k)}$.
Согласно лемме
\RefLemma{map rk is homomorphism},
отображение $r_{(k)}$ является гомоморфизмом
$\Omega_{(k)}$\Hyph алгебры $A_{(k)}$ в
$\Omega_{(k)}$\Hyph алгебру $B_{(k)}$.
Для доказательства теоремы достаточно показать, что если
существует представление
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
то пара отображений $(r_j\ \ r_i)$ является
морфизмом представлений из $f_{ji}$ в $g_{ji}$
(определение
\RefDefinition{Morphism of Diagram of Representations}).

Мы будем доказывать теорему индукцией по сложности
$\Omega_i$\Hyph слова.

Если
\ShowEq{aij in Xij}
то предположение индукции является следствием утверждения
\EqRef{map of words of diagram of representations, morphism}

Пусть предположение индукции верно для
\ShowEq{map of words of diagram of representations, r(a), a i j, 1}
Согласно условию
\RefItem{words of element, diagram of representations, a i j},
\ShowEq{map of words of diagram of representations, r(a), a i j, 2}
Согласно условию
\RefItem{map of words of diagram of representations, am},
равенство
\ShowEq{map of words of diagram of representations, r(a), a j i, 3}
является следствием равенств
\EqRef{morphism based on map of words of diagram of representations},
\EqRef{map of words of diagram of representations, r(a), a i j, 2},
Из равенств
\EqRef{morphism of diagram of representations, levels k k+1},
\EqRef{map of words of diagram of representations, r(a), a j i, 3}
следует, что отображение $r$ является морфизмом
диаграммы представлений $(f,A)$.
\end{proof}

\begin{remark}
Теорема \RefTheorem{map of words of diagram of representations, 1}
- это теорема о продолжении отображения.
Единственное, что нам известно о кортеже множеств $X$ - это то, что
$X$ - кортеж множеств образующих диаграммы представлений $(f,A)$.
Однако, между элементами множества $X_{(k)}$,
\ShowEq{(k)=(1n)},
могут существовать соотношения,
порождённые либо операциями $\Omega_{(k)}$\Hyph алгебры $A_{(k)}$, либо
преобразованиями представления $f_{jk}$.
Поэтому произвольное отображение кортежа множеств $X$, вообще говоря,
не может быть продолжено до эндоморфизма диаграммы представлений $(f,A)$.\,\footnote{
В теореме
\RefTheorem{automorphism uniquely defined by image of basis, diagram of representations},
требования к кортежу множеств образующих более жёсткие. Поэтому теорема
\RefTheorem{automorphism uniquely defined by image of basis, diagram of representations}
говорит о продолжении произвольного отображения.
Более подробный анализ дан в замечании
\RefRemark{automorphism uniquely defined by image of basis, diagram of representations}.}
Однако, если для каждого
\ShowEq{(k)=1n}
отображение $R_{(k)}$ согласованно со структурой диаграммы представлений,
то мы можем построить продолжение этого отображения,
которое является морфизмом диаграммы представлений $(f,A)$.
\qed
\end{remark}

\begin{sloppypar}
\begin{definition}
Пусть $X$ - кортеж множеств образующих диаграммы представлений $(f,A)$.
Пусть $Y$ - кортеж множеств образующих диаграммы представлений $(g,B)$.
Пусть $r$ - морфизм диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$.
Множество координат
\ShowEq{coordinates of morphism, 2, diagram of representations}{}
называется
\AddIndex{координатами морфизма диаграммы представлений}
{coordinates of morphism, diagram of representations}.
\qed
\end{definition}
\end{sloppypar}

\begin{definition}
\labelDefinition{superposition of coordinates, diagram of representations}
Пусть $X$ - кортеж множеств образующих диаграммы представлений $(f,A)$.
Пусть $Y$ - кортеж множеств образующих диаграммы представлений $(g,B)$.
Пусть $r$ - морфизм диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$.
Пусть для
\ShowEq{(k)=(1n)},
$a_{(k)}\in A_{(k)}$.
Мы определим
\AddIndex{суперпозицию координат}{superposition of coordinates}
морфизма $r$ диаграммы представлений и $A_{(k)}$\Hyph числа $a_{(k)}$
как координаты, определённые согласно правилу
\ShowEq{superposition of coordinates}
\ShowEq{superposition of coordinates, diagram of representations}
Пусть $Y_{(k)}\subset A_{(k)}$.
Мы определим
суперпозицию координат
морфизма $r$ диаграммы представлений и множества $Y_{(k)}$
согласно правилу
\ShowEq{superposition of coordinates, 1, diagram of representations}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map of coordinates of diagram of representations}
Морфизм $r$ диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$
порождает отображение координат диаграммы представлений
\ShowEq{map of coordinates of diagram of representations}
\ShowEq{(k)=(1n)},
такое, что
\ShowEq{map of coordinates of diagram of representations, 1}
\ShowEq{map of coordinates of diagram of representations, 1a}
\end{theorem}
\begin{proof}
Согласно замечанию
\RefRemark{coordinates of diagram of representations},
мы можем рассматривать равенства
\EqRef{superposition of coordinates, diagram of representations},
\EqRef{map of coordinates of diagram of representations}
относительно заданного кортежа множеств образующих $X$.
При этом координатам $W_{(k)}[f,X,a_{(k)}]$
соответствует кортеж слов
\ShowEq{map of coordinates of diagram of representations, 2}
а координатам
\ShowEq{map of coordinates of diagram of representations, 3a}{}
соответствует кортеж слов
\ShowEq{map of coordinates of diagram of representations, 3}
Поэтому для того, чтобы доказать теорему,
нам достаточно показать, что отображению
\ShowEq{map of coordinates, diagram of representations}W{(k)}{}
соответствует отображение
\ShowEq{map of coordinates, diagram of representations}w{(k)}.
%Мы докажем утверждение индукцией по диаграмме представлений.

%Если $\Omega_{(k)}\Hyph алгебра $A_{(k)}$ принадлежит множеству $A_{[1]}$,
%то утверждение теоремы является следствием теоремы
%\RefTheorem{map of coordinates of representation}.
%Пусть утверждение теоремы верно для $n-1$.
Мы будем доказывать теорему индукцией по сложности
$\Omega_{(k)}$\Hyph слова.

Если
\ShowEq{map of words of diagram of representations, a in X, 1}
то, согласно равенствам
\EqRef{map of coordinates of diagram of representations, 2},
\EqRef{map of coordinates of diagram of representations, 3},
отображения
\ShowEq{map of coordinates, diagram of representations}W{(k)}{}
и
\ShowEq{map of coordinates, diagram of representations}w{(k)}{}
согласованы.

Пусть для
\ShowEq{superposition of coordinates, diagram of representations, omega, 1}
отображения
\ShowEq{map of coordinates, diagram of representations}W{(k)}{}
и
\ShowEq{map of coordinates, diagram of representations}w{(k)}{}
согласованы.
Пусть $\omega\in\Omega_{(k)}(p)$.
Согласно теореме
\RefTheorem{set of coordinates, representation, omega}
\ShowEq{superposition of coordinates, diagram of representations, omega, 2}
Так как отображение
\ShowEq{map of coordinates of diagram of representations, r}
является гомоморфизмом $\Omega_{(k)}$\Hyph алгебры,
то из равенства
\EqRef{superposition of coordinates, diagram of representations, omega, 2}
следует
\ShowEq{superposition of coordinates, diagram of representations, omega, 3}
Из равенств
\EqRef{superposition of coordinates, diagram of representations, omega, 2},
\EqRef{superposition of coordinates, diagram of representations, omega, 3}
и предположения индукции следует, что
отображения
\ShowEq{map of coordinates, diagram of representations}W{(k)}{}
и
\ShowEq{map of coordinates, diagram of representations}w{(k)}{}
согласованы для $a_{(k)}=a_{(k)1}...a_{(k)p}\omega$.

Пусть для
$a_{j1}\in A_j$
отображения
\ShowEq{map of coordinates, diagram of representations}Wj{}
и
\ShowEq{map of coordinates, diagram of representations}wj{}
согласованы.
Пусть для
$a_{i1}\in A_i$
отображения
\ShowEq{map of coordinates, diagram of representations}Wi{}
и
\ShowEq{map of coordinates, diagram of representations}wi{}
согласованы.
Согласно теореме
\RefTheorem{set of coordinates, diagram of representations, am}
\ShowEq{superposition of coordinates, diagram of representations, a j i, 1}
Так как отображение
$(r_j,r_i)$
является морфизмом представления $f_{ji}$
в представление $F_{ji}$,
то из равенства
\EqRef{superposition of coordinates, diagram of representations, a j i, 1}
следует
\ShowEq{superposition of coordinates, diagram of representations, a j i, 2}
Из равенств
\EqRef{superposition of coordinates, diagram of representations, a j i, 1},
\EqRef{superposition of coordinates, diagram of representations, a j i, 2}
и предположения индукции следует, что
отображения
\ShowEq{map of coordinates, diagram of representations}Wi{}
и
\ShowEq{map of coordinates, diagram of representations}wi{}
согласованы для
$b_i=f_{ji}(a_j)(a_i)$.
\end{proof}

\begin{corollary}
\labelCorollary{map of coordinates of diagram of representations}
Пусть $X$ - кортеж множеств образующих диаграммы представлений $(f,A)$.
Пусть $Y$ - кортеж множеств образующих диаграммы представлений $(g,B)$.
Пусть $r$ - морфизм диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$.
Отображение
\ShowEq{map of coordinates of diagram of representations, tuple}
является морфизмом диаграммы представлений
\ShowEq{(F,W[])}FfX{}
в диаграмму представлений
\ShowEq{(F,W[])}GgY.
\qed
\end{corollary}

В дальнейшем мы будем отождествлять отображение
\ShowEq{map of coordinates of diagram of representations, W f->g}
и множество координат
\ShowEq{coordinates of morphism, 2, diagram of representations}.

\begin{theorem}
Пусть $X$ - кортеж множеств образующих диаграммы представлений $(f,A)$.
Пусть $Y$ - кортеж множеств образующих диаграммы представлений $(g,B)$.
Пусть $r$ - морфизм диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$.
Пусть $Y\subset A$.
Тогда
\ShowEq{superposition of coordinates, 2, diagram of representations}
\ShowEq{superposition of coordinates, 2a, diagram of representations}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 2, diagram of representations}
является следствием равенства
\ShowEq{superposition of coordinates, 3, diagram of representations}
а также равенств
\EqRef{superposition of coordinates, diagram of representations},
\EqRef{superposition of coordinates, 1, diagram of representations}.
Равенство
\EqRef{superposition of coordinates, 2a, diagram of representations}
является следствием равенств
\EqRef{superposition of coordinates, 2, diagram of representations},
\EqRef{map of coordinates of diagram of representations, 1}.
\end{proof}

\begin{theorem}
\labelTheorem{superposition of coordinates of endomorphisms, diagram of representations}
Пусть $X$ - кортеж множеств образующих диаграммы представлений $(f,A)$.
Пусть $Y$ - кортеж множеств образующих диаграммы представлений $(g,B)$.
Пусть $Z$ - кортеж множеств образующих диаграммы представлений $(h,C)$.
Пусть $r$ - морфизм диаграммы представлений $(f,A)$
в диаграмму представлений $(g,B)$.
Пусть $s$ - морфизм диаграммы представлений $(g,B)$
в диаграмму представлений $(h,C)$.
Тогда
\ShowEq{superposition of coordinates, 4, diagram of representations}
\ShowEq{superposition of coordinates, 4a, diagram of representations}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{superposition of coordinates, 4c, diagram of representations}
следует из равенства
\EqRef{superposition of coordinates, 2, diagram of representations}.
Равенство
\EqRef{superposition of coordinates, 4, diagram of representations}
следует из равенства
\EqRef{superposition of coordinates, 4c, diagram of representations},
если положить $Y'=r(X)$.
Равенство
\EqRef{superposition of coordinates, 4a, diagram of representations}
следует из равенства
\EqRef{superposition of coordinates, 4, diagram of representations}.
\end{proof}

\begin{definition}
\labelDefinition{superposition of coordinates and words, diagram of representations}
Мы можем обобщить определение суперпозиции координат и предположить,
что один из множителей является кортежем множеств $\Omega$\Hyph слов.
Соответственно, определение суперпозиции координат имеет вид
\ShowEq{superposition of coordinates, 5, diagram of representations}
\qed
\end{definition}

Следующие формы записи образа кортежа множеств $X'$
при морфизме $r$ диаграммы представлений эквивалентны
\ShowEq{superposition of coordinates, 6, diagram of representations}
Из равенств
\EqRef{superposition of coordinates, 2, diagram of representations},
\EqRef{superposition of coordinates, 6, diagram of representations}
следует, что
\ShowEq{superposition of coordinates, 7, diagram of representations}
Равенство
\EqRef{superposition of coordinates, 7, diagram of representations}
является законом ассоциативности для операции композиции и позволяет
записать выражение
\ShowEq{superposition of coordinates, 8, diagram of representations}
без использования скобок.

\begin{definition}
\labelDefinition{endomorphism of representation, regular on tuple}
Пусть
\ShowEq{tuple of sets 1 n}X
множество образующих диаграммы представлений
$(f,A)$.
Пусть отображение
$r$
является эндоморфизмом диаграммы представления $(f,A)$.
Пусть кортеж множеств
\ShowEq{endomorphism of representation, regular on tuple}
является образом кортежа множеств $X$
при отображении $r$.
Эндоморфизм $r$ диаграммы представлений $(f,A)$ называется
невырожденным на кортеже множеств образующих $X$,
если кортеж множеств $Y$ является кортежем множеств образующих
диаграммы представлений $(f,A)$.
В противном случае, эндоморфизм $r$ называется
вырожденным на кортеже множеств образующих $X$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{regular endomorphism of diagram of representations}
Эндоморфизм $r$ диаграммы представлений $(f,A)$ называется
\AddIndex{невырожденным}{regular endomorphism},
если он невырожден на любом кортеже множеств образующих.
В противном случае, эндоморфизм $r$ называется
\AddIndex{вырожденным}{singular endomorphism}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Automorphism of diagram of representations is regular endomorphism}
Автоморфизм $r$ диаграммы представлений
$(f,A)$
является невырожденным эндоморфизмом.
\end{theorem}
\begin{proof}
Пусть $X$ - кортеж множеств образующих
диаграммы представлений $(f,A)$.
Пусть $Y=r(X)$.
Согласно теореме
\RefTheorem{map of coordinates of diagram of representations}
эндоморфизм $r$
порождает отображение $\Omega$\Hyph слов
\ShowEq{map of coordinates, diagram of representations}w{}.
Пусть $a'\in A$. Так как $r$
- автоморфизм, то существует
\ShowEq{Automorphism of diagram of representations is regular endomorphism, 0}
Согласно определению
\RefDefinition{words of element, diagram of representations},
$w[f,X, a]$ - кортеж $\Omega$\Hyph слов, представляющих
$a$ относительно кортежа множеств образующих $X$.
Согласно теореме
\RefTheorem{map of coordinates of diagram of representations},
$w[f,X',a']$
- кортеж $\Omega$\Hyph слов, представляющих
$a'$ относительно кортежа множеств $Y$
\ShowEq{Automorphism of diagram of representations is regular endomorphism, 1}
Следовательно, $Y$ - множество образующих диаграммы представлений $(f,A)$.
Согласно определению
\RefDefinition{regular endomorphism of diagram of representations},
автоморфизм $r$ - невырожден.
\end{proof}

\section{Базис диаграммы представлений}

\begin{definition}
Пусть
$(f,A)$
- диаграмма представлений
и
\ShowEq{Gen fA =}
Если для кортежа множеств
$X\subset A_2$
верно
\ShowEq{in Gen}X{f,A},
то для любого кортежа множеств
\ShowEq{X in Y in A(k)}
также верно
\ShowEq{in Gen}Y{f,A}.
Если существует минимальный кортеж множеств
\ShowEq{in Gen}X{f,A},
то такой кортеж множеств $X$ называется
\AddIndex{квазибазисом диаграммы представлений}
{quasibasis of diagram of representations}
$(f,A)$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{X is quasibasis of diagram of representations}
Если кортеж множеств $X$ является квазибазисом
диаграммы представлений $(f,A)$,
то, для любого
\ShowEq{(k)=1n}
и любого $m\in X_{(k)}$,
кортеж множеств
\ShowEq{X'=...Xk-m}
не является
множеством образующих диаграммы представлений $(f,A)$.
\end{theorem}
\begin{proof}
Пусть $X$ - квазибазис диаграммы представлений $(f,A)$.
Допустим для некоторого $m\in X_{(k)}$ существует $\Omega_{(k)}$\Hyph слово
\ShowEq{X is quasibasis of diagram of representations, 1}
Рассмотрим $A_{(k)}$\Hyph число $m'$, для
которого $\Omega_{(k)}$\Hyph слово
\ShowEq{X is quasibasis of diagram of representations, 2}
зависит от $m$.
Согласно определению
\RefDefinition{words of element, diagram of representations},
любое вхождение $A_{(k)}$\Hyph числа $m$ в $\Omega_{(k)}$\Hyph слово $w'$ может быть заменено
$\Omega_{(k)}$\Hyph словом $w$. Следовательно,
$\Omega_{(k)}$\Hyph слово $w'$ не зависит от $m$,
а кортеж множеств $X'$ является
множеством образующих диаграммы представлений $(f,A)$.
Следовательно, $X$ не является квазибазисом диаграммы представлений $(f,A)$.
\end{proof}

\begin{remark}
\labelRemark{X is quasibasis of diagram of representations}
Доказательство теоремы
\RefTheorem{X is quasibasis of diagram of representations}
даёт нам эффективный метод построения квазибазиса
диаграммы представлений $(f,A)$.
Квазибазис диаграммы представлений определён индукцией по диаграмме представлений.
Мы начинаем строить квазибазис в
$\Omega$\Hyph алгебрах из множества $A_{[0]}$.
Когда квазибазис построен в $\Omega$\Hyph алгебрах из множества $A_{[i]}$,
мы можем перейти к построению квазибазиса
в $\Omega$\Hyph алгебрах из множества $A_{[i+1]}$.
\qed
\end{remark}

Для каждого
\ShowEq{(k)=1n}
мы ввели $\Omega_{(k)}$\Hyph слово $A_{(k)}$\Hyph числа $x$ относительно множества образующих $X$
в определении\,\footnote{
Рассуждения в начале этого раздела естественно повторяют
рассуждения в начале раздела
\RefSection{Basis of representation}
и я сохранил эти рассуждения для полноты текста.
}
\RefDefinition{words of element, diagram of representations}.
Из теоремы
\RefTheorem{X is quasibasis of diagram of representations}
следует, что если множество образующих $X$ не является квазибазисом,
то выбор $\Omega_{(k)}$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является квазибазисом,
то представление $m\in A_{(k)}$ в виде $\Omega_{(k)}$\Hyph слова неоднозначно.

\begin{remark}
Существует три источника неоднозначности в записи
$\Omega_{(k)}$\Hyph слова.
\StartLabelItem
\begin{enumerate}
\item
В $\Omega_{(k)}$\Hyph алгебре $A_{(k)}$,
\ShowEq{(k)=(1n)},
могут быть определены равенства.
Например, если $e$ - единица мультипликативной группы $A_{(k)}$,
то верно равенство
\[ae=a\]
для любого $a\in A_{(k)}$.
\item
\begin{sloppypar}
Неоднозначность выбора $\Omega_{(k)}$\Hyph слова
может быть связана со свойствами представления.
Например,
допустим существует представление $f_{ik}$
$\Omega_i$\Hyph алгебры $A_i$ в $\Omega_k$\Hyph алгебре $A_k$.
Если $m_1$, ..., $m_n$ - $\Omega_k$\Hyph слова,
$\omega\in\Omega_k(n)$ и
$a$ - $\Omega_i$\Hyph слово,
то\,\footnote{
Например, пусть
$\{e_1,e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1ik}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1ik}
В тоже время, если $\omega$ является операцией
$\Omega_i$\Hyph алгебры $A_i$ и операцией
$\Omega_k$\Hyph алгебры $A_k$, то мы можем потребовать,
что $\Omega_k$\Hyph слова
\ShowEq{a1n omega x}
и
\ShowEq{a1n x omega}
описывают один и тот же
элемент $\Omega_k$\Hyph алгебры $A_k$.\,\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{diagram}
\end{sloppypar}
\item
Равенства вида
\EqRef{ambiguity of coordinates 1ik},
\eqRef{ambiguity of coordinates 2}{diagram}
сохраняются при морфизме диаграммы представлений.
Поэтому мы можем игнорировать эту
форму неоднозначности записи $\Omega_{(k)}$\Hyph слова.
Однако возможна принципиально другая форма неоднозначности,
пример которой можно найти
в теоремах
\RefTheorem{linear dependence between vectors of basis, module},
\RefTheorem{coordinates of vector with linear dependence, module}.
\end{enumerate}
Таким образом, мы видим, что на множестве $\Omega_{(k)}$\Hyph слов
можно определить различные отношения эквивалентности.\,\footnote{
Очевидно, что каждое из равенств
\EqRef{ambiguity of coordinates 1ik},
\eqRef{ambiguity of coordinates 2}{diagram}
порождает некоторое отношение эквивалентности.
}
Наша задача - найти максимальное отношение эквивалентности
на множестве $\Omega_{(k)}$\Hyph слов, которое
сохраняется при морфизме представления.

Аналогичное замечание касается отображения $W[f,X,m]$,
определённого в замечании
\RefRemark{coordinates of diagram of representations}.\,\footnote{Если базис
векторного пространства - конечен, то мы можем представить базис
в виде матрицы строки
\ShowEq{representation, vector space, basis}
Мы можем представить отображение $W[f,\Basis e](v)$
в виде матрицы столбца
\ShowEq{representation, vector space, coordinate}
Тогда
\ShowEq{representation, vector space, word}
имеет вид произведения матриц.
}
\qed
\end{remark}

\begin{theorem}
Пусть $X$ - квазибазис диаграммы представлений $(f,A)$.
Рассмотрим кортеж отношений эквивалентности
\ShowEq{lambda=(1n)}
\ShowEq{lk fX in w fX}
которое порождено исключительно следующими утверждениями.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX k}
Если в $\Omega_{(k)}$\Hyph алгебре $A_{(k)}$ существует равенство
\ShowEq{wk1=wk2}
определяющее структуру $\Omega_{(k)}$\Hyph алгебры, то
\ShowEq{wk1 wk2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
Если существует представление $f_{ik}$
и в $\Omega_i$\Hyph алгебре $A_i$ существует равенство
\ShowEq{wi1=wi2}
определяющее структуру $\Omega_i$\Hyph алгебры, то
\ShowEq{fwi1m fwi2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
Если существует представление $f_{ik}$,
то для любой операции
\ShowEq{omega n ari}{}in,
\ShowEq{(f(a1n)a2,f(a)a2) in lk}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
Если существует представление $f_{ik}$,
то для любой операции
\ShowEq{omega n ari}{}kn,
\ShowEq{(fa1(a21n),fa1(a2)) in lk}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Если существует представление $f_{ik}$,
\ShowEq{omega in O1AO2}ik{}
и представление $f_{ik}$ удовлетворяет равенству\,\footnote{
Рассмотрим представление коммутативного кольца $D$
в $D$\Hyph алгебре $A$. Мы будем пользоваться записью
\ShowEq{f(a)(v)=av}
В обеих алгебрах определены операции сложения и умножения.
Однако равенство
\ShowEq{f(a+b)v=}
верно, а равенство
\ShowEq{f(ab)v=}
является ошибочным.
}
\ShowEq{f(ai1n)a2=f(a)a2}
то мы можем предположить, что верно равенство
\ShowEq{(f(ai1n)a2,f(a)a2) in l 1}
\end{enumerate}
\end{theorem}

\begin{proof}
Теорема верна, так как рассмотренные равенства
сохраняются при гомоморфизмах
универсальных алгебр $A_{(k)}$.
\end{proof}

\begin{definition}
\labelDefinition{basis of diagram of representations}
Квазибазис $\Basis e$ диаграммы представлений $(f,A)$ такой, что
\ShowEq{rho=lambda}
называется
\AddIndex{базисом диаграммы представлений}{basis of diagram of representations}
$(f,A)$.
\qed
\end{definition}

\begin{remark}
Мы будем записывать базис также в виде 
\ShowEq{tuple of basis, diagram of representations}
\ShowEq{notation for basis of diagram of representations 1}
Если базис - конечный, то мы будем также пользоваться записью
\ShowEq{notation for basis of diagram of representations 2}
\qed
\end{remark}

\begin{theorem}
\labelTheorem{Automorphism of diagram of representations maps a basis into basis}
Автоморфизм диаграммы представлений $(f,A)$ отображает базис
диаграммы представлений $(f,A)$ в базис.
\end{theorem}
\begin{proof}
Пусть отображение $r$ - автоморфизм
диаграммы представлений $(f,A)$.
Пусть кортеж множеств $\Basis e$
- базис диаграммы представлений $(f,A)$.
Пусть\,\footnote{
Согласно определениям
\RefDefinition{left-side representation of group},
\RefDefinition{active representation in basis manifold, diagram of representations},
мы будем пользоваться записью
\ShowEq{r(e)=r o e}
}
\ShowEq{e'=r o e}
Допустим кортеж множеств $\Basis e'$ не является базисом.
Согласно теореме
\RefTheorem{X is quasibasis of diagram of representations}
существуют
\ShowEq{(k)=1n}
и
\ShowEq{e'ki in e'k}
такие, что кортеж множеств
\ShowEq{map of basis of diagram of representations, 1}
является множеством образующих
диаграммы представлений $(f,A)$.
Согласно теореме
\RefTheorem{group of automorphisms of diagram of representations}
отображение $r^{-1}$ является автоморфизмом
диаграммы представлений $(f,A)$.
Согласно теореме
\RefTheorem{Automorphism of diagram of representations is regular endomorphism}
и определению
\RefDefinition{regular endomorphism of diagram of representations},
кортеж множеств
\ShowEq{map of basis of diagram of representations, 2}
является множеством образующих
диаграммы представлений $(f,A)$.
Полученное противоречие доказывает теорему.
\end{proof}

\begin{theorem}
\labelTheorem{automorphism uniquely defined by image of basis, diagram of representations}
Пусть $\Basis e$ - базис диаграммы представлений $(f,A)$.
Пусть $(g,B)$ - диаграмма представлений.
Пусть
\ShowEq{f:A->B}R{\Basis e}Y
произвольное отображение кортежа множеств $\Basis e$,
\ShowEq{Yk in Bk}
Рассмотрим кортеж отображений
\ShowEq{map of words of diagram of representations, W}
удовлетворяющих условиям
\RefItem{map of words of diagram of representations, a in X},
\RefItem{map of words of diagram of representations, omega},
\RefItem{map of words of diagram of representations, am},
и такое, что
\ShowEq{map of words of diagram of representations, W in X}
Существует единственный морфизм диаграммы представлений\,\footnote{
Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{f:A->B}rAB
определённый правилом
\ShowEq{endomorphism r based on map of words of diagram of representations}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\RefTheorem{map of words of representation},
\RefTheorem{map of words of representation, 1}.
\end{proof}

\begin{corollary}
\labelCorollary{automorphism uniquely defined by image of basis, diagram of representations}
Пусть $\Basis e$, $\Basis e'$ - базисы представления $(f,A)$.
Пусть $r$ - автоморфизм представления $(f,A)$
такой, что
\ShowEq{e'=r o e}
Автоморфизм $r$ определён однозначно.
\qed
\end{corollary}

\begin{remark}
\labelRemark{automorphism uniquely defined by image of basis, diagram of representations}
Теорема \RefTheorem{automorphism uniquely defined by image of basis, diagram of representations},
так же как и
теорема \RefTheorem{map of words of diagram of representations, 1},
является теоремой о продолжении отображения.
Одако здесь $\Basis e$ - не произвольное множество образующих диаграммы представлений,
а базис.
Согласно замечанию
\RefRemark{X is quasibasis of diagram of representations},
мы не можем определить координаты любого элемента базиса
через остальные элементы этого же базиса.
Поэтому отпадает необходимость в согласованности отображения базиса с представлением.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{coordinates of identity transformation, diagram of representations}
Набор координат
\ShowEq{W[f,e,e]}
соответствует тождественному преобразованию
\ShowEq{identity transformation, representation}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{coordinates of identity transformation, representation}a
\end{proof}

\begin{theorem}
\labelTheorem{coordinates of inverse transformation, diagram of representations}
Пусть
\ShowEq{set of coordinates of automorphism}r{}
- множество координат автоморфизма $r$.
Определено множество координат
\ShowEq{set of coordinates of inverce automorphism}r,
соответствующее
автоморфизму $r^{-1}$. Множество координат
\ShowEq{set of coordinates of inverce automorphism}r{}
удовлетворяет равенству\,\footnote{
Смотри также замечание 
\RefRemark{coordinates of inverse transformation, representation}.}
\DrawEq[r]{coordinates of inverse transformation}{diagram of representations}
\ShowEq{coordinates of inverse transformation, a}r
\end{theorem}
\begin{proof}
Поскольку $r$ - автоморфизм диаграммы представлений $(f,A)$, то, согласно теореме
\RefTheorem{Automorphism of diagram of representations maps a basis into basis},
множество
\ShowEq{coordinates of endomorphism, 4, diagram of representations}
- базис диаграммы представлений $(f,A)$. Следовательно, определено
множество координат
\ShowEq{set of coordinates of inverce automorphism}r.
Равенство
\eqRef{coordinates of inverse transformation}{diagram of representations}
следует из цепочки равенств
\ShowEq{coordinates of inverse transformation, 1}r
\end{proof}

\ShowTheorem{coordinates of product of inverse transformation}{diagram of representations}rs
\ShowProof{coordinates of product of inverse transformation}{diagram of representations}rs

\begin{theorem}
Группа автоморфизмов $GA(f)$
диаграммы эффективных представлений $(f,A)$
порождает эффективное левостороннее представление
в диаграмме представлений $(f,A)$.
\end{theorem}
\begin{proof}
Из следствия
\RefCorollary{automorphism uniquely defined by image of basis, diagram of representations}
следует, что если автоморфизм $r$ отображает базис $\Basis e$ в базис $\Basis e'$,
то множество координат
\ShowEq{W[f,e,e']}
однозначно определяет автоморфизм $r$.
Из теоремы
\RefTheorem{map of coordinates of diagram of representations}
следует, что
множество координат
\ShowEq{W[f,e,e']}
определяет правило
отображения координат относительно
базиса $\Basis e$ при автоморфизме диаграммы представлений $(f,A)$.
Из равенства
\EqRef{superposition of coordinates, 6, diagram of representations}
следует, что автоморфизм $r$ действует слева на элементы
$\Omega_{(k)}$\Hyph алгебры $A_{(k)}$,
\ShowEq{(k)=(1n)}.
Из равенства
\EqRef{superposition of coordinates, 4, diagram of representations}
следует, что представление группы является левосторонним представлением.
Согласно теореме
\RefTheorem{coordinates of identity transformation, diagram of representations}
набор координат
\ShowEq{W[f,e,e]}
соответствует тождественному преобразованию.
Из теоремы
\RefTheorem{coordinates of inverse transformation, diagram of representations}
следует, что набор координат
\ShowEq{set of coordinates of inverce automorphism}r{}
соответствует преобразованию, обратному преобразованию
\ShowEq{set of coordinates of automorphism}r.
\end{proof}

\section{Многообразие базисов диаграммы представлений}

\ShowDefinition{basis manifold}{диаграммы представлений}{(f,A)}

\ShowDefinition{active representation in basis manifold}
{diagram of representations}{диаграммы представлений}{(f,A)}r

\ShowRemark{active representation}{diagram of representations}
{диаграммы представлений}{(f,A)}{диаграмма представлений}

\ShowTheorem{passive representation in basis manifold}{diagram of representations}
\ShowProof{passive representation in basis manifold}

\ShowTheorem{passive transformation}{diagram of representations}{диаграммы представлений}s
\ShowProof{passive transformation}{diagram of representations}

\ShowTheorem{passive transformation is automorphism of A(f)}{diagram of representations}
\ShowProof{passive transformation is automorphism of A(f)}

\ShowTheorem{select second basis of representation}rs{диаграммы представлений}{(f,A)}
\ShowProof{select second basis of representation}rs{diagram of representations}

\section{Геометрический объект диаграммы представлений}

\ShowRemark{active and passive transformation}
{диаграммы представлений}{кортеж $\Omega$\Hyph чисел}{кортежа $\Omega$\Hyph чисел}

\ShowTheorem{Coordinate transformation does not depend}
{diagram of representations}sa{кортежа $A$\Hyph чисел}
{кортеж $\Omega$\Hyph слов}{кортеж $A$\Hyph чисел}
\ShowProof{Coordinate transformation does not depend}{diagram of representations}sa

\ShowTheorem{Coordinate transformations form right-side representation}
{diagram of representations}{кортеже $\Omega$\Hyph алгебр}
\ShowProof{Coordinate transformations form right-side representation}{diagram of representations}sa
{диаграммы представлений}{$(F,W[f,\Basis e_1])$.}{(f,A)}
{кортеж $A$\Hyph чисел}t

Рассмотрим диаграммы представлени $(f,A)$, $(B,g)$.
\ShowRemark{geometric object}{diagram of representations}s{диаграмме представлений}{(B,g)}a

\ShowDefinition{coordinate of geometric object}{diagram of representations}sa
{диаграмме представлений}{(f,A)}

\ShowDefinition{geometric object}{diagram of representations}sa{диаграмме представлений}{(f,A)}
{кортеж $A$\Hyph чисел}{который}

\ShowRemark{2 views on geometric object}{diagram of representations}

\ShowTheorem{invariance principle}{diagram of representations}
\ShowProof{invariance principle}{diagram of representations}{диаграммы представлений}{(f,A)}{(B,g)}bs


==> Basis.Representation.Russian.tex <==
%auto-ignore
\input{Basis.Representation.Eq}

\chapter{Базис представления универсальной алгебры}
\labelChapter{Basis of Representation of Universal Algebra}

\section{Множество образующих представления}
\labelSection{generating set of representation}

\begin{definition}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
\qed
\end{definition}

Мы также будем говорить, что множество $A_2$
стабильно относительно представления $f$.

\begin{theorem}%
\labelTheorem{subrepresentation of representation}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением}{subrepresentation}
представления $f$.
\end{theorem}
\begin{proof}
Пусть $\omega_1$ - $n$\Hyph арная операция $\Omega_1$\Hyph алгебры $A_1$.
Тогда для любых
$a_1$, ..., $a_n\in A_1$
и любого $b\in B_2$
\ShowEq{representation of algebra A in algebra N, 1}
Пусть $\omega_2$ - $n$\Hyph арная операция $\Omega_2$\Hyph алгебры $A_2$.
Тогда для любых
$b_1$, ..., $b_n\in B_2$
и любого
\ShowEq{a in A1}{}
\ShowEq{representation of algebra A in algebra B, 2}
Утверждение теоремы доказано.
\end{proof}

Из теоремы \RefTheorem{subrepresentation of representation}
следует, что если $f_{B_2}$ - подпредставление представления $f$,
то отображение
\ShowEq{id:A->A B->A}
является морфизмом представлений.

\begin{theorem}%
\labelTheorem{lattice of subrepresentations}
Множество\,\footnote{
Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94).
Вообще говоря, в этой и последующих теоремах 
этой главы необходимо рассмотреть структуру универсальных алгебр
$A_1$ и $A_2$.
Так как основная задача этой главы -
это изучение структуры представления,
я сознательно упростил теоремы, чтобы детали не заслоняли
основные утверждения.
Более подробно эта тема будет раскрыта в главе
\RefChapter{Basis of Diagram of Representations of Universal Algebra},
где теоремы будут сформулированы в общем виде.
}
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
\end{theorem}
\begin{proof}
Пусть $(K_{\lambda})_{\lambda\in\Lambda}$
- семейство подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
стабильных относительно представления $f$.
Операцию пересечения на множестве $\mathcal B_f$
мы определим согласно правилу
\ShowEq{set of subrepresentations, intersection}
Операция пересечения подпредставлений определена корректно.
$\cap K_{\lambda}$ - подалгебра
$\Omega_2$\Hyph алгебры $A_2$.
Пусть $m\in \cap K_{\lambda}$.
%Если $K$ и $L$ - стабильные множества представления, то
Для любого $\lambda\in\Lambda$ и для любого
\ShowEq{a in A1},
$f(a)(m)\in K_{\lambda}$.
Следовательно, $f(a)(m)\in\cap K_{\lambda}$.
Следовательно, $\cap K_{\lambda}$ - стабильное множество представления $f$.
\end{proof}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.

\ShowTheorem{structure of subrepresentations}
\begin{proof}
Если положим $U=\cup X_k$, то по определению $X_k$
имеем
\EqParm{X subset JX}{i=0,=c}
и если
\EqParm{X subset JX}{i=k,=c}
то
\EqParm{X subset JX}{i=k+1,=.}
По индукции следует, что
\EqParm{X subset JX}{i=k,=z}
для всех $k$.
Следовательно,
\ShowEq{structure of subrepresentations, U subset J_f}

Если $a\in U^n$, $a=(a_1,...,a_n)$, где $a_i\in X_{k_i}$, и
если $k=\max \{k_1,...,k_n\}$, то
\ShowEq{structure of subrepresentations, 2}
Следовательно,
$U$ является подалгеброй $\Omega_2$\Hyph алгебры $A_2$.

Если $m\in U$, то $m\in X_k$ для некоторого $k$. Следовательно,
$f(a)(m)\in X_{k+1}\subset U$ для любого
\ShowEq{a in A1}.
Следовательно, $U$ - стабильное множество представления $f$.

Так как $U$ - подалгебра $\Omega_2$\Hyph алгебры $A_2$
и стабильное множество представления $f$,
то определено подпредставление $f_U$.
Следовательно,
\ShowEq{structure of subrepresentations, J_f subset U}
Из \EqRef{structure of subrepresentations, U subset J_f},
\EqRef{structure of subrepresentations, J_f subset U},
следует $J[f,X]=U$.
\end{proof}

\begin{definition}
\labelDefinition{generating set of representation}
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением}{subrepresentation},
порождённым множеством $X$,
а $X$ -
множеством образующих
подпредставления $J[f,X]$.
В частности,
\AddIndex{множеством образующих}{generating set}
представления $f$
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
\qed
\end{definition}

Следующее определение
является следствием теоремы
\RefTheorem{structure of subrepresentations}.

\begin{definition}
\labelDefinition{word of element relative to set, representation}
Пусть $X\subset A_2$.
Для любого
\ShowEq{x in JX}m{}
существует
\AddIndex{$\Omega_2$\Hyph слово}
{word of element relative to generating set, representation}
\ShowEq{word of element relative to generating set, representation},
определённое согласно следующему правилам.
\StartLabelItem
\begin{enumerate}
\item Если $m\in X$, то $m$ - $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, m in X}
\item Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова и
$\omega\in\Omega_2(n)$, то $m_1...m_n\omega$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, omega}
\item Если $m$ - $\Omega_2$\Hyph слово и
\ShowEq{a in A1},
то $f(a)(m)$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, am}
\end{enumerate}
Мы будем отождествлять элемент
\ShowEq{x in JX}m{}
и соответствующее ему $\Omega_2$\Hyph слово, выражая это равенством
\ShowEq{identify element jf(X) and word}
Аналогично, для произвольного множества
\ShowEq{subset of representation}{}
рассмотрим множество $\Omega_2$\Hyph слов\,\footnote{Выражение $\wXm$
является частным случаем
выражения $\wXm[B]$, а именно
\ShowEq{subset of words of representation, 2}
}
\ShowEq{subset of words of representation}
Мы будем также пользоваться записью
\ShowEq{subset of words of representation, 1}
Обозначим
\ShowEq{word set of representation}
\AddIndex{множество $\Omega_2$\Hyph слов представления $J[f,X]$}
{word set of representation}.
\qed
\end{definition}

\begin{theorem}
$w[f,X,X]=X$.
\end{theorem}

\begin{proof}
Теорема является следствием утверждения
\RefItem{word of element relative to set, representation, m in X}.
\end{proof}

\begin{theorem}
Пусть $X$, $Y$ - множества образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Пусть $\wXm$ - $\Omega_2$\Hyph слово $A_2$\Hyph числа $m$
относительно множества образующих $X$.
Пусть $\wYm[X]$ - множество $\Omega_2$\Hyph слов множества $X$
относительно множества образующих $Y$.
Если в слове $\wXm$
вместо каждого $x\in X$ подставить его образ
$\wYm[x]$,
то
мы получим $\Omega_2$\Hyph слово
$\wYm$ $A_2$\Hyph числа $m$
относительно множества образующих $Y$.

Преобразование $\Omega_2$\Hyph слов
\ShowEq{wXm->wYm}m
\ShowEq{wYm=...wXm}
называется суперпозицией координат.
\end{theorem}

\begin{proof}
Мы будем доказывать теорему индукцией по сложности
$\Omega_2$\Hyph слова.

Если $m\in X$, то 
\ShowEq{map of words of representation, w(m)=m}.
Если вместо $m$ подставить его образ
$\wYm$,
то мы получим $\Omega_2$\Hyph слово
$\wYm$ $A_2$\Hyph числа $m$
относительно множества образующих $Y$.

Пусть $\Omega_2$\Hyph слово
$\wXm$ $A_2$\Hyph числа $m$
имеет вид
\ShowEq{wXm=wXm1n o}
где
\ShowEq{omega n ari}{}2n{}
и для каждого $A_2$\Hyph числа $m_i$ мы определили отображение
\ShowEq{wXm->wYm}{m_i}
Согласно утверждению
\RefItem{word of element relative to set, representation, omega}
выражение
\ShowEq{wYm1n o}
является $\Omega_2$\Hyph словом
$\wYm$ $A_2$\Hyph числа $m$
относительно множества образующих $Y$.
Следовательно, мы определили отображение
\ShowEq{wXm->wYm}{m}
для $A_2$\Hyph числа $m$.

Пусть $\Omega_2$\Hyph слово
$\wXm$ $A_2$\Hyph числа $m$
имеет вид
\ShowEq{wXm=fa wXm1}
где для $A_2$\Hyph числа $m_1$ мы определили отображение
\ShowEq{wXm->wYm}{m_1}
Согласно утверждению
\RefItem{word of element relative to set, representation, am}
выражение
\ShowEq{fa wYm1}
является $\Omega_2$\Hyph словом
$\wYm$ $A_2$\Hyph числа $m$
относительно множества образующих $Y$.
Следовательно, мы определили отображение
\ShowEq{wXm->wYm}{m}
для $A_2$\Hyph числа $m$.
\end{proof}

Выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Поэтому, если $\Omega_2$\Hyph число имеет различные
$\Omega_2$\Hyph слова, то мы, чтобы их отличать, будем пользоваться индексами:
\ShowEq{w w1 w2[fXm]}

\begin{definition}
\labelDefinition{equivalence on the set of Omega2-words}
Множество образующих $X$ представления $f$
порождает отношение эквивалентности
\ShowEq{rho fX=}
на множестве $\Omega_2$\Hyph слов.
\qed
\end{definition}

Согласно определению
\RefDefinition{equivalence on the set of Omega2-words},
два $\Omega_2$\Hyph слова относительно
множества образующих $X$ представления $f$
эквивалентны тогда и только тогда, когда
они соответствуют одному и тому же $A_2$\Hyph числу.
Когда мы будем записывать равенство
двух $\Omega_2$\Hyph слов относительно
множества образующих $X$ представления $f$,
мы будем иметь в виду, что это равенство верно
с точностью до отношения эквивалентности
\ShowEq{rho fX}

\begin{theorem}
\labelTheorem{map of words of representation}
\ShowEq{Let A->*AB2 be representations}
Пусть $X$ - множество образующих представления $f$.
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления\,\footnote{
Я рассмотрел морфизм представления в теореме
\RefTheorem{map of words of diagram of representations}.
}
и $X'=R(X)$.
Приведенный морфизм $R$ представления
порождает отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation}
такое, что
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of words of representation, m in X, 1}
то
\ShowEq{map of words of representation, m in X}
\item Если
\ShowEq{map of words of representation, omega, 1}
то для операции
$\omega\in\Omega_2(n)$ справедливо
\ShowEq{map of words of representation, omega}
\item Если
\ShowEq{map of words of representation, am, 1}
то
\ShowEq{map of words of representation, am}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждения
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega}
справедливы в силу определения приведенного морфизма $R$.
Утверждение
\RefItem{map of words of representation, am}
является следствием равенства
\eqRef{reduced morphism representation =}{definition}.
\end{proof}

\begin{remark}
\labelRemark{coordinates of representation}
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления.
Пусть
\ShowEq{map of words of representation 1}
Теорема
\RefTheorem{map of words of representation}
утверждает, что
\ShowEq{map of words of representation 2}
Теорема
\RefTheorem{map of words of representation}
также утверждает, что
$\Omega_2$\Hyph слово, представляющее $m$, относительно $X$ и
$\Omega_2$\Hyph слово, представляющее $m'$, относительно $X'$
формируются согласно одному и тому же алгоритму.
Это позволяет рассматривать множество $\Omega_2$\Hyph слов $w[g,X',m']$
как отображение
\ShowEq{coordinates of element relative to generating set}{}m
\DrawEq[{}m]{coordinates of representation 3 fg}{representation}
где
\ShowEq{coordinates of representation 4}
для некоторого приведенного морфизма $R$.

Если $f=g$, то вместо отображения
\eqRef{coordinates of representation 3 fg}{representation}
мы будем рассматривать отображение
\ShowEq{coordinates of representation 3}
такое, что, если для некоторого эндоморфизма $R$ 
\ShowEq{coordinates of representation 4}
то
\ShowEq{coordinates of representation 5}

Отображение
$\ShowSymbol{coordinates relative to set}{}$
называется
\AddIndex{координатами $A_2$\Hyph числа $m$}{coordinates relative to set}
относительно множества $X$.
Аналогично, мы можем рассмотреть координаты множества
\ShowEq{subset of representation}{}
относительно множества $X$
\ShowEq{subset of coordinates of representation}{}m
Обозначим
\ShowEq{coordinate set of representation}{}m
\AddIndex{множество координат представления $J[f,X]$}
{coordinate set of representation}.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{set of coordinates, representation, omega}
На множестве координат $W[f,X]$ определена структура $\Omega_2$\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть $\omega\in\Omega_2(n)$. Тогда для любых
\ShowEq{set of coordinates, 1, omega}
положим
\ShowEq{set of coordinates, omega}
Согласно замечанию
\ref{remark: coordinates of representation},
из равенства
\EqRef{set of coordinates, omega}
следует
\ShowEq{set of coordinates, 2, omega}
Согласно правилу
\RefItem{word of element relative to set, representation, omega},
из равенства
\EqRef{set of coordinates, 2, omega}
следует
\ShowEq{set of coordinates, 3, omega}
Из равенства
\EqRef{set of coordinates, 3, omega}
следует корректность определения
\EqRef{set of coordinates, omega}
операции $\omega$ на множестве координат.
\end{proof}

\begin{theorem}
\labelTheorem{set of coordinates, representation, am}
Определено представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $W[f,X]$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{a in A1}.
Тогда для любого
\ShowEq{x in JX}m{}
положим
\ShowEq{set of coordinates, am}
Согласно замечанию
\ref{remark: coordinates of representation},
из равенства
\EqRef{set of coordinates, am}
следует
\ShowEq{set of coordinates, 2, am}
Согласно правилу
\RefItem{word of element relative to set, representation, am},
из равенства
\EqRef{set of coordinates, 2, am}
следует
\ShowEq{set of coordinates, 3, am}
Из равенства
\EqRef{set of coordinates, 3, am}
следует корректность определения
\EqRef{set of coordinates, am}
представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $W[f,X]$.
\end{proof}

\begin{theorem}
\labelTheorem{map of words of representation, 1}
\ShowEq{Let A->*AB2 be representations}
Для заданных множеств $X\subset A_2$, $X'\subset B_2$,
пусть отображение
\ShowEq{R1 X->}X
согласовано со структурой представления $f$,
т. е.
\ShowEq{map of words of representation, 1}
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}X
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}xX
Существует единственное отображение
\ShowEq{f:A->B}R{A_2}{B_2}
определённое правилом
\ShowEq{endomorphism based on map of words of representation}X
которое является приведенным морфизмом представлнений
$J[f,X]$ и $J[g,X']$.
\end{theorem}
\begin{proof}
Мы будем доказывать теорему индукцией по сложности
$\Omega_2$\Hyph слова.

Если
\ShowEq{map of words of representation, w(m)=m},
то $m\in X$.
Согласно условию
\RefItem{map of words of representation, m in X},
\ShowEq{map of words of representation, R(m)=R1(m)}
Следовательно, на множестве $X$ отображения $R$ и $R_1$ совпадают,
и отображение $R$ согласовано со структурой представления $f$.

Пусть $\omega\in\Omega_2(n)$.
Пусть отображение $R$ определено для
\ShowEq{m1n in JX}
Пусть
\ShowEq{coordinates of representation, omega, 2}
Если $m=m_1...m_n\omega$, то согласно правилу
\RefItem{word of element relative to set, representation, omega},
\ShowEq{coordinates of representation, omega}
Согласно условию
\RefItem{map of words of representation, omega},
\ShowEq{coordinates of representation, omega, 1}
Следовательно, отображение $R$ является эндоморфизмом
$\Omega_2$\Hyph алгебры $A_2$.

Пусть отображение $R$ определено для
\ShowEq{map of words of representation, a, m, 1}
Пусть
\ShowEq{a in A1}.
Если $m=f(a)(m_1)$, то согласно правилу
\RefItem{word of element relative to set, representation, am},
\ShowEq{map of words of representation, a, m, 2}
Согласно условию
\RefItem{map of words of representation, am},
\ShowEq{map of words of representation, a, m, 3}
Из равенства
\eqRef{morphism of representations of universal algebra, 2m}{definition}
следует, что отображение $R$ является морфизмом представления $f$.

Единственность эндоморфизма $R$,
а следовательно, корректность
его определения,
следует из следующего рассуждения.
Допустим, $m\in A_2$ имеет различные $\Omega_2$\Hyph слова относительно множества $X$,
например
\ShowEq{unique endomorphism, 1}
Так как $R$ - эндомоморфизм представления, то из равенства
\EqRef{unique endomorphism, 1}
следует
\ShowEq{unique endomorphism, 2}
Из равенства
\EqRef{unique endomorphism, 2}
следует
\ShowEq{unique endomorphism, 3}
Из равенств
\EqRef{unique endomorphism, 1},
\EqRef{unique endomorphism, 3}
следует, что равенство
\EqRef{unique endomorphism, 1}
сохраняется при отображении. Следовательно, образ $A_2$
не зависит от выбора координат.
\end{proof}

\begin{remark}
\labelRemark{coordinates of representation, 1}
Теорема \RefTheorem{map of words of representation, 1}
- это теорема о продолжении отображения.
Единственное, что нам известно о множестве $X$ - это то, что
$X$ - множество образующих представления $f$.
Однако, между элементами множества $X$ могут существовать соотношения,
порождённые либо операциями $\Omega_2$\Hyph алгебры $A_2$, либо
преобразованиями представления $f$.
Поэтому произвольное отображение множества $X$, вообще говоря,
не может быть продолжено до приведенного морфизма представления $f$.\,\footnote{В теореме
\RefTheorem{automorphism uniquely defined by image of basis},
требования к множеству образующих более жёсткие. Поэтому теорема
\RefTheorem{automorphism uniquely defined by image of basis}
говорит о продолжении произвольного отображения.
Более подробный анализ дан в замечании
\ref{remark: automorphism uniquely defined by image of basis}.}
Однако, если отображение $R_1$ согласованно со структурой представления на
множестве $X$, то мы можем построить продолжение этого отображения,
которое является приведенным морфизмом представления $f$.
\qed
\end{remark}

\begin{sloppypar}
\begin{definition}
\labelDefinition{coordinates of endomorphism of representation}
\ShowEq{Let XY be generating sets}
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления $f$.
Множество координат
\ShowEq{coordinates of endomorphism, 2, representation}
называется
\AddIndex{координатами приведенного морфизма представления}
{coordinates of reduced morphism of representation}.
\qed
\end{definition}
\end{sloppypar}

\ifx\texFuture\Defined
\begin{theorem}
\ShowEq{Let XY be generating sets}
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления
и $X'=R(X)$.
\end{theorem}

\begin{proof}
\end{proof}
\fi

Из определений
\RefDefinition{word of element relative to set, representation},
\RefDefinition{coordinates of endomorphism of representation}
следует, что
\ShowEq{W[RoX]=}
Пусть $m\in A_2$.
Если в слове $\wXm$
вместо каждого $x\in X$ подставить его образ
\ShowEq{image of generating set, morphism},
то,
согласно теореме
\RefTheorem{map of words of representation, 1},
мы получим $\Omega_2$\Hyph слово
\ShowEq{image of word, morphism}
Из этого утверждения
следует определение
\RefDefinition{superposition of coordinates, representation}.

\begin{definition}
\labelDefinition{superposition of coordinates, representation}
\ShowEq{Let XY be generating sets}
Пусть $R$
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления $f$.
Пусть $m\in A_2$.
Мы определим
\AddIndex{суперпозицию координат}{superposition of coordinates}
приведенного морфизма $R$ представления $f$ и $A_2$\Hyph числа $m$
как координаты, определённые согласно правилу
\ShowEq{superposition of coordinates, representation}
\ShowEq{superposition of coordinates of representation}
Мы определим
суперпозицию координат
приведенного морфизма $R$ представления $f$ и множества $B\subseteq A_2$
согласно правилу
\ShowEq{superposition of coordinates, 1, representation}
\ShowEq{superposition of coordinates, 5, representation}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map of coordinates of representation}
\ShowEq{Let XY be generating sets}
Приведенный морфизм представления
\ShowEq{f:A->B}R{A_2}{B_2}
порождает отображение координат представления
\ShowEq{map of coordinates of representation}
такое, что
\ShowEq{map of coordinates of representation, 1}
\end{theorem}
\begin{proof}
Согласно замечанию
\ref{remark: coordinates of representation},
мы можем рассматривать равенства
\EqRef{superposition of coordinates of representation},
\EqRef{map of coordinates of representation}
относительно заданных множеств образующих $X$, $Y$.
При этом координатам $W[f,X,m]$
соответствует слово
\ShowEq{map of coordinates of representation, 2}
а координатам $W[g,Y,R(m)]$
соответствует слово
\ShowEq{map of coordinates of representation, 3}
Поэтому для того, чтобы доказать теорему,
нам достаточно показать, что отображению $W[f,X,R]$
соответствует отображение $w[f,X,R]$.
Мы будем доказывать это утверждение индукцией по сложности
$\Omega_2$\Hyph слова.

Если
\ShowEq{map of words of representation, m in X, 1}
то, согласно равенствам
\EqRef{map of coordinates of representation, 2},
\EqRef{map of coordinates of representation, 3},
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы.

Пусть для
\ShowEq{superposition of coordinates, representation, omega, 1}
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы.
Пусть $\omega\in\Omega_2(n)$.
Согласно теореме
\RefTheorem{set of coordinates, representation, omega}
\ShowEq{superposition of coordinates, representation, omega, 2}
Так как $R$ - эндоморфизм $\Omega_2$\Hyph алгебры $A_2$,
то из равенства
\EqRef{superposition of coordinates, representation, omega, 2}
следует
\ShowEq{superposition of coordinates, representation, omega, 3}
Из равенств
\EqRef{superposition of coordinates, representation, omega, 2},
\EqRef{superposition of coordinates, representation, omega, 3}
и предположения индукции следует, что
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы для $m=m_1...m_n\omega$.

Пусть для
$m_1\in A_2$
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы.
Пусть
\ShowEq{a in A1}.
Согласно теореме
\RefTheorem{set of coordinates, representation, am}
\ShowEq{superposition of coordinates, representation, am, 1}
Так как $R$ - эндоморфизм представления $f$,
то из равенства
\EqRef{superposition of coordinates, representation, am, 1}
следует
\ShowEq{superposition of coordinates, representation, am, 2}
Из равенств
\EqRef{superposition of coordinates, representation, am, 1},
\EqRef{superposition of coordinates, representation, am, 2}
и предположения индукции следует, что
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы для $m=f(a)(m_1)$.
\end{proof}

\begin{corollary}
\labelCorollary{map of coordinates of representation}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$ - эндоморфизм представления $f$.
Отображение $W[f,X,R]$ является эндоморфизмом представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре $W[f,X]$.
\qed
\end{corollary}

В дальнейшем мы будем отождествлять отображение $W[f,X,R]$
и множество координат $W[f,X,R\circ X]$.

\begin{theorem}
\labelTheorem{superposition of coordinates, representation}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$ - эндоморфизм представления $f$.
Пусть $Y\subset A_2$.
Тогда
\ShowEq{superposition of coordinates, 2, representation}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 2, representation}
является следствием равенства
\ShowEq{superposition of coordinates, 3, representation}
а также равенств
\EqRef{superposition of coordinates of representation},
\EqRef{superposition of coordinates, 1, representation}.
\end{proof}

\begin{theorem}
\labelTheorem{superposition of coordinates of endomorphisms, representation}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$, $S$ - эндоморфизмы представления $f$.
Тогда
\ShowEq{superposition of coordinates, 4, representation}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 4, representation}
следует из равенства
\EqRef{superposition of coordinates, 2, representation},
если положить $Y=\ScX$.
\end{proof}

Концепция суперпозиции координат очень проста
и напоминает своеобразную машину Тюринга.
Если элемент $m\in A_2$
имеет вид
\[m=m_1...m_n\omega\]
или
\[m=f(a)(m_1)\]
то мы ищем координаты элементов $m_i$, для того чтобы подставить
их в соответствующее выражение.
Как только элемент $m\in A_2$
принадлежит множеству образующих $\Omega_2$\Hyph алгебры $A_2$,
мы выбираем координаты соответствующего элемента из второго множителя.
Поэтому мы требуем, чтобы второй множитель в суперпозиции был
множеством координат образа множества образующих $X$.

Следующие формы записи образа множества $Y$
при эндоморфизме $R$ эквивалентны.
\ShowEq{superposition of coordinates, 6, representation}
Из равенств
\EqRef{superposition of coordinates, 2, representation},
\EqRef{superposition of coordinates, 6, representation}
следует, что
\ShowEq{superposition of coordinates, 7, representation}
Равенство
\EqRef{superposition of coordinates, 7, representation}
является законом ассоциативности для операции композиции и позволяет
записать выражение
\ShowEq{superposition of coordinates, 8, representation}
без использования скобок.

\begin{definition}
\labelDefinition{endomorphism of representation, regular on set}
Пусть $X\subset A_2$ - множество образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Пусть отображение
\ShowEq{f:A->B}H{A_2}{A_2}
является эндоморфизмом представления $f$.
Пусть множество $X'=H\circ X$ является образом множества $X$
при отображении $H$.
Эндоморфизм $H$ представления $f$ называется
невырожденным на множестве образующих $X$,
если множество $X'$ является множеством образующих представления $f$.
В противном случае, эндоморфизм $H$ представления $f$ называется
вырожденным на множестве образующих $X$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{regular endomorphism of representation}
Эндоморфизм представления $f$ называется
\AddIndex{невырожденным}{regular endomorphism},
если он невырожден на любом множестве образующих.
В противном случае, эндоморфизм $H$ представления $f$ называется
\AddIndex{вырожденным}{singular endomorphism}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Automorphism of representation is regular endomorphism}
Автоморфизм $R$ представления
\ShowEq{f:A->*B}f{A_1}{A_2}
является невырожденным эндоморфизмом.
\end{theorem}
\begin{proof}
Пусть $X$ - множество образующих представления $f$.
Пусть $X'=\RcX$.

Согласно теореме
\RefTheorem{map of words of representation}
эндоморфизм $R$
порождает отображение $\Omega_2$\Hyph слов
$\wXR$.

Пусть $m'\in A_2$. Так как $R$ - автоморфизм, то существует
$m\in A_2$, $R\circ m=m'$. Согласно определению
\RefDefinition{word of element relative to set, representation},
$\wXm$ - $\Omega_2$\Hyph слово,
представляющее $A_2$ относительно множества образующих $X$.
Согласно теореме
\RefTheorem{map of words of representation},
$w[f,X',m']$ - $\Omega_2$\Hyph слово,
представляющее $m'$ относительно множества образующих $X'$
\ShowEq{Automorphism of representation is regular endomorphism, 1}
Следовательно, $X'$ - множество образующих представления $f$.
Согласно определению
\RefDefinition{regular endomorphism of representation},
автоморфизм $R$ - невырожден.
\end{proof}
%\fi

\section{Базис представления}
\labelSection{Basis of representation}

\begin{definition}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
и
\ShowEq{Gen f =}
Если для множества $X\subset A_2$ верно
\ShowEq{in Gen}Xf,
то для любого множества $Y$, $X\subset Y\subset A_2$,
также верно
\ShowEq{in Gen}Yf.
Если существует минимальное множество
\ShowEq{in Gen}Xf,
то множество $X$ называется
\AddIndex{квазибазисом представления}{quasibasis of representation}
$f$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{X is quasibasis of representation}
Если множество $X$ является квазибазисом представления $f$,
то для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{theorem}
\begin{proof}
Пусть $X$ - квазибазис представления $f$.
Допустим для некоторого $m\in X$ существует $\Omega_2$\Hyph слово
\ShowEq{X is quasibasis of representation, 1}
Рассмотрим $A_2$\Hyph число $m'$, для
которого $\Omega_2$\Hyph слово
\ShowEq{X is quasibasis of representation, 2}
зависит от $m$.
Согласно определению
\RefDefinition{word of element relative to set, representation},
любое вхождение $A_2$\Hyph числа $m$ в $\Omega_2$\Hyph слово $w'$ может быть заменено
$\Omega_2$\Hyph словом $w$. Следовательно,
$\Omega_2$\Hyph слово $w'$ не зависит от $m$,
а множество $X\setminus\{m\}$ является
множеством образующих представления $f$.
Следовательно, $X$ не является квазибазисом расслоения $f$.
\end{proof}

\begin{remark}
\labelRemark{X is quasibasis of representation}
Доказательство теоремы
\RefTheorem{X is quasibasis of representation}
даёт нам эффективный метод построения квазибазиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить квазибазис этого представления.
\qed
\end{remark}

\ShowEq{=module}

Мы ввели $\Omega_2$\Hyph слово элемента $x\in A_2$ относительно множества образующих $X$
в определении
\RefDefinition{word of element relative to set, representation}.
Из теоремы
\RefTheorem{X is quasibasis of representation}
следует, что если множество образующих $X$ не является квазибазисом,
то выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является квазибазисом,
то представление $m\in A_2$ в виде $\Omega_2$\Hyph слова неоднозначно.

\begin{remark}
Существует три источника неоднозначности в записи
$\Omega_2$\Hyph слова.
\StartLabelItem
\begin{enumerate}
\item
В $\Omega_i$\Hyph алгебре $A_i$, $i=1$, $2$,
могут быть определены равенства.
Например, если $e$ - единица мультипликативной группы $A_i$,
то верно равенство
\[ae=a\]
для любого $a\in A_i$.
\item
\begin{sloppypar}
Неоднозначность выбора $\Omega_2$\Hyph слова
может быть связана со свойствами представления.
Например, если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова,
$\omega\in\Omega_2(n)$ и
\ShowEq{a in A1},
то\,\footnote{
Например, пусть
$\{e_1,e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1}
В тоже время, если $\omega$ является операцией
$\Omega_1$\Hyph алгебры $A_1$ и операцией
$\Omega_2$\Hyph алгебры $A_2$, то мы можем потребовать,
что $\Omega_2$\Hyph слова
\ShowEq{a1n omega x}
и
\ShowEq{a1n x omega}
описывают один и тот же
элемент $\Omega_2$\Hyph алгебры $A_2$.\,\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{representation}
\end{sloppypar}
\item
Равенства вида
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
сохраняются при морфизме представления.
Поэтому мы можем игнорировать эту
форму неоднозначности записи $\Omega_2$\Hyph слова.
Однако возможна принципиально другая форма неоднозначности,
пример которой можно найти
в теоремах
\RefTheorem{linear dependence between vectors of basis, \SideWS module},
\RefTheorem{coordinates of vector with linear dependence, \SideWS module}.
\end{enumerate}
Таким образом, мы видим, что на множестве $\Omega_2$\Hyph слов
можно определить различные отношения эквивалентности.\,\footnote{
Очевидно, что каждое из равенств
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
порождает некоторое отношение эквивалентности.
}
Наша задача - найти максимальное отношение эквивалентности
на множестве $\Omega_2$\Hyph слов, которое
сохраняется при морфизме представления.

Аналогичное замечание касается отображения $W[f,X,m]$,
определённого в замечании
\RefRemark{coordinates of representation}.\,\footnote{Если базис
векторного пространства - конечен, то мы можем представить базис
в виде матрицы строки
\ShowEq{representation, vector space, basis}
Мы можем представить отображение $W[f,\Basis e](v)$
в виде матрицы столбца
\ShowEq{representation, vector space, coordinate}
Тогда
\ShowEq{representation, vector space, word}
имеет вид произведения матриц.
}
\qed
\end{remark}

\begin{theorem}
Пусть $X$ - квазибазис представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Рассмотрим отношение эквивалентности
\ShowEq{l fX in w fX}
которое порождено исключительно следующими утверждениями.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX}
Если в $\Omega_2$\Hyph алгебре $A_2$ существует равенство
\ShowEq{w1=w2}
определяющее структуру $\Omega_2$\Hyph алгебры, то
\ShowEq{w1 w2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
Если в $\Omega_1$\Hyph алгебре $A_1$ существует равенство
\ShowEq{w1=w2}
определяющее структуру $\Omega_1$\Hyph алгебры, то
\ShowEq{fw1m fw2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
Для любой операции
\ShowEq{omega n ari}{}1n,
\ShowEq{(f(a1n)a2,f(a)a2) in l}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
Для любой операции
\ShowEq{omega n ari}{}2n,
\ShowEq{(fa1(a21n),fa1(a2)) in l}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Пусть
\ShowEq{omega in O1AO2}12.
Если представление $f$ удовлетворяет равенству\,\footnote{
Рассмотрим представление коммутативного кольца $D$
в $D$\Hyph алгебре $A$. Мы будем пользоваться записью
\ShowEq{f(a)(v)=av}
В обеих алгебрах определены операции сложения и умножения.
Однако равенство
\ShowEq{f(a+b)v=}
верно, а равенство
\ShowEq{f(ab)v=}
является ошибочным.
}
\ShowEq{f(a1n)a2=f(a)a2}
то мы можем предположить, что верно равенство
\ShowEq{(f(a1n)a2,f(a)a2) in l 1}
\end{enumerate}
\end{theorem}

\begin{proof}
Теорема верна, так как рассмотренные равенства
сохраняются при гомоморфизмах
универсальных алгебр $A_1$ и $A_2$.
\end{proof}

\begin{definition}
\labelDefinition{basis of representation}
Квазибазис $\Basis e$ представления $f$ такой, что
\ShowEq{rho=lambda}
называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{definition}

\begin{remark}
Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}

\begin{remark}
Мы будем записывать базис также в виде 
\ShowEq{notation for basis of representation 1}
Если базис - конечный, то мы будем также пользоваться записью
\ShowEq{notation for basis of representation 2}
\qed
\end{remark}

\begin{theorem}
\labelTheorem{Automorphism of representation maps a basis into basis}
Автоморфизм представления $f$ отображает базис
представления $f$ в базис.
\end{theorem}
\begin{proof}
Пусть отображение $R$ - автоморфизм представления $f$.
Пусть множество $\Basis e$ - базис представления $f$.
Пусть\,\footnote{
Согласно определениям
\RefDefinition{left-side representation of group},
\RefDefinition{active representation in basis manifold, representation},
мы будем пользоваться записью
\ShowEq{R(e)=Roe}
}
\ShowEq{e'=Roe}
Допустим множество $\Basis e'$ не является базисом.
Согласно теореме
\RefTheorem{X is quasibasis of representation}
существует
\ShowEq{in basis 1}
такое, что
\ShowEq{in basis 2}
является множеством образующих представления $f$.
Согласно теореме
\RefTheorem{group of automorphisms of representation}
отображение $R^{-1}$ является автоморфизмом представления $f$.
Согласно теореме
\RefTheorem{Automorphism of representation is regular endomorphism}
и определению
\RefDefinition{regular endomorphism of representation},
множество
\ShowEq{in basis 3}
является множеством образующих
представления $f$.
Полученное противоречие доказывает теорему.
\end{proof}

\begin{theorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $\Basis e$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}{\Basis e}
произвольное отображение множества $X$.
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}{\Basis e}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}e{\Basis e}
Существует единственный эндоморфизм представлнения $f$\,\footnote{Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}{\Basis e}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\RefTheorem{map of words of representation},
\RefTheorem{map of words of representation, 1}.
\end{proof}

\begin{corollary}
\labelCorollary{automorphism uniquely defined by image of basis, representation}
Пусть $\Basis e$, $\Basis e'$ - базисы представления $f$.
Пусть $R$ - автоморфизм представления $f$
такой, что
\ShowEq{e'=Roe}
Автоморфизм $R$ определён однозначно.
\qed
\end{corollary}

\begin{remark}
\labelRemark{automorphism uniquely defined by image of basis}
Теорема \RefTheorem{automorphism uniquely defined by image of basis},
так же как и
теорема \RefTheorem{map of words of representation, 1},
является теоремой о продолжении отображения.
Однако здесь $\Basis e$ - не произвольное множество образующих представления,
а базис.
Согласно замечанию
\RefRemark{X is quasibasis of representation},
мы не можем определить координаты любого элемента базиса
через остальные элементы этого же базиса.
Поэтому отпадает необходимость в согласованности отображения базиса с представлением.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{coordinates of identity transformation, representation}
Набор координат
\ShowEq{W[f,e,e]}
соответствует тождественному преобразованию
\ShowEq{identity transformation, representation}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{coordinates of identity transformation, representation}m
\end{proof}

\begin{theorem}
\labelTheorem{coordinates of inverse transformation, representation}
Пусть
\ShowEq{set of coordinates of automorphism}R{}
- множество координат автоморфизма $R$.
Определено множество координат
\ShowEq{set of coordinates of inverce automorphism}R,
соответствующее
автоморфизму $R^{-1}$. Множество координат
\ShowEq{set of coordinates of inverce automorphism}R{}
удовлетворяют равенству
\DrawEq[R]{coordinates of inverse transformation}{representation}
\ShowEq{coordinates of inverse transformation, a}R
\end{theorem}
\begin{proof}
Поскольку $R$ - автоморфизм представления $f$, то, согласно теореме
\RefTheorem{Automorphism of representation maps a basis into basis},
множество $\Rce$ - базис представления $f$. Следовательно, определено
множество координат
\ShowEq{set of coordinates of inverce automorphism}R.
Равенство
\eqRef{coordinates of inverse transformation}{representation}
следует из цепочки равенств
\ShowEq{coordinates of inverse transformation, 1}R
\end{proof}

\begin{remark}
\labelRemark{coordinates of inverse transformation, representation}
В $\Omega_2$\Hyph алгебре $A_2$ не существует универсального алгоритма
определения множества координат
\ShowEq{set of coordinates of inverce automorphism}R{}
для заданного множества
\ShowEq{set of coordinates of automorphism}R.\,\footnote{В векторном пространстве линейному преобразованию
соответствует матрица чисел. Соответственно, обратному преобразованию
соответствует обратная матрица.
}
Мы полагаем, что в теореме
\RefTheorem{coordinates of inverse transformation, representation}
этот алгоритм задан неявно.
Очевидно также, что множество $\Omega_2$\Hyph слов
\ShowEq{coordinates of inverse transformation, 2, representation}
вообще говоря, не совпадает с множеством $\Omega_2$\Hyph слов
\ShowEq{coordinates of inverse transformation, 3, representation}
Теорема
\RefTheorem{coordinates of inverse transformation, representation}
утверждает, что множества $\Omega_2$\Hyph слов
\EqRef{coordinates of inverse transformation, 2, representation}
и
\EqRef{coordinates of inverse transformation, 3, representation}
совпадают с точностью до отношения эквивалентности, порождённой представлением $f$.
\qed
\end{remark}

\ShowTheorem{coordinates of product of inverse transformation}{representation}RS
\ShowProof{coordinates of product of inverse transformation}{representation}RS

\begin{theorem}
Группа автоморфизмов $GA(f)$ эффективного представления $f$
в $\Omega_2$\Hyph алгебре $A_2$ порождает эффективное левостороннее представление
в $\Omega_2$\Hyph алгебре $A_2$.
\end{theorem}
\begin{proof}
Из следствия
\RefCorollary{automorphism uniquely defined by image of basis, representation}
следует, что если автоморфизм $R$ отображает базис $\Basis e$ в базис $\Basis e'$,
то множество координат $W[f,\Basis e,\Basis e']$ однозначно определяет автоморфизм $R$.
Из теоремы
\RefTheorem{map of coordinates of representation}
следует, что
множество координат
\ShowEq{W[f,e,e']}
определяет правило
отображения координат относительно
базиса $\Basis e$ при автоморфизме представления $f$.
Из равенства
\EqRef{superposition of coordinates, 6, representation}
следует, что автоморфизм $R$ действует слева на элементы
$\Omega_2$\Hyph алгебры $A_2$.
Из равенства
\EqRef{superposition of coordinates, 4, representation}
следует, что представление группы является левосторонним представлением.
Согласно теореме
\RefTheorem{coordinates of identity transformation, representation}
набор координат $W[f,\Basis e,\Basis e]$
соответствует тождественному преобразованию.
Из теоремы
\RefTheorem{coordinates of inverse transformation, representation}
следует, что набор координат
\ShowEq{set of coordinates of inverce automorphism}R{}
соответствует преобразованию, обратному преобразованию
\ShowEq{set of coordinates of automorphism}R.
\end{proof}

\section{Свободное представление}

В разделе
\RefSection{Representation of Universal Algebra}
мы рассмотрели определение
\RefDefinition{free representation of algebra}
свободного представления.
Однако мы можем рассмотреть другое определение,
которое аналогично определению свободного модуля.

\begin{definition}
\labelDefinition{free representation has basis}
Представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется свободным, если это представление имеет базис.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{free has basis -> free representation}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
свободное представление согласно определению
\RefDefinition{free representation has basis}.
Тогда представление $f$ свободно согласно определению
\RefDefinition{free representation of algebra}.
\end{theorem}

\begin{proof}
Пусть $\Basis e$ - базис представления $f$
и $m\in\Basis e$.
Пусть существуют $A_1$\Hyph числа $a_1$, $b_1$ такие, что
$f(a_1)=f(b_1)$.
Согласно предположению
$f(a_1)(m)=f(b_1)(m)$.
Однако, если $a_1\ne b_1$, то
$f(a_1)(m)$ и $f(b_1)(m)$
различные $\Omega_2$\Hyph слова.
Следовательно, $\Basis e$ не является базисом.
Из полученного противоречия следует, что $a_1=b_1$.
Следовательно представление $f$ свободно согласно определению
\RefDefinition{free representation of algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{free representation -> free has basis}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
свободное представление согласно определению
\RefDefinition{free representation of algebra}.
Тогда представление $f$ свободно согласно определению
\RefDefinition{free representation has basis}.
\end{theorem}

%\begin{proof}
%\end{proof}

\begin{question}
Очень важно найти доказательство теоремы
\RefTheorem{free representation -> free has basis}
или найти пример, когда эта теорема не верна.
Мы увидим в главе
\RefChapter{Diagram of Representations of Universal Algebras}
какую роль играет свободное представление согласно определению
\RefDefinition{free representation has basis}.
Так как в дальнейшем я буду предполагать,
что представление всегда имеет базис,
то в рамках этой книги я могу ограничиться теоремой
\RefTheorem{free has basis -> free representation}.
\qed
\end{question}

\section{Многообразие базисов представления}
\labelSection{Basis Manifold of Representation}

\ShowDefinition{basis manifold}{представления}f

\ShowDefinition{active representation in basis manifold}
{representation}{представления}fR

\ShowRemark{active representation}{representation}{представления}f{представление}

\ShowTheorem{passive representation in basis manifold}{representation}
\ShowProof{passive representation in basis manifold}

\ShowTheorem{passive transformation}{representation}{представления}S
\ShowProof{passive transformation}{representation}

\ShowTheorem{passive transformation is automorphism of A(f)}{representation}
\ShowProof{passive transformation is automorphism of A(f)}

\ShowTheorem{select second basis of representation}RS{представления}f
\ShowProof{select second basis of representation}RS{representation}

\section{Геометрический объект представления универсальной алгебры}
\labelSection{Geometric Object of Representation of Universal Algebra}

\ShowRemark{active and passive transformation}
{представления}{$\Omega_2$\Hyph число}{$\Omega_2$\Hyph числа}

\ShowTheorem{Coordinate transformation does not depend}{representation}Sm{$A_2$\Hyph числа}
{$\Omega_2$\Hyph слово}{$A_2$\Hyph число}
\ShowProof{Coordinate transformation does not depend}{representation}Sm

\ShowTheorem{Coordinate transformations form right-side representation}
{representation}{$\Omega_2$\Hyph алгебре}
\ShowProof{Coordinate transformations form right-side representation}{representation}Sm
{представления}
{\ShowEq{f:A->*B}f{A_1}{W[f,\Basis e_1]}}f{$A_2$\Hyph число}T

Пусть $f$ - представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $g$ - представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_3$\Hyph алгебре $A_3$.
\ShowRemark{geometric object}{representation}S{представлении}gm

\ShowDefinition{coordinate of geometric object}{representation}Sm
{представлении}f

\ShowDefinition{geometric object}{representation}Sm{представлении}f{$A_2$\Hyph число}{которое}

\ShowRemark{2 views on geometric object}{representation}

\ShowTheorem{invariance principle}{representation}
\ShowProof{invariance principle}{representation}{представления}fgnS

\begin{theorem}
Множество геометрических объектов типа $H$
является $\Omega_3$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{geometric object, 1, omega}
Для операции
\ShowEq{geometric object, 2, omega}
мы положим
\ShowEq{geometric object, 3, omega}
Так как отображение
\ShowEq{W[g,eN,eNHS]}
для произвольного эндоморфизма $S$ $\Omega_2$\Hyph алгебры $A_2$ является эндоморфизмом
$\Omega_3$\Hyph алгебры $A_3$, то определение
\EqRef{geometric object, 3, omega}
корректно.
\end{proof}

\begin{theorem}
Определено представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_3$\Hyph алгебре $N$ геометрических объектов типа $H$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{geometric object, 1, am}
Для
\ShowEq{a in A1},
мы положим
\ShowEq{geometric object, 3, am}
Так как отображение
\ShowEq{W[g,eN,eNHS]}
для произвольного эндоморфизма $S$ $\Omega_2$\Hyph алгебры $A_2$
является эндоморфизмом
представления $g$, то определение
\EqRef{geometric object, 3, am}
корректно.
\end{proof}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\BiblioItem{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}%

\BiblioItem{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}%

\BiblioItem{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\BiblioItem{MVector}
{
Александр Клейн,
Линейное отображение D-алгебры,\\
eprint \href{http://arxiv.org/abs/MVector}{arXiv:MVector} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Теория представлений универсальной алгебры,\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{1812.03397}
{
Ivan Kyrchei,
Linear differential systems over the quaternion skew field,\\
eprint \href{http://arxiv.org/abs/1812.03397}{arXiv:1812.03397} (2018)
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{1510.02224}
{
Kit Ian Kou, Yong-Hui Xia.
Linear Quaternion Differential Equations: Basic Theory and Fundamental Results.\\
eprint \href{http://arxiv.org/abs/1510.02224}{arXiv:1510.02224} (2017)
}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,\\
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Diagram.Representation.Russian.tex <==
%auto-ignore
\input{Diagram.Representation.Eq}
\chapter{Диаграмма представлений универсальных алгебр}
\labelChapter{Diagram of Representations of Universal Algebras}

\section{Диаграмма представлений универсальных алгебр}
\labelSection{Diagram of Representations of Universal Algebras}

Из сравнения теорем
\RefTheorem{structure of subrepresentations}
и
\citeBib{Cohn: Universal Algebra}\Hyph 5.1
следует, что
нет жёсткой границы между универсальной алгеброй
и представлением универсальной алгебры.
Отсюда следует возможность обобщения теории представлений
универсальной алгебры.

Самая простая конструкция возникает следующим образом.
Пусть
\ShowEq{f:i->*j}12
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Если мы вместо $\Omega_2$\Hyph алгебры $A_2$
рассмотрим представление
\ShowEq{f:i->*j}23
$\Omega_2$\Hyph алгебры $A_2$
в $\Omega_3$\Hyph алгебре $A_3$,
то мы получим диаграмму вида
\DrawEq[123]{Ai->*Aj->*Ak}{tower}
Очевидно, что в диаграмме
\eqRef{Ai->*Aj->*Ak}{tower}
мы можем положить, что $A_3$ является представлением
\ShowEq{f:i->*j}34
Цепочку представлений универсальных алгебр можно сделать сколь угодно длиной.
Таким образом мы получаем следующее определение.

\ShowDefinition{tower of representations}

Башню представлений $(f,A)$
можно описать с помощью диаграммы
\ShowEq{tower of representations}

Рассматривая башню представлений
мы можем снова предположить, что $A_2$ или $A_3$
являются представлениями универсальных алгебр
или башнями представлений.
В этом случае диаграмма
\eqRef{Ai->*Aj->*Ak}{tower}
примет вид
\ShowEq{A1->*A2->*A3 1}
либо
\ShowEq{A1->*A2->*A3 2}
Мы также допускаем, что некоторые алгебры или отображения
на диаграмме совпадают.
Таким образом, мы будем считать, что диаграммы
\ShowEq{diagram A123 1}
и
\ShowEq{diagram A123 2}
эквивалентны.

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowTheorem{diagram of representations}

\begin{proof}
Теорема является следствием принципа математической индукции.
\end{proof}

\ShowDefinition{commutative diagram of representations}

\ShowTheorem{diagram of representations, define map fik}
\begin{proof}

\begin{lemma}
\labelLemma{The map fijk is injection}
{\it
Отображуние $f_{ijk}$ является инъекцией.
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{ab in ker13}
Тогда
\ShowEq{ab in ker13 1}
Если представление $f_{jk}$ эффективно,
то равенство
\ShowEq{ab in ker13 2}
является следствием
определения
\RefDefinition{effective representation of algebra}
и равенства
\EqRef{ab in ker13 1}
для любого
\ShowEq{a in A}j.
Утверждение $a_i=b_i$ следует из определения
\RefDefinition{free representation of algebra}.
\hfill\(\odot\)

\begin{sloppypar}
%{\hangindent=1cm
%\setlength{\parindent}{1.6cm}
\begin{lemma}
{\it
На множестве
\ShowEq{End 2 3}
определена
структура $\Omega_i$\Hyph алгебры.
}
\end{lemma}
%}%\hangindent
\end{sloppypar}

%{\hangindent=1cm
%\setlength{\parindent}{1.6cm}
{\sc Доказательство.}
Пусть
\ShowEq{omega in Omega}i.
Пусть $a_1$, ..., $a_m\in A_i$.
Мы определим операцию $\omega$ на множестве
\ShowEq{End 2 3}
с помощью равенства
\ShowEq{omega f1 on level 3}
Согласно лемме
\RefLemma{The map fijk is injection},
операция $\omega$ корректно определена
равенством
\EqRef{omega f1 on level 3}.
\hfill\(\odot\)
%}%\hangindent

\begin{corollary}
\labelCorollary{f13 is homomorphism of Omega1 algebra}
{\it
Отображение $f_{ijk}$ является гомоморфизмом $\Omega_i$\Hyph алгебры.
}
\hfill\(\odot\)
\end{corollary}

\begin{lemma}
\labelLemma{f13(a) is homomorphism of Omega2 algebra}
{\it
Отображение $f_{ijk}(a)$ является гомоморфизмом $\Omega_j$\Hyph алгебры.
}
\end{lemma}

{\sc Доказательство.}
Пусть $b_1$, ..., $b_m\in A_j$.
Тогда равенство
\ShowEq{f a b1n omega}
является следствием равенства
\EqRef{define map f13}.
Так как отображения
\ShowEq{f12a f23}
являются гомоморфизмами $\Omega_j$\Hyph алгебры, то равенство
\ShowEq{f a b1n omega 1}
является следствием равенства
\EqRef{f a b1n omega}.
Равенство
\ShowEq{f a b1n omega 2}
является следствием равенств
\EqRef{define map f13},
\EqRef{f a b1n omega 1}.
Так как отображение
$f_{jk}$
является гомоморфизмом $\Omega_2$\Hyph алгебры, то равенство
\ShowEq{f a b1n omega 3}
является следствием равенства
\EqRef{f a b1n omega 2}.
\hfill\(\odot\)

Теорема является следствием следствия
\RefCorollary{f13 is homomorphism of Omega1 algebra}
и леммы
\RefLemma{f13(a) is homomorphism of Omega2 algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{morphism representations f23}
Отображение $f_{jk}$ является приведенным морфизмом представлений
%$\Omega_i$\Hyph алгебры $A_i$
из $f_{ij}$ в $f_{ijk}$.
\end{theorem}
\begin{proof}
Рассмотрим более детально диаграмму \EqRef{tower of representations, 1 2 3}.
\ShowEq{morphism representations f23}
Утверждение теоремы следует
из равенства \EqRef{define map f13} и
определения \RefDefinition{reduced morphism of representations}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f:i->*j}ij
представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре $A_j$.
Пусть
\ShowEq{f:i->*j}jk
представление $\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
Тогда существует представление
\ShowEq{f:ij->*k}
множества\,\footnote{
Так как $\Omega_i$\Hyph алгебра $A_i$
и $\Omega_j$\Hyph алгебра $A_j$
имеют различный набор операций,
мы не можем определить структуру универсальной алгебры на множестве
$A_i\times A_j$.
}
$A_i\times A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
\end{theorem}

\begin{proof}
Мы можем описать фрагмент
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
диаграмы представлений с помощью диаграммы
\ShowEq{tower of representations, ij,k}
Из диаграммы
\EqRef{tower of representations, ij,k}
следует, что отображение $f_{ij,k}$ определено равенством
\ShowEq{f ij->k}
\end{proof}

\section{Морфизм диаграммы представлений}
\labelSection{Morphism of Diagram of Representations}

\ShowDefinition{Morphism of Diagram of Representations}

Мы будем пользоваться записью
\ShowEq{f:A->B}hAB
если кортеж отображений $h$ является
морфизмом из диаграммы представлений
$(f,A)$ в диаграмму представлений $(B,g)$.

Очень часто при изучении морфизма представления универсальной алгебры,
мы предполагаем, что алгебра, порождающая представление,
задана. Поэтому нас не интересует отображение этой алгебры,
и это соглашение упрощает структуру морфизма.
Такой морфизм представления мы называем
приведенным морфизмом представления.

Похожая задача встречается при изучении морфизма диаграммы представлений.
Для каждой универсальной алгебры из диаграммы представлений
существует множество алгебр, предшествующих этой алгебре в соответствующем графе.
Мы можем предположить, что некоторые из этих алгебр заданы
и не рассматривать соответствующие гомоморфизмы.
Соответствующий морфизм диаграммы представлений также называется приведенным.
Однако в виду сложности структуры диаграммы представлений,
мы не будем рассматривать приведенные морфизмы диаграммы представлений.

\ShowRemark{Morphism of Diagram of Representations}

Пусть определены представления
$f_{ij}$ и $f_{jk}$
универсальных алгебр.
Учитывая диаграмму
\EqRef{morphism of diagram of representations of F algebra, level k, diagram}
для представлений $f_{ij}$ и $f_{jk}$,
мы получим следующую диаграмму
\ShowEq{morphism h3}
Очевидно, что существует морфизм из
\ShowEq{End Ak}Ak{}
в
\ShowEq{End Ak}Bk,
отображающий $f_{ijk}(a_i)$ в $g_{ijk}(h_k(a_i))$.

\begin{theorem}
\labelTheorem{morphism representations h3 h1}
Если представление $f_{jk}$ эффективно
и представление $f_{ij}$ свободно,
то\,\footnote{
Смотри определение отображения $h^*$ в теореме
\RefTheorem{morphism of representations and homomorphism of algebra}.
}
$(h_i,h^*_k)$ является морфизмом представлений
из представления $f_{ijk}$ в представление $g_{ijk}$
$\Omega_i$\Hyph алгебры.
\end{theorem}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{morphism representations h3 h1}
Существование отображения $h^*_k$ и
коммутативность диаграмм $(2)$ и $(3)$ следует
из эффективности отображения $f_{jk}$ и
теоремы \RefTheorem{morphism of representations and homomorphism of algebra}.
Коммутативность диаграмм $(4)$ и $(5)$ следует
из теоремы \RefTheorem{morphism representations f23}.

Из коммутативности диаграммы $(4)$ следует
\ShowEq{Morphism of Tower of Representations, diagram 4}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 4} следует
\ShowEq{Morphism of Tower of Representations, diagram 4a}
Из коммутативности диаграммы $(3)$ следует
\ShowEq{Morphism of Tower of Representations, diagram 3}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 3} следует
\ShowEq{Morphism of Tower of Representations, diagram 3a}
Из равенств \EqRef{Morphism of Tower of Representations, diagram 4a}
и \EqRef{Morphism of Tower of Representations, diagram 3a} следует
\ShowEq{Morphism of Tower of Representations, diagrams 4, 3}

Из коммутативности диаграммы $(5)$ следует
\ShowEq{Morphism of Tower of Representations, diagram 5}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 5} следует
\ShowEq{Morphism of Tower of Representations, diagram 5a}
Из коммутативности диаграммы $(2)$ следует
\ShowEq{Morphism of Tower of Representations, diagram 2}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 2} следует
\ShowEq{Morphism of Tower of Representations, diagram 2a}
Из равенств \EqRef{Morphism of Tower of Representations, diagram 5a}
и \EqRef{Morphism of Tower of Representations, diagram 2a} следует
\ShowEq{Morphism of Tower of Representations, diagrams 5, 2}

Внешняя диаграмма является диаграммой
\EqRef{morphism of diagram of representations of F algebra, level k, diagram}
при $i=1$. Следовательно, внешняя диаграмма коммутативна
\ShowEq{morphism of tower of representations of F algebra, level 1}
Из равенства \EqRef{morphism of tower of representations of F algebra, level 1} следует
\ShowEq{morphism of tower of representations of F algebra, level 1, a}
Из равенств \EqRef{Morphism of Tower of Representations, diagrams 4, 3},
\EqRef{Morphism of Tower of Representations, diagrams 5, 2}
и \EqRef{morphism of tower of representations of F algebra, level 1, a} следует
\ShowEq{morphism of tower of representations of F algebra, level 2}
Так как отображение $f_{i+1,i+2}$ - инъекция, то из равенства
\EqRef{morphism of tower of representations of F algebra, level 2} следует
\ShowEq{morphism of tower of representations of F algebra, level 2, a}
Из равенства \EqRef{morphism of tower of representations of F algebra, level 2, a}
следует коммутативность диаграммы $(1)$, откуда следует утверждение теоремы.
\end{proof}

Теорема \RefTheorem{morphism representations h3 h1} утверждает,
что неизвестное отображение на диаграмме \EqRef{morphism h3}
является отображением $h^*_k$.
Смысл теорем
\RefTheorem{morphism representations f23}
и \RefTheorem{morphism representations h3 h1}
состоит в том, что, если все представления свободны,
то все отображения в диаграмме представлений действуют согласовано.

\begin{theorem}
\labelTheorem{product of morphisms of tower of representations}
Рассмотрим множество $\Omega_i$\Hyph алгебр
\ShowEq{product of morphisms of tower of representations, 0}
Пусть определены
морфизмы диаграм представлений
\ShowEq{product of morphisms of tower of representations, 1}
Тогда определён морфизм представлений $\Omega$\Hyph алгебры
\ShowEq{product of morphisms of tower of representations, 2}
где
\ShowEq{product of morphisms of tower of representations, 3}
Мы будем называть морфизм $r$ диаграммы представлений
из $f$ в $h$
\AddIndex{произведением морфизмов $p$ и $q$ диаграммы представлений}
{product of morphisms of diagram of representations}.
\end{theorem}
\begin{proof}
Для любых $i$, $j$
таких, что $A_{(j)}=A_j$,
если существует представление $f_{ij}$,
мы можем представить утверждение теоремы,
пользуясь диаграммой
\ShowEq{product of morphisms of tower of representations, diagram}
Отображение $r_i$ является гомоморфизмом
$\Omega_i$\Hyph алгебры $A_i$ в
$\Omega_i$\Hyph алгебру $C_i$.
Нам надо показать, что пара отображений $(r_i,r_j)$ удовлетворяет
\EqRef{morphism of diagram of representations, level k}:
\ShowEq{product of morphisms of tower of representations, k-1 k}
\end{proof}

\section{Автоморфизм диаграммы представлений}

\begin{definition}
\labelDefinition{endomorphism of diagram of representations}
Пусть
$(f,A)$
- диаграмма представлений универсальных алгебр.
Морфизм диаграммы представлений
\ShowEq{endomorphism of tower of representations}
такой, что для любого
\ShowEq{endomorphism of tower of representations, 1}
является эндоморфизмом $\Omega_{(k)}$\Hyph алгебры $A_{(k)}$,
называется
\AddIndex{эндоморфизмом диаграммы представлений}
{endomorphism of diagram of representations}.
\qed
\end{definition}

\begin{definition}
\labelDefinition{automorphism of tower of representations}
Пусть
$(f,A)$
- диаграмма представлений универсальных алгебр.
Морфизм диаграммы представлений
\ShowEq{endomorphism of tower of representations}
такой, что для любого
\ShowEq{endomorphism of tower of representations, 1}
является автоморфизмом $\Omega_{(k)}$\Hyph алгебры $A_{(k)}$,
называется
\AddIndex{автоморфизмом диаграммы представлений}
{automorphism of diagram of representations}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{group of automorphisms of diagram of representations}
Пусть
$(f,A)$
- диаграмма представлений универсальных алгебр.
Множество автоморфизмов диаграммы $(f,A)$ представлений порождает
\AddIndex{группу}{group of automorphisms of representation}
\ShowEq{group of automorphisms of representation}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{a=(a(i))}r,
\ShowEq{a=(a(i))}p{}
- автоморфизмы диаграммы представлений $(f,A)$.
Согласно определению
\RefDefinition{automorphism of tower of representations}
для любого $(k)$, \Kb1,
отображения $r_{(k)}$, $p_{(k)}$ являются автоморфизмами
$\Omega_{(k)}$\Hyph алгебры $A_{(k)}$.
Согласно теореме II.3.2
(\citeBib{Cohn: Universal Algebra}, c. 60)
для любого $(k)$, \Kb1,
отображение $r_{(k)}\circ p_{(k)}$ является автоморфизмом
$\Omega_{(k)}$\Hyph алгебры $A_{(k)}$.
Из теоремы
\RefTheorem{product of morphisms of tower of representations}
и определения
\RefDefinition{automorphism of tower of representations}
следует, что произведение автоморфизмов
$r\circ p$ диаграммы представлений $(f,A)$
является автоморфизмом диаграммы представлений $(f,A)$.

Согласно доказательству теоремы
\RefTheorem{group of automorphisms of representation},
для любого $(k)$, \Kb1,
произведение автоморфизмов $\Omega_{(k)}$\Hyph алгебры ассоциативно.
Следовательно, ассоциативно произведение
автоморфизмов диаграммы представлений.

Пусть
\ShowEq{a=(a(i))}r{}
- автоморфизм диаграммы представлений $(f,A)$.
Согласно определению
\RefDefinition{automorphism of tower of representations}
для любого $(k)$, \Kb1,
отображение $r_{(k)}$ является автоморфизмом
$\Omega_{(k)}$\Hyph алгебры $A_{(k)}$.
Следовательно,
для любого $(k)$, \Kb1,
отображение $r_{(k)}^{-1}$ является автоморфизмом
$\Omega_{(k)}$\Hyph алгебры $A_{(k)}$.
Для автоморфизма
\ShowEq{a=(a(i))}r{}
справедливо равенство
\EqRef{morphism of diagram of representations, levels k k+1}.
Пусть $j$ - индекс такой, что $j=(k)$.
Положим
\ShowEq{morphism of tower of representations, level k, 1}
Так как $r_j$
- автоморфизм,
то
\ShowEq{morphism of tower of representations, level k, 3}
и равенство
\EqRef{morphism of diagram of representations, levels k k+1}
можно записать в виде
\ShowEq{morphism of diagram of representations, levels k k+1, 1}
для любых $i$, $j$ при условии, что представление $f_{ij}$ существует.
Аналогично, из равенства
\EqRef{morphism of diagram of representations, levels k k+1, 1}
следует
\ShowEq{morphism of diagram of representations, levels k k+1, 2}
Равенство
\EqRef{morphism of diagram of representations, levels k k+1, 2}
соответствует равенству
\EqRef{morphism of diagram of representations, levels k k+1}
для отображения $r^{-1}$.
Следовательно, отображение $r^{-1}$ является автоморфизмом
диаграммы представлений $(f,A)$.
\end{proof}


==> Group.Representation.15.Russian.tex <==
%auto-ignore
\input{Group.Representation.15.Eq}

\chapter{Представление мультипликативной \texorpdfstring{$\Omega$}{Omega}-группы}
\labelChapter{Representation of Group}

\section{Представление мультипликативной \texorpdfstring{$\Omega$}{Omega}-группы}
\labelSection{Representation of Group}

Согласованность произведения в мультипликативной $\Omega$\Hyph группе $G$
и соответствующих преобразований представления $f$
позволяет нам рассмотреть больше деталей представления $f$.
Однако конструкция, рассмотренная в теореме
\RefTheorem{permits reduced polymorphism of representation},
не полна в случае некоммутативного произведения.

Если для заданного представления
\ShowEq{f:A->*B}g{A_1}{A_2}
для любых $A_1$\Hyph чисел $a_1$, $b_1$,
однозначно определено $A_1$\Hyph число $c_1$
такое, что
\ShowEq{f(c)=f(a)f(b)1}
то какой формат произведения
мы должны выбрать:
\DrawEq{c=ab}{choice}
или
\ShowEq{c=ba}

\begin{example}
\labelExample{h(g)=f(-g)}
Пусть
\ShowEq{row basis e=ei}en
базис левого векторного пространства $V$
над ассоциативной алгеброй с делением $A$.
Мы можем представить произвольный вектор
\ShowEq{vector v in V}
как \CR произведение матриц
\ShowEq{vector v=v cr e}
где
\DrawEq[v]{matrix of vector coordinates}{}
матрица координат вектора $\Vector v$
относительно базиса $\Basis e$.

Рассмотрим однотранзитивное действие группы $G$,
определённое равенством
\ShowEq{action of the group on basis manifold}
где мы отождествляем $G$\Hyph число $g$ и невырожденную матрицу
\ShowEq{matrix gnn}
Действие группы $G$ на многообразии базисов
является представлением, так как верно равенство
\ShowEq{g cr (h cr e)=}

Пусть
\DrawEq[{v_i}{}]{matrix of vector coordinates}i
матрица координат вектора $\Vector v$
относительно базиса $\Basis e_i$, $i=1$, $2$, $3$.
Тогда
\ShowEq{v=vi ei 123}
Пусть $G$\Hyph число $g_1$ отображает базис $\Basis e_1$ в базис $\Basis e_2$
\DrawEq[121]{e2=g cr e1}1
Пусть $G$\Hyph число $g_2$ отображает базис $\Basis e_2$ в базис $\Basis e_3$
\DrawEq[232]{e2=g cr e1}2
Равенство
\ShowEq{e3=g12 cr e1}
является следствием равенств
\eqRef{e2=g cr e1}1,
\eqRef{e2=g cr e1}2.
Равенство
\ShowEq{v1 cr e1=v2 cr g cr e1}
является следствием равенств
\EqRef{v=vi ei 123},
\eqRef{e2=g cr e1}1.
Равенство
\ShowEq{v1=v2 cr g}
является следствием равенства
\EqRef{v1 cr e1=v2 cr g cr e1},
так как координаты вектора $\Vector v$ определены однозначно относительно базиса $\Basis e_1$.
Равенство
\DrawEq[121]{v2=v1 cr g}1
является следствием равенства
\EqRef{v1=v2 cr g}.
Аналогично,
равенство
\DrawEq[232]{v2=v1 cr g}{23}
является следствием равенств
\EqRef{v=vi ei 123},
\eqRef{e2=g cr e1}2
и
равенство
\ShowEq{v3=v1 cr g21-}
является следствием равенств
\EqRef{v=vi ei 123},
\EqRef{e3=g12 cr e1}.
Равенство
\ShowEq{v3=v1 cr g1- cr g2-}
является следствием равенств
\eqRef{v2=v1 cr g}1,
\eqRef{v2=v1 cr g}{23}.
\qed
\end{example}

\begin{example}
\labelExample{left module over ring}
Пусть $V$ - левый модуль над кольцом $D$.
Это значит, что определено представление
\DrawEq{D->*V}{}
такое, что
\ShowEq{D->*V =}
Отображение
\ShowEq{w:V->D}
называется аддитивным, если
\ShowEq{wv12=}
Мы пользуемся записью
\ShowEq{(wv)=}
для образа аддитивного отображения.
Мы определим сумму аддитивных отображений равенством
\ShowEq{w1+w2=}
Нетрудно показать, что множество $W$ аддитивных отображений
является абелевой группой.

Мы определим отображение
\ShowEq{D->*W}
равенством
\ShowEq{wd,v=w,dv}
Из равенств
\ShowEq{w12d=}
\ShowEq{wd12=}
\ShowEq{wd1d2=}
следует, что отображение $h$ является представлением группы $G$.
Однако мы можем записать равенство
\EqRef{wd1d2=}
в виде
\ShowEq{wd1d2= h}
откуда следует, что отображение $h$ не является гомоморфизмом группы $G$.
\qed
\end{example}

Мы предполагаем, что преобразования представления мультипликативной $\Omega$\Hyph группы $A_1$
могут действовать на $A_2$\Hyph числа либо слева, либо справа. В этом случае
нам достаточно ограничиться произведением
\eqRef{c=ab}{choice}
в мультипликативной $\Omega$\Hyph группе $A_1$.
Таким образом, концепция представления мультипликативной $\Omega$\Hyph группы состоит в том,
что в каком порядке мы перемножаем элементы мультипликативной $\Omega$\Hyph группы,
в том же порядке перемножаются соответствующие преобразования представления.
Эта точка зрения отражена в примере
\ref{example: left module over ring}.
Мы также видим, что мы должны изменить формат записи,
прежде чем мы можем перейти к этой точке зрения.
Вместо того, чтобы рассматривать
\ShowEq{f in End A2}
как отображение
\ShowEq{f:A2->A2}
мы должны рассматривать эндоморфизм $f$ как оператор.

\ShowDefinition{representation of group}

Из анализа примера
\ref{example: left module over ring}
следует, что выбор между левосторонним и правосторонним представлением
зависит от рассматриваемой модели.
\ShowTheorem{duality principle, algebra representation}

\begin{remark}
Если $\Omega_1$\Hyph алгебра не является мультипликативной $\Omega$\Hyph группой,
то мы не можем сказать, действует ли представление
слева или справа.
В этом случае мы сохраним функциональную запись
$f(a_1)(a_2)$
для представления $\Omega_1$\Hyph алгебры.
\qed
\end{remark}

Из анализа равенств
\EqRef{v3=v1 cr g21-},
\EqRef{v3=v1 cr g1- cr g2-}
следует, что действие группы $G$
на множестве координат вектора $\Vector v$
(пример
\ref{example: h(g)=f(-g)})
не соответствует ни левостороннему, ни правостороннему представлению.
следует, что у нас есть два выбора.
Мы согласны, что в мультипликативной $\Omega$\Hyph группе $A_1$
мы можем определить оба варианта произведения:
\eqRef{c=ab}{choice}
и
\EqRef{c=ba} -
с целью согласовать произведение в мультипликативной $\Omega$\Hyph группе $A_1$
и произведение преобразований представления мультипликативной $\Omega$\Hyph группы $A_1$.
Эта точка зрения отражена в определениях
\RefDefinition{Left side covariant representation},
\RefDefinition{Left side contravariant representation}.

\begin{definition}
\labelDefinition{Left side covariant representation}
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{ковариантным}{covariant representation},
если равенство
\ShowEq{Left side covariant representation}
верно.
\qed
\end{definition}

\begin{definition}
\labelDefinition{Left side contravariant representation}
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{контравариантным}{contravariant representation},
если равенство
\ShowEq{Left side contravariant representation}
верно.
\qed
\end{definition}

Если тип представления не указан,
мы будем предполагать, что представление ковариантно.
Из равенств
\EqRef{v3=v1 cr g21-},
\EqRef{v3=v1 cr g1- cr g2-}
следует, что действие группы $G$
на множестве координат вектора $\Vector v$
(пример
\ref{example: h(g)=f(-g)})
является контравариантным правосторонним представлением.

Насколько велика разница между ковариантным и контравариантным представлениями.
Поскольку
\ShowEq{ab-=a-b-}
то равенство
\ShowEq{a-(b-.)=(a-b-).}
является следствием равенства
\EqRef{Left side contravariant representation}.
Из равенства
\EqRef{a-(b-.)=(a-b-).}
следует, что
мы можем рассматривать контравариантное представление группы $G$
как ковариантное представление группы $G$,
порождённое $G$\Hyph числами вида $a^{-1}$.
Так же как в примере
\ref{example: h(g)=f(-g)},
мы рассматриваем два согласованных представления группы $G$
\ShowEq{f:A->*B}fG{A_2}
\ShowEq{f:A->*B}hG{B_2}
причём $G$\Hyph число $g$ порождает преобразование
\ShowEq{a1:a2->a1a2}
в универсальной алгебре $A_2$ и преобразование
\ShowEq{a1:b2->a1-b2}
в универсальной алгебре $B_2$.

\section{Левый и правый сдвиги}

\ShowTheorem{left right shift}
\begin{proof}
Согласно определению
\RefDefinition{multiplicative Omega group},
левый и правый сдвиги являются эндоморфизмами
$\Omega$\Hyph алгебры $A$.
Согласно определению
\RefDefinition{multiplicative Omega group},
мы можем определить $\Omega$\Hyph алгебру
на множестве левых сдвигов.
Согласно определению мультипликативной группы,\,\footnote{
Смотри, например, определение на страницах
\citeBib{Serge Lang}\Hyph 17,
\citeBib{Serge Lang}\Hyph 21.
}
равенство
$a_1=a_2$
является следствием равенства
\ShowEq{a1*=a2*}
для любого $x$.
В частности, равенство
\EqRef{left shift, product}
является следствием равенства
\ShowEq{L(cb)a=}
Следовательно, отображение
\ShowEq{A->L(A)}
является левовосторонним представлением
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$.
Аналогичное рассуждение верно для правого сдвига.
\end{proof}

Ассоциативная $D$\Hyph алгебра
является мультипликативной $\Omega$\Hyph группой.
Неассоциативная $D$\Hyph алгебра $A$
не является $\Omega$\Hyph группой,
так как относительно произведения $A$ является группоидом.
Однако нас также будет интересовать представление
неассоциативной $D$\Hyph алгебры.

\begin{definition}
\labelDefinition{Omega groupoid}
Пусть произведение
\DrawEq{c=ab}{}
является операцией $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o}
Если $\Omega_1$\Hyph алгебра $A$ является группоидом
относительно произведения
и для любой операции
\ShowEq{omega n ari}{}{}n{}
умножение дистрибутивно относительно операция $\omega$
\DrawEq{a omega=omega a left}{}
\DrawEq{a omega=omega a right}{}
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph группоидом}{Omega groupoid}.
\qed
\end{definition}

Мы будем пользоваться тем же форматом записи
для представления $\Omega$\Hyph группоида,
что мы пользуемся для представления мультипликативной $\Omega$\Hyph группы.

\begin{theorem}
\labelTheorem{left right shift groupoid}
Произведение в неассоциативном $\Omega$\Hyph группоиде $A$
определяет два различных представления.
\begin{itemize}
\EqParm{non associative shift}{=left}
\EqParm{non associative shift}{=right}
\end{itemize}
\end{theorem}

\begin{proof}
Согласно определению
\RefDefinition{multiplicative Omega group},
левый и правый сдвиги являются эндоморфизмами
$\Omega$\Hyph алгебры $A$.
Согласно определению
\RefDefinition{Omega groupoid},
мы можем определить $\Omega$\Hyph алгебру
на множестве левых сдвигов.
Следовательно, отображение
\ShowEq{A->L(A)}
является представлением
$\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебре $A$.
\end{proof}

\begin{theorem}
\labelTheorem{non associative product is different from the superposition}
Пусть
\ShowEq{f:A->*B}LAA
представление неассоциативного $\Omega$\Hyph группоида $A$
в $\Omega$\Hyph алгебре $A$.
Тогда на множестве
\ShowEq{End Ak}A{}{}
определена операция произведения, отличная от суперпозиции эндоморфизмов.
\end{theorem}
\begin{proof}
Рассмотрим отображение
\ShowEq{L:A->End A}
Поскольку произведение в $\Omega$\Hyph группоиде $A$ не ассоциативно,
то, вообще говоря,
\ShowEq{La Lb ne Lab}
Следовательно,
\ShowEq{Lab ne LaLb}
\end{proof}

Согласно теореме
\RefTheorem{left right shift},
если $A$ - мультипликативная $\Omega$\Hyph группа,
то равенство
\EqRef{left shift, product}
гарантирует, что левый сдвиг порождает
левосторонним представление
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$.
Согласно теореме
\RefTheorem{non associative product is different from the superposition}
это равенство не верно в
неассоциативном $\Omega$\Hyph группоиде $A$.
Однако теоремы
\RefTheorem{left right shift groupoid},
\RefTheorem{non associative product is different from the superposition}
не отвечают на вопрос
о возможности рассмотрения
левостороннего представления
неассоциативного $\Omega$\Hyph группоида $A$
в $\Omega$\Hyph алгебре $A$.
Согласно примеру
\RefExample{left shift Lie algebra},
существует возможность подобного представления,
даже если произведение в $\Omega$\Hyph группоиде неассоциативно.

\begin{example}
\labelExample{left shift Lie algebra}
{\it
Пусть $A$ - алгебре Ли.
Произведение\,\footnote{
Смотри определение
\citeBib{Bourbaki: Group Lie}\Hyph 1
на странице 9.
}
$[a,b]$ $A$\Hyph чисел $a$, $b$ удовлетворяет равенству
\ShowEq{[ab]=-}
а также тождеству Ли
\ShowEq{Lee identity}
Левый сдвиг на алгебре Ли $A$ определён равенством
\ShowEq{L(b)a=}
Из равенства
\EqRef{L(b)a=}
следует, что
\ShowEq{L(c)L(b)a=}
Равенство
\ShowEq{[L(c)L(b)]a=}
является следствием равенств
\EqRef{[ab]=-},
\EqRef{L(c)L(b)a=}.
Равенство
\ShowEq{Lee identity 1}
является следствием равенств
\EqRef{[ab]=-},
\EqRef{Lee identity}.
Равенство
\ShowEq{[L(c)L(b)]a= 1}
является следствием равенств
\EqRef{L(b)a=},
\EqRef{[L(c)L(b)]a=},
\EqRef{Lee identity 1}.

Если я определю произведение Ли
\ShowEq{Lie product on set of left shifts}
на множестве левых сдигов,
то равенство
\EqRef{[L(c)L(b)]a= 1}
принимает вид
\ShowEq{[L(c)L(b)]a= 2}
Следовательно, алгебра Ли $A$ с произведением $[a,b]$
порождает представление в векторном пространстве $A$.
}
\qed
\end{example}

\section{Орбита представления мультипликативной \texorpdfstring{$\Omega$}{Omega}-группы}

\begin{theorem}
\labelTheorem{identity transformation}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega_1$\Hyph группы $A_1$
и $e$ - единица
мультипликативной $\Omega_1$\Hyph группы $A_1$.
Тогда
\ShowEq{f(e)=}
где $\delta$ - тождественное преобразование
$\Omega_2$\Hyph алгебры $A_2$.
\end{theorem}

\begin{proof}
Теорема является следствием равенства
\ShowEq{fa=fafe}
для любого $A_1$\Hyph числа.
\end{proof}

\begin{theorem}
\labelTheorem{inverse transformation}
Пусть отображение
\ShowEq{f:A->*B}g{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Для любого $g\in A_1$ преобразование $f(g)$ имет обратное отображение
и удовлетворяет равенству
\ShowEq{inverse transformation}
\end{theorem}
\begin{proof}
Пусть $e$ - единица мультипликативной $\Omega$\Hyph группы $A_1$
и $\delta$ - тождественное преобразование множества $A_2$.
На основании
\eqRef{left-side representation of group}{def}
и теоремы
\RefTheorem{identity transformation}
мы можем записать
\ShowEq{=f(g-g)u=}
Это завершает доказательство.
\end{proof}

\ShowEq{=left}
\ShowDefinition{orbit of representation}

\ShowEq{=right}
\ShowDefinition{orbit of representation}

\begin{theorem}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Then
\ShowEq{a2 in A1a2}
\end{theorem}

\begin{proof}
Согласно теореме
\RefTheorem{identity transformation}
\ShowEq{a2=fea2}
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f:A->*B}LAA
представление алгебры Ли, порождённое множеством левых сдвигов. Тогда
\ShowEq{a not in Aa}
\end{theorem}

\begin{proof}
Теорема является следствием отсутствия единицы в алгебре Ли.
Кроме того, самый простой пример алгебры Ли -
это множество векторов трёх мерного пространства на котором определена
операция векторного произведения. Очевидно, что не существует вектора $b$ такого, что
\ShowEq{a=b x a}
\end{proof}

\begin{theorem}
\labelTheorem{proper definition of orbit}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Если
\ShowEq{orbit, proposition}
то
\ShowEq{A1a2=A1b2}
\end{theorem}
\begin{proof}
Из \EqRef{orbit, proposition} следует существование
\ShowEq{a in A}1{}
такого, что
\ShowEq{orbit, 1}
Если
\ShowEq{c2 in A1b2},
то существует
\ShowEq{b in A}1{}
такой, что
\ShowEq{orbit, 2}
Подставив \EqRef{orbit, 1}
в \EqRef{orbit, 2}, мы получим
\ShowEq{orbit, 3}
На основании \eqRef{left-side representation of group}{def}
из \EqRef{orbit, 3}
следует, что
\ShowEq{c2 in A1a2}
Таким образом,
\ShowEq{A1b2 in A1a2}

На основании \EqRef{inverse transformation}
из \EqRef{orbit, 1}
следует, что
\ShowEq{orbit, 4}
Равенство \EqRef{orbit, 4} означает, что
\ShowEq{a2 in A1b2}
и, следовательно,
\ShowEq{A1a2 in A1b2}
Равенство
\EqRef{A1a2=A1b2}
является следствием утверждений
\EqRef{A1b2 in A1a2},
\EqRef{A1a2 in A1b2}.
\end{proof}

Таким образом, левостороннее представление
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
порождает отношение эквивалентности $S$ и
орбита $A_1*a_2$ является классом эквивалентности.
Мы будем пользоваться обозначением
\ShowEq{space of orbits of representation}
для фактор множества $A_2/S$ и мы будем называть
это множество
\AddIndex{пространством орбит левостороннего представления}
{space of orbits of left side representation} $f$.

\section{Представление в \texorpdfstring{$\Omega$}{Omega}-группе}

\begin{theorem}
\labelTheorem{kernel of inefficiency, representation of group}
Мы будем называть
ядром неэффективности левостороннего представления
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
множество
\ShowEq{kernel of inefficiency of representation}
Ядро неэффективности левостороннего представления - это подгруппа
мультипликативной группы $A_1$.
\end{theorem}
\begin{proof}
Допустим
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\ShowEq{f(a1a2)=e}
\ShowEq{f(-a)=e}
\end{proof}

\begin{theorem}
\labelTheorem{effective representation of multiplicative Omega-group}
Левостороннее представление
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
\AddIndex{эффективно}{effective representation}
тогда и только тогда, когда ядро неэффективности $K_f=\{e\}$.
\end{theorem}
\begin{proof}
Утверждение является следствием определения
\RefDefinition{effective representation of algebra} и
теоремы \RefTheorem{kernel of inefficiency, representation of group}.
\end{proof}

\begin{theorem}
\labelTheorem{not effective representation into effective}
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
не эффективно, мы можем перейти к эффективному
заменив мультипликативную $\Omega$\Hyph группу $A_1$
мультипликативной $\Omega$\Hyph группой
\ShowEq{=A1/Kf}
%пользуясь факторизацией по ядру неэффективности.
\end{theorem}
\begin{proof}
Пусть операция
\ShowEq{omega n ari}{}{}n.
Чтобы доказать теорему, мы должны показать, что равенство
\ShowEq{fa1no=fb1no}
является следствием утверждения
\ShowEq{fai=fbi}
Действительно, равенство
\EqRef{fa1no=fb1no}
является следствием равенства
\ShowEq{fa1no=fb1no 1}
\end{proof}

Теорема
\RefTheorem{not effective representation into effective}
означает, что мы можем изучать только эффективное действие.

\section{Однотранзитивное правостороннее представление группы}
\labelSection{Single Transitive Representation of Group}

\begin{theorem}
\labelTheorem{free representation of group, little group}
Пусть отображение
\ShowEq{f:A->*B}g{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
\AddIndex{Малая группа}{little group} или
\AddIndex{группа стабилизации}{stability group} элемента
\ShowEq{a in A}2{}
- это множество
\ShowEq{little group}
Представление $f$
\AddIndex{свободно}{free representation}
тогда и только тогда, когда для любого
\ShowEq{a in A}2{}
группа стабилизации
\ShowEq{stability group=e}
\end{theorem}
\begin{proof}
Согласно определению
\RefDefinition{free representation of algebra},
представление $f$ свободно тогда и только тогда, когда
равенство $a_1=b_1$ является следтсвием
утверждения
\DrawEq[{a_1}{b_1}]{fa=fb}{group}
Равенство
\eqRef{fa=fb}{group}
эквивалентно равенству
\ShowEq{f(-ba)=e}
Равенство $a_1=b_1$ является следтсвием
утверждения
\EqRef{f(-ba)=e}
тогда и только тогда, когда для любого
\ShowEq{a in A}2{}
группа стабилизации
\ShowEq{stability group=e}
\end{proof}

\begin{theorem}%
\labelTheorem{free representation of group}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является свободным левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует взаимно однозначное соответствие между
любыми двумя орбитами представления,
а также между орбитой представления и мультипликативной $\Omega$\Hyph группой $A_1$.
\end{theorem}
\begin{proof}
Допустим для точки
\ShowEq{a in A}2{}
существуют
\ShowEq{a b in A}1{}
\ShowEq{free representation of group, 1}
Умножим обе части равенства
\EqRef{free representation of group, 1}
на
\ShowEq{free representation of group, 2}
Поскольку представление свободное, $a_1=b_1$. Теорема доказана,
так как мы установили взаимно однозначное соответствие между
орбитой и мультипликативной $\Omega$\Hyph группой $A_1$.
\end{proof}

\begin{theorem}%однотранзитивное
Левостороннее представление
\ShowEq{f:A->*B}g{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
\AddIndex{однотранзитивно}{single transitive representation of algebra}
тогда и только тогда, когда для любых
\ShowEq{a b in A}2{}
существует одно и только одно
\ShowEq{a in A}1{}
такое, что
\ShowEq{a=fab}
\end{theorem}
\begin{proof}
Следствие определений \RefDefinition{effective representation of algebra}
и \RefDefinition{transitive representation of algebra}.
\end{proof}

\begin{theorem}%
\labelTheorem{single transitive representation of group}
Если существует однотранзитивное представление
\ShowEq{f:A->*B}f{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$,
то мы можем однозначно определить координаты на $A_2$, пользуясь $A_1$\Hyph числами.

Если $f$ - левостороннее однотранзитивное однотранзитивное представление,
то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $A_1$.
Если $f$ - правостороннее однотранзитивное представление, то $f(a)$ эквивалентно
правому сдвигу $R(a)$ на группе $A_1$.
\end{theorem}
\begin{proof}
Пусть $f$ - левостороннее представление.
Мы выберем $A_2$\Hyph число $a_2$
и определим координаты $A_2$\Hyph числа $b_2$
как $A_1$\Hyph число $a_1$
такое, что
\ShowEq{b=faa...}
Координаты, определённые таким образом, однозначны
с точностью до выбора $A_2$\Hyph числа $a_2$,
так как действие эффективно.
Для левостороннего однотранзитивного представления
мы будем также пользоваться записью
\ShowEq{left side single transitive shift}
Мы пользуемся записью
\ShowEq{left side shift notation}
для левостороннего однотранзитивного представления $f$
так как, согласно теореме
\RefTheorem{left right shift},
произведение левых сдвигов совпадает с их композицией.

Пусть $f$ - правостороннее однотранзитивное представление.
Мы выберем $A_2$\Hyph число $a_2$
и определим координаты $A_2$\Hyph числа $b_2$
как $A_1$\Hyph число $a_1$
такое, что
\ShowEq{b=afa...}
Координаты, определённые таким образом, однозначны
с точностью до выбора $A_2$\Hyph числа $a_2$,
так как действие эффективно.
Для правостороннего однотранзитивного представления
мы будем также пользоваться записью
\ShowEq{rigt side single transitive shift}
Мы пользуемся записью
\ShowEq{rigt side shift notation}
для правостороннего однотранзитивного представления $f$
так как, согласно теореме
\RefTheorem{left right shift},
произведение правых сдвигов совпадает с их композицией.
\end{proof}

\begin{definition}
Мы будем называть $\Omega_2$\Hyph алгебру $A_2$
\AddIndex{однородным пространством}{homogeneous space} мультипликативной $\Omega$\Hyph группы $A_1$,
если существует однотранзитивное левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Free representation is single transitive}
Свободное левостороннее представление
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
однотранзитивно на орбите.
\end{theorem}
\begin{proof}
Следствие теоремы
\RefTheorem{free representation of group}.
\end{proof}

\begin{theorem}%
\labelTheorem{shifts on group commuting}
Правый и левый сдвиги на мультипликативной $\Omega$\Hyph группе $A_1$ перестановочны.
\end{theorem}
\begin{proof}
Теорема является следствием ассоциативности произведения в мультипликативной $\Omega$\Hyph группе $A_1$
\ShowEq{L(a)oR(b)=}
\end{proof}

Теорема \RefTheorem{shifts on group commuting} может
быть сформулирована следующим образом.

\begin{theorem}%
\labelTheorem{shift is automorphism of representation}
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа. Для любого
\ShowEq{a in A}1{}
отображение
$L(a_1)$ является автоморфизмом представления $R$.
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{shifts on group commuting}
\ShowEq{shifts on group commuting}
Равенство \EqRef{shifts on group commuting}
совпадает с равенством
\EqRef{morphism of representations of universal algebra, definition, 2}
из определения
\RefDefinition{morphism of representations of universal algebra}
при условии
\ShowEq{r1=id r2=L}
\end{proof}

\begin{theorem}%
\labelTheorem{two representations of group}
Пусть левостороннее $A_1$\Hyph представление $f$
на $\Omega_2$\Hyph алгебре $A_2$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное правостороннее $A_1$\Hyph представление $h$
на $\Omega_2$\Hyph алгебре $A_2$
такое, что диаграмма
\ShowEq{two representations of group}
коммутативна для любых $a_1$, $b_1\in A_1$.\,\footnote{Это
утверждение можно также найти в \citeBib{Rashevsky}.}
\end{theorem}
\begin{proof}
Мы будем пользоваться групповыми координатами для $A_2$\Hyph чисел $a_2$.
Тогда согласно теореме \RefTheorem{single transitive representation of group}
мы можем записать левый сдвиг $L(a_1)$ вместо преобразования $f(a_1)$.

Пусть
\ShowEq{a b in A}2.
Тогда мы можем найти
одно и только одно
\ShowEq{a in A}1{}
такое, что
\ShowEq{b=aRa}
Мы предположим
\ShowEq{ha=Ra}
Существует
\ShowEq{b in A}1{}
такое, что
\ShowEq{c=Lba}
Согласно теореме \RefTheorem{shifts on group commuting} диаграмма
\ShowEq{Diagram: two representations of group}
коммутативна.

Изменяя $b_1$ мы получим, что $c_2$ - это произвольное $A_2$\Hyph число.

Мы видим из диаграммы, что, если $a_2=b_2$, то $c_2=d_2$ и следовательно $h(e)=\delta$.
С другой стороны, если $a_2\neq b_2$, то $c_2\neq d_2$ потому, что
левостороннее $A_1$\Hyph представление $f$ однотранзитивно.
Следовательно правостороннее $A_1$\Hyph представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $c_2$ мы можем найти $a_1$
такое, что
\ShowEq{d2=c2 h}
Следовательно правостороннее $A_1$\Hyph представление $h$ однотранзитивно.

В общем случае, произведение преобразований левостороннего $A_1$\Hyph представления $f$
не коммутативно и следовательно
правосторонним $A_1$\Hyph представление $h$ отлично от левостороннего $A_1$\Hyph представления $f$.
Таким же образом мы можем создать левостороннее $A_1$\Hyph представление $f$,
пользуясь правосторонним $A_1$\Hyph представлением $h$.
\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями}{twin representations}
мультипликативной $\Omega$\Hyph группы $A_1$.

\begin{remark}
\labelRemark{one representation of group}
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если мультипликативная $\Omega$\Hyph группа $A_1$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $A_2$,
то мы можем определить два перестановочных представления на множестве $A_2$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму
\EqRef{Diagram: two representations of group}
и предположить
\ShowEq{haa=Laa}
вместо
\ShowEq{haa=aRa}
и проанализировать, какое выражение $h(a_1)$ имеет в
точке $c_2$. Диаграмма
\ShowEq{Diagram: two representations of group 1}
эквивалентна диаграмме
\ShowEq{Diagram: two representations of group 2}
и мы имеем
\ShowEq{d2=...c2 1}
Следовательно
\ShowEq{d2=...c2}
Мы видим, что представление $h$
зависит от его аргумента.
\qed  
%There is interesting question. Если I имею преобразование $a\star$ in точке $b$
%what is $c$ такое, что $a\star b = R_c b$. Мы можем find it из равенства
%$ab=bc$, so $c=b^{-1}ab$, следовательно
%\[a\star b = R_{b^{-1}ab} b\]?????
\end{remark}

\begin{theorem}%
\labelTheorem{twin representations of group, automorphism}
Пусть $f$ и $h$ - парные преставления мультипликативной $\Omega$\Hyph группы $A_1$.
Для любого
\ShowEq{a in A}1{}
отображение $h(a_1)$ является автоморфизмом представления $f$.
\end{theorem}
\begin{proof}
Следствие теорем
\RefTheorem{shift is automorphism of representation} и
\RefTheorem{two representations of group}.
\end{proof}

\begin{question}
Существует ли морфизм представлений
из $L$ в $L$, отличный от автоморфизма $R(a_1)$?
Если мы положим
\ShowEq{morphism of representations from L to L}
то нетрудно убедиться, что отображение
\ShowEq{r r(a)}
является морфизмом представлений из $L$ в $L$.
Но это отображение не является
автоморфизмом представления $L$,
так как $r_1\ne\id$.
\qed
\end{question}


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%966%C%cr собственная строка
   {\CR собственная строка}%
   {cr eigenrow}%
\Index%964%C%cr собственное значение
   {\CR собственное значени}%
   {cr eigenvalue}%
\Index%947%C%cr собственный столбец
   {\CR собственный столбец}%
   {cr eigencolumn}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%965%R%rc собственная строка
   {\RC собственная строка}%
   {rc eigenrow}%
\Index%963%R%rc собственное значение
   {\RC собственное значение}%
   {rc eigenvalue}%
\Index%946%R%rc собственный столбец
   {\RC собственный столбец}%
   {rc eigencolumn}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%913%Б%базис абелевой группы
   {базис абелевой группы}%
   {basis of Abelian group}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate representation}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%701%К%квазибазис диаграммы представлений
   {квазибазис диаграммы представлений}%
   {quasibasis of diagram of representations}%
\Index%535%К%квазибазис представления
   {квазибазис представления}%
   {quasibasis of representation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация столбцов
   {левая линейная комбинация столбцов}%
   {left linear combination of columns}%
\Index%954%Л%левая линейная комбинация строк
   {левая линейная комбинация строк}%
   {left linear combination of rows}%
\Index%959%Л%левое A subs векторное пространство
   {левое $A_*$\Hyph векторное пространство}%
   {left A subs vector space}%
\Index%958%Л%левое A sups векторное пространство
   {левое $A^*$\Hyph векторное пространство}%
   {left A sups vector space}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное *G представление
   {пассивное \sT{G}представление}%
   {passive *G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%912%П%подмодуль, порождённым множеством
   {подмодуль, порождённым множеством}%
   {submodule generated by set}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация столбцов
   {правая линейная комбинация столбцов}%
   {right linear combination of columns}%
\Index%956%П%правая линейная комбинация строк
   {правая линейная комбинация строк}%
   {right linear combination of rows}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%960%П%правое A sups векторное пространство
   {правое $A^*$\Hyph векторное пространство}%
   {right A sups vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%384%П%принцип инвариантности
   {принцип инвариантности}%
   {invariance principle}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Omega.Group.Russian.tex <==
%auto-ignore
\input{Omega.Group.Eq}

\chapter{\texorpdfstring{$\Omega$}{Omega}-группа}

\section{Множество гомоморфизмов \texorpdfstring{$\Omega$}{Omega}-алгебры}

\begin{theorem}
\labelTheorem{aijo1o2=aijo2o1}
Пусть множества $A$, $B$ являются $\Omega$\Hyph алгебрами.
Множество
\ShowEq{hom Omega A B}
является $\Omega$\Hyph алгеброй,
если для любых операций
\EqParm{o12 in Omn}{=c}
верно следующее равенство
\DrawEq{aijo1o2=aijo2o1}{algebra}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{Cartesian power is universal algebra},
множество $B^A$
является $\Omega$\Hyph алгеброй.
Пусть
\ShowEq{omega n ari}{}{}n.
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{o1}

Пусть
\EqParm{o12 in Omn}{=.}
Пусть отображения
\ShowEq{f1m in Hom AB}
являются гомоморфизмами
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
В частности, для любых
\ShowEq{a1n in A}
\ShowEq{f1ma1no2=}
Если мы требуем, что отображение
\ShowEq{f1mo1}
является гомоморфизмом
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$, то
\ShowEq{f1mo1a1no2=}
Согласно определению
\eqRef{f1n omega=}{o1},
равенство
\ShowEq{f1mo1a1no2= 1}
является следствием равенства
\EqRef{f1mo1a1no2=}.
Равенство
\ShowEq{f1mo1a1no2= 2}
является следствием равенств
\EqRef{f1ma1no2=},
\EqRef{f1mo1a1no2= 1}.
Положим
\ShowEq{aij=fi(aj)}
Равенство
\eqRef{aijo1o2=aijo2o1}{algebra}
является следствием равенств
\EqRef{f1mo1a1no2= 2},
\EqRef{aij=fi(aj)}.
\end{proof}

Не всякая $\Omega$\Hyph алгебра удовлетворяет условиям теоремы
\RefTheorem{aijo1o2=aijo2o1}.

\begin{theorem}
\labelTheorem{Hom+G12 is Abelian group}
Если $G_1$, $G_2$ - абелевые полугруппы, то множество\newline
\ShowEq{Hom+G12}
также является абелевой полугруппой.
\end{theorem}
\begin{proof}
Поскольку операция сложения в абелевой полугруппе
коммутативна и ассоциативна,
то теорема является следствием теоремы
\RefTheorem{aijo1o2=aijo2o1}.
\end{proof}

\begin{theorem}
\labelTheorem{set of endomorphism of Abelian group}
Множество
\ShowEq{End+A}
эндоморфизмов абелевой группы $A$
является абелевой группой.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{End A=Hom AA},
\RefTheorem{Hom+G12 is Abelian group}
и утверждения, что уравнение
\[x+a=0\]
в абелевой группе имеет решение.
\end{proof}

\begin{theorem}
\labelTheorem{Hom+*D12 is not ring}
Если $D_1$, $D_2$ - кольца, то множество
\EqParm{Hom+*D12}{=c}
вообще говоря, кольцом не является.
\end{theorem}
\begin{proof}
В кольце определены две операции: сложение, которое
коммутативно и ассоциативно, и произведение, которое
дистрибутивно относительно сложения.
Согласно теореме
\RefTheorem{aijo1o2=aijo2o1},
сложение и произведение должны удовлетворять равенству
\DrawEq{a * b + =}{ring}
Однако правая часть равенства
\eqRef{a * b + =}{ring}
имеет вид
\ShowEq{a+a a+a}
Следовательно, равенство
\eqRef{a * b + =}{ring}
не верно.
\end{proof}

Анализ теорем
\RefTheorem{Hom+G12 is Abelian group},
\RefTheorem{Hom+*D12 is not ring}
говорит о том, что множество $\Omega$\Hyph алгебр,
удовлетворяеющих условиям теоремы
\RefTheorem{aijo1o2=aijo2o1},
невелико.

\begin{question}
\labelQuest{Is there aijo1o2=aijo2o1 algebra which is different from semigroup}
Существует ли универсальная алгебра, отличная от абелевой полугруппы и
удовлетворяеющая условиям теоремы
\RefTheorem{aijo1o2=aijo2o1}?
\qed
\end{question}

Из нашего опыта следует, что многие $\Omega$\Hyph алгебры содержат
операцию, которая соло порождала бы полугруппу.
Поэтому мы изменим формулировку теоремы
\RefTheorem{aijo1o2=aijo2o1}.

\begin{theorem}
\labelTheorem{aijoo=...}
Пусть множества $A$, $B$ являются $\Omega$\Hyph алгебрами.
Пусть
\ShowEq{omega n ari}{}{}n.
Множество
\ShowEq{hom Omega A B}
замкнуто относительно операции $\omega$,
если верно следующее равенство
\ShowEq{aijoo=...}
\end{theorem}
\begin{proof}
Вообще говоря, мы рассматриваем множество\newline
\ShowEq{hom omega AB}
Теорема является следствием теоремы
\RefTheorem{aijo1o2=aijo2o1}.
\end{proof}

\begin{theorem}
\labelTheorem{omega 2 ari commutative and associative}
Пусть операция
\ShowEq{omega n ari}{}{}2{}
коммутативна и ассоциативна.
Множество
\ShowEq{hom Omega A B}
замкнуто относительно операции $\omega$.
\end{theorem}
\begin{proof}
Так как операция
\ShowEq{omega n ari}{}{}2{}
коммутативна и ассоциативна,
то
\ShowEq{aijoo=... 2}
Теорема является следствием равенства
\EqRef{aijoo=... 2}
и теоремы
\RefTheorem{aijoo=...}.
\end{proof}

\begin{theorem}
Пусть операция
\ShowEq{omega n ari}{}{}2{}
имеет нейтральный элемент
и множество
\ShowEq{hom Omega A B}
замкнуто относительно операции $\omega$.
Тогда операция $\omega$
коммутативна и ассоциативна.
\end{theorem}
\begin{proof}
Равенства
\ShowEq{omega 2 ari commutative}
\ShowEq{omega 2 ari associative}
являются следствием равенств
\EqRef{left neutral element},
\EqRef{right neutral element},
\EqRef{aijoo=...}.
Ассоциативность операции $\omega$ является следствием равенства
\EqRef{omega 2 ari commutative}.
Коммутативность операции $\omega$ является следствием равенства
\EqRef{omega 2 ari associative}.
\end{proof}

\begin{question}
Существует ли область операторов $\Omega$,
для которой верны следующие утверждения?
\begin{itemize}
\item
Множество
\ShowEq{hom Omega A B}
замкнуто относительно операции
\ShowEq{omega n ari}{}{}2.
\item
Операция $\omega$ не является коммутативной или ассоциативной.
\end{itemize}
\qed
\end{question}

\section{\texorpdfstring{$\Omega$}{Omega}-группа}

Пусть в $\Omega_2$\Hyph алгебре $A_2$
определена операция
\EqParm{omega 2 ari 2}{=c}
%сложения,
%которая не обязательно коммутативна.
которая коммутативна и ассоциативна.
Мы будем отождествлять операцию $\omega$ с суммой.
Мы пользуемся символом $+$ для обозначения операции суммы.
Положим
\ShowEq{Omega=2...-+}

\begin{definition}
\labelDefinition{additive map}
Отображение
\ShowEq{f:A2->B2}
$\Omega_2$\Hyph алгебры $A_2$ в $\Omega_2$\Hyph алгебру $B_2$
называется
\AddIndex{аддитивным отображением}{additive map},
если
\ShowEq{f(a+b)=}
Обозначим
\ShowEq{set additive maps, AB}
множество аддитивных отображений
$\Omega_2$\Hyph алгебры $A_2$ в $\Omega_2$\Hyph алгебру $B_2$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{A(A,B)=Mor(+,A,B)}
\ShowEq{A(A,B)=Mor(+,A,B)}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{additive map}.
\end{proof}

\ShowDefinition{polyadditive map}

\begin{theorem}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является эффективным представлением $\Omega$\Hyph алгебры $A_1$
в абелевой полугруппе $A_2$.
\StartLabelItem
\begin{enumerate}
\item
На множестве $A_1$ можно определить структуру абелевой полугруппы
\labelItem{effective representation, Abelian semigroup}%
\ShowEq{(a+b)(m)=a(m)+b(m)}%
\item
Отображение $f$ является аддитивным отображением.
\labelItem{effective representation is additive map}
\item
Отображение $f$ является
представлением $\Omega_1$\Hyph алгебры $A_1$, где
\ShowEq{Omega1=...-+}
\labelItem{map f is representation of Omega1-algebra}
%\item
%Любая операция $\omega\in\Omega$
%является полиаддитивным отображением.
\end{enumerate}
\end{theorem}
\begin{proof}
Согласно теоремам
\RefTheorem{End A=Hom AA},
\RefTheorem{omega 2 ari commutative and associative},
множество
\ShowEq{End+A2}
является абелевой полугруппой.
Поскольку представление $f$ эффективно,
то, согласно теоремам
\RefTheorem{representation is effective},
\RefTheorem{aijo1o2=aijo2o1},
для любых $A_1$\Hyph чисел $a$, $b$
существует единственное $A_1$\Hyph число $c$ такое, что
\ShowEq{c(m)=a(m)+b(m)}
Опираясь на равенство
\EqRef{c(m)=a(m)+b(m)},
мы определяем сумму $A_1$\Hyph чисел
\ShowEq{c=a+b}
Равенство
\EqRef{(a+b)(m)=a(m)+b(m)}
является следствием равенств
\EqRef{c(m)=a(m)+b(m)},
\EqRef{c=a+b}.

\begin{lemma}
{\it
\labelLemma{effective representation, sum is commutative}
Сумма $A_1$\Hyph чисел коммутативна.
}
\end{lemma}

{\sc Доказательство.}
Поскольку сумма $A_2$\Hyph чисел коммутативна, то равенство
\ShowEq{(a+b)(m)=(b+a)(m)}
является следствием равенства
\EqRef{(a+b)(m)=a(m)+b(m)}.
Лемма является следствием равенства
\EqRef{(a+b)(m)=(b+a)(m)}.
\hfill\(\odot\)

\begin{lemma}
{\it
\labelLemma{effective representation, sum is associative}
Сумма $A_1$\Hyph чисел ассоциативна.
}
\end{lemma}

{\sc Доказательство.}
Поскольку сумма $A_2$\Hyph чисел ассоциативна, то равенство
\ShowEq{((a+b)+c)(m)=}
является следствием равенства
\EqRef{(a+b)(m)=a(m)+b(m)}.
Лемма является следствием равенства
\EqRef{((a+b)+c)(m)=}.
\hfill\(\odot\)

Утверждение
\RefItem{effective representation, Abelian semigroup}
является следствием равенства
\EqRef{c=a+b},
лемм
\RefLemma{effective representation, sum is commutative},
\RefLemma{effective representation, sum is associative}
и определения
\RefDefinition{semigroup}.

Утверждение
\RefItem{effective representation is additive map}
является следствием равенства
\EqRef{c=a+b}.
Утверждение
\RefItem{map f is representation of Omega1-algebra}
является следствием утверждения
\RefItem{effective representation is additive map},
так как отображение $f$ является гомоморфизмом $\Omega$\Hyph алгебры.
\end{proof}

\begin{theorem}
\labelTheorem{a omega omega1}
Пусть
\ShowEq{omega n ari}{}{}n,
\ShowEq{omega n ari}1{}m.
Отображение
\DrawEq{ai->omega}{theorem}
согласовано с операцией $\omega_1$,
если верно следующее равенство
\ShowEq{a omega omega1}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{fa omega omega1}
является следствием равенств
\EqRef{a omega omega1},
\eqRef{ai->omega}{theorem}.
Теорема является следствием определения
\RefDefinition{homomorphism}
и равенства
\EqRef{fa omega omega1}.
\end{proof}

Равенство
\EqRef{a omega omega1}
является менее жёстким, чем равенство
\eqRef{aijo1o2=aijo2o1}{algebra}.
Тем не менее, также как и в случае теоремы
\RefTheorem{aijo1o2=aijo2o1},
большинство операций универсальной алгебры
не удовлетворяет условиям теоремы
\RefTheorem{a omega omega1}.
Поскольку операция сложения
удовлетворяет условиям теоремы
\RefTheorem{aijo1o2=aijo2o1},
мы ожидаем, что существуют условия,
когда операция сложения удовлетворяет условиям теоремы
\RefTheorem{a omega omega1}.

\begin{theorem}
\labelTheorem{operation omega is polyadditive map}
Пусть
\ShowEq{omega n ari}{}{}n.
Если отображение
\DrawEq{ai->omega}{operation}
согласовано со сложением для любого $i$,
то операция $\omega$ является полиаддитивным отображением.
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{a omega omega1},
если отображение
\eqRef{ai->omega}{operation}
согласовано со сложением,
то верно следующее равенство
\ShowEq{a omega +}
Теорема является следствием равенства
\EqRef{a omega +}
и определения
\RefDefinition{polyadditive map}.
\end{proof}

\ShowTheorem{operation is distributive over addition}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{operation omega is polyadditive map}.
\end{proof}

\ShowDefinition{Omega group}

\begin{example}
Группа является наиболее очевидным примером $\Omega$\Hyph группы.

Кольцо является $\Omega$\Hyph группой.

Бикольцо матриц над телом
(\citeBib{0612.111})
является $\Omega$\Hyph группой.
\qed
\end{example}

\begin{remark}
Бурбаки рассматривают похожее определение,
а именно группы с операторами
(смотри определение 10 в
\citeBib{Bourbaki: Algebra 1}
на странице 100).
\ifx\texFuture\Defined
Различие в определении состоит в том,
что Бурбаки рассматривают группу $A$ и множество отображений
\ShowEq{BxA->A}
таких, что для заданных $i$, $b$, отображение $f_i(b,a)$
является эндоморфизмом группы $A$.
Согласно определениям
\RefDefinition{transformation of universal algebra},
\RefDefinition{representation of algebra},
определение Бурбаки соответствует представлению $B$ в группе $A$.
можете найти определение $\Omega$\Hyph группы по адресу
\begin{center}\url{http://ncatlab.org/nlab/show/Omega-group}\end{center}
\fi
\qed
\end{remark}

\begin{theorem}
\labelTheorem{ai->omega is endomorphism}
Пусть $A$ - $\Omega$\Hyph группа.
Пусть
\ShowEq{omega n ari}{}{}n.
Отображение
\DrawEq{ai->omega}{}
является эндоморфизмом аддитивной группы $A$.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{operation is distributive over addition}
и определения
\RefDefinition{Omega group}.
\end{proof}

\begin{theorem}
Пусть отображение
\ShowEq{f:A->*B}g{A_1}{A_2}
является представлением
$\Omega$\Hyph группы $A_1$.
Тогда отображение
\ShowEq{fai->omega}
является морфизмом представления $f$ аддитивной группы $A_1$.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{ai->omega is endomorphism}
и определений
\RefDefinition{representation of algebra},
\RefDefinition{morphism of representations of universal algebra}.
\end{proof}




==> Preface.1908.04418.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Preface}

\section{Representation Theory}

In my papers, I often explore problems relating to the representation of
universal algebra. Initially it was small sketches
which I repeatedly corrected and rewrote.
However gradually there were new observations.
As a result, auxiliary tool became a consistent theory.

I realized this when I was writing book
\citeBib{0906.0135}, and I decided to dedicate a separate book
to the questions related with representation of universal algebra.
Exploring of the theory of representations of universal algebra
shows that this theory has a lot of common with theory of
universal algebra.

The definition of vector space as representation of field
in the Abelian group was the main impetus of deeper exploring
of representations of
universal algebra.
I put attention that this definition changes role 
of linear map.
It was found that linear map is the map
that preserves the structure of the representation.
It is easy to generalize this structure for an arbitrary representation of
universal algebra.
Thus I came to the notion of morphism of representation.

The set of regular automorphisms of vector space
forms a group. This group is single transitive on the set of
basises of vector space. This statement is the foundation of
the theory of invariants of vector space.

The natural question arises. Can we generalize this structure
to arbitrary representation?
The basis is not the only set that forms
the vector space.
If we add an arbitrary vector to the set of vectors of basis,
then a new set also generates the same vector
space, however this set is not basis.
This statement is initial point where I started
exploring of generating set of representation.
Generating set of representation is one more interesting
parallel between theory of representations and
theory of universal algebra.

The set of automorphisms of representations is loop.
Nonassociativity of the product is the source of numerous
questions which require additional research.
All these questions lead to the need to understand the
theory of invariants of a given representation.

If we consider the theory of representations of universal algebra
as an extension of the theory of universal algebra,
then why not consider the representation of one representation
in another representation.
Thus the concept of the tower representations appeared.
The most amazing fact is the statement that all maps in the
tower of representations are coordinated.

\ifx\texFuture\Defined
%Несмотря на обнаруженные в начале XX века проблемы в основаниях
%математики, математика остаётся мощным и надёжным инструментом.
В молодости, изучая теорию множеств по Бурбаки,
я обратил внимание на парадоксальную ситуацию.
В главе I Бурбаки рассматривают основы математической логики.
Это - достаточно стандартный и хорошо известный курс.
Сюрприз ждал меня в приложении
(\citeBib{Bourbaki: Set Theory}, стр. 66 - 70),
где Бурбаки рассматривают логические термы как элементы моноида
(\citeBib{Bourbaki: Set Theory}, гл. I, ).
\fi

\ifx\texFuture\Defined
Морфизм представлений во многом похож на морфизм расслоений.
В обоих случаях я работаю с диаграммой вида
\[
\xymatrix{
A\ar[rr]^f&&B
\\
C\ar[u]^p\ar[rr]^g&&D\ar[u]^q
}
\]
Отображения $f$, $g$ описывают морфизм. При этом каждая
стрелка по отдельности является морфизмом некоторой
universal алгебры.\,\footnote{Если на множестве
не задана некоторая universal алгебра, то мы можем
полагать, что множество операций, определённых на этом множестве,
пусто.}
Отображения $p$, $q$
согласуют отображения $f$, $g$
таким образом, что диаграмма коммутативна
(определения \RefDefinition{morphism of representations of universal algebra}
и \xRef[0702.561]{definition: fibered morphism}).

Let us define an additional structure on vector space $\mathcal{V}$
(for instance, a scalar product or a norm of a vector).
Then not every \drc linear map keeps properties of the selected structure.
In this case we need subgroup
$G$ of the group $\RCGL nD$
\drc linear maps from which hold properties of the selected structure.
We usually call group $G$
symmetry group.
Without loss of generality we identify element $g$ of group $G$
with corresponding transformation of representation
and write its action on vector $\Vector V\in\mathcal{V}$ as $v\RCstar g$.

Not every two bases can be mapped by a transformation
from the symmetry group
because not every nonsingular linear transformation belongs to
the representation of group $G$. Therefore, we can represent
the set of bases
as a union of orbits of group $G$.

Properties of basis depend on the symmetry group.
We can select basis $\Basis{e}$ vectors of which are
in a relationship which is invariant relative to symmetry group.
In this case all bases from orbit $\Basis{e}G$
have vectors which satisfy the same relationship. Such a basis we call
\AddIndex{$G$\Hyph basis}{G-basis}.
In each particular case we need to prove the existence of a basis
with certain properties. If such a basis does not exist
we can choose an arbitrary basis.

Basis $\Basis{e}$ creates coordinates in $\mathcal{V}$.
In different types of space it may be done in different ways.
In affine space if node of basis is point $A$ then
point $B$ has the same coordinates as vector $\overset{\longrightarrow}{AB}$
relative basis $\Basis{e}$.
In a general case we introduce coordinates of a vector as coordinates
relative to the selected basis.
Using only bases of type $G$ means using of specific coordinates on $\mathcal{A}_n$.
To distinguish them we call this \AddIndex{$G$\Hyph coordinates}{G-coordinates}.
We also call the space $\mathcal{V}$ with such coordinates
\AddIndex{$G$\Hyph space}{GSpace}.
\fi

\section{On the Edge of Theory}

Over the years, I believed
that representation theory is the main tool
to study covariance principle.
However, in the process of writing this book, I suddenly found myself
on the edge of representation theory.
It was extremely important event.

More precisely, it was two different discoveries,
interconnected by topic of non commutative addition.
At the beginning, I discovered that I can study affine geometry
on affine manifold.
(This is not new discovery.
I think people have known about this since Descartes and Gauss).
The most important for me here was the statement
that sum is not defined for every pairs of vectors.
I met similar problem when I was studying basis manifold of Minkowski space
(\citeBib{1201.4158}).
If connection on affine manifold has nonzero torsion,
then sum of vectors becomes non commutative.

Later, I decided to study representation of ring in non\Hyph abelian group.
Although algebra is closed relative operation,
I see opportunity for further development of representation theory.
We can use the definition of basis from this book;
however some important details will be hiden.
I am interested in the version that elements of basis may have a given order;
but right now I do not have a clear idea of what may follow from this assumption.


==> Preface.1908.04418.Eq.tex <==
%auto-ignore

\DefEq
{
$\Vector u+\Vector v=\Vector v+\Vector u$
}
{vector sum 1}

\DefEq
{
$\Vector u+(-\Vector u)=\Vector 0$
}
{vector sum 4}

\DefEq
{
$\Vector 0+\Vector v=\Vector v$
}
{vector sum 3}

\DefEq
{
$\Vector u+(\Vector v+\Vector w)=(\Vector u+\Vector v)+\Vector w$
}
{vector sum 2}

\DefEq
{
$1\Vector u=\Vector u$
}
{vector am 1}

\DefEq
{
$a(b\Vector u)=(ab)\Vector u$
}
{vector am 2}

\DefEq
{
$(a+b)\Vector u=a\Vector u+b\Vector u$
}
{vector am 3}

\DefEq
{
\begin{align*}
(a+b)\Vector u&=a\Vector u+b\Vector u&
a(\Vector u+\Vector v)&=a\Vector u+a\Vector v&
a,b\in F&&\Vector u,\Vector v\in\Vector V
\end{align*}
}
{vector am 5}

\DefEq
{
$a(\Vector u+\Vector v)=a\Vector u+a\Vector v$
}
{vector am 4}


==> Preface.1908.04418.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Предисловие}

\section{Теория представлений}

В статьях я часто рассматриваю вопросы, связанные с представлением
универсальной алгебры. Вначале это были небольшие наброски,
которые я многократно исправлял и переписывал.
Но постепенно появлялись новые наблюдения.
В результате вспомогательный инструмент превратился в стройную теорию.

Я это понял, когда я работал над книгой
\citeBib{0906.0135}, и решил посвятить отдельную книгу
вопросам, связанным с представлением универсальной алгебры.
Изучение теории представлений универсальной алгебры
показывает, что эта теория имеет много общего с теорией
универсальной алгебры.

Основным толчком к более глубокому изучению представлений
универсальной алгебры послужило определение векторного
пространства как представление поля в абелевой группе.
Я обратил внимание, что это определение меняет роль
линейного отображения.
По сути, линейное отображение - это отображение,
которое сохраняет структуру представления.
Эту конструкцию легко обобщить на произвольное представление
универсальной алгебры.
Таким образом появилось понятие морфизма представлений.

Множество невырожденных автоморфизмов векторного пространства
порождает группу. Эта группа действует однотранзитивно на множестве
базисов векторного пространства. Это утверждение является фундаментом
теории инвариантов векторного пространства.

Возникает естественный вопрос. Можно ли обобщить эту конструкцию
на произвольное представление?
Базис - это не единственное множество, которое порождает
векторное пространство.
Если мы к множеству векторов базиса добавим произвольный вектор,
то новое множество по прежнему порождает тоже самое векторное
пространство, но базисом не является.
Это утверждение является исходной точкой, от которой я начал
изучение множества образующих представления.
Множество образующих представления - это ещё одна интересная
параллель теории представлений с теорией универсальной алгебры.

Множество автоморфизмов представления является лупой.
Неассоциативность произведения порождает многочисленные
вопросы, которые требуют дополнительное исследование.
Все эти вопросы ведут к необходимости понимания теории инвариантов
заданного представления.

Если мы рассматриваем теорию представлений универсальной алгебры
как расширение теории универсальной алгебры,
то почему не рассмотреть представление одного представления
в другом представлении. Так появилась концепция башни представлений.
Самый удивительный факт - это то, что все отображения в
башне представлений действуют согласовано.

\ifx\texFuture\Defined
%Несмотря на обнаруженные в начале XX века проблемы в основаниях
%математики, математика остаётся мощным и надёжным инструментом.
В молодости, изучая теорию множеств по Бурбаки,
я обратил внимание на парадоксальную ситуацию.
В главе I Бурбаки рассматривают основы математической логики.
Это - достаточно стандартный и хорошо известный курс.
Сюрприз ждал меня в приложении
(\citeBib{Bourbaki: Set Theory}, стр. 66 - 70),
где Бурбаки рассматривают логические термы как элементы моноида
(\citeBib{Bourbaki: Set Theory}, гл. I, ).
\fi

\ifx\texFuture\Defined
Морфизм представлений во многом похож на морфизм расслоений.
В обоих случаях я работаю с диаграммой вида
\[
\xymatrix{
A\ar[rr]^f&&B
\\
C\ar[u]^p\ar[rr]^g&&D\ar[u]^q
}
\]
Отображения $f$, $g$ описывают морфизм. При этом каждая
стрелка по отдельности является морфизмом некоторой
универсальной алгебры.\,\footnote{Если на множестве
не задана некоторая универсальная алгебра, то мы можем
полагать, что множество операций, определённых на этом множестве,
пусто.}
Отображения $p$, $q$
согласуют отображения $f$, $g$
таким образом, что диаграмма коммутативна
(определения \RefDefinition{morphism of representations of universal algebra}
и \xRef[0702.561]{definition: fibered morphism}).

Если на векторном пространстве $\mathcal{V}$ определена дополнительная структура
(например, скалярное произведение или норма вектора),
не всякий \drc линейное отображение сохраняет свойства заданной структуры.
В этом случае нас интересует подгруппа
$G$ группы $\RCGL nD$,
\drc линейное отображения которой сохраняют свойства заданной структуры.
Мы обычно будем называть группу $G$
группой симметрии.
Не нарушая общности, мы будем отождествлять элемент $g$ группы $G$
с соответствующим преобразованием представления
и записывать его действие на вектор $\Vector V\in\mathcal{V}$
в виде $v\RCstar g$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Таким образом, множество базисов
можно представить как объединение орбит группы $G$.

Свойства базиса зависят от группы симметрии.
Мы можем выбрать базисы $\Basis{e}$, векторы которых находятся
в отношении, которое инвариантно относительно группы симметрии.
В этом случае все базисы из орбиты $\Basis{e}G$
имеют векторы, которые удовлетворяют одному и тому же отношению.
Такой базис мы будем называть
\AddIndex{$G$\Hyph базисом}{G-basis}.
В каждом конкретном случае мы должны доказать существование
базиса с искомыми свойствами. Если подобного типа базиса
не существует, мы можем выбрать произвольный базис.

Базис $\Basis{e}$ порождает координаты на $\mathcal{V}$.
В различных типах пространства это может быть сделано различным образом.
В аффинном пространстве, если вершина базиса является точкой $A$, то
точка $B$ имеет те же координаты, что и вектор $\overset{\longrightarrow}{AB}$
относительно базиса $\Basis{e}$.
В общем случае мы вводим координаты вектора как координаты
относительно выбранного базиса.
Использование только \Gspaceа означает использование специальных координат на $\mathcal{A}_n$.
Для того, чтобы отличать их, мы будем называть их
\AddIndex{$G$\Hyph координатами}{G-coordinates}.
Мы также будем называть пространство $\mathcal{V}$ с такими координатами
\AddIndex{$G$\Hyph пространством}{GSpace}.
\fi

\section{На грани теории}

На протяжении многих лет я считал,
что теория представлений является основным инструментом
для изучения принципа общековариантности.
Однако в процессе подготовки этой книги я неожиданно оказался
на грани применимости теории представлений.
Я не мог пройти мимо этого крайне важного события.

Точнее это было два разных открытия,
связанных между собой темой некоммутативного сложения.
Сначала я обнаружил, что я могу моделировать аффинную геометрию
на многообразии аффинной связности
(Тоже мне открытие.
Думаю люди об этом знали со времён Декарта и Гауса).
Здесь самым главным для меня было утверждение,
что сумма определена не для любой пары векторов.
Похожую задачу я видел, когда изучал многообразие базисов пространства Минковского
(\citeBib{1201.4158}).
Если связность на аффинном многообразии имеет ненулевое кручение,
то сумма векторов становится некоммутативной.

Позднее я решил исследовать представление кольца в неабелевой группе.
Хотя алгебра замкнута относительно операции,
я вижу возможность дальнейшего развития теории представлений.
Мы можем пользоваться определением базиса из этой книги,
однако некоторые важные детали будут спрятаны.
Для меня интересна версия, что элементы базиса могут иметь заданный порядок,
но сейчас я недостаточно ясно представляю какие из этого могут быть следствия.


==> Preliminary.Russian.tex <==
%auto-ignore
\def\Preliminary{on}
\ifx\setCACAA\Defined
\maketitle
\input{Preliminary.Eq}
\Input{Abstract.\BookNumber}
%\tableofcontents
\Input{Preface.\BookNumber}
\else
\Prolog
\fi

\Chapter{Предварительные определения}

\ifx\PrintBook\undefined
В этом разделе
\else
В этой главе
\fi
собраны определения и теоремы,
которые необходимы для понимания текста предлагаемой
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
Поэтому читатель может обращаться к утвердениям из
\ifx\PrintBook\undefined
этого раздела
\else
этой главы
\fi
по мере чтения основного текста
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi

\ePrints{4975-6381,1506.00061,BQuater,5148-4632,1908.04418,6860-2955}%,MVector
\Items{1601.03259,5410-9916,9835-2163,7287-9339}
\ifx\Semafor\ValueOn

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Отношение эквивалентности}

\begin{definition}
\labelDefinition{equivalence}
Соответствие
\ShowEq{Phi in AxA}
называется
\AddIndex{отношением эквивалентности}{equivalence},
если\,\footnote{
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 27.
}
\StartLabelItem
\begin{enumerate}
\item
соответствие $\Phi$
\AddIndex{рефлексивно}{reflexive correspondence}
\ShowEq{reflexive correspondence}
\item
соответствие $\Phi$
\AddIndex{симметрично}{symmetric correspondence}
\ShowEq{symmetric correspondence}
\item
соответствие $\Phi$
\AddIndex{транзитивно}{transitive correspondence}
\ShowEq{transitive correspondence}
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{kernel of map}
\ShowEq{def kernel of map}
является отношением эквивалентности и
называется
\AddIndex{ядром отображения}{kernel of map}.\,\footnote{
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 28.
}
\end{theorem}
\begin{proof}
\begin{lemma}
\labelLemma{ker - reflexive correspondence}
{\it
Соответствие
\ShowEq{ker f}
рефлексивно.
}
\end{lemma}

{\sc Доказательство.}
Из равенства
\ShowEq{fa=fa}
и определения
\EqRef{def kernel of map}
следует, что
\DrawEq[aa]{ab in ker}{aa}
Лемма является следствием утверждения
\eqRef{ab in ker}{aa}
и определения
\RefItem{reflexive correspondence}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{ker - symmetric correspondence}
{\it
Соответствие
\ShowEq{ker f}
симметрично.
}
\end{lemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab symmetric}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ba]{fa=fb}{ba}
является следствием равенства
\eqRef{fa=fb}{ab symmetric}.
Утверждение
\DrawEq[ba]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ba}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab in ker -> ba in ker}
Лемма является следствием утверждения
\EqRef{ab in ker -> ba in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{ker - transitive correspondence}
{\it
Соответствие
\ShowEq{ker f}
транзитивно.
}
\end{lemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab transitive}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[bc]{fa=fb}{bc}
является следствием утверждения
\DrawEq[bc]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ac]{fa=fb}{ac}
является следствием равенств
\eqRef{fa=fb}{ab transitive},
\eqRef{fa=fb}{bc}.
Утверждение
\DrawEq[ac]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ac}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab,ac in ker -> ac in ker}
Лемма является следствием утверждения
\EqRef{ab,ac in ker -> ac in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

Утверждение теоремы является следствием лем
\ShowEq{lemmas for ker}
и определения
\RefDefinition{equivalence}.
\end{proof}
\else
\Section{Универсальная алгебра}
\fi

\ePrints{5410-9916,9835-2163}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\footnote{
Утверждение леммы аналогично утверждению 
на с. \citeBib{Serge Lang}-94.}
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnote{Определение
универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.}
\end{theorem}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Универсальная алгебра}
\fi

\begin{definition}
\labelDefinition{Cartesian power}
{\it
Для любых множеств\,\footnote{
Я следую определению из примера (iV),
\citeBib{Cohn: Universal Algebra}, страницы 17, 18.
}
$A$, $B$,
\AddIndex{декартова степень}{Cartesian power}
\ShowEq{Cartesian power}
- это множество отображений
\ShowEq{f:A->B}fAB
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{operation on set}
{\it
Пусть дано множество $A$ и целое число $n\ge 0$. Отображение\,\footnote{
\ePrints{MVector,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Определения
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
опираются
\else
Определение
\RefDefinition{operation on set}
опирается
\fi
на определение в примере (vi),
страница \citeBib{Cohn: Universal Algebra}\Hyph 26.
}
\ShowEq{o:An->A}
называется
\AddIndex{$n$\Hyph арной операцией на множестве}{n-ary operation on set}
$A$ или просто
\AddIndex{операцией на множестве}{operation on set}
$A$.
Для любых
\EqParm{b1n in B}{B=A}
мы пользуемся любой из форм записи
\ShowEq{a1no=oa1n}
для обозначения образа отображения $\omega$.
}
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\begin{remark}
\labelRemark{o in AAn}
Согласно определениям
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph арная операция
\ShowEq{o in AAn}
\qed
\end{remark}
\fi

\begin{definition}
{\it
\AddIndex{Область операторов}{operator domain}
- это множество операторов\,\footnote{
Я следую определению 1,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\ShowEq{operator domain}
вместе с отображением
\ShowEq{a:O->N}
Если
\ShowEq{omega in Omega}{},
то $a(\omega)$ называется
\AddIndex{арностью}{arity}
оператора $\omega$. Если
\ShowEq{a(o)=n}
то оператор $\omega$ называется $n$\Hyph арным.
\ShowEq{set of n-ary operators}
Мы пользуемся обозначением
\ShowEq{set of n-ary operators =}
для множества $n$\Hyph арных операторов.
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{Omega-algebra}
{\it
Пусть $A$ - множество, а $\Omega$ - область операторов.\,\footnote{
Я следую определению 2,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
Семейство отображений
\ShowEq{O(n)->AAn}
называется структурой $\Omega$\Hyph алгебры на $A$.
Множество $A$ со структурой $\Omega$\Hyph алгебры называется
\AddIndex{$\Omega$\Hyph алгеброй}{Omega-algebra}
\ShowEq{Omega-algebra}
или
\AddIndex{универсальной алгеброй}{universal algebra}.
\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOff
Множество $A$ называется
\AddIndex{носителем $\Omega$\Hyph алгебры}{carrier of Omega-algebra}.
\fi
}
\qed
\end{definition}

\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOff
Область операторов $\Omega$ описывает множество $\Omega$\Hyph алгебр.
Элемент множества $\Omega$ называется оператором,
так как операция предполагает некоторое множество.
Согласно замечанию
\ref{remark: o in AAn}
и определению
\RefDefinition{Omega-algebra},
каждому оператору
\ShowEq{omega n ari}{}{}n{}
сопоставляется $n$\Hyph арная операция $\omega$ на $A$.
\fi

\ePrints{MVector,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{Cartesian power is universal algebra}
Пусть множество $B$ является $\Omega$\Hyph алгеброй.
Тогда множество $B^A$ отображений
\ShowEq{f:A->B}fAB
также является $\Omega$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega n ari}{}{}n.
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{MVector,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{set is closed with respect to operation}
{\it
Пусть
\ShowEq{B subset A}.
Если для любых
\EqParm{b1n in B}{B=B}
\ShowEq{b1no in B}
то мы говорим, что $B$
\AddIndex{замкнуто относительно}{set is closed with respect to operation}
$\omega$ или что $B$
\AddIndex{допускает операцию}{set admits operation}
$\omega$.
}
\qed
\end{definition}

\begin{definition}
$\Omega$\Hyph алгебра $B_{\Omega}$ является
\AddIndex{подалгеброй}{subalgebra of Omega-algebra}
$\Omega$\Hyph алгебры $A_{\Omega}$,
если верны следующие утверждения\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
Если оператор
\ShowEq{omega in Omega}{}{}
определяет операции $\omega_A$ на $A$ и $\omega_B$ на $B$, то
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{homomorphism}
{\it
Пусть $A$, $B$ - $\Omega$\Hyph алгебры и
\ShowEq{omega n ari}{}{}n.
Отображение\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\ShowEq{f:A->B}fAB
\AddIndex{согласовано с операцией}{map is compatible with operation}
$\omega$, если, для любых
\EqParm{b1n in B}{B=A}
\ShowEq{afo=aof}
Отображение $f$ называется
\AddIndex{гомоморфизмом}{homomorphism}
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$,
если $f$ согласовано с каждым
\ShowEq{omega in Omega}{}.
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of homomorphisms}
множество гомоморфизмов
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
\fi
}
\qed
\end{definition}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Hom empty A B=B**A}
Если область операторов пуста,
то гомоморфизм
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$
- это отображение
\ShowEq{f:A->B}fAB
Следовательно,
\ShowEq{Hom empty A B=B**A}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{MVector,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{isomorphism}
{\it
Гомоморфизм $f$ назывется\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\AddIndex{изоморфизмом}{isomorphism}
между $A$ и $B$, если соответствие $f^{-1}$ является гомоморфизмом.
Если существует изоморфизм между $A$ и $B$, то говорят,
что $A$ и $B$ изоморфны, и пишут
\ShowEq{isomorphic}
Инъективный гомоморфизм называется
\AddIndex{мономорфизмом}{monomorphism}.
Суръективный гомоморфизм называется
\AddIndex{эпиморфизмом}{epimorphism}.
}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{endomorphism}
{\it
Гомоморфизм, источником и целью которого является одна и таже алгебра, называется
\AddIndex{эндоморфизмом}{endomorphism}.
%\ePrints{1908.04418,6860-2955}%
%\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of endomorphisms}
множество эндоморфизмов
$\Omega$\Hyph алгебры $A$.
%\fi
\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,5148-4632,9835-2163,0767-8264}%
\ifx\Semafor\ValueOff%
Эндоморфизм, который является изоморфизмом, называется
\AddIndex{автоморфизмом}{automorphism}.
\fi
}
\qed
\end{definition}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{theorem}
\labelTheorem{End empty A=A**A}
Если область операторов пуста,
то эндоморфизм множества $A$
- это отображение
\ShowEq{t:A->A}
Следовательно,
\ShowEq{End empty A=A**A}
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,5148-4632,5410-9916,9835-2163,0767-8264}%
\ifx\Semafor\ValueOff%
\begin{definition}
{\it
Если существует мономорфизм $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебру $B$, то говорят, что
\AddIndex{$A$ может быть вложена в $B$}{can be embeded}.
}
\qed
\end{definition}

\begin{definition}
{\it
Если существует эпиморфизм из $A$ в $B$, то $B$ называется
\AddIndex{гомоморфным образом}{homomorphic image} алгебры $A$.
}
\qed
\end{definition}
\fi
\fi

\ePrints{MVector,5148-4632,5410-9916,9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
$\Omega$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\Section{Декартово произведение универсальных алгебр}

\ShowDefinition{product in category}

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{
Смотри также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\RefDefinition{product in category},
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{theorem}
\labelTheorem{product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}
\item
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\labelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\RefDefinition{product in category},
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\ifx\texFuture\Defined

\begin{lemma}
\labelLemma{tuple represent A number}
{\it
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{projection on i factor}
является произведением в категории \(\mathcal A\).
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a ne b}
- такие \(A\)\Hyph числа, что для любого \iI
\ShowEq{p(a)=p(b)}
Если предположить, что неравные \(A\)\Hyph числа
имеют равные разложения в виде кортежа,
то мы можем определить отношение эквивалентности,
фактор по которому скорее кандидат на произведение.
\hfill\(\odot\)

Из равенства
\ShowEq{pj(a)=aj}
следует, что отображение \(p_j\) является проекцией.
\fi
\end{proof}

\begin{definition}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Bi iI}.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{theorem}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{theorem}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Bi iI}.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}fAB
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{definition}
{\it
Эквивалентность на $\Omega$\Hyph алгебре $A$,
которая является подалгеброй $\Omega$\Hyph алгебры $A^2$,
называется
\AddIndex{конгруенцией}{}\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 71.
}
на $A$.
}
\qed
\end{definition}

\begin{theorem}[первая теорема об изоморфизмах]
\labelTheorem{first isomorphism theorem}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм $\Omega$\Hyph алгебр с ядром $s$.
Тогда отображение $f$ имеет разложение
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{Ядро гомоморфизма}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
является конгруэнцией на $\Omega$\Hyph алгебре $A$.
\labelItem{kernel of homomorphism}
\item
Множество
\ShowEq{A/ker f}
является $\Omega$\Hyph алгеброй.
\labelItem{A/ker f is Omega-algebra}
\item
Отображение
\ShowEq{p:A->/ker}
является эпиморфизмом и называется
\AddIndex{естественным гомоморфизмом}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
Отображение
\ShowEq{q:A/ker->f(A)}
является изоморфизмом.
\labelItem{q:A/ker->f(A) isomorphism}
\item
Отображение
\ShowEq{r:f(A)->B}
является мономорфизмом.
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждение
\RefItem{kernel of homomorphism}
является следствием предложения II.3.4
(\citeBib{Cohn: Universal Algebra}, страница 72).
Утверждения
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
являются следствием теоремы II.3.5
(\citeBib{Cohn: Universal Algebra}, страница 72)
и последующего определения.
Утверждения
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
являются следствием теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, страница 74).
\end{proof}
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Полугруппа}

Обычно операция
\ShowEq{omega n ari}{}{}2{}
называется произведением
\ShowEq{abo=ab}
либо суммой
\ShowEq{abo=a+b}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй и
\ShowEq{omega n ari}{}{}2.
$A$\Hyph число $e$ называется
\AddIndex{нейтральным элементом операции}{neutral element of operation}
$\omega$, если для любого $A$\Hyph числа $a$ верны равенства
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{ассоциативной}{associative operation},
если верно равенство
\ShowEq{associative operation}
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{коммутативной}{commutative operation},
если верно равенство
\ShowEq{commutative operation}
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{semigroup}
{\it
Пусть
\ShowEq{Omega=omega}
Если операция
\ShowEq{omega n ari}{}{}2{}
ассоциативна, то $\Omega$\Hyph алгебра называется
\AddIndex{полугруппой}{semigroup}.
Если операция в полугруппе коммутативна,
то полугруппа называется
\AddIndex{абелевой полугруппой}{Abelian semigroup}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,BQuater,1601.03259,5148-4632}%
\Items{MVector,5410-9916,9835-2163,0767-8264}%
\ifx\Semafor\ValueOn%
\Section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\begin{definition}
\labelDefinition{representation of algebra} 
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
\qed
\end{definition}

Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

\begin{definition}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnote{
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
}
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\qed
\end{definition}

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что\,\footnote{
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a\ne e$
существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{fam ne m}
}
}
\ShowEq{fam ne fbm}
\end{theorem}
\ProofTheorem{\RefRepresentation}{representation is effective}

\begin{theorem}
\labelTheorem{effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}
\fi

\ePrints{1506.00061}%
\ifx\Semafor\ValueOn%
\begin{definition}
\labelDefinition{free representation of algebra}
{\it
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnote{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
}
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что $a=b$.
}
\qed
\end{definition}

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff%
\begin{theorem}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{theorem}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{definition}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnote{
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}
если для любых
\EqParm{ab in A}{A=2,=z}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\labelTheorem{Representation is single transitive iff}
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{single transitive representation generates algebra}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi
\fi

\begin{definition}
\labelDefinition{morphism of representations of universal algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Матрица отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
\qed
\end{definition}

\begin{remark}
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем матрицу отображений
\ShowEq{map r12}r{}
мы будем также называть отображением.
\qed
\end{remark}

\ePrints{5148-4632,MVector}
\ifx\Semafor\ValueOn

\begin{remark}
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглашению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{Tuple of maps is morphism of representations iff}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{definition}
\end{theorem}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\begin{remark}
\labelRemark{morphism of representations of universal algebra}
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{definition}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{definition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{definition}.
\qed
\end{remark}
\fi

\begin{definition}
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
\qed
\end{definition}

\ePrints{aa}%MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{unique morphism of representations of universal algebra}
Если представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\begin{definition}
\labelDefinition{transformation coordinated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}
следует
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{transformation correlated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование $f\in{}^* A_2$ согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве ${}^*(A_2/S)$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\begin{theorem}
\labelTheorem{decompositions of morphism of representations}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s_1$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}
\fi

\ePrints{5148-4632,MVector,5410-9916}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{MVector,5148-4632,BQuater}
\ifx\Semafor\ValueOn

\Section{Базис представления универсальной алгебры}

\begin{definition}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{subrepresentation of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением представления}
{subrepresentation of representation} $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\begin{theorem}%
\labelTheorem{lattice of subrepresentations}
Множество\,\footnote{Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94)}
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
\end{theorem}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.

\begin{definition}
\labelDefinition{generating set of representation}
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением, порождённым множеством $X$}
{subrepresentation generated by set},
а $X$ -
\AddIndex{множеством образующих подпредставления $J_f(X)$}
{generating set of subrepresentation}.
В частности,
\AddIndex{множеством образующих представления $f$}
{generating set of representation}
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
\qed
\end{definition}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\begin{definition}
\labelDefinition{basis of representation}
Если множество $X\subset A_2$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset A_2$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
Доказательство теоремы
\RefTheorem{X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $X$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}X
произвольное отображение множества $X$.
%Рассмотрим отображение $\Omega_2$\Hyph слов
%\ShowEq{map of words of representation, W}
%удовлетворяющее условиям
%\RefItem{map of words of representation, m in X},
%\RefItem{map of words of representation, omega},
%\RefItem{map of words of representation, am},
%и такое, что
%\ShowEq{map of words of representation, W in X}
Существует единственный эндоморфизм представления $f$\,\footnote{Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{Rm=R1m}
%\ShowEq{endomorphism based on map of words of representation}
\end{theorem}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\Section{Диаграмма представлений универсальных алгебр}

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowDefinition{commutative diagram of representations}

Мы можем проиллюстрировать определение
\RefDefinition{tower of representations}
с помощью теоремы
\RefTheorem{diagram of representations, define map fik}.

\ShowTheorem{diagram of representations, define map fik}
\ProofTheorem{\RefRepresentation}{diagram of representations, define map fik}

\ShowDefinition{Morphism of Diagram of Representations}

\ShowRemark{Morphism of Diagram of Representations}
Для любого $k$, $k=1$, ..., $n-1$, мы имеем диаграмму
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
выражают коммутативность диаграммы (1).

\begin{definition}
{\it
Пусть
\ShowEq{Aij}
- множество
\ShowEq{Omegaij}%
алгебр.
}
\qed
\end{definition}
\fi

\ePrints{MVector,5148-4632,4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Section{Перестановка}

\begin{definition}
{\it
Инъективное отображение конечного множества в себя называется
\AddIndex{перестановкой}{permutation}.\,\footnote{
Смотри определение и свойства перестановки в
\citeBib{Kurosh: High Algebra}, страницы 28 - 32,
\citeBib{Cohn: Algebra 1}, страницы 58, 59.
}
}
\qed
\end{definition}

Обычно перестановку $\sigma$ мы записываем в виде матрицы
\ShowEq{permutation as matrix}
Запись
\EqRef{permutation as matrix}
перестановки эквивалентна утверждению
\ShowEq{a->sigma a}
Поэтому порядок столбцов в записи
\EqRef{permutation as matrix}
несущественен.

Если на множестве
\EqParm{set a1n}{=z}
задан некоторый порядок
(например, мы предполагаем, что $a_i$ предшествует $a_j$,
если $i<j$),
то мы можем подразумевать, что элементы первой строки
записаны согласно предполагаемому порядку
и будем отождествлять перестановку со второй строкой
\ShowEq{permutation as matrix 2}

\begin{definition}
{\it
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,309618526,CACAA.06.121,9835-2163,0767-8264}%
\ifx\Semafor\ValueOn%
\Section{Модуль над кольцом}

\ShowEq{=module}

\ShowDefinition{module over commutative ring}

\ShowTheorem{definition of module over commutative ring}
%\ProofTheorem{\RefLinearMap}{definition of module over commutative ring}
\ProofTheorem{\RefLinearMap}{definition of module}

\ShowDefinition{coordinates of vector 2016}

\ePrints{}
\ifx\Semafor\ValueOn

\ShowEq{=left}
\ShowTheorem{set of vectors generated by set of vectors}
\ProofTheorem{\RefLinearMap}{set of vectors generated by set of vectors}

\ShowDefinition{vector linearly dependent on vectors}

\ShowEq{remark: scalars and vectors as matrix}

\ShowDefinition{linearly independent vectors}

\ShowTheorem{basis of module}
\ProofTheorem{\RefLinearMap}{basis of module}

\ShowDefinition{free module over ring}

\ShowTheorem{division algebra, basis}
\ProofTheorem{\RefLinearMap}{division algebra, basis}
\fi

\ShowDefinition{linear map from A1 to A2, commutative module}

\ShowEq{=DD}
\ShowEq{=module}
\ShowTheorem{linear map of module}
\ePrints{7287-9339,0767-8264}%
\ifx\Semafor\ValueOn%
\ProofTheorem{\RefLinearMap}{linear map from A1 to A2, commutative module}
\else
\ProofTheorem{\RefLinearMap}{linear map, DA1->DA2, module}
\fi

\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\ShowTheorem{linear map of module, coordinates}
\ProofTheorem{4993-2400}{linear map of rcd vector space}
\fi

\ePrints{4975-6381,BQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{linear map, 0, D algebra}
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{linear map, 0, D algebra}
\fi

\ePrints{1601.03259,4975-6381,9835-2163,0767-8264}
\ifx\Semafor\ValueOn
%\ePrints{4975-6381}
%\ifx\Semafor\ValueOff
%\ShowTheorem{sum of linear maps, D module}
%\ProofTheorem{\RefLinearMap}{sum of linear maps, D module}
%\fi

\begin{definition}
\labelDefinition{polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением}{polylinear map} модулей
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\ShowTheorem{sum of polylinear maps, module}
\ProofTheorem{\RefLinearMap}{sum of polylinear maps, module}

\ShowCorollary{sum of linear maps, D module}
\fi

\ePrints{1601.03259,4975-6381,9835-2163}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{tensor product of algebras}
Пусть $A_1$, ..., $A_n$ -
свободные модули над  коммутативным кольцом $D$.\,\footnote{
Я определяю
тензорное произведение $D$\Hyph модулей
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
Рассмотрим категорию $\mathcal A_1$ объектами которой являются
полилинейные отображения
\ShowEq{polylinear maps category}
где $S_1$, $S_2$ - модули над кольцом $D$.
Мы определим морфизм
\ShowEq{f->g}fg
как линейное отображение
\ShowEq{f->g 1}
такое, что коммутативна диаграмма
\ShowEq{polylinear maps category, diagram}
Универсальный объект
\ShowEq{tensor product of algebras}
категории $\mathcal A_1$ называется
\AddIndex{тензорным произведением}{tensor product}
модулей $A_1$, ..., $A_n$.
\qed
\end{definition}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Tensor product is distributive over sum}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$ - $D$\Hyph модули.
Тензорное произведение дистрибутивно относительно сложения
\ShowEq{tensors 1, tensor product}
Представление кольца $D$
в тензорном произведении определено равенством
\ShowEq{tensors 2, tensor product}
\end{theorem}
\ProofTheorem{\RefLinearMap}{Tensor product is distributive over sum}

\begin{theorem}
\labelTheorem{tensor product and polylinear map}
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Тензорное произведение
\ShowEq{f:xA->oxA}
существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
Пусть
\ShowEq{map g, algebra, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, algebra, tensor product}
такое, что диаграмма
\ShowEq{map gh, algebra, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, algebra, tensor product}
\end{theorem}
\begin{proof}
Смотри доказательство теорем
\ShowEq{ref tensor product and polylinear map}
\end{proof}

\begin{convention}
\labelConvention{isomorphic representations S1=S2}
Алгебры $S_1$, $S_2$ могут быть различными множествами.
Однако они неразличимы для нас, если мы рассматриваем их
как изоморфные представления.
В этом случае мы будем писать $S_1=S_2$.
\qed
\end{convention}

\begin{theorem}
\labelTheorem{tensor product is associative}
\ShowEq{A1xA2xA3}
\end{theorem}
\ProofTheorem{\RefLinearMap}{tensor product is associative}

\begin{definition}
\labelDefinition{tensor power of algebra}
Тензорное произведение
\ShowEq{tensor power of algebra}
называется
\AddIndex{тензорной степенью}{tensor power} модуля $A_1$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{V times->V otimes}
Отображение
\ShowEq{V times->V otimes}
является полилинейным отображением.
\end{theorem}
\ProofTheorem{\RefLinearMap}{V times->V otimes}
\fi

\ePrints{4975-6381,BQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{standard component of tensor, algebra}
Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Мы будем
называть выражение
$\ShowSymbol{standard component of tensor}{}$
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
\end{theorem}
\ProofTheorem{\RefLinearMap}{standard component of tensor, algebra}
\fi
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{BQuater,1601.03259,MVector,309618526,CACAA.06.121,9835-2163,0767-8264}%
\ifx\Semafor\ValueOn%
\Section{Алгебра над коммутативным кольцом}

\ShowDefinition{algebra over ring}

\ePrints{1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{multiplication in algebra is distributive over addition}
Произведение в алгебре $A_1$ дистрибутивно по отношению к сложению.
\end{theorem}
\ProofTheorem{\RefLinearMap}{multiplication in algebra is distributive over addition}
\fi

\ePrints{1506.00061,7287-9339}%
\Items{BQuater,4975-6381,1601.03259,309618526,CACAA.06.121}%
\ifx\Semafor\ValueOn%
\begin{convention}
Элемент
$D$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данных в \citeBib{Richard D. Schafer}, страница 13.

\ShowDefinition{commutator of algebra}

\ShowDefinition{associator of algebra}

\ShowDefinition{nucleus of algebra}

\ShowDefinition{center of algebra}

\ShowEq{convention: we use separate color for index of element}

\ShowEq{convention: unit of algebra in basis}

\ePrints{309618526,CACAA.06.121,1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{product in algebra}
Пусть $\Basis e$ - базис свободной алгебры $A_1$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы}{structural constants}
алгебры $A_1$ над кольцом $D$.
Произведение базисных векторов в алгебре $A_1$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{product in algebra}
\fi

\ePrints{4975-6381,1601.03259,309618526,CACAA.06.121,BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{Free Algebra over Ring}
\begin{proof}
\TheoremFollows
\RefTheorem[\RefLinearMap]{endomorphism of module from product}
и следствия
\RefCorollary[\RefLinearMap]{Free Algebra over Ring}.
\end{proof}
\fi

\ShowEq{=DD}

\ShowDefinition{linear map from A1 to A2, algebra}

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль $\mathcal L(D;A;A)$, оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
является алгеброй над $D$.
\end{theorem}
\ProofTheorem{\RefLinearMap}{module L(A;A) is algebra}
\fi

\begin{definition}
\labelDefinition{polylinear map of algebras}
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Мы будем называть
полилинейное отображение
\ShowEq{polylinear map of algebras}
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\AddIndex{полилинейным отображением}{polylinear map}
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A_1$ ($A_1=...=A_n=A_1$)
в $D$\Hyph алгебру
$S$.
\qed
\end{definition}

\ePrints{9835-2163}
\ifx\Semafor\ValueOff
\ShowTheorem{tensor product of D-algebras is D-algebra}
\ProofTheorem{\RefLinearMap}{tensor product of D-algebras is D-algebra}
\fi

\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowDefinition{algebra, left and right action on L}
\fi

\ShowTheorem{representation of algebra A2 in LA}
\ProofTheorem{\RefLinearMap}{representation of algebra A2 in LA}

\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $i$.
\qed
\end{convention}

%\ShowTheorem{h generated by f, associative algebra}
%\ProofTheorem{\RefLinearMap}{h generated by f, associative algebra}

\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ShowDefinition{component of linear map}

\ShowTheorem{set FoG generates left module L(A;B), n<m}
\ShowProof{set FoG generates left module L(A;B), n<m}

\ShowTheorem{set FoG generates left module L(A;B), n>m}
\ShowProof{set FoG generates left module L(A;B), n>m}

\ShowRemark{set FoG generates left module L(A;B), n>m}
\fi

\ePrints{9835-2163,BQuater}
\ifx\Semafor\ValueOn
\ShowTheorem{set FoG generates left module L(A;B)}
\ePrints{BQuater}
\ifx\Semafor\ValueOn
\ShowProof{set FoG generates left module L(A;B)}
\else
\ProofTheorem{BQuater}{set FoG generates left module L(A;B)}
\fi
\fi

\ePrints{BQuater,9835-2163}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2 FoG, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,1601.03259}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A->A, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ePrints{4975-6381}
\ifx\Semafor\ValueOff
\ShowDefinition{component of linear map}
\fi

\ShowTheorem{conjugation transformation}
\ProofTheorem{\RefLinearMap}{conjugation transformation}

\ShowTheorem{representation of composition of linear maps}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps}

\ShowTheorem{representation of composition of linear maps A->A}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps A->A}

%\ShowTheorem{linear map in L(A,A), associative algebra}
%\ProofTheorem{\RefLinearMap}{linear map in L(A,A), associative algebra}
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}

По определению
\ShowEq{Basis F=...}
Мы также рассматриваем множество
\ShowEq{F=...}
имея в виду, что возможно равенство
\ShowEq{Fi=Fj}
при условии $i\ne j$.
\fi

\ePrints{4975-6381,1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\begin{convention}
В равенстве
\ShowEq{n linear map A LA}
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.
\qed
\end{convention}
\fi

\ePrints{1601.03259,4975-6381,1506.00061,7287-9339,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{L(An;B) is free D module}
\ProofTheorem{\RefLinearMap}{L(An;B) is free D module}

\begin{theorem}
\labelTheorem{polylinear map, algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Полилинейное отображение
\ShowEq{polylinear map, algebra}
порождённое отображениями
\ShowEq{I1n in L(A;A)},
имеет вид
\ShowEq{polylinear map, algebra, canonical morphism}
где $\sigma_s$ - перестановка множества переменных
\ShowEq{transposition of set of variables, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{polylinear map, algebra}

\ShowTheorem{representation of algebra An in LAnA}
\ProofTheorem{\RefLinearMap}{representation of algebra An in LAnA}

\begin{convention}
Если тензор
\EqParm{a in Aoxn+1}{=z}
имеет разложение
\ShowEq{a=oxi}
то множество перестановок
\ShowEq{si in Sn}
и тензор $a$
порождают отображение
\ShowEq{ox:An->A}
определённое равенством
\ShowEq{ox circ =}
\qed
\end{convention}
\fi
\fi

\ePrints{}
\ifx\Semafor\ValueOn
\Section{Модуль над алгеброй}

\ShowEq{=left}

\ShowDefinition{module over algebra}

\ShowTheorem{definition of A module}
\ShowTheorem{definition of A module, property}
\ProofTheorem{\RefLinearMap}{definition of left A module}

\ShowEq{=right}
\ShowDefinition{module over algebra}
\fi

\ePrints{1506.00061,7287-9339}
\ifx\Semafor\ValueOn
\Section{Алгебра с сопряжением}

Пусть $D$ - коммутативное кольцо.
Пусть $A$ - $D$\hyph алгебра с единицей $e$, $A\ne D$.

Пусть существует подалгебра $F$ алгебры $A$ такая, что
$F\ne A$, $D\subseteq F\subseteq Z(A)$, и алгебра $A$ является свободным
модулем над кольцом $F$.
Пусть $\Basis e$ - базис свободного модуля $A$ над кольцом $F$.
Мы будем полагать $e_{\gi 0}=1$.

\begin{theorem}
\labelTheorem{structural constant of algebra with unit}
Структурные константы
$D$\hyph алгебры с единицей $e$ удовлетворяют условию
\ShowEq{structural constant re algebra, 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref structural constant of algebra with unit}
\end{proof}

Рассмотрим отображения
\ShowEq{Re Im A->A}
определенные равенством
\ShowEq{Re Im A->F 0}
\ShowEq{Re Im A->F 1}
Выражение
\ShowEq{Re Im A->F 2}
называется
\AddIndex{скаляром элемента}{scalar of algebra} $d$.
Выражение
\ShowEq{Re Im A->F 3}
называется
\AddIndex{вектором элемента}{vector of algebra} $d$.

Согласно
\EqRef{Re Im A->F 1}
\ShowEq{Re Im A->F 4}
Мы будем пользоваться записью
\ShowEq{scalar algebra of algebra}
для обозначения
\AddIndex{алгебры скаляров алгебры}{scalar algebra of algebra} $A$.

\begin{theorem}
\labelTheorem{Re Im A->F}
Множество
\ShowEq{vector module of algebra}
является $(\re A)$\Hyph модулем,
который мы называем
\AddIndex{модуль векторов алгебры}{vector module of algebra} $A$.
\ShowEq{A=re+im}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref Re Im A->F}
\end{proof}

Согласно теореме \RefTheorem{Re Im A->F},
однозначно определенно представление
\ShowEq{d Re Im}

\begin{definition}
\labelDefinition{conjugation in algebra}
Отображение
\ShowEq{conjugation in algebra}
\ShowEq{conjugation in algebra, 0}
называется
\AddIndex{сопряжением в алгебре}{conjugation in algebra}
при условии, если это отображение удовлетворяет равенству
\ShowEq{conjugation in algebra, 1}
$(\re A)$\Hyph алгебра $A$,
в которой определено сопряжение, называется
\AddIndex{алгеброй с сопряжением}{algebra with conjugation}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{conjugation in algebra}
$(\re A)$\Hyph алгебра $A$ является
алгеброй с сопряжением
тогда и только тогда, когда структурные константы
$(\re A)$\Hyph алгебры $A$ удовлетворяют условию
\ShowEq{conjugation in algebra, 5}
\ShowEq{conjugation in algebra, 4}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref conjugation in algebra}
\end{proof}
\fi

\ePrints{1601.03259,7287-9339,4975-6381,1506.00061}
\ifx\Semafor\ValueOn
\Section{Многочлен над ассоциативной \texorpdfstring{$D$}{D}-алгеброй}

Пусть $D$ - коммутативное кольцо и
$A$ - ассоциативная $D$\Hyph алгебра с единицей.
Пусть $\Basis F$ - базис алгебры
\ShowEq{L(A;B)}DAA.

\begin{theorem}
\labelTheorem{monomial of power k}
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\ShowEq{monomial of power k}
где $a_k\in A$ и  $F\in\Basis F$.
\end{enumerate}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref monomial of power k}
\end{proof}

В частности, одночлен степени $1$ имеет вид
\ShowEq{p1(x)=aFxa}

\begin{definition}
\labelDefinition{Abelian group of homogeneous polynomials over algebra}
Обозначим
\ShowEq{module of homogeneous polynomials over algebra}
абелевую группу,
порождённую множеством одночленов степени $k$.
Элемент $p_k(x)$ абелевой группы $A_k[x]$ называется
\AddIndex{однородным многочленом степени}
{homogeneous polynomial of power} $k$.
\qed
\end{definition}

\begin{convention}
Пусть тензор
\EqParm{a in Aoxn+1}{=.}
Пусть
\ShowEq{F1n in F}
Если
\ShowEq{x1=xn=x}
то мы положим
\ShowEq{a xn=}
\qed
\end{convention}

\begin{convention}
Если мы имеем несколько кортежей отображений $F\in\Basis F$,
то мы будем пользоваться индексом вида $[k]$
для индексирования кортежа
\ShowEq{F[k]=...}
\qed
\end{convention}

\begin{theorem}
\labelTheorem{homogeneous polynomial a circ xk}
Однородный многочлен $p(x)$
может быть записан в виде
\ShowEq{p(x)=a circ xk}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref map A(k+1)->pk otimes is polylinear map}
\end{proof}

\begin{definition}
\labelDefinition{Polynomial over algebra}
Обозначим
\ShowEq{algebra of polynomials over algebra}
прямую сумму\,\footnote{Смотри определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}
$A$\Hyph модулей $A_n[x]$.
Элемент $p(x)$ $A$\Hyph модуля $A[x]$ называется
\AddIndex{многочленом}{polynomial}
над $D$\Hyph алгеброй $A$.
\qed
\end{definition}

\ePrints{4975-6381,1601.03259}
\ifx\Semafor\ValueOn
Следующее определение
\RefDefinition{otimes -}
опирается на определение
\xRef[1302.7204]{definition: otimes -}.

\ShowDefinition{otimes -}

\begin{definition}
\labelDefinition{product of homogeneous polynomials}
Произведение однородных многочленов
\ShowEq{polynomials p,r}
определено равенством\,\footnote{
Определение
\RefDefinition{product of homogeneous polynomials}
опирается на определение
\xRef[1302.7204]{definition: product of homogeneous polynomials}.
}
\ShowEq{pr=p circ r}
\qed
\end{definition}

\ePrints{}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{p(x)=a k-1 k}
Пусть
\ShowEq{p(x)=a circ xk}
одночлен степени $k>1$.
Тогда многочлен $p(x)$ может быть представлен в 
одной из следующих форм
\ShowEq{p(x)=a k-1 k 1}
\ShowEq{p(x)=a k-1 k 2}
где
\ShowEq{p(x)=a k-1 k 3}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\RefTheorem[1302.7204]{p(x)=a k-1 k}.
\end{proof}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%

\begin{definition}
\labelDefinition{divisor of polynomial}
Многочлен $p(x)$ называется
\AddIndex{делителем многочлена}{divisor of polynomial} $r(x)$,
если мы можем представить многочлен $r(x)$ в виде
\ShowEq{r=qpq(x)}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{r=+q circ p}
Пусть
\ShowEq{p=p circ x}
- однородный многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p}
\end{proof}

\begin{theorem}
\labelTheorem{r=+q circ p 1}
Пусть
\ShowEq{p=p+p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p 1}
\end{proof}
\fi
\fi

\ePrints{BQuater,309618526,CACAA.06.121,9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\Section{Производная отображения банаховой алгебры}

\begin{definition}
Нормированная $D$\Hyph алгебра $A_1$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A_1$ сходится, т. е.
имеет предел в алгебре $A_1$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{continuous map, algebra}
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264}
\ifx\Semafor\ValueOff

\ShowTheorem{set of A->B is D module}
\begin{proof}
\TheoremFollows
ффф
\end{proof}

\else

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|f(a)|<|f||a| 1n}
\else
\ShowProof{|f(a)|<|f||a| 1n}
\fi

\ShowTheorem{|on|->0 ona1p->0}
\ePrints{CACAA.06.121}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|on|->0 ona1p->0}
\else
\ShowProof{|on|->0 ona1p->0}
\fi
\fi

\ShowDefinition{differentiable map}DAB{algebra}

\begin{definition}
\labelDefinition{differential of map}
{\it
Если, для данного $x$, приращение
\eqRef{derivative of map, def}{algebra}
отображения
\ShowEq{f:A->B}fAA
рассматривать как функцию дифференциала $dx$ переменной $x$,
то линейная часть этой функции
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{}
называется
\AddIndex{дифференциалом отображения}{differential of map}
$f$.
}
\qed
\end{definition}

\ShowEq{remark: differential L(A,A)}

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{derivative, representation in algebra}
\ProofTheorem{\RefCalculus}{derivative, representation in algebra}
\fi

\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOff
\ShowTheorem{representation of derivative, algebra A->B}
\begin{proof}
\TheoremFollows
\ShowEq{ref differentiable map A->B}
\end{proof}

\ShowDefinition{coordinates of derivative, algebra A->B}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowTheorem{dfa1p/dx=df/dx a1p}
\ShowProof{dfa1p/dx=df/dx a1p}

\ShowTheorem{bilinear map and differential}

\ShowTheorem{derivative of tensor product}

%\ShowTheorem{map is continuous, derivative}
%\begin{proof}
%\TheoremFollows
%\ShowEq{ref map is continuous, derivative}
%\end{proof}
\fi

\ePrints{309618526,CACAA.06.121,9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\ShowDefinition{derivative of Second Order, algebra}

\ShowDefinition{derivative of Order n, algebra}
\fi
\fi

\ePrints{0767-8264}
\ifx\Semafor\ValueOn
\ShowDefinition{indefinite integral 2017}
\fi

\ePrints{1601.03259,4975-6381,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\Section{Комплексное поле}

\ShowTheorem{complex field over real field}
\ShowProof{complex field over real field}

\ShowDefinition{maps of conjugation, complex field}

\ShowTheorem{linear map of complex field}
\ProofTheorem{1003.1544}{additive map of complex field, structure}

\begin{corollary}
\labelCorollary{basis of L(R;C;C)}
{\it
$C\otimes C$\Hyph модуль
\ShowEq{L(A;B)}RCC{}
является $C$\Hyph векторным пространством
и имеет базис
\ShowEq{e=(E,I)}.
}
\qed
\end{corollary}

\begin{theorem}
\labelTheorem{CE is algebra isomorphic to complex field}
Множество
\ShowEq{CE set}
является $R$\Hyph алгеброй, изоморфной полю комплексных чисел.
\end{theorem}
\begin{proof}
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map of complex field}.
\end{proof}

\begin{theorem}
\labelTheorem{L(CCC)=CE}
\ShowEq{L(CCC)=CE}
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\EqRef{linear map of algebra C, structure, 2}
и коммутативности произведения комплексных чисел.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations linear}
Матрица линейного отображения $f\in CE$
\ShowEq{yi=xj fji}
удовлетворяет соотношению
\ShowEq{complex field over real field}
\end{theorem}
\ProofTheorem{1003.1544}{complex field over real field}

\begin{theorem}
\labelTheorem{matrix of linear map f in CI}
Матрица линейного отображения $f\in CI$
\ShowEq{yi=xj fji}
удовлетворяет соотношению\,\footnote{
Смотри также раздел
\xRef[1003.1544]{section: System of Additive Equations in Complex Field}.
}
\ShowEq{matrix of linear map f in CI}
\end{theorem}
\begin{proof}
Утверждение следует из равенств
\ShowEq{congugate map complex field, 3}
\end{proof}

\ePrints{4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
Множество
\ShowEq{CI set}
не является $R$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{aI o bI=...E}
опирающегося на теорему
\RefTheorem{linear map of complex field}.
\end{proof}

\ePrints{...}
\ifx\Semafor\ValueOn

\begin{definition}
\labelDefinition{differentiable map of complex field}
{\it
Отображение
\ShowEq{f:C->C}
поля комплексных чисел
называется
\AddIndex{дифференцируемым}{differentiable map}
на множестве $U\subset C$,
если в каждой точке $x\in U$
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{}
где
\ShowEq{df:A->B}CC
- линейное отображение $C$\Hyph векторного пространства $C$ и
\ShowEq{o:A->B}oCC
- такое непрерывное отображение, что
\ShowEq{lim |o|/|a|}CC
Линейное отображение
$\displaystyle\ShowSymbol{derivative of map}{}$
называется
\AddIndex{производной отображения}{derivative of map}
$f$.
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{dx fx in CE}
Если отображение
\ShowEq{f:C->C}
поля комплексных чисел
дифференцируемо,
то
\ShowEq{dx fx in CE}
\end{theorem}
\begin{proof}
\TheoremFollows
\RefTheorem{CE is algebra isomorphic to complex field}
и определения
\RefDefinition{differentiable map of complex field}.
\end{proof}

\begin{definition}
{\it
Дифференцируемое отображение поля комплексных чисел называется
\AddIndex{голоморфным}{holomorphic map}.
}
\qed
\end{definition}

\ShowTheorem{Cauchy Riemann equations, complex field, 1}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Cauchy Riemann equations linear},
\RefTheorem{dx fx in CE}.
\end{proof}

\ShowEq{theorem: Cauchy Riemann equations, complex field}f
\ShowEq{proof: Cauchy Riemann equations, complex field}f

\ShowDefinition{projection maps, complex field}

\ShowTheorem{Expansion of projection maps relative E,I}
\ShowProof{Expansion of projection maps relative E,I}

\begin{theorem}
\labelTheorem{df=...dx= CE}
Производная отображения
\ShowEq{f:C->C}
поля комплексных чисел
имеет вид\,\footnote{
Теоремы в этом разделе
аналогичны теоремам в \citeBib{Shabat: Complex Analysis}, с. 31 - 33.}
\ShowEq{df=...dx= CE}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{Expansion of projection maps relative E,I},
\ShowEq{dx01=}
является следствием равенства
\ShowEq{dx=dx0+dx1}
Равенство
\ShowEq{df=...dx}
является следствием равенств
\EqRef{dx01=}
и
\ShowEq{df=df/dx0+df/dx1}
Равенство
\DrawEq{df/dx= complex field}{theorem}
является следствием равенства
\EqRef{df=...dx}
и определения
\RefDefinition{differential of map}.
Равенство
\EqRef{df=...dx= CE}
является следствием равенства
\eqRef{df/dx= complex field}{theorem}
и теоремы
\RefTheorem{Cauchy Riemann equations, complex field}.
\end{proof}
\fi
\fi
\fi

\ePrints{1506.00061,7287-9339,309618526,CACAA.06.121,9835-2163,0767-8264}%
\ifx\Semafor\ValueOn%

\Section{Алгебра кватернионов}

\begin{definition}
\labelDefinition{quaternion algebra}
Пусть $R$ - поле действительных чисел.
Расширение
\ShowEq{quaternion algebra}
поля $R$ называется
\AddIndex{алгеброй кватернионов}{quaternion algebra},
если произведение в алгебре $H$ определено согласно правилам
\ShowEq{product of quaternions}
\qed
\end{definition}

Элементы алгебры $H$ имеют вид
\ShowEq{quaternion algebra, element}
Кватернион
\ShowEq{conjugate to the quaternion}x
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion}
Из равенства
\EqRef{norm of quaternion}
следует, что обратный элемент имеет вид
\ShowEq{inverce quaternion}

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{quaternion conjugation}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref quaternion conjugation}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{Quaternion over real field}
Положим
\ShowEq{basis of quaternion}
базис алгебры кватернионов $H$.
Тогда структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product of quaternions}.
\end{proof}
\fi

\ePrints{...}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\ShowEq{basis of quaternion}
Стандартные компоненты линейного отображения над полем $R$
и координаты этого отображения над полем $R$
удовлетворяют соотношениям
\ShowEq{quaternion fUD<-fUU}
\ShowEq{quaternion fUD->fUU}
где
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref Quaternion over real field, matrix}
\end{proof}
\fi

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\ShowDefinition{quaternion maps of conjugation}

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{ao Jacobian matrix}EHl
\begin{proof}
\TheoremFollows
\ShowEq{ref aE, quaternion, Jacobian matrix}
\end{proof}
\fi

\ShowTheorem{linear map, maps of conjugation, algebra}H
\begin{proof}
\TheoremFollows
\ShowEq{ref expand linear mapping, quaternion}
\end{proof}

\ShowTheorem{L is left vector space}H

\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOff
\ShowTheorem{HE is algebra isomorphic to quaternion algebra}
\ShowProof{HE is algebra isomorphic to quaternion algebra}
\fi
\fi

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOn%
\begin{theorem}
\labelTheorem{ax-xa=1 quaternion algebra}
Уравнение
\ShowEq{ax-xa=1}
в алгебре кватернионов не имеет решений.
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref ax-xa=1 quaternion algebra}
\end{proof}
\fi
\fi

\def\Preliminary{off}
\ShowEq{SetupRef}


==> Representation.Examples.1.Russian.tex <==
%auto-ignore

\input{Representation.Examples.1.Eq}

\chapter{Примеры диаграммы представлений: модуль}
\labelChapter{Examples of Diagram of Representations: Module}

\section{Об этой главе}

Теория представлений
универсальной алгебры - это важный инструмент,
которым я пользуюсь на протяжении многих лет
для изучения алгебры, геометрии, математического анализа.
Основная задача этой и следующей глав -
показать как работает теория представлений
универсальной алгебры в различных разделах математики.

Примеры в этой главе имеют отношение к различным конструкциям,
связанным с модулем над кольцом.

Первый пример - это абелевая группа.
Модуль - это эффективное представление кольца в абелевой группе.
Поэтому существует параллель между абелевой группой и модулем.
Я рассматриваю это сходство в разделе
\RefSection{Abelian Group}.

Модуль над коммутативным кольцом - это относительно простая конструкция.
С другой стороны, многие определения теории представлений
(базис представления, морфизм представлений, свободное представления)
опираются на аналогичные определения в модуле.
Поэтому раздел
\RefSection{Vector Space}
посвящён детальному рассмотрению модуля над коммутативным кольцом.

Я рассматриваю алгебру над коммутативным кольцом в разделе
\RefSection{Algebra over Ring}
и левый модуль над $D$\Hyph алгеброй в разделе
\RefSection{Module over Algebra}.
Мы можем рассматривать модуль над некоммутативным кольцом
также как мы рассматривали модуль над коммутативным кольцом.
Однако мы встречаем серьёзные проблемы при
изучении линейного отображения.

Рассмотрение некоммутативного кольца как
алгебры над центром кольца существенно меняет картину.
Анализ диаграммы представлений,
описывающей модуль $V$ над
$D$\Hyph алгеброй $A$,
позволяет рассмотреть различные группы отображений,
сохраняющих структуру алгебры.
Среди этих отображений мы выделяем
линейные отображения $A$\Hyph модуля $V$
(приведенный морфизм $D$\Hyph модуля $V$)
и гомоморфизм $A$\Hyph модуля $V$
(приведенный морфизм диаграммы представлений).
Такое определение линейного отображения
позволяет рассмотреть полилинейное отображение модуля над
$D$\Hyph алгеброй $A$.

Если $D$\Hyph алгебра $A$ является банаховой,
то мы получаем инструмент для изучения математического анализа
функций нескольких переменных.
К сожалению, структура линейного отображения некоммутативной алгебры
лежит вне рамок этой главы.
Подробнее эту тему читатель может изучить в книге
\ShowEq{citeBib RefLinearMap}

\section{Абелевая группа}
\labelSection{Abelian Group}

\ShowDefinition{action of rational integers in Abelian group}

\ShowTheorem{action of ring of rational integers in Abelian group}
\ShowProof{action of ring of rational integers in Abelian group}

\ShowTheorem{structure of Abelian group}
\ShowProof{structure of Abelian group}

\section{Векторное пространство}
\labelSection{Vector Space}

\subsection{Модуль над коммутативным кольцом}

\ShowEq{=module}

\ShowDefinition{module over commutative ring}

\ShowTheorem{module over algebra}
\ShowProof{module over algebra}

\ShowTheorem{definition of A module}
\ShowTheorem{definition of A module, property}
\ShowProof{definition of A module}

\ShowEq{show linear combination of vectors}

\ShowEq{show basis of module}

\ShowExample{Abelian Group is Z module}

\subsection{Линейное отображение}

\ShowEq{show linear map from D1 A1 to D2 A2, module}

\ShowEq{=DD}

\ShowDefinition{linear map from A1 to A2, commutative module}

\ShowTheorem{linear map of module}
\ShowProof{linear map, DA1->DA2, module}

\ShowTheorem{linear map of module, coordinates}
\ShowProof{linear map of module, coordinates}

\subsection{Полилинейное отображение}

\ShowDefinition{polylinear map of modules}

\ShowTheorem{polylinear map of modules}
\ShowProof{polylinear map of modules}

\ShowTheorem{sum of polylinear maps, module}
\ShowProof{sum of polylinear maps, module}

\ShowCorollary{sum of linear maps, D module}

\ShowTheorem{module of polylinear maps}
\ShowProof{module of polylinear maps}

\ShowCorollary{product of linear map over scalar, D module}

\section{Алгебра над коммутативным кольцом}
\labelSection{Algebra over Ring}

\ShowDefinition{algebra over ring}

\ShowTheorem{Free Algebra over Ring}
\ShowProof{Free Algebra over Ring}

Обычно, когда мы рассматриваем $D$\Hyph алгебру $A$, мы
выбираем базис $\Basis e$ соответствующего $D$\Hyph модуля $A$.
Этот выбор удобен, так как
если $D$\Hyph модулЬ $A$ является свободным $D$\Hyph модулем,
то разложение вектора однозначно
относительно базиса $D$\Hyph модуля $A$.
Это, в частности, позволяет описать операции произведения, указав структурные константы
алгебры относительно заданого базиса.

В общем случае, базис $R$\Hyph модуля $A$ может оказаться множеством образующих.
Например, если в векторном пространстве $H$, в котором задана алгебра
кватернионов над полем действительных чисел, рассмотреть базис
\ShowEq{quaternion basis over R}
то в алгебре $H$ верно равенство
\ShowEq{quaternion basis over R 1}
Следовательно, множество
\ShowEq{quaternion basis over R 2}
является базисом алгебры $H$.
Следствием равенства
\EqRef{quaternion basis over R 1}
является неоднозначность представления кватерниона относительно
заданного базиса.
А именно, кватернион $a\in H$ можно записать в виде
\ShowEq{quaternion basis over R 3}
где $a^{\gi 4}$ - произвольно.

\section{Левый модуль над алгеброй}
\labelSection{Module over Algebra}

\ShowEq{=left}

\ShowEq{show definition of A module}

Билинейное отображение
\ShowEq{AV->V}
порождённое левосторонним представлением $g_{2,3}$ называется
\AddIndex{левосторонним произведением}{left-side product}
вектора на скаляр.

\ShowEq{show linear combination of vectors}

\ShowEq{show basis of module}

\section{Правый модуль над алгеброй}

\ShowEq{=right}

\ShowEq{show definition of A module}

Билинейное отображение
\ShowEq{VA->V}
порождённое правосторонним представлением $g_{2,3}$ называется
\AddIndex{правосторонним произведением}{right-side product}
вектора на скаляр.

\ShowEq{show linear combination of vectors}

\ShowEq{show basis of module}

\section{Левый модуль над неассоциативной алгеброй}

Теоремы
\RefTheorem{definition of \SideWS module},
\RefTheorem{definition of \SideWS module, property}
рассматривают структуру модуля над ассоциативной $D$\Hyph алгеброй $A$.
Нетрудно заметить, что с учётом некоторых поправок,
эти теоремы остаются верны если $A$ -
неассоциативная $D$\Hyph алгебра.
Однако, так как произведение в $D$\Hyph алгебре $A$ неассоциативно,
а произведение преобразований в модуле над $D$\Hyph алгеброй $A$ ассоциативно,
то отображение $g_{34}$ не может быть представлением
неассоциативной $D$\Hyph алгебры $A$.

Мы подошли к той границе, где определена теория представлений универсальной алгебры.
Для того, чтобы сохранить возможность применения рассмотренного в этой книге аппарата,
мы можем согласиться, что отображение
\ShowEq{f:A->B}{g_{34}}{A\times V}V
является представлением, если отображение $g_{34}$ является билинейным отображением.
Появляются новые вопросы, рассмотрение которых выходит за рамки этой книги.

Однако мы можем рассмотреть эту задачу с другой стороны.
Если отображение $g_{34}$ не сохраняет операцию произведения,
то мы полагаем, что отображение $g_{34}$ - это
представление $D$\Hyph алгебры $A$, в которой
не определено произведение.
Другими словами, отображение $g_{34}$ - это
представление $D$\Hyph модуля.
Следовательно, диаграмма представлений будет иметь вид
\ShowEq{diagram of representations, left module nonassociative 1}
Однако мы потеряли структуру $D$\Hyph алгебры $A$ в диаграмме представлений
\EqRef{diagram of representations, left module nonassociative 1}.
Следовательно, правильная диаграмма представлений будет иметь вид
\ShowEq{diagram of representations, left module nonassociative}


==> Representation.Examples.2.Russian.tex <==
%auto-ignore

\input{Representation.Examples.2.Eq}

\chapter{Примеры диаграммы представлений: аффинная геометрия}

\section{Об этой главе}

В главе
\RefChapter{Examples of Diagram of Representations: Module}
мы рассмотрели примеры диаграммы представлений,
связанные с модулем над кольцом.
Если бы теория представлений сводилась бы к изучению модулей,
вряд ли это была бы интересная теория.

В этой главе я рассмотрел примеры диаграммы представлений,
связанные с аффинной геометрией.
Внешне простая алгебраическая конструкция
оказалась для меня богатейшим источником вдохновения.
Я дважды встретил интересные идеи в этой области математики.
Сперва изучая аффинную геометрию, я обнаружил, что я могу
описать аффинную геометрию с помощью башни представлений.
Впоследствии, изучая таким же образом алгебру над коммутативным кольцом,
я стал изучать диаграмму представлений.

Однако второе открытие пришло ко мне случайно.
Когда я просматривал учебник по математическому анализу,
я встретил определение знакомое с детства.
Сумма векторов.
Определение крайне простое.
При определении многообразия аффинной связности
мы имем сумму векторов в касательной плоскости.
Но в этот раз я понял, что я могу определить
сумму векторов пользуясь параллелограммом из геодезических.
Это позволило построить аффинную геометрию на многообразии аффинной связности.

Ещё один шаг, и от многообразия аффинной связности
я перешёл к метрико аффинному многообразию.
Так как параллелограм из геодезических не замкнут,
то сумма векторов в метрико аффинном многообразии не коммутативна.
Без сомнения, это исследование, которое выходит за рамки этой книги
и к которому я надеюсь вернуться в будущем.
Однако я решил написать набросок этой конструкции
в разделе
\RefSection{Noncommutative Sum},
чтобы показать читателю границы теории,
изложенной в этой книге.
%так как читатель видит что теория представлений расслоенной
%универсальной алгебры имеет другой вид.

Теория представлений является естественным продолжением
теории универсальных алгебр.
Предполагается, что бинарная операция на универсальной алгебре $A$
определена для любой пары $A$\Hyph чисел.
Однако очевидно, что сумма векторов в аффинной геометрии на
дифференцируемом многообразии хорошо определена только
в достаточно малой окрестности.

С похожей задачей я столкнулся в статье
\citeBib{1201.4158},
где я и Александр Ложье
изучали ортогональные преобразования в пространстве Минковского.
Мы обнаружили, что произведение ортогональных преобразований
не всегда является ортогональным преобразованием,
и следовательно множество ортогональных преобразований
не является группой.

\section{Представление группы на множестве}
\labelSection{representation of group on the set}

Пусть $G$ - абелевая группа, и $M$ - множество.
Рассмотрим эфективное представление группы $G$ на множестве $M$.
Для заданных $a\in G$, $A\in M$ положим
\ShowEq{A=>A+a}.
Мы будем также пользоваться
записью $a=\overset{\rightarrow}{AB}$, если
\ShowEq{representation of group on the set, 1}
Тогда действие группы можно представить в виде
\ShowEq{representation of group on the set, 2}
Поскольку представление эффективно, то из равенств
\EqRef{representation of group on the set, 1},
\EqRef{representation of group on the set, 2}
и равенства
\ShowEq{representation of group on the set, 3}
следует, что
\ShowEq{representation of group on the set, 4}

Мы будем называть вектором
$G$\Hyph число $a$
и соответствующее преобразование $\Vect AB$.
Мы интерпретируем равенство
\EqRef{representation of group on the set, 4}
как независимость вектора $a$ от выбора $M$\Hyph числа $A$.

Мы можем рассматривать множество $M$ как объединение орбит представления группы $G$.
В качестве базиса представления можно выбрать
множество точек таким образом, что одна и только одна точка
принадлежит каждой орбите представления.
Если $X$ - базис представления, $A\in X$, $g\in G$, то $\Omega_2$\Hyph слово
имеет вид $A+g$. Поскольку на множестве $M$ не определены операции,
то не существует $\Omega_2$\Hyph слово, содержащее различные элементы базиса.
Если представление группы $G$ однотранзитивно,
то базис представления состоит из одной точки.
Этой точкой может быть любая точка множества $M$.

\begin{theorem}
\labelTheorem{determine sum of vectors}
Пусть представление
\ShowEq{A=>A+a}{}
абелевой группы $G$ на множестве $M$ однотранзитивно.
Тогда, для любых $M$\Hyph чисел $A$, $B$, $C$,
определена сумма векторов $\Vect AB$ и $\Vect BC$
и сумма векторов удовлетворяет равенству
\ShowEq{AB+BC=AC}
\end{theorem}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
\setlength{\parindent}{.8cm}
{\sc Доказательство.}
Поскольку представление однотранзитивно,
то, для любых $M$\Hyph чисел $A$, $B$, $C$,
существуют векторы $\Vect AB$, $\Vect BC$
такие, что
\DrawEq[{\Vect{A}{B}}AB]{B=A+a}B
\DrawEq[{\Vect BC}BC]{B=A+a}C
\end{minipage}
&
\ShowEq{Vector v+w=AC}ab{}
\end{tabular}

\noindent
Равенство
\ShowEq{C=A+a+b}
является следствием равенств
\eqRef{B=A+a}B,
\eqRef{B=A+a}C
и ассоциативности сложения в абелевой группе $G$.
Поскольку представление однотранзитивно,
то равенство
\EqRef{AB+BC=AC}
является следствием равенства
\EqRef{C=A+a+b}
и равенства
\DrawEq[{\Vect AC}AC]{B=A+a}{}
Это определение суммы называется
правилом треугольника.
\qed

\begin{remark}
Так как $G$ - абелева группа, то утверждения
\RefItem{AA=0},
\RefItem{AB=-BA},
следуют из теоремы
\RefTheorem{determine sum of vectors}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{AA=0}
\item
\ShowEq{AB=-BA}
\item
Сложение коммутативно.
\labelItem{Addition is commutative}
\item
Сложение ассоциативно.
\labelItem{Addition is associative}
\end{enumerate}
\qed
\end{remark}

\begin{theorem}
\labelTheorem{parallelogram G->*M}
Для заданных $a$, $b\in G$ и $A\in M$
рассмотрим следующее множество $M$\Hyph чисел.
\ShowEq{parallelogram G->*M}
\end{theorem}

\begin{proof}
Теорема является следствием утверждения
\RefItem{Addition is commutative}.
\end{proof}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{180pt}
\setlength{\parindent}{5mm}
\begin{theorem}
\labelTheorem{Axiom of parallelogram}
Если
\ShowEq{axiom: 4, drc affine space, 11}
то
\ShowEq{axiom: 4, drc affine space, 12}
\end{theorem}
\end{minipage}
&
\begin{minipage}{140pt}
\ShowEq{AB=CD...}
\end{minipage}
\end{tabular}

\begin{proof}
Положим
\ShowEq{AB=a AC=b}
Согласно утверждению
\RefItem{AB=-BA},
\ShowEq{BA=-a}
Теорема является следствием равенства
\ShowEq{D=B+...}
\end{proof}

\section{Аффинное пространство}
\labelSection{Affine space is single transitive representation}

\begin{definition}
\labelDefinition{drc affine space, 1}
Пусть $D$ - коммутативное кольцо и $V$ - свободный $D$\Hyph модуль.
Множество точек $\Vcirc$ называется
\AddIndex{аффинным пространством}{affine space}
над $D$\Hyph модулем $V$,
если множество точек $\Vcirc$ удовлетворяет
следующим аксиомам.\,\footnote{Я написал определения и теоремы
в этом разделе согласно определению аффинного пространства в
\citeBib{Rashevsky}, с. 86 - 93.}
\StartLabelItem
\begin{enumerate}
\item
\label{axiom: 1, drc affine space}
Существует по крайней мере одна точка
\item
\labelItem{axiom: 2, affine space}
Каждой паре точек $(A, B)$ поставлен в соответствие один и
только один вектор. Этот вектор мы будем обозначать $\Vect AB$.
Вектор $\Vect AB$ имеет начало в точке $A$ и конец в точке B.
\item
\labelItem{axiom: 3, affine space}
Для каждой точки $A$ и любого вектора $a$ существует одна
и только одна точка $B$ такая, что
\ShowEq{axiom: 3, drc affine space, 1}
Мы будем также пользоваться записью\,\footnote{\citeBib{Bamberg Sternberg},
с. 9.}
\ShowEq{axiom: 3, drc affine space}
\item
\labelItem{axiom: 4, affine space}
(Аксиома параллелограмма.) Если
\ShowEq{axiom: 4, drc affine space, 11}
то
\ShowEq{axiom: 4, drc affine space, 12}
\end{enumerate}
Множество $V$ называется множеством свободных векторов.
$\Vcirc$\Hyph числа называются
точками аффинного пространства $\Vcirc$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{sum of vectors, affine space}
Пусть $A\in\Vcirc$ - произвольная точка.

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
Пусть $v$ - вектор.
Согласно аксиоме
\RefItem{axiom: 3, affine space},
существует
$B\in\Vcirc$,
$B=A+v$.
\end{minipage}
&
\ShowEq{Vector v=AB}
\end{tabular}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
Пусть $w$ - вектор. 
Согласно аксиоме
\RefItem{axiom: 3, affine space},
существует
$C\in\Vcirc$,
$C=B+w$.
\end{minipage}
&
\ShowEq{Vector w=BC}
\end{tabular}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{190pt}
Согласно аксиоме
\RefItem{axiom: 2, affine space},
существует вектор $\Vect AC$.
Вектор $\Vect AC$ называется суммой векторов
$v$ и $w$
\ShowEq{sum of vectors, affine space}
Это определение суммы называется
правилом треугольника.
\end{minipage}
&
\ShowEq{Vector v+w=AC}vw{}
\end{tabular}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{vectors of affine space, zero vector}
Вектор $\Vect AA$
является нулём по отношению к операции сложения
и не зависит от выбора точки $A$.
Вектор $\Vect AA$ называется нуль\Hyph вектором
и мы полагаем $\Vect AA=0$.
\end{theorem}
\begin{proof}
Мы можем записать правило сложения
\EqRef{sum of vectors, affine space} в виде
\ShowEq{sum of vectors, affine space, 1}
Если $B=C$, то из равенства
\EqRef{sum of vectors, affine space, 1} следует
\ShowEq{sum of vectors, affine space, 2}
Из равенства
\EqRef{sum of vectors, affine space, 2}
следует, что
вектор $\Vect BB$
является нулём по отношению к операции сложения.
Если $C=A$, $B=D$, то
из аксиомы
\RefItem{axiom: 4, affine space}
следует
\ShowEq{sum of vectors, affine space, 3}
Следовательно,
нуль\Hyph вектор $\Vect AA$ не зависит от выбора точки $A$.
\end{proof}

\begin{theorem}
\labelTheorem{vectors of affine space, opposite vector}
Пусть
\ShowEq{a = AB}aAB.
Тогда
\ShowEq{vectors of affine space, opposite vector}
и это равенство
не зависит от выбора точки $A$.
\end{theorem}
\begin{proof}
Из равенства
\EqRef{sum of vectors, affine space, 1}
и теоремы
\RefTheorem{vectors of affine space, zero vector}
следует
\ShowEq{sum of vectors, affine space, 4}
Равенство \EqRef{vectors of affine space, opposite vector}
следует из равенства \EqRef{sum of vectors, affine space, 4}.
Применяя аксиому
\RefItem{axiom: 4, affine space}
к равенству
\ShowEq{sum of vectors, affine space, 9}
получим
\ShowEq{sum of vectors, affine space, 10}
или, что то же,
\ShowEq{sum of vectors, affine space, 11}
Из равенства
\EqRef{sum of vectors, affine space, 11}
и аксиомы
\RefItem{axiom: 4, affine space}
следует, что
\ShowEq{sum of vectors, affine space, 12}
Следовательно, равенство \EqRef{vectors of affine space, opposite vector}
не зависит от выбора точки $A$.
\end{proof}

\begin{theorem}
\labelTheorem{vectors of affine space, independence of sum on point}
Сумма векторов $v$ и $w$ не зависит от выбора точки $A$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{vectors AB BC}

Сумма векторов $v$ и $w$ определена
согласно определению
\RefDefinition{sum of vectors, affine space}.
\ShowEq{sum of vectors, affine space, 16}
Согласно аксиоме
\RefItem{axiom: 4, affine space},
из равенств
\EqRef{AB=A'B'},
\EqRef{BC=B'C'}
следует, что
\ShowEq{sum of vectors, affine space, 5}
Применяя аксиому
\RefItem{axiom: 4, affine space}
к крайним членам равенства \EqRef{sum of vectors, affine space, 5},
получаем
\ShowEq{sum of vectors, affine space, 6}
Из равенства \EqRef{sum of vectors, affine space, 6}
следует утверждение теоремы.
\end{proof}

\begin{theorem}
\labelTheorem{vectors of affine space, sum associative}
Сложение векторов ассоциативно.
\end{theorem}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{180pt}
\setlength{\parindent}{5mm}
{\sc Доказательство.}
Пусть
\ShowEq{a = AB}vAB,
\ShowEq{a = AB}wBC,
\ShowEq{a = AB}uCD.
Из равенства
\ShowEq{vectors of affine space, sum associative, 3}
\end{minipage}
&
\begin{minipage}{140pt}
\setlength{\parindent}{5mm}
\ShowEq{vAB+wBC+uCD}
\end{minipage}
\end{tabular}

{
\setlength{\parindent}{0mm}
следует
\ShowEq{vectors of affine space, sum associative, 1}
Из равенства
\ShowEq{vectors of affine space, sum associative, 4}
следует
\ShowEq{vectors of affine space, sum associative, 2}
Теорема следует из сравнения равенств
\EqRef{vectors of affine space, sum associative, 1} и
\EqRef{vectors of affine space, sum associative, 2}.
\qed
}

\begin{theorem}
\labelTheorem{vectors of affine space, Abelian group}
На множестве $V$ определена структура абелевой группы.
\end{theorem}
\begin{proof}
Из теорем \RefTheorem{vectors of affine space, zero vector},
\RefTheorem{vectors of affine space, opposite vector},
\RefTheorem{vectors of affine space, independence of sum on point},
\RefTheorem{vectors of affine space, sum associative}
следует, что операция сложение векторов определяет группу.
\newline
%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{190pt}
Пусть
\ShowEq{a = AB}vAB,
\ShowEq{a = AB}wBC.
\ShowEq{sum of vectors, affine space, 7}
Согласно аксиоме
\RefItem{axiom: 3, affine space}
существует точка $D$ такая, что
\ShowEq{sum of vectors, affine space, 17}
\end{minipage}
&
\begin{minipage}{130pt}
\ShowEq{Vector v+w=w+v ABCD}
Правило параллелограмма.
\end{minipage}
\end{tabular}

\setlength{\parindent}{0mm}
Согласно аксиоме
\RefItem{axiom: 4, affine space},
\ShowEq{sum of vectors, affine space, 18}
Согласно определению суммы векторов
\ShowEq{sum of vectors, affine space, 8}
Из равенств
\EqRef{sum of vectors, affine space, 7} и
\EqRef{sum of vectors, affine space, 8}
следует коммутативность сложения.
\end{proof}

\begin{theorem}
\labelTheorem{vectors of affine space, Abelian group representation}
Отображение
\ShowEq{drc affine space, map to A circle}
определённое равенством
\EqRef{axiom: 3, drc affine space},
является однотранзитивным представлением абелевой группы $V$.
\end{theorem}
\begin{proof}
Аксиома
\RefItem{axiom: 3, affine space}
определяет отображение
\EqRef{drc affine space, map to A circle}.
Из теоремы
\RefTheorem{vectors of affine space, independence of sum on point}
следует, что отображение \EqRef{drc affine space, map to A circle}
является представлением.
Эффективность представления следует
из теоремы \RefTheorem{vectors of affine space, zero vector}
и аксиомы
\RefItem{axiom: 2, affine space}.
Из аксиомы 
\RefItem{axiom: 2, affine space}
следует также, что представление транзитивно.
Эффективное и транзитивное представление однотранзитивно.
\end{proof}

Сравнение теоремы
\RefTheorem{vectors of affine space, Abelian group representation}
и утверждений раздела
\RefSection{representation of group on the set}
видно, что
однотранзитивное представление абелевой группы $V$
на множестве $\Vcirc$
эквивалентно аксиомам аффинного пространства.
Однако, пользуясь теоремой
\RefTheorem{vectors of affine space, Abelian group representation}
как определением аффинного пространства,
мы теряем многие важные конструкции в аффинном пространстве.
Например, вектор определяет преобразование параллельного переноса
в аффинном пространстве.
Но у нас нет инструмента, чтобы определить преобразование
поворота аффинного пространства.

Если мы внимательно посмотрим на определение
\RefDefinition{drc affine space, 1},
то мы увидим, что абелевая группа $V$ имеет дополнительную структуру,
поскольку абелевая группа $V$ является $D$\Hyph модулем.
Таким образом, мы получаем следующую теорему.

\begin{theorem}
Пусть $D$ - коммутативное кольцо,  $V$ - абелева группа
и $\Vcirc$ - множество.
Если $A\in\Vcirc$ и $v\in V$,
то мы будем обозначать действие вектора $v$
на точку $A$ выражением $A+v$.
\AddIndex{Аффинное пространство}{affine space}
над $D$\Hyph модулем $V$
- это диаграмма представлений
\ShowEq{drc affine space, tower of representations}
где $f_{12}$ - эффективное представление
коммутативного кольца $D$ в абелевой группе $V$
и $f_{23}$ - однотранзитивное правостороннее представление абелевой группы $V$
в множестве $\Vcirc$.
\end{theorem}

\begin{proof}
Мы полагаем, что множество $\Vcirc$ не пусто;
следовательно множество $\Vcirc$ удовлетворяет аксиоме
\ref{axiom: 1, drc affine space}.
Поскольку $v\in V$ порождает преобразование множества,
то для любого $A\in M$ однозначно определён $B\in M$ такое, что
\DrawEq[vAB]{B=A+a}{}
Это утверждение доказывает аксиому
\RefItem{axiom: 3, affine space}.
Поскольку представление $f_{23}$ однотранзитивно, то для любых
$A$, $B\in\Vcirc$ существует единственное $v\in V$ такое, что
\DrawEq[vAB]{B=A+a}{}
Это утверждение позволяет ввести обозначение
\ShowEq{affine structure on set, 1}
а также доказывает аксиому
\RefItem{axiom: 2, affine space}.
Аксиома
\RefItem{axiom: 4, affine space}
следует из утверждения теоремы
\RefTheorem{Axiom of parallelogram}.

Представление $f_{12}$ гарантирует, что абелевая группа $V$
является $D$\Hyph модулем.
\end{proof}

Абелевая группа $V$ действует однотранзитивно на множестве $\Vcirc$.
Из построений в разделе
\RefSection{representation of group on the set}
следует, что базис множества $\Vcirc$ относительно представления
абелевой группы $V$ состоит из одной точки. Эту точку обычно обозначают
буквой $O$ и называют
\AddIndex{началом системы координат аффинного пространства}
{origin of coordinate system of affine space}.
Следовательно, произвольную точку $A\in\Vcirc$
можно представить с помощью вектора
\ShowEq{affine space coordinates, 1}

Пусть $\Basis e$ - базис $D$\Hyph модуля $V$.
Тогда вектор $\Vect OA$ имеет вид
\ShowEq{affine space coordinates, 2}

Множество
\ShowEq{affine space coordinates, 3}
называется
\AddIndex{координатами точки $A$ аффинного пространства $\overset{\circ}{A}$
относительно базиса $(O,\Basis e)$}
{coordinates in affine space}.

\section{Аффинное пространство на дифференцируемом многообразии}
\labelSection{Noncommutative Sum}

В разделе
\RefSection{Affine space is single transitive representation}
мы рассмотрели определение аффинной геометрии.
\ShowEq{note: sum of vectors 2}vw

\ShowEq{note: sum of vectors 3}

\ShowEq{note: sum of vectors 4}

\ShowEq{note: sum of vectors 5}

\ShowLemma{increase of coordinate along geodesic}
\ShowProof{increase of coordinate along geodesic}

\ShowTheorem{parallelogram is not closed}
\ShowProof{parallelogram is not closed}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
\begin{theorem}
В римановом пространстве параллелограм $ABCD$ замкнут.
В точке $A$ геодезическая $AC$ имеет касательный вектор $u$,
который является суммой векторов $v$ и $w$
\DrawEq{uk=v+w}1
Следовательно, сумма векторов
в римановом пространстве коммутативна.
\end{theorem}
\end{minipage}
&
\begin{minipage}{160pt}
\ShowEq{Vector v+w=w+v Riemann}vw
\end{minipage}
\end{tabular}

\begin{proof}
Мы будем полагать $\pi$ - длина вектора $u$.
Пусть $U$ - единичный вектор, колинеарный вектору $u$
\ShowEq{U pi=u}
Согласно лемме
\RefLemma{increase of coordinate along geodesic},
приращение координаты $x^k$ вдоль геодезической $L_u$
имеет следующий вид
\ShowEq{Delta AC=}
Равенства
\ShowEq{U pi=V rho +W sigma}
\ShowEq{U pi=V rho +W sigma, Gamma}
являются следствием равенств
\EqRef{Delta ABC=},
\EqRef{Delta AC=}.
Равенство
\eqRef{uk=v+w}1
является следствием равенств
\ShowEq{ref uk=v+w}
Равенство
\ShowEq{u=v +w, Gamma}
является следствием равенств
\ShowEq{ref uk=v+w, Gamma}
Равенство
\ShowEq{u=v +w, Gamma 1}
является следствием равенства
\eqRef{uk=v+w}1.
Равенство
\EqRef{u=v +w, Gamma}
является следствием равенства
\EqRef{u=v +w, Gamma 1}
и симметрии связности.
Следовательно, геодезическая $AC$ является
суммой геодезических $AB$ и $BC$.
\end{proof}

Если связность не симметрична,
то геодезическая $L_u$
не содержит точек $C$ и $E$.
Следовательно, сумма векторов в метрико\hyph аффинном многообразии
некоммутативна.

\begin{theorem}
\labelTheorem{v+w=.+t w+v=.-t}
Существует вектор $t$ такой, что
\ShowEq{v+w=.+t}
\ShowEq{w+v=.-t}
Координаты вектора $t$ удовлетворяют системе уравнений
\ShowEq{v+w=.+/-t}
\end{theorem}

\begin{proof}
Рассмотрим сперва вектор $v+w$.
Равенство
\ShowEq{v+w=.+t, Gamma}
является следствием равенства
\EqRef{Delta ABC=}
и леммы
\RefLemma{increase of coordinate along geodesic}.
Равенство
\ShowEq{v+w=.+t, Gamma 1}
является следствием равенства
\EqRef{v+w=.+t, Gamma}
Равенство
\ShowEq{v+w=.+t, Gamma 2}
является следствием равенства
\EqRef{v+w=.+t, Gamma 1}
Равенство
\ShowEq{v+w=.+t, Gamma 3}
является следствием равенства
\EqRef{v+w=.+t, Gamma 2}
Равенство
\EqRef{v+w=.+/-t}
является следствием равенства
\EqRef{v+w=.+t, Gamma 3}

Рассмотрим теперь вектор $w+v$.
Равенство
\ShowEq{w+v=.-t, Gamma}
является следствием равенства
\EqRef{Delta ADE=}
и леммы
\RefLemma{increase of coordinate along geodesic}.
Равенство
\ShowEq{w+v=.-t, Gamma 1}
является следствием равенства
\EqRef{w+v=.-t, Gamma}
Равенство
\ShowEq{w+v=.-t, Gamma 2}
является следствием равенства
\EqRef{w+v=.-t, Gamma 1}
Равенство
\ShowEq{w+v=.-t, Gamma 3}
является следствием равенства
\EqRef{w+v=.-t, Gamma 2}
Равенство
\EqRef{v+w=.+/-t}
является следствием равенства
\EqRef{w+v=.-t, Gamma 3}
\end{proof}

Ответить на вопрос, имеет ли система уравнений
\EqRef{v+w=.+/-t}
решение - задача непростая.
Однако есть другой способ найти координаты вектора $t$.

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_{v+w}$ через точку $A$, используя вектор $v+w$
как касательный вектор к $L_{v+w}$ в точке $A$.
Мы проведём геодезическую $L_{w+v}$ через точку $A$, используя вектор $w+v$
как касательный вектор к $L_{w+v}$ в точке $A$.
Мы проведём геодезическую $L_u$ через точку $A$, используя вектор $u$
\DrawEq{uk=v+w}{}
как касательный вектор к $L_u$ в точке $A$.
\end{minipage}
&
\ShowEq{v+w w+v u}
\end{tabular}

Согласно теоремам
\RefTheorem{parallelogram is not closed},
\RefTheorem{v+w=.+t w+v=.-t}
точка $F$ является серединой отрезка $EC$.
Следовательно, мы можем рассматривать отрезок $AF$
как медиану треугольника $ACE$.
Согласно теореме
\RefTheorem{v+w=.+t w+v=.-t}
мы можем отождествить отрезок $FC$ и вектор $t$.
Следовательно, теорема
\RefTheorem{parallelogram is not closed}
даёт нам способ найти координаты вектора $t$.

\section{Некоммутативный модуль}

В разделе
\RefSection{Noncommutative Sum},
мы рассмотрели возможность изучения аффинной геометрии
на многообразии аффинной связности.
Эта геометрия имеет две особенности.
Множество векторов не замкнуто относительно сложения
и операция сложения может быть некоммутативной.

Мы ещё не готовы рассмотреть первую проблему,
однако мы можем рассмотреть вопросы,
связанные с некоммутативностью суммы векторов.
Представление
\ShowEq{f:A->*B}fDG
коммутативного кольца $D$ в произвольной группе $G$
называется некоммутативным модулем.
Это представление во многом похоже на модуль,
поэтому все теоремы о структуре модуля верны.
Однако вопрос о структуре базиса остаётся открытым. 

Вообще говоря,
\ShowEq{av+bw ne}
Поэтому возникает вопрос, какое множество группы $G$ мы хотим рассмотреть в качестве базиса.

Мы можем построить базис аналогично тому,
как мы строим базис модуля.
Тогда этот базис должен допускать выражение вида
\[av+bw+cv\]
Либо мы можем потребовать, чтобы элементы базиса
в линейной комбинации имели строгий порядок.
При этом предполагается, что если $(v,w)$ - базис
некоммутативного модуля $V$, то для любого
выражения $bw+av$ существуют $c$, $d\in D$ такие, что
\ShowEq{cv+dw=bw+av}


==> Representation.Product.15.Russian.tex <==
%auto-ignore

\input{Representation.Product.15.Eq}

%\chapter{Произведение представлений}

\section{Декартово произведение представлений}

\begin{lemma}
\labelLemma{product of *algebras is *algebra}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение семейства \(\Omega_2\)\Hyph алгебр
\ShowEq{Ai iI}.
Для каждого \iI, пусть множество
\ShowEq{End O2}{A_i}{}
является \(\Omega_1\)\Hyph алгеброй.
Тогда множество
\ShowEq{f in *A =}
является декартовым произведением \(\Omega_1\)\Hyph алгебр
\ShowEq{End O2}{A_i}.
\end{lemma}
\begin{proof}
Согласно определению
\EqRef{f in *A =},
мы можем представить отображение
\ShowEq{f in *A}
в виде кортежа
\ShowEq{f=(fi)}
отображений
\ShowEq{fi in *Ai}
Согласно определению
\EqRef{f in *A =},
\ShowEq{(fi)(ai)=}
Пусть
\ShowEq{omega in 2}
- n\Hyph арная операция.
Мы определим операцию $\omega$
на множестве
\ShowEq{circ A}
равенством
\ShowEq{circ A omega}
\end{proof}

\begin{definition}
%\labelDefinition{category of representations of F algebra from category}
Пусть $\mathcal A_1$ - категория $\Omega_1$\Hyph алгебр.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{mA1(mA2) symb}
$\ $ представлений}
{category of representations}.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются морфизмы соответствующих представлений.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{product of single transitive representations}
В категории
\ShowEq{mA1(mA2)}
существует произведение
однотранзитивных представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре.
\end{theorem}
\begin{proof}
Для
\ShowEq{j=12}
пусть
\EqParm{P=xBi}{P=P}
произведение семейства $\Omega_j$\Hyph алгебр
\EqParm{Bi}{P=P}
и для любого $\Ii$ отображение
\EqParm{ti:P->Bi}{P=P}
является проекцией на множитель $i$.
Для каждого $\Ii$, пусть
\EqParm{F:P->*P}{P=B}
однотранзитивное $B_{1i}$\Hyph представление в \(\Omega_2\)\Hyph алгебре $B_{2i}$.

Пусть
\(b_1\in P_1\).
Согласно утверждению
\RefItem{tuple represent A number},
\(P_1\)\Hyph число \(b_1\)
может быть представлено в виде кортежа \(B_{1i}\)\Hyph чисел
\ShowEq{b=t(b)1i}
Пусть
\(b_2\in P_2\).
Согласно утверждению
\RefItem{tuple represent A number},
\(P_2\)\Hyph число \(b_2\)
может быть представлено в виде кортежа \(B_{2i}\)\Hyph чисел
\ShowEq{b=t(b)2i}

\begin{lemma}
Для каждого $\Ii$, рассмотрим диаграмму отображений
\ShowEq{define product of single transitive representations}
Пусть отображение
\EqParm{g:P1->*P2}{P=P}
определено равенством
\ShowEq{g(b1)(b2)=}
Тогда отображение \(g\) является
однотранзитивным $P_1$\Hyph представлением в \(\Omega_2\)\Hyph алгебре $P_2$
\EqParm{F:P->*P}{P=P}
Отображение
\ShowEq{ti12}
является морфизмом представления \(g\) в представление \(h_i\).
\end{lemma}

{\sc Доказательство.}
\StartLabelItem
\begin{enumerate}
\item
Согласно определениям
\ShowEq{ref representation of algebra}
отображение $h_i(b_{1i})$ является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $B_{2i}$.
Согласно теореме
\RefTheorem{homomorphism of Cartesian product of Omega algebras},
из коммутативности диаграммы $(1)$ для каждого \iI,
следует, что отображение
\EqParm{g(b):P->P}{P=P}
определённое равенством
\EqRef{g(b1)(b2)=}
является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $P_2$.
\labelItem{g(b) is homomorphism of Omega2 algebra P2}
\item
Согласно определению
\ShowEq{ref representation of algebra}
множество
\EqParm{*B2i}{P=P}
является $\Omega_1$\Hyph алгеброй.
Согласно лемме
\RefLemma{product of *algebras is *algebra},
множество
\EqParm{*P2}{P=P}
является $\Omega_1$\Hyph алгеброй.
\item
Согласно определению
\ShowEq{ref representation of algebra}
отображение
\ShowEq{h:B1->*B2 i}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
Согласно теореме
\RefTheorem{homomorphism of Cartesian product of Omega algebras},
отображение
\EqParm{g:P1->*P2}{P=P}
определённое равенством
\ShowEq{g(b1)=}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
\labelItem{g is homomorphism of Omega1 algebra P1->*P2}
\end{enumerate}

Согласно утверждениям
\RefItem{g(b) is homomorphism of Omega2 algebra P2},
\RefItem{g is homomorphism of Omega1 algebra P1->*P2}
и определению
\ShowEq{ref representation of algebra}
отображение $g$ является $P_1$\Hyph представлением
в $\Omega_2$\Hyph алгебре $P_2$.

Пусть
\EqParm{b2 12 in P2}{P=P}
Согласно утверждению
\RefItem{tuple represent A number},
\(P_2\)\Hyph числа
\ShowEq{b2 12}
могут быть представлены в виде кортежей \(B_{2i}\)\Hyph чисел
\ShowEq{b=t(b)2i 12}
Согласно теореме
\ShowEq{ref Representation is single transitive iff}
поскольку представление $h_i$ однотранзитивно,
то существует единственное \(B_{1i}\)\Hyph число $b_{1i}$ такое, что
\ShowEq{b22=h(b1)b21}
Согласно определениям
\EqRef{b=t(b)1i},
\EqRef{g(b1)(b2)=},
\EqRef{b=t(b)2i 12},
существует единственное \(P_1\)\Hyph число $b_1$ такое, что
\ShowEq{b22=g(b1)b21}
Согласно теореме
\ShowEq{ref Representation is single transitive iff}
представление $g$ однотранзитивно.

Из коммутативности диаграммы $(1)$ и определения
\ShowEq{ref morphism of representations of universal algebra}
следует, что отображение
\ShowEq{ti12}
является морфизмом представления \(g\) в представление \(h_i\).
\hfill\(\odot\)

Пусть
\DrawEq{d=g(b)(b)}{regular}
Из равенств
\EqRef{g(b1)(b2)=},
\eqRef{d=g(b)(b)}{regular}
следует, что
\ShowEq{d=h(b)(b)}

Для
\ShowEq{j=12}
пусть $R_j$ - другой объект категории $\mathcal A_j$. Для любого $\Ii$, пусть отображение
\EqParm{ti:P->Bi}{P=R1}
является морфизмом из $\Omega_1$\Hyph алгебра $R_1$ в
$\Omega_1$\Hyph алгебру $B_{1i}$.
Согласно определению
\RefDefinition{product in category},
существует единственный морфизм $\Omega_1$\Hyph алгебры
\ShowEq{s:R->P,1}
такой, что коммутативна диаграмма
\ShowEq{t*s=r1}
Пусть
\ShowEq{a in R1}
Пусть
\ShowEq{b=s(a)1}
Из коммутативности диаграммы
\EqRef{t*s=r1}
и утверждений
\EqRef{b=s(a)1},
\EqRef{b=t(b)1i}
следует, что
\ShowEq{b=r(a)1i}

Пусть
\EqParm{F:P->*P}{P=R}
однотранзитивное $R_1$\Hyph представление в \(\Omega_2\)\Hyph алгебре $R_2$.
Согласно теореме
\ShowEq{ref unique morphism of representations of universal algebra}
морфизм $\Omega_2$\Hyph алгебры
\EqParm{ti:P->Bi}{P=R2}
такой, что отображение
\ShowEq{(r12)}
является морфизмом
представлений из $f$ в $h_i$,
определён однозначно
с точностью до выбора образа $R_2$\Hyph числа $a_2$.
Согласно замечанию
\ShowEq{ref remark morphism of representations of universal algebra}
в диаграмме отображений
\ShowEq{r12 product of single transitive representations}
диаграмма $(2)$ коммутативна. 
Согласно определению
\RefDefinition{product in category},
существует единственный морфизм $\Omega_2$\Hyph алгебры
\ShowEq{s:R->P,2}
такой, что коммутативна диаграмма
\ShowEq{t*s=r2}
Пусть
\ShowEq{a in R2}
Пусть
\ShowEq{b=s(a)2}
Из коммутативности диаграммы
\EqRef{t*s=r2}
и утверждений
\EqRef{b=s(a)2},
\EqRef{b=t(b)2i}
следует, что
\ShowEq{b=r(a)2i}
Пусть
\DrawEq{c=f(a)a}{regular}
Из коммутативности диаграммы $(2)$ и равенств
\EqRef{d=h(b)(b)},
\EqRef{b=r(a)2i},
\eqRef{c=f(a)a}{regular}
следует, что
\ShowEq{d=r(c)2i}
Из равенств
\EqRef{d=h(b)(b)},
\EqRef{d=r(c)2i}
следует, что
\ShowEq{d=s(c)2}
что согласуется с коммутативносью диаграммы
\EqRef{t*s=r2}.

Для каждого $\Ii$, мы объединим диаграммы отображений
\EqRef{define product of single transitive representations},
\EqRef{t*s=r1},
\EqRef{t*s=r2},
\EqRef{r12 product of single transitive representations}
\ShowEq{product of single transitive representations}
Из равенств
\eqRef{d=g(b)(b)}{regular}
\EqRef{b=s(a)2}
и из равенств
\eqRef{c=f(a)a}{regular},
\EqRef{d=s(c)2},
следует коммутативность диаграммы $(3)$.
Следовательно, отображение
\ShowEq{(s12)}
является морфизмом
представлений из $f$ в $g$.,
Согласно теореме
\ShowEq{ref unique morphism of representations of universal algebra}
морфизм
\ShowEq{(s12)}
определён однозначно,
так как мы требуем
\EqRef{d=s(c)2}.

Согласно определению
\RefDefinition{product in category},
представление $g$
и семейство морфизмов представления
\ShowEq{ti12, family}
является произведением в категории
\ShowEq{mA1(mA2)}.
\end{proof}

\ShowDefinition{polymorphism of representations}

Мы также будем говорить, что отображение
\ShowEq{map r12}r{}
является полиморфизмом
представлений в $\Omega_2$\Hyph алгебрах $B_1$, ..., $B_n$ в представление
в $\Omega_2$\Hyph алгебре $B$.

\ShowTheorem{polymorphism of representations}
\begin{proof}
Равенство
\EqRef{polymorphism of representation, ak}
следует из определения
\RefDefinition{polymorphism of representations}
и равенства
\ShowEq{ref morphism of representations of universal algebra, 2m}
Равенство
\EqRef{polymorphism of representation, omega1}
следует из утверждения, что, для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in A_k$
имеют заданное значение, отображение $r_1$
является гомоморфизмом $\Omega_1$\Hyph алгебры $A_k$ в $\Omega_1$\Hyph алгебру $A$.
Равенство
\EqRef{polymorphism of representation, omega2}
следует из утверждения, что, для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $m_k\in B_k$
имеют заданное значение, отображение $r_2$
является гомоморфизмом $\Omega_2$\Hyph алгебры $B_k$ в $\Omega_2$\Hyph алгебру $B$.
\end{proof}

\section{Приведенное декартово произведение представлений}

\ShowDefinition{category of representations A1(mA2)}

\begin{theorem}
\labelTheorem{product of effective representations}
В категории
\ShowEq{A1(mA2)}
существует произведение
эффективных представлений $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре
и это произведение является
эффективным представлением $\Omega_1$\Hyph алгебры $A_1$.
\end{theorem}
\begin{proof}
Пусть
\EqParm{P=xBi}{P=A}
произведение семейства $\Omega_2$\Hyph алгебр
\EqParm{Bi}{P=A}
и для любого $\Ii$ отображение
\EqParm{ti:P->Bi}{P=A}
является проекцией на множитель $i$.
Для каждого $\Ii$, пусть
\EqParm{F:A->*P}{P=A}
эффективное $A_1$\Hyph представление в \(\Omega_2\)\Hyph алгебре $A_{2i}$.

Пусть
\(b_1\in A_1\).
Пусть
\(b_2\in A_2\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A_2\)\Hyph число \(b_2\)
может быть представлено в виде кортежа \(A_{2i}\)\Hyph чисел
\ShowEq{b=t(b)i}

\begin{lemma}
Для каждого $\Ii$, рассмотрим диаграмму отображений
\ShowEq{define product of single transitive representations, reduced}
Пусть отображение
\EqParm{g:P1->*P2}{P=A}
определено равенством
\ShowEq{g(b1)(b2)=, reduced}
Тогда отображение \(g\) является
эффективным $A_1$\Hyph представлением в \(\Omega_2\)\Hyph алгебре $A_2$
\EqParm{F:P->*P}{P=A}
Отображение
\(t_i\)
является приведенным морфизмом представления \(g\) в представление \(h_i\).
\end{lemma}

{\sc Доказательство.}
\StartLabelItem
\begin{enumerate}
\item
Согласно определениям
\ShowEq{ref representation of algebra}
отображение $h_i(b_1)$ является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $A_{2i}$.
Согласно теореме
\RefTheorem{homomorphism of Cartesian product of Omega algebras},
из коммутативности диаграммы $(1)$ для каждого \iI,
следует, что отображение
\EqParm{g(b):P->P}{P=A}
определённое равенством
\EqRef{g(b1)(b2)=, reduced}
является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $A_2$.
\labelItem{g(b) is homomorphism of Omega2 algebra A2}
\item
Согласно определению
\ShowEq{ref representation of algebra}
множество
\EqParm{*B2i}{P=A}
является $\Omega_1$\Hyph алгеброй.
Согласно лемме
\RefLemma{product of *algebras is *algebra},
множество
\EqParm{*P2}{P=A}
является $\Omega_1$\Hyph алгеброй.
\item
Согласно определению
\ShowEq{ref representation of algebra}
отображение
\ShowEq{h:A1->*A2i}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
Согласно теореме
\RefTheorem{homomorphism of Cartesian product of Omega algebras},
отображение
\EqParm{g:P1->*P2}{P=A}
определённое равенством
\ShowEq{g(b1)=,}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
\labelItem{g is homomorphism of Omega1 algebra A1->*A2}
\end{enumerate}

Согласно утверждениям
\RefItem{g(b) is homomorphism of Omega2 algebra A2},
\RefItem{g is homomorphism of Omega1 algebra A1->*A2}
и определению
\ShowEq{ref representation of algebra}
отображение $g$ является $A_1$\Hyph представлением
в $\Omega_2$\Hyph алгебре $A_2$.

Для любого $\Ii$,
согласно определению
\ShowEq{ref effective representation of algebra}
$A_1$\Hyph число $a_1$ порождает единственное преобразование
\ShowEq{b22=a1*b21 i}
Пусть
\EqParm{b2 12 in P2}{P=A}
Согласно утверждению
\RefItem{tuple represent A number},
\(A_2\)\Hyph числа
\ShowEq{b2 12}
могут быть представлены в виде кортежей \(A_{2i}\)\Hyph чисел
\ShowEq{b=t(b)i 12}
Согласно определению
\EqRef{g(b1)(b2)=, reduced}
представления $g$,
из равенств
\EqRef{b22=a1*b21 i},
\EqRef{b=t(b)i 12}
следует, что
$A_1$\Hyph число $a_1$ порождает единственное преобразование
\ShowEq{b22=a1*b21}
Согласно определению
\ShowEq{ref effective representation of algebra}
представление $g$ эффективно.

Из коммутативности диаграммы $(1)$ и определения
\ShowEq{ref morphism of representations of universal algebra}
следует, что отображение
$t_i$
является приведенным морфизмом представления \(g\) в представление \(h_i\).
\hfill\(\odot\)

Пусть
\DrawEq{d=g(b)(b)}{reduced}
Из равенств
\EqRef{g(b1)(b2)=, reduced},
\eqRef{d=g(b)(b)}{reduced}
следует, что
\ShowEq{d=h(b)(b),}

Пусть $R_2$ - другой объект категории $\mathcal A_2$.
Пусть
\ShowEq{f:A->*R}
эффективное $A_1$\Hyph представление в \(\Omega_2\)\Hyph алгебре $R_2$.
Для любого $\Ii$,
пусть существует морфизм
\EqParm{ti:P->Bi}{P=A2}
представлений из $f$ в $h_i$.
Согласно замечанию
\ShowEq{ref remark morphism of representations of universal algebra}
в диаграмме отображений
\ShowEq{r12 product of effective representations}
диаграмма $(2)$ коммутативна. 
Согласно определению
\RefDefinition{product in category},
существует единственный морфизм $\Omega_2$\Hyph алгебры
\ShowEq{s:R->A}
такой, что коммутативна диаграмма
\ShowEq{t*s=r}
Пусть
\ShowEq{a in R2}
Пусть
\ShowEq{b=s(a)}
Из коммутативности диаграммы
\EqRef{t*s=r}
и утверждений
\EqRef{b=s(a)},
\EqRef{b=t(b)i}
следует, что
\ShowEq{b=r(a)i}
Пусть
\DrawEq{c=f(a)a}{reduced}
Из коммутативности диаграммы $(2)$ и равенств
\EqRef{d=h(b)(b),},
\EqRef{b=r(a)i},
\eqRef{c=f(a)a}{reduced}
следует, что
\ShowEq{d=r(c)i}
Из равенств
\EqRef{d=h(b)(b),},
\EqRef{d=r(c)i}
следует, что
\ShowEq{d=s(c)}
что согласуется с коммутативносью диаграммы
\EqRef{t*s=r}.

Для каждого $\Ii$, мы объединим диаграммы отображений
\EqRef{define product of single transitive representations, reduced},
\EqRef{t*s=r},
\EqRef{r12 product of effective representations}
\ShowEq{product of effective representations}
Из равенств
\eqRef{d=g(b)(b)}{reduced},
\EqRef{b=s(a)}
и из равенств
\eqRef{c=f(a)a}{reduced},
\EqRef{d=s(c)},
следует коммутативность диаграммы $(3)$.
Следовательно, отображение
\(s\)
является приведенным морфизмом
представлений из $f$ в $g$.
Согласно определению
\ShowEq{ref reduced morphism of representations}
отображение $s$ является гомоморфизмом $\Omega_2$ алгебры.
Согласно теореме
\RefTheorem{product exists in category of Omega algebras}
и определению
\RefDefinition{product in category},
приведенный морфизм
$s$
определён однозначно.

Согласно определению
\RefDefinition{product in category},
представление $g$
и семейство морфизмов представления
\ShowEq{ti, family}
является произведением в категории
\ShowEq{A1(mA2)}.
\end{proof}

\ShowDefinition{reduced polymorphism of representations}

\ShowTheorem{reduced polymorphism of representations}
\begin{proof}
Равенство
\EqRef{reduced polymorphism of representation, ak}
следует из определения
\RefDefinition{reduced polymorphism of representations}
и равенства
\ShowEq{eqref morphism of representations of universal algebra}
Равенство
\EqRef{reduced polymorphism of representation, akl}
следует из равенства
\EqRef{reduced polymorphism of representation, ak}.
Равенство
\EqRef{reduced polymorphism of representation, omega2}
следует из утверждения, что, для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $m_k\in B_k$
имеют заданное значение, отображение $r_2$
является гомоморфизмом $\Omega_2$\Hyph алгебры $B_k$ в $\Omega_2$\Hyph алгебру $B$.
\end{proof}

Мы также будем говорить, что отображение $r_2$ является приведенным полиморфизмом
представлений в $\Omega_2$\Hyph алгебрах $B_1$, ..., $B_n$ в представление
в $\Omega_2$\Hyph алгебре $B$.

\section{Мультипликативная \texorpdfstring{$\Omega$}{Omega}-группа}

Пусть отображение
\ShowEq{f:A->*B}fAB
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$.
Согласно теореме
\RefTheorem{Endomorphisms of representation form semigroup},
множество
\ShowEq{End A(O2) B}{}
является полугруппой.
В тоже время\,\footnote{
В утверждении
\EqRef{End A(O2) B in End B},
я обозначил $\Omega_2$ категорию $\Omega_2$\Hyph алгебр
и $A(\Omega_2)$ категорию представлений $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре.
}
\ShowEq{End A(O2) B in End B}
Согласно определению
\RefDefinition{representation of algebra},
множество
\ShowEq{End O2}B{}
является $\Omega_2$\Hyph алгеброй.
Однако из утверждения
\EqRef{End A(O2) B in End B}
не следует, что
множество
\ShowEq{End A(O2) B}{}
является $\Omega_2$\Hyph алгеброй.

Чтобы понять, при каких условиях
множество
\ShowEq{End A(O2) B}{}
является $\Omega_2$\Hyph алгеброй,
мы рассмотрим связь между
множеством представлений
$\Omega_1$\Hyph алгебры $A$ в
$\Omega_2$\Hyph алгебре $B$ и
множеством приведенных морфизмов этих представлений.

\begin{theorem}
\labelTheorem{reduced endomorphism -> representation}
Пусть отображение
\ShowEq{f:A->B}rBB
является приведенным эндоморфизмом представления
\ShowEq{f:A->*B}fAB
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$.
Отображение
\ShowEq{rf:A->end B}
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$
тогда и только тогда, когда
на множестве
\ShowEq{fA in End O2 B}{}
произведение $\circ$ отображений
дистрибутивно слева относительно произвольной операции
\ShowEq{omega in Omega}1{}
\ShowEq{r fa1p=rf a1p}
\end{theorem}
\begin{proof}
Согласно определению
\RefDefinition{representation of algebra},
отображение $f(a)$ является эндоморфизмом $\Omega_2$\Hyph алгебры $B$.
Согласно определениям
\RefDefinition{morphism of representations of universal algebra},
\RefDefinition{reduced morphism of representations},
отображение $r$ является эндоморфизмом $\Omega_2$\Hyph алгебры $B$.
Следовательно, отображение
\ShowEq{r f(a)}
является эндоморфизмом $\Omega_2$\Hyph алгебры $B$.

\StartLabelItem
\begin{enumerate}
\item
Согласно определению
\RefDefinition{representation of algebra},
отображение $rf$
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$
тогда и только тогда, когда
отображение $rf$ является гомоморфизмом $\Omega_1$\Hyph алгебры.
\labelItem{rf is homomorphism}
\item
Утверждение
\RefItem{rf is homomorphism}
означает, что
для любой операции
\ShowEq{omega in Omega}1{}
верно равенство
\ShowEq{rf omega}
Поскольку отображение $f$
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$,
то, согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом $\Omega_1$\Hyph алгебры
\ShowEq{rf omega 1}
Равенство
\EqRef{r fa1p=rf a1p}
является следствием равенств
\EqRef{rf omega},
\EqRef{rf omega 1}.
\labelItem{product of maps is distributive}
\end{enumerate}
Теорема является следствием утверждения
\RefItem{product of maps is distributive}.
\end{proof}

\begin{theorem}
\labelTheorem{Im f=End A(O2) B}
Пусть отображение
\ShowEq{f:A->*B}fAB
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$.
Пусть
\DrawEq{Im f=End A(O2) B}1
\StartLabelItem
\begin{enumerate}
\item
\labelItem{product in semigroup is commutative}
Произведение в полугруппе
\ShowEq{End A(O2) B}{}
коммутативно.
\item
\labelItem{product o generates product *}
Произведение $\circ$ в полугруппе
\ShowEq{End A(O2) B}{}
порождает произведение $*$ в $\Omega_1$\Hyph алгебре $A$ таким образом, что
\ShowEq{f(a*b)=fa o fb}
\item
\labelItem{semigroup is Omega algebra}
Полугруппа
\ShowEq{End A(O2) B}{}
является $\Omega_1$\Hyph алгеброй.
%\item
%\labelItem{product is distributive over any operation}
%Произведение
%дистрибутивно относительно произвольной операции
%\ShowEq{omega in Omega}1.
\end{enumerate}
\end{theorem}
\begin{proof}
Пусть отображение $h$ является эндоморфизмом представления $f$.
Согласно утверждению
\eqRef{Im f=End A(O2) B}1,
существует $b\in A$ такое, что $h=f(b)$.
Следовательно, равенство
\ShowEq{fa fb=fb fa}
является следствием равенства
\EqRef{morphism of representations of universal algebra}.
Согласно утверждению
\eqRef{Im f=End A(O2) B}1,
отображения $f(a)$, $f(b)$ являются эндоморфизмами представления $f$.
Следовательно, произведение $\circ$ в полугруппе
\ShowEq{End A(O2) B}{}
коммутативно.

Согласно теореме
\RefTheorem{Endomorphisms of representation form semigroup},
произведение эндоморфизмов $f(a)$, $f(b)$ представления $f$
является эндоморфизмом $h$ представления $f$.
Согласно утверждению
\eqRef{Im f=End A(O2) B}1,
существует $c\in A$ такое, что $h=f(c)$.
Бинарная операция $*$ на множестве $A$ определена равенством
\[c=a*b\]
Следовательно, утверждение
\RefItem{product o generates product *}
верно.

Пусть отображения
\ShowEq{h1n}h
являются эндоморфизмами представления $f$.
Согласно утверждению
\eqRef{Im f=End A(O2) B}1,
существуют $A$\Hyph числа
\ShowEq{h1n}a
такие, что
\ShowEq{hi=fai}
Поскольку отображение $f$
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$,
то, согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$
\ShowEq{h1p o=f1p o}
Согласно утверждению
\eqRef{Im f=End A(O2) B}1,
\ShowEq{h1p o in End A(O2) B}
Следовательно, утверждение
\RefItem{semigroup is Omega algebra}
верно.
\end{proof}

Согласно теореме
\RefTheorem{Im f=End A(O2) B},
если утверждение
\eqRef{Im f=End A(O2) B}1
выполнено, то на множестве
\ShowEq{End A(O2) B}{}
определены две алгебраические структуры.
А именно, множество
\ShowEq{End A(O2) B}{}
является полугруппой и в тоже время это множество является $\Omega_1$\Hyph алгеброй.
Аналогичное утверждение верно для $\Omega_1$\Hyph алгебры $A$.
Однако мы не можем утверждать, что операция произведения в $\Omega_1$\Hyph алгебре $A$
дистрибутивна по отношению к произвольной операции
\ShowEq{omega in Omega}1{}
(смотри теорему
\RefTheorem{reduced endomorphism -> representation}).

\begin{theorem}
\labelTheorem{product in algebra is distributive over any operation}
Пусть отображение
\ShowEq{f:A->*B}fAB
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$
и
\DrawEq{Im f=End A(O2) B}{}
Произведение $*$,
определённое в $\Omega_1$\Hyph алгебре $A$,
дистрибутивно относительно произвольной операции
\ShowEq{omega in Omega}1{}
тогда и только тогда, когда
отображение
\ShowEq{fb:A->end B}
является представлением
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$ алгебре $B$
\end{theorem}
\begin{sloppypar}
\begin{proof}
Согласно утверждению
\RefItem{product o generates product *},
для нас не имеет значение рассматриваем ли мы $\Omega_1$\Hyph алгебру $A$
или мы рассматриваем $\Omega_1$\Hyph алгебру
\ShowEq{End A(O2) B}.
Теорема является следствием определения
\EqRef{f(a*b)=fa o fb}
произведения $*$ в $\Omega_1$\Hyph алгебре $A$,
а также теоремы
\RefTheorem{reduced endomorphism -> representation}
и утверждений
\RefItem{product in semigroup is commutative},
\RefItem{semigroup is Omega algebra}.
\end{proof}
\end{sloppypar}

В теореме
\RefTheorem{product in algebra is distributive over any operation},
мы встречаем универсальную алгебру, похожую на $\Omega$\Hyph группу,
однако эта алгебра отличается от $\Omega$\Hyph группы.
Поскольку эта универсальная алгебра
играет важную роль в теории представлений,
мы рассмотрим определения
\RefDefinition{multiplicative Omega group},
\RefDefinition{Abelian multiplicative Omega group}.

\ShowDefinition{multiplicative Omega group}

\ShowDefinition{Abelian multiplicative Omega group}

\begin{definition}
Если
\ShowEq{associative multiplicative Omega group}
то мультипликативная $\Omega$\Hyph группа называется
\AddIndex{асоциативной}{associative multiplicative Omega group}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{permits reduced polymorphism of representation}
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Пусть отображение
\ShowEq{reduced polymorphism of representation}
является
приведенным полиморфизмом представлений
$f_1$, ..., $f_n$ в представление $f$.
Произведение $\circ$,
определённое в $\Omega_1$\Hyph алгебре $f(A)$,
коммутативно.

Представление
\ShowEq{f:A->*B}fAB
допускает приведенный полиморфизм представлений
тогда и только тогда, когда
следующие условия выполнены
\StartLabelItem
\begin{enumerate}
\item
Произведение $\circ$,
определённое в $\Omega_1$\Hyph алгебре
\ShowEq{End A(O2) B},
дистрибутивно относительно произвольной операции
\ShowEq{omega in Omega}1{}
%В $\Omega_1$\Hyph алгебре $A_1$
%определено умножение $*$.
%\labelItem{product circ is defined}
\item
\labelItem{f(ab)=f(a)f(b)}
\DrawEq{f(ab)=f(a)f(b)}-
\end{enumerate}
\end{theorem}
\begin{proof}
Пользуясь равенством
\EqRef{reduced polymorphism of representation, ak},
мы можем записать выражение
\ShowEq{reduced polymorphism of representation 1, ak}
либо в виде
\ShowEq{reduced polymorphism of representation 2, ak}
либо в виде
\ShowEq{reduced polymorphism of representation 3, ak}
Коммутативность произведения $\circ$
следует из равенств
\EqRef{reduced polymorphism of representation 2, ak},
\EqRef{reduced polymorphism of representation 3, ak}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$ и
\DrawEq{Im f=End A(O2) B}3
Тогда представление $f$
допускает приведенный полиморфизм представлений.

Пусть
\ShowEq{Omega=...-o}
Представление
\ShowEq{A1->End A1}
полугруппы $A_1$ в $\Omega$\Hyph алгебре $A_1$
существует тогда и только тогда, когда
для любой операции
\ShowEq{omega n ari}{}{}n{}
умножение
\AddIndex{дистрибутивно}{distributive law}
относительно операции $\omega$
\DrawEq{a omega=omega a left}1
\DrawEq{a omega=omega a right}1
\end{theorem}
\begin{proof}
Согласно определению
\RefDefinition{representation of algebra},
равенства
\eqRef{a omega=omega a left}1,
\eqRef{a omega=omega a right}1
верны тогда и только тогда, когда отображение $h$ является представлением
полугруппы $A_1$ в $\Omega$\Hyph алгебре $A_1$.
Одновременно
равенства
\eqRef{a omega=omega a left}1,
\eqRef{a omega=omega a right}1
выражают закон дистрибутивности
умножения относительно операции $\omega$.
\end{proof}

В $\Omega_1$\Hyph алгебре $A_1$, мы определили произведение,
согласованное с однотранзитивным представлением в $\Omega_2$\Hyph алгебре $A_2$.
Эту конструкцию можно построить в случае произвольного представления
при условии, что произведение в $\Omega_1$\Hyph алгебре $A_1$
определено однозначно. Однако в общем случае произведение может быть некоммутативным.

\begin{theorem}
\labelTheorem{existence of reduced polymorphism, a omega b omega}
Пусть
\ShowEq{->B 12}
эффективные представления
абелевой мультиплиткативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебрах
\ShowEq{B 12}
Допустим $\Omega_2$\Hyph алгебра имеет 2 операции, а именно
\EqParm{o12 in Omn}{=.}
Необходимым условием существования приведенного полиморфизма
\ShowEq{R:B1B2->B}
является равенство 
\DrawEq{aijo1o2=aijo2o1}{representation}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{a in 1 b in 2}
Согласно равенству
\EqRef{reduced polymorphism of representation, omega2},
выражение
\ShowEq{r2 aw1 aw2}
может иметь $2$ значения
\ShowEq{r2 aw1 aw2 1}
\ShowEq{r2 aw1 aw2 2}
Из равенств
\EqRef{r2 aw1 aw2 1},
\EqRef{r2 aw1 aw2 2}
следует, что
\ShowEq{r2 aw1 aw2 1=2}
Следовательно, выражение
\EqRef{r2 aw1 aw2}
определенно корректно тогда и только тогда, когда равенство
\EqRef{r2 aw1 aw2 1=2}
верно.
Положим
\ShowEq{a=Rij}
Равенство
\eqRef{aijo1o2=aijo2o1}{representation}
является следствием равенств
\EqRef{r2 aw1 aw2 1=2},
\EqRef{a=Rij}.
\end{proof}

\begin{theorem}
Существует приведенный полиморфизм эффективного представления
абелевой мультиплиткативной $\Omega$\Hyph группы
в абелевой группе.
\end{theorem}
\begin{proof}
Поскольку операция сложения в абелевой группе
коммутативна и ассоциативна,
то теорема является следствием теоремы
\RefTheorem{existence of reduced polymorphism, a omega b omega}.
\end{proof}

\begin{theorem}
\labelTheorem{no reduced polymorphism in ring}
Не существует приведенный полиморфизм эффективного представления
абелевой мультиплиткативной $\Omega$\Hyph группы
в кольце.
\end{theorem}
\begin{proof}
В кольце определены две операции: сложение, которое
коммутативно и ассоциативно, и произведение, которое
дистрибутивно относительно сложения.
Согласно теореме
\RefTheorem{existence of reduced polymorphism, a omega b omega},
если существует полиморфизм эффективного представления в кольцо,
то сложение и произведение должны удовлетворять равенству
\DrawEq{a * b + =}{polymorphism}
Однако правая часть равенства
\eqRef{a * b + =}{polymorphism}
имеет вид
\ShowEq{a+a a+a}
Следовательно, равенство
\eqRef{a * b + =}{polymorphism}
не верно.
\end{proof}

\begin{question}
Возможно, что полиморфизм представлений существует
только для эффективного представления в
Абелевая группе.
Однако это утверждение пока не доказано.
\qed
\end{question}

\section{\texorpdfstring{$\Omega$}{Omega}-кольцо}

\ShowDefinition{Omega ring}

\ShowTheorem{product in Omega ring is distributive over addition}
\ShowProof{product in Omega ring is distributive over addition}

\ShowDefinition{matrix over Omega ring}

\ShowEq{convention: Einstein summation}

\ShowEq{matrix operations}

\ShowEq{remark: pronunciation of product}

\ShowTheorem{rcstar transpose}
\ShowProof{rcstar transpose}

\ShowDefinition{biring}

\ShowTheorem{duality principle for biring}

\ShowTheorem{duality principle for biring of matrices}

\ShowEq{remark: reducible biring}


==> Representation.Tensor.Russian.tex <==
%auto-ignore
\input{Representation.Tensor.Eq}

%\chapter{Тензорное произведение представлений}

\section{Тензорное произведение представлений}

\ShowDefinition{tensor product of representations}

\begin{theorem}
\labelTheorem{tensor product is unique}
Если тензорное произведение эффективных представлений существует,
то тензорное произведение определено однозначно
с точностью до изоморфизма представлений.
\end{theorem}
\begin{proof}
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{a1n}An{}
- $\Omega_2$\Hyph алгебры.
Пусть для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть эффективные представления
\ShowEq{representation of algebra in S1 S2}
являются тензорным произведением
представлений $B_1$, ..., $B_n$.
Из коммутативности диаграммы
\ShowEq{polymorphisms category, diagram 1}
следует, что
\ShowEq{R1= R2=}
Из равенств
\EqRef{R1= R2=}
следует, что морфизмы представления
\ShowEq{h1*h2}
являются тождественными отображениями.
Следовательно, морфизмы представления $h_1$, $h_2$
являются изоморфизмами.
\end{proof}

\begin{convention}
\labelConvention{isomorphic representations S1=S2}
Алгебры $S_1$, $S_2$ могут быть различными множествами.
Однако они неразличимы для нас, если мы рассматриваем их
как изоморфные представления.
В этом случае мы будем писать $S_1=S_2$.
\qed
\end{convention}

\begin{definition}
\labelDefinition{tensor power of representation}
Тензорное произведение
\ShowEq{tensor power of representation}
называется
\AddIndex{тензорной степенью}{tensor power} представления $B$.
\qed
\end{definition}

\ShowTheorem{tensor product of representations}
\begin{proof}
Пусть
\ShowEq{f:A->M}
представление $\Omega_1$\Hyph алгебры $A$, порождённое
декартовым произведением $\Times$
множеств $B_1$, ..., $B_n$.\,\footnote{Согласно теоремам
\RefTheorem{product exists in category of Omega algebras},
\RefTheorem{product of effective representations},
множество, порождённое приведенным декартовым произведением
представлений $B_1$, ..., $B_n$
совпадает с декартовым произведением $\Times$
множеств $B_1$, ..., $B_n$.
В этом месте доказательства
нас не интересует алгебраическая структра на множестве $\Times$.
}
Инъекция
\ShowEq{map i, representation, tensor product, 1}
определена по правилу\,\footnote{Равенство
\EqRef{map i, representation, tensor product}
утверждает, что мы отождествляем базис представления $M$
с множеством $\Times$.
}
\ShowEq{map i, representation, tensor product}
Пусть $N$ - отношение эквивалентности, порождённое равенствами\,\footnote{
Я рассматриваю формирование элементов представления из элементов базиса
согласно теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.
Теорема
\RefTheorem{representation, tensor product}
требует выполнения условий
\EqRef{equivalence 1, representation, tensor product},
\EqRef{equivalence 2, representation, tensor product}.
}
\ShowEq{equivalence, representation, tensor product}
\ShowEq{equivalence, 1, representation, tensor product}

\begin{lemma}
\labelLemma{endomorphism coordinated with equivalence 1}
{\it
Пусть $\omega\in\Omega_2(p)$. Тогда
\ShowEq{equivalence 1 5, representation, tensor product}
}
\end{lemma}

{\sc Доказательство.}
Из равенства
\EqRef{equivalence 2, representation, tensor product}
следует
\ShowEq{equivalence 1 1, representation, tensor product}
Так как $f_i(c)$ - эндоморфизм $\Omega_2$\Hyph алгебры $B_i$, то
из равенства
\EqRef{equivalence 1 1, representation, tensor product}
следует
\ShowEq{equivalence 1 2, representation, tensor product}
Из равенств
\EqRef{equivalence 1 2, representation, tensor product},
\EqRef{equivalence 1, representation, tensor product}
следует
\ShowEq{equivalence 1 3, representation, tensor product}
Из равенств
\EqRef{equivalence 1 3, representation, tensor product},
\EqRef{equivalence 2, representation, tensor product}
следует
\ShowEq{equivalence 1 4, representation, tensor product}
Так как $f(c)$ - эндоморфизм $\Omega_2$\Hyph алгебры $B$, то
равенство
\EqRef{equivalence 1 5, representation, tensor product}
следует из равенства
\EqRef{equivalence 1 4, representation, tensor product}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{endomorphism coordinated with equivalence 2}
\ShowEq{equivalence 2 1, representation, tensor product}
\end{lemma}

{\sc Доказательство.}
Из равенства
\EqRef{equivalence 2, representation, tensor product}
следует, что
\ShowEq{equivalence 2, 1, representation, tensor product}
Равенство
\EqRef{equivalence 2 1, representation, tensor product}
следует из равенства
\EqRef{equivalence 2, 1, representation, tensor product}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{endomorphism coordinated with equivalence}
Для любого $c\in A$ эндоморфизм $f(c)$ $\Omega_2$\Hyph алгебры $M$
согласовано с эквивалентностью $N$.
\end{lemma}

{\sc Доказательство.}
Утверждение леммы следует
из лемм
\RefLemma{endomorphism coordinated with equivalence 1},
\RefLemma{endomorphism coordinated with equivalence 2}
и определения
\ShowEq{ref transformation coordinated with equivalence}
\hfill\(\odot\)

Из леммы
\RefLemma{endomorphism coordinated with equivalence}
и теоремы
\RefTheorem{transformation correlated with equivalence}
следует, что на множестве ${}^*M/N$ определена $\Omega_1$\Hyph алгебра.
Рассмотрим диаграмму
\ShowEq{endomorphism coordinated with equivalence, diagram}
Согласно лемме
\RefLemma{endomorphism coordinated with equivalence},
из условия
\ShowEq{endomorphism coordinated with equivalence, diagram 1}
следует
\ShowEq{endomorphism coordinated with equivalence, diagram 2}
Следовательно, преобразование $F(a)$ определено корректно и
\ShowEq{endomorphism coordinated with equivalence, diagram 3}
Если $\omega\in\Omega_1(p)$, то мы положим
\ShowEq{endomorphism coordinated with equivalence, diagram 4}
Следовательно, отображение $F$ является представлением
$\Omega_1$\Hyph алгебры $A$.
Из \EqRef{endomorphism coordinated with equivalence, diagram 3}
следует, что $j$ является приведенным морфизмом представлений $f$ и $F$.

Рассмотрим коммутативную диаграмму
\ShowEq{diagram top, representation, tensor product}
Из коммутативности диаграммы
\EqRef{diagram top, representation, tensor product}
и равенства
\EqRef{map i, representation, tensor product}
следует, что
\ShowEq{g1()=j()}
Из равенств
\EqRef{map i, representation, tensor product},
\EqRef{equivalence 1, representation, tensor product},
\EqRef{equivalence 2, representation, tensor product}
следует
\ShowEq{g_1 1, representation, tensor product}
\ShowEq{g_1 2, representation, tensor product}
Из равенств \EqRef{g_1 1, representation, tensor product}
и \EqRef{g_1 2, representation, tensor product}
следует, что отображение $g_1$
является приведенным полиморфизмом представлений $f_1$, ..., $f_n$.

Поскольку $\Times$ - базис представления $M$ $\Omega_1$\Hyph алгебры $A$,
то, согласно теореме
\RefTheorem{automorphism uniquely defined by image of basis},
для любого представления
\ShowEq{representation A V}
и любого
приведенного полиморфизма
\ShowEq{diagram bottom, 1, representation, tensor product}
существует единственный морфизм представлений $k:M\rightarrow V$,
для которого коммутативна следующая диаграмма
\ShowEq{diagram bottom, representation, tensor product}
Так как $g_2$ - приведенный полиморфизм, то
\ShowEq{ker k supseteq N}

Согласно теореме
\RefTheorem{morphism representations and kernel equivalence}
отображение $j$ универсально в категории морфизмов
представления $f$,
ядро которых содержит $N$.
Следовательно, определён морфизм представлений
\[
h:M/N\rightarrow V
\]
для которого коммутативна диаграмма
\ShowEq{diagram right, representation, tensor product}
Объединяя диаграммы
\ShowEq{diagrams, representation, tensor product}
получим коммутативную диаграмму
\ShowEq{diagram, representation, tensor product}
Так как $\mathrm{Im}\,g_1$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\RefTheorem{tensor product of representations}
\ShowEq{B 1n M N}
Для $d_i\in A_i$ будем записывать
\ShowEq{map j, representation, tensor product}
Из равенств
\EqRef{g1()=j()},
\EqRef{map j, representation, tensor product}
следует, что
\ShowEq{g1()=otimes}

\ShowTheorem{B times->B otimes}
\begin{proof}
Теорема является следствием определений
\RefDefinition{reduced polymorphism of representations},
\RefDefinition{tensor product of representations}.
\end{proof}

\ShowTheorem{tensor product and polymorphism}
\begin{proof}
Равенство
\EqRef{map f, representation, tensor product}
следует
из равенств
\EqRef{map i, representation, tensor product} и
\EqRef{map j, representation, tensor product}.
Существование отображения $h$ следует из определения
\RefDefinition{tensor product of representations}
и построений, выполненных при доказательстве теоремы
\RefTheorem{tensor product of representations}.
\end{proof}

\ShowTheorem{representation, tensor product}
\begin{proof}
Равенство
\EqRef{tensors 1, representation, tensor product}
является следствием равенства\\
\EqRef{g_1 1, representation, tensor product}
и определения
\EqRef{g1()=otimes}.
Равенство
\EqRef{tensors 2, representation, tensor product}
является следствием равенства
\EqRef{g_1 2, representation, tensor product}
и определения
\EqRef{g1()=otimes}.
\end{proof}

\section{Ассоциативность тензорного произведения}

Пусть $A$ является мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{B1,B2,B3}
- $\Omega_2$\Hyph алгебры.
Пусть для $k=1$, $2$, $3$
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $B_k$.

\begin{lemma}
\labelLemma{ox12x3->ox123 morphism of oxB12}
{\it
Для заданного значения
\ShowEq{x3 in B3}
отображение
\ShowEq{ox12x3->ox123}
определённое равенством
\ShowEq{ox12x3->ox123=}
является приведенным морфизмом представления
\ShowEq{oxB12}
в представление
\ShowEq{oxB13}.
}
\end{lemma}
\begin{proof}
Согласно теореме
\RefTheorem{B times->B otimes},
для заданного значения
\ShowEq{x3 in B3}
отображение
\ShowEq{x123->ox123}
является полиморфизмом по переменным
\ShowEq{x in B 12}
Следовательно,
для заданного значения
\ShowEq{x3 in B3}
лемма является следствием теоремы
\RefTheorem{tensor product and polymorphism}.
\end{proof}

\begin{lemma}
\labelLemma{ox12x3->ox123 morphism of B3}
{\it
Для заданного значения
\ShowEq{x12 in B12}
отображение
$h_{12}$
является приведенным морфизмом представления
$B_3$
в представление
\ShowEq{oxB13}.
}
\end{lemma}
\begin{proof}
Согласно теореме
\RefTheorem{B times->B otimes}
и равенству
\EqRef{g1()=otimes},
для заданного значения
\ShowEq{x in B 12,}
отображение
\ShowEq{x ox12 3->ox123}
является морфизмом по переменной
\ShowEq{x in B 3}
Следовательно,
теорема является следсвием равенства
\EqRef{reduced polymorphism of representation, ak}
и теоремы
\RefTheorem{existence of reduced polymorphism, a omega b omega}.
\end{proof}

\begin{lemma}
\labelLemma{h:ox(12)3->ox123}
{\it
Существует приведенный морфизм представлений
\ShowEq{h:ox(12)3->ox123}
}
\end{lemma}
\begin{proof}
Согласно леммам
\RefLemma{ox12x3->ox123 morphism of oxB12},
\RefLemma{ox12x3->ox123 morphism of B3}
и определению
\RefDefinition{reduced polymorphism of representations},
отображение $h_{12}$ является приведенным полиморфизмом представлений.
Утверждение леммы является следствием теоремы
\RefTheorem{tensor product and polymorphism}.
\end{proof}

\begin{lemma}
\labelLemma{g:ox123->ox(12)3}
{\it
Существует приведенный морфизм представлений
\ShowEq{g:ox123->ox(12)3}
}
\end{lemma}
\begin{proof}
Отображение
\ShowEq{x123->ox(12)3}
является полиморфизмом по переменным
\ShowEq{x in B 13}
Следовательно,
лемма является следствием теоремы
\RefTheorem{tensor product and polymorphism}.
\end{proof}

\begin{theorem}
\labelTheorem{tensor product is associative}
\ShowEq{A1xA2xA3}
\end{theorem}
\begin{proof}
Согласно лемме
\RefLemma{h:ox(12)3->ox123},
существует приведенный морфизм представлений
\ShowEq{h:ox(12)3->ox123}
Согласно лемме
\RefLemma{g:ox123->ox(12)3},
существует приведенный морфизм представлений
\ShowEq{g:ox123->ox(12)3}
Следовательно, приведенные морфизмы представлений $h$, $g$
являются изоморфизмами, откуда следует равенство
\ShowEq{B1xB2xB3=(B1xB2)xB3}
Аналогично мы можем доказать равенство
\ShowEq{B1xB2xB3=B1x(B2xB3)}
\end{proof}

\begin{remark}
Очевидно, что структура $\Omega_2$\Hyph алгебр
\ShowEq{x(12)3 123}
слегка различна.
Мы записываем равенство
\EqRef{B1xB2xB3=(B1xB2)xB3},
опираясь на соглашение
\RefConvention{isomorphic representations S1=S2}
и это позволяет нам говорить об ассоциативности тензорного произведения представлений.
\qed
\end{remark}




==> Stmt.1908.04418.Russian.tex <==
%auto-ignore
\input{Stmt.1908.04418.Eq}

\AddEq[3]{theorem: coordinates of product of inverse transformation}
{
\begin{theorem}
\labelTheorem{coordinates of product of inverse transformation, #1}
Пусть
\ShowEq{set of coordinates of automorphism}{#2}{}
- множество координат автоморфизма $#2$.
Пусть
\ShowEq{set of coordinates of automorphism}{#3}
- множество координат автоморфизма $#3$.
Множество координат автоморфизма
\ShowEq{1o2-}{#2}{#3}
удовлетворяет равенству
\DrawEq[{#2}{#3}]{coordinates of product of inverse transformation}{#1}
\end{theorem}
}

\AddEq[3]{proof: coordinates of product of inverse transformation}
{
\begin{proof}
Равенство
\DrawEq[{#2}{#3}]{coordinates of product of inverse transformation 1}{#1}
является следствием теорем
\RefTheorem{superposition of coordinates of endomorphisms, #1},
\RefTheorem{coordinates of inverse transformation, #1}.
Равенство
\eqRef{coordinates of product of inverse transformation}{#1}
является следствием равенства
\eqRef{coordinates of product of inverse transformation 1}{#1}.
\end{proof}
}


==> Stmt.Gravity.Russian.tex <==
%auto-ignore
\input{Stmt.Gravity.Eq}

\AddEq[2]{note: sum of vectors 1}
{
Сумма векторов
%TabPage
\noindent
\begin{tabular}{@{}lcr}
\ShowEq{Vector v}{#1}
&
и
&
\ShowEq{Vector w}{#2}
\end{tabular}
определена правилом треугольника
\ShowEq{Vector v+w}{#1}{#2}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
Из правила параллелограмма
следует коммутативность сложения.
\end{minipage}
&
\begin{minipage}{160pt}
\ShowEq{Vector v+w=w+v}{#1}{#2}
\end{minipage}
\end{tabular}
}

\AddEq[2]{note: sum of vectors 2}
{
Ниже мы рассмотрим модель аффинного пространства
в метрико\hyph аффинном многообразии.
\ePrints{0803.3276,0405.027}
\ifx\Semafor\ValueOff
Когда мы рассматриваем связность $\Gamma^k_{ij}$ в римановом пространстве,
мы накладываем на связность ограничение,\,\footnote{
Смотри определение аффинной связности в римановом пространстве
на странице
\citeBib{Rashevsky}\Hyph 443.
}
что тензор кручения
\ShowEq{T=G-G}
обращается в $0$ (симметрия связности)
и скалярное произведение векторов при параллельном переносе не меняется.
Если на дифференцируемом многообразии определены
метрический тензор и произвольная связность,
то это многообразие называется
\AddIndex{метрико\Hyph аффинным многообразием}{metric-affine manifold}.\,\footnote{
Смотри также определение
\RefDefinition[\RefGravity]{metric-affine manifold}.
}
В частности, связность в метрико\Hyph аффинном многообразии имеет кручение.
\fi

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
\setlength{\parindent}{5mm}
В римановом пространстве, мы пользуемся геодезическими
вместо прямых.
Поэтому вектор $#1$ мы можем представить
с помощью отрезка $AB$ геодезической $L_{#1}$
при условии, что
вектор $#1$ касается геодезической $L_{#1}$ в точке $A$
и длина отрезка $AB$ равна длине вектора $#1$.
\end{minipage}
&
\ShowEq{Vector v Riemann}{#1}
\end{tabular}

\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{210pt}
\setlength{\parindent}{5mm}
Это определение позволяет отождествить вектор $#1$
и отрезок $AB$ геодезической $L_{#1}$.
\end{minipage}
&
\end{tabular}

\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
\setlength{\parindent}{5mm}
Для заданных векторов $#1$ и $#2$ в касательной плоскости к точке $A$,
мы будем полагать $\rho>0$ - длина вектора $#1$
и $\sigma>0$ - длина вектора $#2$.
\ePrints{323966352,0921-2370}
\ifx\Semafor\ValueOff
Пусть $V$ - единичный вектор, колинеарный вектору $#1$
\ShowEq{V rho=v}
Пусть $W$ - единичный вектор, колинеарный вектору $#2$
\ShowEq{W sigma=w}
\fi
%\ShowEq{triangle ABC}
\end{minipage}
&
\ShowEq{Vector w Riemann}{#2}
\end{tabular}
}

\AddEq{note: sum of vectors 3}
{
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{240pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_v$ через точку $A$, используя вектор $v$
как касательный вектор к $L_v$ в точке $A$.
Пусть $\tau$ - канонический параметр на $L_v$ и
\ShowEq{dx/dt=A}{\tau}V
Мы перенесём вектор $w$ вдоль геодезической $L_v$ из точки $A$
в точку $B$, определённую значением параметра $\tau=\rho$.
Мы обозначим результат $w'$.
\end{minipage}
&
\ShowEq{Vector v+w= 1 Riemann}vw
\end{tabular}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_{w'}$ через точку $B$, используя вектор $W'$
как касательный вектор к $L_{w'}$ в точке $B$.
Пусть $\varphi'$ - канонический параметр на $L_{w'}$ и 
\ShowEq{dx/dt=A}{\varphi'}{W'}
Мы определим точку $C$ на геодезической $L_{w'}$
значением параметра $\varphi'=\sigma$
\end{minipage}
&
\ShowEq{Vector v+w= Riemann}vw
\end{tabular}

Я полагаю, что длина векторов $v$ и $w$ мала.
Тогда существует единственная геодезическая $L_u$
из точки $A$ в точку $C$.
Я буду отождествлять отрезок $AC$ геодезической $L_u$
и вектор $v+w$.
}

\AddEq{note: sum of vectors 4}
{
Аналогичным образом я строю треугольник $ADE$,
чтобы определить вектор $w+v$.

\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_w$ через точку $A$, используя вектор $w$
как касательный вектор к $L_w$ в точке $A$.
Пусть $\varphi$ - канонический параметр на $L_w$ и
\ShowEq{dx/dt=A}{\varphi}W
Мы перенесём вектор $v$ вдоль геодезической $L_w$ из точки $A$
в точку $D$, определённую значением параметра $\varphi=\sigma$.
Мы обозначим результат $v'$.
\end{minipage}
&
\ShowEq{Vector w+v= 1}
\end{tabular}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_{v'}$ через точку $D$, используя вектор $v'$
как касательный вектор к $L_{v'}$ в точке $D$.
Пусть $\tau'$ - канонический параметр на $L_{v'}$ и 
\ShowEq{dx/dt=A}{\tau'}{V'}
Мы определим точку $E$ на геодезической $L_{v'}$
значением параметра $\tau'=\rho$
\end{minipage}
&
\ShowEq{Vector w+v=}
\end{tabular}

Существует единственная геодезическая $L_u$
из точки $A$ в точку $E$.
Я буду отождествлять отрезок $AE$ геодезической $L_u$
и вектор $w+v$.
}

\AddEq{note: sum of vectors 5}
{
%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Формально линии $AB$ и $DE$ так же, как линии $AD$ и $BC$, параллельны.
Длины отрезков $AB$ и $DE$ равны так же, как длины
отрезков $AD$ и $BC$ равны. Мы называем такую фигуру
\AddIndex{параллелограммом}{parallelogram}, построенным на векторах
$v$ и $w$ с вершиной в точке $A$.
\end{minipage}
&
\ShowEq{Vector v+w=w+v Metric-affine}vw
\end{tabular}
}

\DefLemma{increase of coordinate along geodesic}
{
Пусть $L_v$ - геодезическая через точку $A$ и вектор $v$
- касательный вектор к $L_v$ в точке $A$.
Приращение координаты $x^k$ вдоль геодезической $L_v$ имеет вид
\ShowEq{increase of coordinate along geodesic}
где $\tau$ - канонический параметр и мы вычисляем производные и компоненты
$\Gamma^k_{mn}$ в начальной точке. 
}

\DefProof{increase of coordinate along geodesic}
{
Система дифференциальных уравнений геодезической $L_v$
имеет вид
\ShowEq{differential equation of geodesic}
Мы можем записать решение
системы дифференциальных уравнений
\EqRef{differential equation of geodesic}
в виде ряда Тейлора
\ShowEq{increase of coordinate along geodesic 1}
Равенство
\EqRef{increase of coordinate along geodesic}
является следствием равенства
\EqRef{increase of coordinate along geodesic 1}.
}

\DefTheorem{parallelogram is not closed old}
{
Предположим $CBADE$ - параллелограм с вершиной в точке
$A$; тогда построенная фигура не будет замкнута \citeBib{torsion}.
Величина различия координат
точек $C$ и $E$ равна поверхностному интегралу кручения
над этим параллелограммом\,\footnote{Доказательство этого утверждения я нашёл в \citeBib{Shilov}}
\ShowEq{CE = surface integral of the torsion}
}

\AddEq{theorem: parallelogram is not closed}
{
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
\begin{theorem}
\labelTheorem{parallelogram is not closed}
Предположим $CBADE$ - параллелограм с вершиной в точке
$A$; тогда построенная фигура не будет замкнута \citeBib{torsion}.
Величина различия координат
точек $C$ и $E$ равна поверхностному интегралу кручения
над этим параллелограммом
\ShowEq{CE = surface integral of the torsion}
\end{theorem}
\end{minipage}
&
\ShowEq{Vector v+w=w+v Metric-affine}vw
\end{tabular}
}

\DefProof{parallelogram is not closed}
{
Согласно лемме
\RefLemma{increase of coordinate along geodesic},
приращение координаты $x^k$ вдоль геодезической $L_v$
имеет следующий вид\,\footnote{
Доказательство этого утверждения я нашёл в \citeBib{Shilov}}
\ShowEq{CE = surface integral of the torsion}
\ShowEq{Delta AB=}
и приращение координаты $x^k$ вдоль геодезической $L_{b'}$
имеет следующий вид
\ShowEq{Delta BC=}
Здесь
\ShowEq{W'k=Wk-...}
результат параллельного переноса вектора $w$ из $A$ в $B$ и
\ShowEq{G(B)=G(A)+...}
с точностью до малой первого порядка. Подставляя
\EqRef{W'k=Wk-...},
\EqRef{G(B)=G(A)+...}
в
\EqRef{Delta BC=},
мы получим
\ShowEq{Delta BC= 1}
Общее приращение координаты $x^K$ вдоль пути $ABC$ имеет вид
\ShowEq{Delta ABC=}
Аналогично общее приращение координаты $x^K$ вдоль пути $ADE$ имеет вид
\ShowEq{Delta ADE=}
Из
\EqRef{Delta ABC=}
и
\EqRef{Delta ADE=}
следует, что
\ShowEq{Delta ADE-ABC=}
и мы получаем интегральную сумму для выражения
\[
\Delta_{ADE}x^k-\Delta_{ABC}x^k
=\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn})dx^m \wedge dx^n
\]

\ePrints{0803.3276,FAlgebra,0405.027}
\ifx\Semafor\ValueOn
Однако недостаточно найти разность
\[\Delta_{ADE}x^k-\Delta_{ABC}x^k\]
чтобы найти разность координат точек $C$ и $E$.
Координаты могут быть неголономными и мы должны учесть, что
координаты вдоль замкнутого пути изменяются \EqRef{change of coordinate along a loop}
\[\Delta x^k=\oint_{ECBADE}dx^k=-\iint_\Sigma c^k_{mn}dx^m \wedge dx^n \]
где $c$ - объект неголономности.

Окончательно разность координат точек $C$ и $E$ имеет вид
\[\Delta_{CE}x^k=\Delta_{ADE}x^k-\Delta_{ABC}x^k+\Delta x^k=
\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn}-c^k_{mn})dx^m \wedge dx^n\]
Используя \EqRef{Torsion coordinates}, мы доказали утверждение.
\fi
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теоремы
\RefTheorem{action of ring of rational integers in Abelian group}
и определения
\RefDefinition{module over commutative ring}
следует, что абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefEq
{
\begin{definition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\qed
\end{definition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в алгебре
\ShowEq{AoxA}A{}
определено согласно правилу
\DrawEq{product in algebra AA}{}
Представление
\ShowEq{h:AoxA->L(A)}
$D$\Hyph алгебры
\ShowEq{AoxA}A{}
в модуле
\ShowEq{L(A;B)}DAA,
определённое равенством
\ShowEq{representation AA in LA}
позволяет отождествить тензор
\ShowEq{d in AxoA}
с линейным отображением
\ShowEq{product in algebra AA 2},
где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}
имеет вид
\ShowEq{a ox b c=}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{direct sum of D modules}
{
Копроизведение в категории $D$\Hyph модулей называется
\AddIndex{прямой суммой}{direct sum}.\,\footnote{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой $D$\Hyph модулей $A$ и $B$.
}

\AddEq{theorem: definition of module over commutative ring}
{
\begin{theorem}
\labelTheorem{definition of module}
Элементы $D$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закону ассоциативности}{associative law}
\DrawEq{associative law, module}2
\item 
\labelItem{distributive law, module}
\AddIndex{закону дистрибутивности}{distributive law}
\ShowEq{distributive law, module}
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, D-module}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
\end{theorem}
}

\AddEq{definition: module over algebra}
{
\begin{definition}
\labelDefinition{\SideWS module over algebra}
Эффективное \SideRu востороннее представление
\DrawEq{\SideWS A->*V}{def}
ассоциативной $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{\SideRu вым модулем}{\SideWS module} над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{\SideRu вым $A$\Hyph модулем}{\SideWS A module}
или
\AddIndex{$\SideA$\Hyph модулем}{\SideA-module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\qed
\end{definition}
}

\DefDefinition{left vector space over algebra}
{
Пусть $A$ - алгебра с делением.
Эффективное левостороннее представление
\DrawEq{left A->*V}{}
%ассоциативной $D$\Hyph алгебры $A$
абелевой группы $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{левым векторным пространством}{left vector space}
над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{левым $A$\Hyph векторным пространством}{left A vector space}
или
\AddIndex{$A*$\Hyph векторным пространством}{A*-vector space}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
}

\DefDefinition{right vector space over algebra}
{
Пусть $A$ - алгебра с делением.
Эффективное правостороннее представление
\DrawEq{right A->*V}{}
%ассоциативной $D$\Hyph алгебры $A$
абелевой группы $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{правым векторным пространством}{right vector space}
над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{правым $A$\Hyph векторным пространством}{right A vector space}
или
\AddIndex{$*A$\Hyph векторным пространством}{*A-vector space}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
}

\AddEq{theorem: module over algebra}
{
\begin{theorem}
\labelTheorem{\SideWS module over algebra}
Следующая диаграмма представлений описывает \SideRu\To $\Base$\Hyph модуль $V$
\ShowEq{diagram of representations, \SideWS module}
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
\end{theorem}
}

\DefProof{module over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\def\Temp{}
\ifx\SideNS\Temp
\RefDefinition{module over commutative ring}
и теоремы
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefDefinition{\SideWS module over algebra}
%и следствия
%\RefCorollary{Free Algebra over Ring}.
и теоремы
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{lemma}
\labelLemma{structure of D algebra is generated by product}
{\it
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
}
\end{lemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\RefDefinition{linear map from A1 to A2, commutative module},
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{representation of D module in D module determines the product}
{\it
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
}
\end{lemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лем
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\AddEq{theorem: A module -> algebra is associative}
{
\begin{theorem}
\labelTheorem{\SideWS A module -> algebra is associative}
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
\end{theorem}
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\AddEq{theorem: definition of A module}
{
\begin{theorem}
\labelTheorem{definition of \SideWS module}
Пусть $V$ является \SideRu\What $\Base$\Hyph модулем.
Для любого вектора $v\in V$,
вектор, порождённый диаграммой представлений
\EqRef{diagram of representations, \SideWS module},
имеет следующий вид
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\ShowEq{\SideWS module, a+n:V->V}
порождает\,\footnote{
Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.
}
\algebrad $\Base_{(1)}$
где сложение определено равенством
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
и произведение определено равенством
\DrawEq{(a+n)(b+m)=}{\SideWS module}
\algebraD $\Base_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\algebrab $\Base$.
\begin{table}[h]
%\caption{Active and Passive Representations}
%\label{table:Passive and Active Representations}
\begin{tabular}{|l|l|l|}
\hline
Если \algebrac $\Base$ имеет единицу, то
\ShowEq{A1=A unital extension}
Если \algebrac $\Base$ является идеалом $\CBase$, то
\ShowEq{A1=D unital extension}
В противном случае
\ShowEq{A1=A+D unital extension}
\end{tabular}
\end{table}
\item
\algebraD $\Base$ является \SideRu\What идеалом \algebrab $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
Множество преобразований
\EqRef{\SideWS module, (a+n)v=av+nv}
порождает \SideRu\HSide представление \algebrab $\Base_{(1)}$ в абелевой группе $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
\end{theorem}
}

\AddEq{theorem: definition of A module, property}
{
\begin{theorem}
\labelTheorem{definition of \SideWS module, property}
Элементы \SideRu\From $\Base$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\ShowEq{distributive law, \SideWS module}
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{p,q in \Base 1, v,w in V}
\end{theorem}
}

\AddEq{proof: definition of A module}
{%
{\sc Доказательство теорем
\RefTheorem{definition of \SideWS module},
\RefTheorem{definition of \SideWS module, property}.}
Пусть $v\in V$.

\begin{lemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Пусть 
\ShowEq{module, d in D}
\ShowEq{module, a in A}
Отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
}
\end{lemma}

{\sc Доказательство.}
Утверждения
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{\SideWS module over algebra}.
Так как $V$ является абелевой группой, то
\ShowEq{\SideWS module, dv+av in V}
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\EqRef{\SideWS module, a+n:V->V}.
Поскольку преобразование $\DTransf(\DArg)$
и \SideRu\HSide преобразование $\ATransf(a)$
являются эндоморфизмами абелевой группы $V$,
то отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
\hfill\(\odot\)

Пусть $\Base_{(1)}$ - множество отображений
\EqRef{\SideWS module, a+n:V->V}.
Равенство
\EqRef{distributive law, \SideWS module, 1}
является следствием леммы
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\EqRef{distributive law, \SideWS module, 2}.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\EqRef{distributive law, \SideWS module, 2}.
Равенство
\ShowEq{distributive law, \CBase, \SideWS module, 2}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\ShowEq{distributive law, \Base, \SideWS module, 2}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \algebrab $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{\SideWS module}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Так как произведение в $D$\Hyph алгебре $A$ может быть неассоциативным,
то опираясь на теорему
\RefTheorem{definition of \SideWS module, property},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
\qed
}

\AddEq{definition: submodule}
{
\begin{definition}
\labelDefinition{submodule, \SideWS module}
Подпредставление $D$\Hyph \SideRu вого модуля $V$ называется
\AddIndex{подмодулем}{submodule}
\SideRu вого $D$\Hyph модуля $V$.
\qed
\end{definition}
}

\AddEq{theorem: submodule}
{
\begin{theorem}
\labelTheorem{submodule, \SideWS module}
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu вого $\Base$\Hyph модуля $V$.
Если векторы
\ShowEq{set vi}
принадлежат подмодулю $V'$ \SideRu вого $\Base$\Hyph модуля $V$,
то линейная комбинация векторов
\ShowEq{set vi}
принадлежат подмодулю $V'$.
\end{theorem}
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определений
\RefDefinition{\SideWS linear combination of vectors},
\RefDefinition{submodule, \SideWS module}.
}

\AddEq{theorem: set of vectors generated by set of vectors}
{
\begin{theorem}
\labelTheorem{set of vectors generated by set of vectors, \SideWS module}
Пусть $V$ - \SideRu\To $\Base$\Hyph модуль.
Множество векторов, порождённое множеством векторов
\ShowEq{vi V},
имеет вид\,\footnote{
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}
\ShowEq{w=sum vi, \SideWS module}
\end{theorem}
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
Согласно теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
мы должны доказать следующие утверждения:
\ShowEq{vectors generated by set of vectors}

\begin{itemize}
\item
Для произвольного
\ShowEq{vk in v}
положим
\ShowEq{ci=dik}{\Base_{(1)}}
Тогда
\ShowEq{vk=sum vi, \SideWS module}
Утверждение
\RefItem{\SideWS module, vk in Jv}
следует из
\EqRef{w=sum vi, \SideWS module},
\EqRef{vk=sum vi, \SideWS module}.
\item
Утверждение
\RefItem{\SideWS module, cvk in Jv}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{definition of \SideWS module}
и утверждения
\RefItem{\SideWS module, vk in Jv}.
\item
Так как $V$ является абелевой группой,
то утверждение
\RefItem{\SideWS module, sum cvk in Jv}
следует из утверждения
\RefItem{\SideWS module, cvk in Jv}
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
и теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.
\else
и теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{structure of Abelian group}.
\fi
\item
Пусть
\ShowEq{w12 in Jv}wv
Так как $V$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\DrawEq{w1+w2 in V}{\SideNS}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{gi12}w
такие, что
\DrawEq[w]{w12= \SideNS}{module}
где множества
\DrawEq[w]{|ci12 ne 0|}{\SideWS module}
конечны.
Так как $V$ является абелевой группой,
то из равенства
\eqRef{w12= \SideNS}{module}
следует, что
\DrawEq[w]{w1+w2= \SideNS}{module}
Равенство
\DrawEq[w]{w1+w2= 1 \SideNS}{module}
является следствием равенств
\EqRef{distributive law, \SideWS module, 2},
\eqRef{w1+w2= \SideNS}{module}.
Из равенства
\eqRef{|ci12 ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}w
конечно.
\item
Пусть
\ShowEq{w in Jv}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{(1)}$\Hyph числа $a$,
\ShowEq{aw in Xk \SideWS module}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{set au vi}w
такие, что
\ShowEq{w= \SideWS module}
где
\DrawEq{|wi ne 0|}{\SideWS module}
Из равенства
\EqRef{w= \SideWS module}
следует, что
\ShowEq{aw= \SideWS module}
Из утверждения
\eqRef{|wi ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |awi ne 0|}
конечно.
\end{itemize}
Из равенств
\eqRef{w1+w2 in V}{\SideNS},
\eqRef{w1+w2= 1 \SideNS}{module},
\EqRef{aw in Xk \SideWS module},
\EqRef{aw= \SideWS module}
следует, что
\ShowEq{Xk+1 in Jv}
}

\AddEq{definition: linear combination of vectors}
{
\begin{definition}
\labelDefinition{\SideWS linear combination of vectors}
Пусть
\ShowEq{vi V}{}
- множество векторов.
\ShowEq{\SideWS linear combination}%
Выражение
\ShowEq{A linear combination =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{vi}
Вектор
\ShowEq{w=wi vi\SideNS}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{vi}
\qed
\end{definition}
}

\AddEq{definition: generating set of module}
{
\begin{definition}
\labelDefinition{generating set of \SideWS module}
$J(v)$
называется
\AddIndex{подмодулем, порождённым множеством}
{submodule generated by set} $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $D$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
\qed
\end{definition}
}

\AddEq{remark: generating set of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\AddEq{remark: basis of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\AddEq{definition: basis of module}
{
\begin{definition}
\labelDefinition{basis of \SideWS module}
Если множество $X\subset V$ является множеством образующих
\SideRu\From $D$\Hyph модуля $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $D$\Hyph модуля $V$.
Если существует минимальное множество $X$, порождающее
\SideRu\To $D$\Hyph модуль $V$, то такое множество $X$ называется
\AddIndex{базисом}{basis} \SideRu\From $D$\Hyph модуля $V$.
\qed
\end{definition}
}

\AddEq{theorem: linearly depends on rest of vectors}
{
\begin{theorem}
\labelTheorem{linearly depends on rest of vectors, \SideWS module}
Пусть $\Base$ - \Algebra.
Если уравнение
\ShowEq{\SideWS wi vi=0}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0},
то вектор $v_{\gij}$
линейно зависит от остальных векторов $v$.
\end{theorem}
}

\AddEq{proof: linearly depends on rest of vectors}
{
\begin{proof}
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}v
и определения
\RefDefinition{\SideWS linear combination of vectors}.
\end{proof}
}

\AddEq{remark: 0=0vi}
{
Очевидно, что для любого множества векторов $v_{\gii}$,
\ShowEq{\SideWS 0=0vi}
}

\AddEq{remark: scalars and vectors as matrix}
{
Представим множество $\Base_{(1)}$\Hyph чисел
\ShowEq{set au vi}w
в виде матрицы
\ShowEq{column vector w=wi}w
Представим множество векторов
\ShowEq{set vi}
в виде матрицы
\ShowEq{row vector w=wi}vn
Тогда мы можем записать линейную комбинацию векторов
\ShowEq{w=wi vi\SideNS}
в виде
\ShowEq{w=w cr v}
}

\AddEq{definition: linearly independent vectors}
{
\begin{definition}
\labelDefinition{\SideWS linearly independent vectors}
Множество векторов\,\footnote{
Я следую определению в
\citeBib{Serge Lang}, страница 100.}
\ShowEq{set vi}
\SideRu\From $\Base$\Hyph модуля $V$
\AddIndex{линейно независимо}{linearly independent set},
если $w=0$ следует из уравнения
\ShowEq{\SideWS wi vi=0}
В противном случае, множество векторов
\ShowEq{set vi}
\AddIndex{линейно зависимо}{linearly dependent set}.
\qed
\end{definition}
}

\AddEq{theorem: basis of module}
{
\begin{theorem}
\labelTheorem{basis of \SideWS module}
Множество векторов
\ShowEq{basis for module over algebra}
является базисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e_{\gii}$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
\end{theorem}
}

\DefProof{basis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определению
\RefDefinition{\SideWS linear combination of vectors},
множество $\Basis e$ порождает \SideRu\To $\Base$\Hyph модуль $V$
(определение
\RefDefinition{generating set of \SideWS module}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRu\To $\Base$\Hyph модуль $V$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество $\Basis e$ является базисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\AddEq{theorem: division algebra, basis}
{
\begin{theorem}
\labelTheorem{division algebra, \SideWS basis}
Пусть $\Base$ - \Algebra.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы $e_{\gii}$ линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{theorem}
}

\DefProof{division algebra, basis}
{
Пусть множество векторов
\ShowEq{ei, i in I}
линейно зависимо. Тогда в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}.
Согласно теореме
\RefTheorem{linearly depends on rest of vectors, \SideWS module},
вектор $e_{\gij}$
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество векторов
\ShowEq{ei, i in I}
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{ei, i in I}
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{ei, i in I},
то множество векторов $v$,
\ShowEq{ei, i in I}
не является линейно независимым.
}

\AddEq{convention: we use separate color for index of element}
{
\begin{convention}
\labelConvention{we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
}

\AddEq{convention: unit of algebra in basis}
{
\begin{convention}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.
\qed
\end{convention}
}

\DefDefinition{linear map from D1 A1 to D2 A2, module}
{
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
$D_1$\Hyph модуля $A_1$
в $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}

\ifx\texFuture\Defined
\AddEq{linear map from D1 A1 to D2 A2, module}
{
\begin{definition}
\labelDefinition{linear map from D1 A1 to D2 A2, \SideNS module}
{\it
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
\SideRu\From $D_1$\Hyph модуля $A_1$
в \SideRu\To $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu\From $D_1$\Hyph модуля $A_1$ в \SideRu\To $D_2$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}
\qed
\end{definition}
}
\fi

\DefDefinition{linear map from A1 to A2, commutative module}
{
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
}

\DefEq
{
\begin{theorem}
\labelTheorem{set of A->B is D module}
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
\end{theorem}
}
{theorem: set of A->B is D module}
%\DefEq

\DefDefinition{coordinates of vector 2016}
{
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Матрица $\Base$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\fi
}

\AddEq{definition: coordinates of vector}
{
\begin{definition}
\labelDefinition{coordinates of vector, \SideWS module}
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base_{(1)}$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
Матрица $\Base_{(1)}$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\qed
\end{definition}
}

\AddEq{theorem: linear dependence between vectors of basis}
{
\begin{theorem}
\labelTheorem{linear dependence between vectors of basis, \SideWS module}
Пусть $\Base$ - \algebra.
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$.
Пусть
\DrawEq[w]{c*e=0, \SideWS module}{1}
линейная зависимость векторов базиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{(1)}$\Hyph число
\ShowEq{wi i in I}
не имеет обратного элемента
в \algebraa $\Base_{(1)}$.
\item
Множество $\Base'$ матриц
\ShowEq{w=wi i in I}
порождает \SideRu\To $\Base$\Hyph модуль.
\end{enumerate}
\end{theorem}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{w=wi i in I}
такая, что равенство
\eqRef{c*e=0, \SideWS module}{1}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Если мы положим, что $\Base_{(1)}$\Hyph число $c^{\gij}$
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}e
является следствием равенства
\eqRef{c*e=0, \SideWS module}{1}.
Следовательно вектор $e_{\gij}$
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является базисом.
Следовательно, наше предположение неверно,
и $\Base_{(1)}$\Hyph число $c^{\gij}$ не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[b]{c*e=0, \SideWS module}{}
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\AddEq{theorem: coordinates of vector with linear dependence}
{
\begin{theorem}
\labelTheorem{coordinates of vector with linear dependence, \SideWS module}
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет базис $\Basis e$ такой, что в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{2}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{w=wi i in I}
определяет координаты вектора $0\in V$ относительно базиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно базиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
\end{theorem}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{c*e=0, \SideWS module}{2}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно базиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{c*e=0, \SideWS module}{2},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.
}

\AddEq{definition: free module over ring}
{
\begin{definition}
\labelDefinition{free \SideWS module}
\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRu\To $\Base$\Hyph модуль}{free module},\,\footnote{
Я следую
определению в \citeBib{Serge Lang}, страница 103.}
если \SideRu\To $\Base$\Hyph модуль $V$ имеет базис
и векторы базиса линейно независимы.
\qed
\end{definition}
}

\AddEq{theorem: coordinates of vector of free module}
{
\begin{theorem}
\labelTheorem{coordinates of vector of free \SideWS module}
Координаты вектора $v\in V$ относительно базиса $\Basis e$
свободного \SideRu\From $\Base$\Hyph модуля $V$
определены однозначно.
\end{theorem}
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\RefTheorem{coordinates of vector with linear dependence, \SideWS module}
и определений
\RefDefinition{\SideWS linearly independent vectors},
\RefDefinition{free \SideWS module}.
}

\DefTheorem{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnote{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}
левого \BoxB{A}модуля
\ShowEq{L(A;B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f:A->B}fAA
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\end{enumerate}
}

\DefTheorem{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnote{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}
\ShowEq{L(A;B)}DAB.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\ShowEq{A->B}AD.
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A;B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A;B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\DefTheorem{direct sum of n D modules}
{
Прямая сумма $D$\Hyph модулей
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}
}

\DefTheorem{foa=fi ai}
{
Пусть
\ShowEq{A1n}An{}
- $D$\Hyph модули и
\ShowEq{A1o+.n}An
Представим $A$\Hyph число
\ShowEq{A1o+.n}an
как вектор столбец
\ShowEq{a=(a1.n)}an
Представим линейное отображение
\ShowEq{f:A->B}fAB
как вектор строку
\ShowEq{f=(f1.n)}
Тогда значение отображения $f$ в $A$\Hyph числе $a$
можно представить как произведение матриц
\ShowEq{foa=fi ai}
}

\DefTheorem{foa=fi a}
{
Пусть
\ShowEq{A1n}Bm{}
- $D$\Hyph модули и
\ShowEq{A1o+.n}Bm
Представим $B$\Hyph число
\ShowEq{A1o+.n}bm
как вектор столбец
\ShowEq{a=(a1.n)}bm
Тогда линейное отображение
\ShowEq{f:A->B}fAB
имеет представление как вектор столбец отображений
\ShowEq{a=(a1.n)}fm
таким образом, что если
$b=f\circ a$,
то
\DrawEq{foa=fi a}{}
}

\DefTheorem{map of direct sum of modules}
{
Пусть
\ShowEq{A1n}An,
\ShowEq{A1n}Bm{}
- $D$\Hyph модули и
\ShowEq{A1o+.n}An
\ShowEq{A1o+.n}Bm
Представим $A$\Hyph число
\ShowEq{A1o+.n}an
как вектор столбец
\ShowEq{a=(a1.n)}an
Представим $B$\Hyph число
\ShowEq{A1o+.n}bm
как вектор столбец
\ShowEq{a=(a1.n)}bm
Тогда линейное отображение $f$
имеет представление как матрица отображений
\ShowEq{matrix of maps}
таким образом, что если
$b=f\circ a$,
то
\ShowEq{b=f rco a}
Отображение
\ShowEq{fij:->}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $f^i_j$
с помощью \BoxB{B^i}чисел.
}

\DefTheorem{direct sum of D modules}
{
Пусть
\ShowEq{set Bi}A
- семейство $D$\Hyph модулей.
Тогда представление
\ShowEq{D->*o+A}
кольца $D$
в прямой сумме абелевых групп
\ShowEq{o+Ai}
является прямой суммой $D$\Hyph модулей
\ShowEq{o+Ai}
}

\AddEq{text: Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\AddEq{theorem: linear map of A module, coordinates}
{
\begin{theorem}
\labelTheorem{linear map of \SideWS A module, coordinates \Base\DF\Base\DT}
\ShowEq{Let e be basis}{\Base_\DF}iI{}{D_1}{\Base_\DF}
\ShowEq{Let e be basis}{\Base_\DT}jJ{}{D_2}{\Base_\DT}
\ShowEq{Let e be basis}{\Module_1}kK{\SideRu\Which}{\Base_\DF}{\Module_1}
\ShowEq{Let e be basis}{\Module_2}lL{\SideRu\Which}{\Base_\DT}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}{\Vector g}{\Vector f}
имеет представление
\DrawEq[g]{r2:A1->A2, \DFDT module}{1 \SideWS g}
\ShowEq{linear map in \SideWS A module}
\DrawEq{linear map in A module}{\SideNS}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
\end{theorem}
}

\DefProof{linear map of A module, coordinates}
{
Равенство
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS g}
является следствием теоремы
\RefTheorem{linear map of D1 D2 module, coordinates}.

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map in A module}{\SideNS}
является следствием теоремы
\RefTheorem{map of direct sum of modules}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}
алгебры $\AOn$
в модуле $\LAnA$,
определённое равенством
\DrawEq{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\ShowEq{product in algebra An 2}
где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\AddEq{remark: notation for linear map}
{
Если отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D_1$\Hyph алгебры $A_1$ в $D_2$\Hyph алгебру $A_2$,
то я пользуюсь обозначением
\ShowEq{f circ a =}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{theorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{theorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefEq
{
\begin{proof}
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
\end{proof}
}
{proof: conjugation transformation}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{theorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
\end{proof}
}
{proof: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A;B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{theorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{h generated by f, associative algebra}
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(D;A_1;A_2)$.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\ShowEq{f:A->B}f{A_1}{A_2}
имеет вид
\ShowEq{h generated by f, associative algebra}
\end{theorem}
}
{theorem: h generated by f, associative algebra}
%\DefEq

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A;B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{theorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{theorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A;B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map of complex field}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\ShowEq{f:A->B}fCC
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a01=}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefTheorem{linear map of complex field}
{
Линейное отображение
\ShowEq{f in LRC y=fx}
поля комплексных чисел имеет вид
\ShowEq{linear map of algebra C, structure, 1}
\ShowEq{linear map of algebra C, structure, 2}
где $C$\Hyph числа
\ShowEq{a... C}
определены равенством
\ShowEq{a01=}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{polylinear map of algebras}
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$ ($A_1=...=A_n=A$)
в $D$\Hyph алгебру
$S$.
}

\DefEq
{
\begin{theorem}
\labelTheorem{sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of linear maps, D module}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{sum of polylinear maps, module}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of polylinear maps, module}
%\DefEq

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\AddEq{definition: linear map A module}
{
\begin{definition}
\labelDefinition{linear map \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set linear maps, \SideWS A12 module}
множество линейных отображений
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{definition}
}

\AddEq{definition: homomorphism A module}
{
\begin{definition}
\labelDefinition{homomorphism \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for homomorphism}1
в диаграмму представлений
\ShowEq{A module diagram for homomorphism}2
называется
\AddIndex{гомоморфизмом}{homomorphism}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set homomorphisms, \SideWS A12 module}
множество гомоморфизмов
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{definition}
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A;B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefEq
{
\begin{definition}
\labelDefinition{linear map from A1 to A2, module}
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.
\qed
\end{definition}
}
{definition: linear map from A1 to A2, module}
%\DefEq

\AddEq{theorem: linear map of module}
{
\begin{theorem}
\labelTheorem{linear map, \Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}hf
\SideRu\From $\Base_{\DF}$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_{\DT}$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnote{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map, \Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
рассматривается как определение.}
\ShowEq{property linear map \MapE}
\end{theorem}
}

\DefProof{linear map, DA1->DA2, module}
{
Из определений
\RefDefinition[\RefRepresentation]{reduced morphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module}
следует, что
отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D }).
Равенство
\eqRef{f(da)=h... module}{\DFDT \SideWS module}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{polylinear map of algebras}
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{polylinear map of algebras}
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module},
\RefDefinition{polylinear map of modules}
и теоремы
\RefTheorem{linear map, DA1->DA2, module}.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\RefDefinition{module over commutative ring}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A;B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A;B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\AddEq{theorem: linear map of A module}
{
\begin{theorem}
\labelTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}gf
\SideRu\From $\Base_\DF$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_\DT$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnote{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
рассматривается как определение.}
\ShowEq{property linear map \MapE}
\end{theorem}
}

\DefProof{linear map of module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map from D1 A1 to D2 A2, module}
следует, что
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
и отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
Равенство
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module}
является следствием равенства
%\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{definition}.
}

\DefProof{linear map of A module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map \SideWS A module}
следует, что
\begin{itemize}
\item
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module});
\item
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{g \DFDT \SideWS module}).
\item
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{f(a+b)=...}{f \DFDT \SideWS module}).
\end{itemize}
Равенства
\eqRef{f(da)=h...}{g \DFDT \SideWS module},
\eqRef{f(da)=h...}{f \DFDT \SideWS module}
являются следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{definition}.
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\AddEq[1]{theorem: maps of conjugation antilinear}
{
\begin{theorem}
\labelTheorem{#1 maps of conjugation antilinear}
Отображения сопряжения
\ShowEq{I... O}
\DoVerb являются антилинейными гомоморфизмами.
\end{theorem}
}

\DefProof{H maps of conjugation antilinear}
{
Произведение $H$\Hyph чисел
\ShowEq{H number Ea}a
и
\ShowEq{H number Ea}b
имеет вид
\DrawEq[ab]{H product aEx}{ab}
\ShowEq{H items maps of conjugation antilinear}
}

\DefProof{O maps of conjugation antilinear}
{
Произведение $O$\Hyph чисел
\ShowEq{O number Ea}a
и
\ShowEq{O number Ea}b
имеет вид
\DrawEq[ab]{O product aEx}{ab}
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{theorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{theorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{theorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{theorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{theorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{theorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{theorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{theorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{theorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A;B)}R{#1}{#1}{}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{theorem}
}

\AddEq [6]{Let e be basis}
{
Пусть
\ShowEq{basis e of module}{#1}{#2}{#3}
базис в #4 $#5$\Hyph модуле $#6$.
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в свободном #3 $#4$\Hyph модуле $#5$.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}1{}
\DrawEq [#1{1}]{va=ae1, \SideWS module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS module}
относительно базиса
\ShowEq{basis e}2{}
\DrawEq [#9{2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}2.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}1{}
и
\ShowEq{basis e}2.
}

\AddEq{theorem: linear map of module, coordinates}
{
\begin{theorem}
\labelTheorem{linear map of \SideWS \DFDT module, coordinates}
\ShowEq{Let e be basis}1iI{}{\Base_{\DF}}{\Module_1}
\ShowEq{Let e be basis}2jJ{}{\Base_{\DT}}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}h{\Vector f}
имеет представление
\DrawEq[f]{r2:A1->A2, \DFDT module}{1 \SideWS f}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Module}fhiI{D_2}{}b
\end{itemize}
\end{theorem}
}

\DefProof{linear map of module, coordinates}
{
Так кaк
\ShowEq{show linear map \MapE}h{\Vector f}
линейное отображение, то равенство
\ShowEq{\DFDT vb=h(e1)a \SideNS}
является следствием равенств
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module},
\eqRef{va=ae1, \SideWS module}{a \DFDT\SideWS module},
\eqRef{vb=f(va)}{a \DFDT\SideWS module}.
$\Module_2$\Hyph число
\ShowEq{f(e1) \SideNS}
имеет разложение
\DrawEq{f(e1)= \SideNS}{\DFDT}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{\DFDT vb=h(e1)a \SideNS}
и \eqRef{f(e1)= \SideNS}{\DFDT}, мы получаем
\ShowEq{\DFDT vb=a f e \SideNS}
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS f}
следует из сравнения
\eqRef{va=ae1, \SideWS module}{b \DFDT\SideWS module}
и \EqRef{\DFDT vb=a f e \SideNS} и
теоремы \RefTheorem{coordinates of vector of free \SideWS module}.
}

\DefDefinition{algebra over ring}
{
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnote{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.} в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinition{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefEq
{
\begin{definition}
\labelDefinition{center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14}
\ShowEq{center of algebra}
\qed
\end{definition}
}
{definition: center of algebra}
%\DefEq

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Stmt.Omega.Russian.tex <==
%auto-ignore
\input{Stmt.Omega.Eq}

\DefDefinition{polyadditive map}
{
Отображение
\ShowEq{f:A->B}g{A^n}A
называется
\AddIndex{полиаддитивным отображением}{polyadditive map},
если для любого
\ShowEq{fi(a+b)=}
}

\DefDefinition{semiring of sets}
{
Непустая система множеств $\mathcal S$ называется
\AddIndex{полукольцом множеств}{semiring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 43.}
если
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\item
\ShowEq{empty in S}
\item
Если
\ShowEq{A, B in S}
то
\ShowEq{AB in S}
\item
Если
\ShowEq{A, A1 in S},
то множество \(A\) может быть представлено в виде 
\DrawEq{A=+Ai}{def}
где
\ShowEq{Ai*Aj=0}
\labelItem{A=+Ai}
\end{enumerate}
Представление
\eqRef{A=+Ai}{def}
множества \(A\) называется
\AddIndex{конечным разложением множества}{finite expansion of set}
\(A\).
}

\DefDefinition{norm on Omega group}
{
\AddIndex{Норма на $\Omega$\Hyph группе}
{norm on Omega group} $A$\,\footnote{
Определение дано согласно определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2, а также согласно
определению \citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.} - это отображение
\ShowEq{d->|d|}
такое, что
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\ShowEq{|a|>=0}
\ShowEq{|a|=0}
равносильно $a=0$
\ShowEq{|a+b|<=|a|+|b|}
\ShowEq{|-a|=|a|}
\end{enumerate}

$\Omega$\Hyph группа $A$,
наделённая структурой, определяемой заданием на $A$ нормы, называется
\AddIndex{нормированной $\Omega$\Hyph группой}{normed Omega group}.
}

\DefTheorem{h=f1...fn omega, converges uniformly}
{
Пусть $A$ - полная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}{}{}
- $n$\Hyph арная операция.
Пусть последовательность отображений
\ShowEq{fim M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f_i$.
Пусть множество значений отображения
$f_i$
компактно.
Тогда последовательность отображений
\ShowEq{hm=f1m...fnm omega}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f1...fn omega}{converges uniformly}
}

\DefTheorem{|int h|<int|omega||f1n|}
{
Пусть
\ShowEq{omega in Omega}{}{}
- $n$\Hyph арная операция в
абелевой \(\Omega\)\Hyph группе \(A\).
Пусть
\ShowEq{fi:X->A}
$\mu$\Hyph измеримое отображение
с компактным множеством значений.
Если отображение \(f_i\), \(i=1\), ..., \(n\),
интегрируемо, то отображение
\DrawEq{h=f1...fn omega}{}
интегрируемо и
\DrawEq{|int h|<int|omega||f1n|}{measurable}
}

\DefTheorem{h=fX g1 g2 representation}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{gi:X->A 12}
интегрируемое отображение
с компактным множеством значений.
Тогда отображение
\ShowEq{h=fX g1 g2}
интегрируемо и
\DrawEq{|int h|<int|g1||g2|}{measurable}
}

\DefTheorem{polymorphism of representations}
{
Пусть отображение
\ShowEq{map r1n,R}
является полиморфизмом
представлений $f_1$, ..., $f_n$ в представление $f$.
Для любого
\ShowEq{k,1n}
отображение
\ShowEq{map r,R}{r_{1k}}{r_2}{}
удовлетворяет равенству
\ShowEq{polymorphism of representation, ak}
Пусть $\omega_1\in\Omega_1(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_{1k}$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega1}
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega2}
}

\DefDefinition{polymorphism of representations}
{
Пусть
\ShowEq{A1n A}
- $\Omega_1$\Hyph алгебры.
Пусть
\ShowEq{B1n}
- $\Omega_2$\Hyph алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}{A_k}{B_k}
представление $\Omega_1$\Hyph алгебры $A_k$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{polymorphism of representation}
называется
\AddIndex{полиморфизмом представлений}
{polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если, для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменных
\ShowEq{ak bk in}
имеют заданное значение, отображение
\ShowEq{map r,R}{r_{1k}}{r_2}{}
является морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение
\ShowEq{map r1n,R}
является полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение
\ShowEq{map r1n,R}
является полиморфизмом представления $f$.
}

\DefDefinition{Omega group}
{
Пусть в $\Omega_1$\Hyph алгебре
$A$ определена операция сложения,
которая не обязательно коммутативна.
Мы пользуемся символом $+$ для обозначения операции суммы.
Положим
\ShowEq{Omega=...-+}
Если $\Omega_1$\Hyph алгебра $A$ является группой
относительно операции сложения
и любая операция $\omega\in\Omega$
является полиаддитивным отображением,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph группой}{Omega group}.
Если $\Omega$\Hyph группа $A$ является ассоциативной группой
относительно операции сложения,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной $\Omega$\Hyph группой}{associative Omega group}.
Если $\Omega$\Hyph группа $A$ является абелевой группой
относительно операции сложения,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{абелевой $\Omega$\Hyph группой}{Abelian Omega group}.
}

\DefTheorem{operation is distributive over addition}
{
Пусть
\ShowEq{omega n ari}{}{}n{}
- полиаддитивное отображение.
Операция $\omega$
\AddIndex{дистрибутивна}{distributive law}
относительно сложения
\ShowEq{omega is distributive over addition}
}

\DefDefinition{multiplicative Omega group}
{
Пусть произведение
\DrawEq{c=ab}{}
является операцией $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o}
Если $\Omega_1$\Hyph алгебра $A$ является группой
относительно произведения
и для любой операции
\ShowEq{omega n ari}{}{}n{}
умножение дистрибутивно относительно операция $\omega$
\DrawEq{a omega=omega a left}{}
\DrawEq{a omega=omega a right}{}
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{мультипликативной $\Omega$\Hyph группой}
{multiplicative Omega group}.
}

\DefDefinition{Abelian multiplicative Omega group}
{
Если
\ShowEq{Abelian multiplicative Omega group}
то мультипликативная $\Omega$\Hyph группа называется
\AddIndex{абелевой}{Abelian multiplicative Omega group}.
}

\DefDefinition{Omega ring}
{
Пусть сложение
\ShowEq{c1=a+b}
которое не обязательно коммутативно,
и произведение
\DrawEq{c=ab}{}
являются операциями $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o+}
Если $\Omega_1$\Hyph алгебра $A$ является
$\Omega\cup\{*\}$\Hyph группой
и
мультипликативной $\Omega\cup\{+\}$\Hyph группой,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph кольцом}{Omega ring}.
}

\DefTheorem{product in Omega ring is distributive over addition}
{
Произведение в $\Omega$\Hyph кольце
\AddIndex{дистрибутивно}{distributive law}
относительно сложения
\ShowEq{a*(b1+b2)=}
}

\DefProof{product in Omega ring is distributive over addition}
{
Теорема является следствием определений
\RefDefinition{Omega group},
\RefDefinition{multiplicative Omega group},
\RefDefinition{Omega ring}.
}

\DefDefinition{matrix over Omega ring}
{
Пусть $A$ - $\Omega$\Hyph кольцо.
\AddIndex{Матрица}{matrix}
над $\Omega$\Hyph кольцом $A$ - это таблица $A$\Hyph чисел $a^i_j$,
где индекс $i$ - это номер строки
и индекс $j$ - это номер столбца.
}


==> Stmt.Representation.Russian.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Кортеж отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
}

\DefDefinition{tower of representations}
{
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $A=(A_1,...,A_n)$.
Положим $f=(f_{1\,2},...,f_{n-1\,n})$.
Множество представлений $f_{k\,k+1}$, \Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(f,A)$ представлений $\Omega$\Hyph алгебр}
{tower of representations of algebras}.
}

\DefDefinition{diagram of representations}
{
\AddIndex{Диаграмма $(f,A)$ представлений универсальных алгебр}
{diagram of representations of algebras}
- это такой ориентированный граф, что
\StartLabelItem
\begin{enumerate}
\item
вершина $A_k$, \Kn1, является $\Omega_k$\Hyph алгеброй;
\item
ребро $f_{kl}$ является представлением
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_l$\Hyph алгебре $A_l$;
\end{enumerate}
Мы будем требовать, чтобы этот граф
был связным и не содержал циклов.
Мы будем полагать, что $A_{[0]}$ - это множество начальных вершин графа.
Мы будем полагать, что $A_{[k]}$ - это множество вершин графа,
для которых максимальный путь от начальных вершин равен $k$.
}

\DefRemark{diagram of representations}
{
Так как в разных вершинах графа
может быть одна и таже алгебра,
то мы обозначим
\ShowEq{A=A1n}A{}
множество универсальных алгебр, которые попарно различны.
Из равенства
\ShowEq{A=A(1n)1n}A
следует, что для любого индекса $(i)$
существует по крайней мере один индекс $i$ такой, что
\ShowEq{A(i)=Ai}i.
Если даны два набора множеств
\ShowEq{A=A1n}A,
\ShowEq{A=A1n}B
и определено отображение
\ShowEq{hi:Ai->Bi}
для некоторого индекса $(i)$,
то также определено отображение
\ShowEq{f:A->B}{h_i}{A_i}{B_i}
для любого индекса $i$ такого, что
\ShowEq{A(i)=Ai}i{}
и в этом случае $h_i=h_{(i)}$.
}

\DefTheorem[индукция по диаграмме представлений]{diagram of representations}
{
\AddIndex{}{induction over diagram of representations}
Пусть теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[0]}$
диаграммы $(f,A)$ представлений универсальных алгебр.
Пусть из утверждения, что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k]}$
диаграммы $(f,A)$ представлений, следует утверждение,
что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k+1]}$
диаграммы $(f,A)$ представлений.
Тогда теорема $\mathcal T$ верна для множества
универсальных алгебр
диаграммы $(f,A)$ представлений.
}

\DefDefinition{commutative diagram of representations}
{
Диаграмма $(f,A)$ представлений универсальных алгебр
называется
\AddIndex{коммутативной}{commutative diagram of representations},
если выполнено следующее условие.
для каждой пары представлений
\ShowEq{f:A->*B}{f_{ik}}{A_i}{A_k}
\ShowEq{f:A->*B}{f_{jk}}{A_j}{A_k}
следующее равенство верно\,\footnote{
Образно говоря,
представления $f_{ik}$ и $f_{jk}$
прозрачны друг для друга.
}
\ShowEq{fik fjk = fjk fik}
}

\DefTheorem{diagram of representations, define map fik}
{
Пусть
\ShowEq{f:i->*j}ij
представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре $A_j$.
Пусть
\ShowEq{f:i->*j}jk
представление $\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
Мы можем описать фрагмент\,\footnote{
Теорема
\RefTheorem{diagram of representations, define map fik}
утверждает, что преобразования в башне представлений согласованы.
}
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
диаграмы представлений с помощью диаграммы
\ShowEq{tower of representations, 1 2 3}
Отображение
\ShowEq{f:A->End 2 3}
определено равенством
\ShowEq{define map f13}
где
\ShowEq{a in A}i,
\ShowEq{a in A}j.
Если представление $f_{jk}$ эффективно
и представление $f_{ij}$ свободно,
то отображение $f_{ijk}$ является свободным представлением
\ShowEq{f:1->*3}
$\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре
\ShowEq{End Ak}Ak.
}

\DefDefinition{Morphism of Diagram of Representations}
{
Пусть
$(f,A)$
- диаграмма представлений, где
\ShowEq{A=A1n}A{}
- множество универсальных алгебр.
Пусть
$(B,g)$
- диаграмма представлений, где
\ShowEq{A=A1n}B{}
- множество универсальных алгебр.
Множество отображений
\ShowEq{A=A1n}h{}
\ShowEq{hi:Ai->Bi}
называется \AddIndex{морфизмом из диаграммы представлений
$(f,A)$ в диаграмму представлений $(B,g)$}
{morphism from diagram of representations into diagram of representations},
если для любых индексов $(i)$, $(j)$, $i$, $j$ таких, что
\ShowEq{A(i)=Ai}i,
\ShowEq{A(i)=Ai}j,
и для каждого представления
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
пара отображений $(h_j\ \ h_i)$ является
морфизмом представлений из $f_{ji}$ в $g_{ji}$.
}

\AddEq{remark: Morphism of Diagram of Representations}
{
Для любого представления $f_{ij}$,
\Kn[i]1, \Kn[j]1,
мы имеем диаграмму
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
выражают коммутативность диаграммы (1).
}

\DefTheorem{reduced polymorphism of representations}
{
Пусть отображение $r_2$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
\begin{itemize}
\item
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
\item
Для любого
\ShowEq{kl,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, akl}
\item
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\AddEq{remark: morphism of representation of Omega group}
{
\begin{remark}
\labelRemark{morphism of \SideWS representation of Omega group}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть отображение
\ShowEq{f:A->*B}g{B_1}{B_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений.
Мы будем пользоваться записью
\ShowEq{r2a=r2 o a}
для образа $A_2$\Hyph числа $a_2$
при отображении $r_2$.
Тогда мы можем записать равенство
\eqRef{morphism of representations of universal algebra, 2m}{definition}
следующим образом
\ShowEq{morphism of \SideWS representation of Omega group}
\qed
\end{remark}
}

\AddEq{definition: orbit of representation}
{
\begin{definition}
\labelDefinition{orbit of \SideNS-side representation}
Пусть $A_1$ является $\Omega$\Hyph группоидом с произведением
\ShowEq{(ab)->ab}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
$\Omega$\Hyph группоида $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\ShowEq{a in A}2,
мы определим
\AddIndex{орбиту представления}{orbit of representation}
$\Omega$\Hyph группоида $A_1$ как множество
\ShowEq{orbit of \SideNS-side representation}
\qed
\end{definition}
}

\AddEq{Let A->*AB2 be representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\AddEq{Let XY be generating sets}
{
Пусть $X$ - множество образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $Y$ - множество образующих представления
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\DefDefinition{product in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}\,\footnote{
Определение дано согласно \citeBib{Serge Lang},
страница 45.}, если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\Ii\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
}

\DefExample{Cartesian product of sets}
{
Пусть \(\mathcal S\) - категория множеств.\,\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\RefDefinition{product in category},
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
}

\DefDefinition{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ePrints{CACAA.07}
\ifx\Semafor\ValueOff
\ShowEq{coproduct in category}
\else
P из $\mathcal A$
\fi
и множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category}\,\footnote{
Определение дано согласно \citeBib{Serge Lang}, страница 46.},
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}g{B_i}R
существует единственный морфизм
\ShowEq{f:A->B}hPR
такой, что диаграмма
\ShowEq{coproduct in category diagram}
коммутативна для всех $i\in I$.

\ePrints{CACAA.07}
\ifx\Semafor\ValueOff
Если $|I|=n$, то для копроизведения множества объектов
\ShowEq{set Bi}B
в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{coproduct in category, 1 n}
\fi
}

\DefTheorem{structure of subrepresentations}
{
Пусть\,\footnote{Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, страница 94.}
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $X\subset A_2$.
Определим подмножество $X_k\subset A_2$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
}

\DefDefinition{direct sum of Abelian groups}
{
Копроизведение в категории абелевых групп $Ab$ называется
\AddIndex{прямой суммой}{direct sum}.\,\footnote{
Определение дано согласно \citeBib{Serge Lang}, страница 55.}
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой суммы абелевых групп $A$ и $B$.
}

\DefTheorem{direct sum of Abelian groups}
{
Пусть
\ShowEq{set Bi}A
- семейство абелевых групп.
Пусть
\ShowEq{A in xAi}
такое множество, что
\ShowEq{(xi)in A},
если
$x_i\ne 0$
для конечного числа индексов $i$.
Тогда\,\footnote{
Смотри также предложение \citeBib{Serge Lang}-10, страница 55.}
\ShowEq{A=o+Ai}
}

\DefProof{direct sum of Abelian groups}
{
Согласно построению
$A$ является подгруппой абелевой группы $\prod A_i$.
Отображение
\ShowEq{f:A->B}{\lambda_j}{A_j}A
определённое равенством
\ShowEq{lj(x)=0x0}
является инъективным гомоморфизмом.

Пусть
\ShowEq{set f:A->B}f{A_i}B
семейство гомоморфизмов в абелевую группу $B$.
Мы определим отображение
\ShowEq{f:A->B}fAB
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{group}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{group}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{group}
следует, что
\ShowEq{f(x+y)i=}
Следовательно, отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{group}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\AddEq{remark: side representation of group}
{
Пусть
\ShowEq{f:A->B}f{A_2}{A_2}
\ShowEq{f:A->B}g{A_2}{A_2}
эндоморфизмы $\Omega_2$\Hyph алгебры $A_2$.
Пусть произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
является композицией эндоморфизмов.
Так как произведение отображений $f$ и $g$ определено в том же порядке,
как эти отображения действуют на $A_2$\Hyph число,
то мы можем рассматривать равенство
\ShowEq{fga= o \SideNS}
как
\AddIndex{закон ассоциативности}{associative law},
который позволяет записывать равенство
\EqRef{fga= o \SideNS}
без использования скобок
\ShowEq{fga= 1 \SideNS}
а также записать равенство
\eqRef{\SideNS-side representation of group}{def}
в виде
\DrawEq{\SideNS-side 1 representation of group}{def}
Из равенства
\eqRef{* \SideNS-side representation of group}{def}
следует, что
\DrawEq{o \SideNS-side representation of group}{def}
Мы можем рассматривать равенство
\eqRef{o \SideNS-side representation of group}{def}
как
\AddIndex{закон ассоциативности}{associative law},
}

\AddEq[4]{theorem: select second basis of representation}
{
\begin{theorem}
\labelTheorem{select second basis of representation, #4}
Пусть $#2$ - пассивное преобразование
многообразия базисов #3 $#4$.
Пусть $\Basis e_1$ - базис #3 $#4$,
\ShowEq{e2=e1 o S}{#2}21
Пусть для базиса $\Basis e_3$ существует активное преобразование $#1$ такое, что
\ShowEq{e3=R o e1}{#1}31
Положим
\ShowEq{e3=R o e1}{#1}42
Тогда
\ShowEq{e2=e1 o S}{#2}43
\end{theorem}
}

\AddEq[3]{proof: select second basis of representation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#3},
активное преобразование координат базиса $\Basis e_3$ имеет вид
\DrawEq{active transformation, 1}{#3}
Пусть
\ShowEq{e2=e1 o S}{#2}53
Из равенства
\eqRef{passive transformation}{#3}
следует, что
\DrawEq{passive transformation, 1}{#3}
Из совпадения выражений в равенствах
\eqRef{active transformation, 1}{#3},
\eqRef{passive transformation, 1}{#3}
следует, что
\ShowEq{Basis e4=Basis e5}
Следовательно,
коммутативна диаграмма
\ShowEq{passive and active maps}{#1}{#2}
\end{proof}
}

\AddEq[2]{definition: basis manifold}
{
Множество
\ShowEq{basis manifold}
базисов #1 $#2$ называется
\AddIndex{многообразием базисов}{basis manifold}
#1 $#2$.
}

\AddEq{ref active representation, representation}
{
Согласно теоремам
\RefTheorem{superposition of coordinates, representation},
\RefTheorem{Automorphism of representation maps a basis into basis},
}

\AddEq{ref active representation, diagram of representations}
{
Согласно теореме
\RefTheorem{Automorphism of diagram of representations maps a basis into basis}
и определению
\RefDefinition{superposition of coordinates and words, diagram of representations},
}

\AddEq[4]{definition: active representation in basis manifold}
{
\begin{definition}
\labelDefinition{active representation in basis manifold, #1}
\ShowEq{ref active representation, #1}
автоморфизм $#4$ #2 $#3$
порождает преобразование
\DrawEq[{#4}]{active transformation}{#1}
многообразия базисов #2.
Это преобразование называется
\AddIndex{активным}{active transformation of basis}.
Согласно теореме
\RefTheorem{group of automorphisms of #1},
определено левостороннее представление
\ShowEq{active representation in basis manifold}
\ShowEq{active representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $A(f)$ называется
\AddIndex{активным представлением}{active representation in basis manifold}.
Согласно следствию
\RefCorollary{automorphism uniquely defined by image of basis, #1},
это представление однотранзитивно.
\qed
\end{definition}
}

\AddEq[4]{remark: active representation}
{
\begin{remark}
\labelRemark{active representation, #1}
Согласно замечанию
\RefRemark{X is quasibasis of #1},
могут существовать базисы #2 $#3$,
не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, #4 $#3$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\end{remark}
}

\AddEq[6]{theorem: Coordinate transformation does not depend}
{
\begin{theorem}
\labelTheorem{Coordinate transformation does not depend, #1}
Допустим пассивное преобразование $#2\in GA(f)$ отображает
базис $\Basis e_1\in\mathcal{B}[f]$
в базис $\Basis e_2\in\mathcal{B}[f]$
\DrawEq[{#2}]{passive transformation S}{#1}
Допустим #6 $#3$ имеет #5
\DrawEq[1{#3}]{Omega_2 word, basis e}{1 #1}
относительно базиса $\Basis e_1$ и имеет #5
\DrawEq[2{#3}]{Omega_2 word, basis e}{2 #1}
относительно базиса $\Basis e_2$.
Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#1}
не зависит от #4 $#3$ или базиса $\Basis e_1$, а
определенно исключительно координатами #4 $#3$
относительно базиса $\Basis e_1$.
\end{theorem}
}

\AddEq[3]{proof: Coordinate transformation does not depend}
{
\begin{proof}
Из \eqRef{passive transformation S}{#1}
и
\eqRef{Omega_2 word, basis e}{2 #1}
следует, что
\DrawEq[{#2}{#3}]{Omega word in representation, basis Y, 1}{#1}
Сравнивая \eqRef{Omega_2 word, basis e}{1 #1}
и
\eqRef{Omega word in representation, basis Y, 1}{#1}
получаем, что
\DrawEq[{#2}{#3}]{coordinate transformation in representation, 1}{#1}
Так как $#2$ - автоморфизм представления, то равенство
\eqRef{coordinate transformation}{#1}
следует из
\eqRef{coordinate transformation in representation, 1}{#1}
и теоремы
\RefTheorem{coordinates of inverse transformation, #1}.
\end{proof}
}

\AddEq[3]{remark: active and passive transformation}
{
Активное преобразование изменяет базис #1 и
#2 согласовано
и координаты #3 относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат #3 относительно базиса.
}

\AddEq[2]{theorem: Coordinate transformations form right-side representation}
{
\begin{theorem}
\labelTheorem{Coordinate transformations form right-side representation, #1}
Преобразования координат
\eqRef{coordinate transformation}{#1}
порождают эффективное контравариантное
правостороннее представление группы $GA(f)$, называемое
\AddIndex{координатным представлением}{coordinate representation}
в #2.
\end{theorem}
}

\AddEq[8]{proof: Coordinate transformations form right-side representation}
{
\begin{proof}
Согласно следствию
\RefCorollary{map of coordinates of #1},
преобразование
\eqRef{coordinate transformation}{#1}
является эндоморфизмом #4\,\footnote{Это преобразование
не порождает эндоморфизма #4 $#6$. Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако
#7, координаты которого мы рассматриваем, не меняется.}
#5

Допустим мы имеем два последовательных пассивных преобразования
$#2$ и $#8$. Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#2 #1}
соответствует пассивному преобразованию $#2$.
Преобразование координат
\DrawEq[{#3}{#8}]{coordinate transformation}{#8 #1}
соответствует пассивному преобразованию $#8$.
Согласно теореме
\RefTheorem{passive representation in basis manifold, #1},
произведение преобразований координат
\eqRef{coordinate transformation}{#2 #1}
и
\eqRef{coordinate transformation}{#8 #1}
имеет вид
\ShowEq{coordinate transformation in representation, TS}{#3}{#2}{#8}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in representation, TS 1}{#8}{#2}
Согласно теоремам
\RefTheorem{coordinates of inverse transformation, #1},
\RefTheorem{coordinates of product of inverse transformation, #1}
и определению
\RefDefinition{Left side contravariant representation}
преобразования координат
порождают
правостороннее контравариантное представление группы $GA(f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $GA(f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}
}

\AddEq[5]{remark: geometric object}
{
Пассивное представление $P(g)$ согласовано
с пассивным представлением $P(f)$,
если существует гомоморфизм $h$ группы $GA(f)$ в группу $GA(g)$.
Рассмотрим диаграмму
\ShowEq{passive representation coordinated with passive representation}
Так как отображения $P(f)$, $P(g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $GA(f)$
в многообразии базисов $\mathcal B(g)$.
Согласно построению, пассивному преобразованию $#2$ многообразии базисов $\mathcal B(f)$
соответствует пассивное преобразование $H(#2)$ многообразия базисов $\mathcal B(g)$
\DrawEq[{#2}]{passive transformation of representation g}{#1}
Тогда координатное преобразование в #3 $#4$ принимает вид
\DrawEq[{#5}{#2}]{coordinate transformation g}{#1}
}

\AddEq[5]{definition: coordinate of geometric object}
{
\begin{definition}
\labelDefinition{coordinate of geometric object, #1}
Мы будем называть
орбиту
\ShowEq{geometric object, coordinate representation}{#3}%
\ShowEq{show geometric object, coordinate representation}{#2}{#3}
\AddIndex{геометрическим объектом в координатном представлении}
{geometric object, coordinate representation},
определённом в #4 $#5$.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка
\eqRef{coordinate transformation g}{#1}
орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometric object}
относительно базиса
\ShowEq{geometric object 2}
\qed
\end{definition}
}

\AddEq[1]{remark: 2 views on geometric object}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Определение
\RefDefinition{coordinate of geometric object, #1}
строит геометрический объект в координатном пространстве.
Определение \RefDefinition{geometric object, #1} предполагает,
что мы выбрали базис представления $g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\AddEq[7]{definition: geometric object}
{
\begin{definition}
\labelDefinition{geometric object, #1}
Мы будем называть
орбиту
\ShowEq{geometric object}{#3}%
\ShowEq{show geometric object}{#2}{#3}%
\AddIndex{геометрическим объектом}{geometric object},
определённым в #4 $#5$.
Мы будем также говорить, что $#3$ - это
\AddIndex{геометрический объект типа $H$}{geometric object of type H}.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка 
\eqRef{coordinate transformation g}{#1}
орбиты  определяет #6
\ShowEq{geometric object 2, g}{#3}%
#7 мы называем
\AddIndex{представителем геометрического объекта}{representative of geometric object}
в #4 $#5$.
\qed
\end{definition}
}

\AddEq[1]{theorem: invariance principle}
{
\begin{theorem}[принцип инвариантности]
\AddIndex{}{invariance principle}
\labelTheorem{invariance principle, #1}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis e_f$.
\end{theorem}
}

\AddEq[6]{proof: invariance principle}
{
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_f$ #2 $#3$,
базис $\Basis e_g$ #2 $#4$
и координаты геометрического объекта
\ShowEq{invariance principle 4}{#5}
Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1}{#5}
Базис $\Basis e_{f1}$ связан с базисом
$\Basis e_f$ пассивным преобразованием
\ShowEq{invariance principle 2}{#6}
Согласно построению это порождает пассивное преобразование
\eqRef{passive transformation of representation g}{#1}
и координатное преобразование
\eqRef{coordinate transformation g}{#1}.
Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3}{#5}{#6}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}
}

\AddEq[1]{theorem: passive representation in basis manifold}
{
\begin{theorem}
\labelTheorem{passive representation in basis manifold, #1}
Существует однотранзитивное правостороннее представление
\ShowEq{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $P(f)$ называется
\AddIndex{пассивным представлением}{passive representation in basis manifold}.
\end{theorem}
}

\DefProof{passive representation in basis manifold}
{
Поскольку $A(f)$ - однотранзитивное левостороннее представление группы $GA(f)$,
то однотранзитивное правостороннее представление $P(f)$
определено однозначно
согласно теореме
\RefTheorem{two representations of group}.
}

\AddEq[1]{theorem: passive transformation is automorphism of A(f)}
{
\begin{theorem}
\labelTheorem{passive transformation is automorphism of A(f), #1}
Пассивное преобразование многообразия базисов
является автоморфизмом представления $A(f)$.
\end{theorem}
}

\DefProof{passive transformation is automorphism of A(f)}
{
Теорема является следствием теоремы
\RefTheorem{twin representations of group, automorphism}.
}

\AddEq[3]{theorem: passive transformation}
{
\begin{theorem}
\labelTheorem{passive transformation, #1}
Преобразование представления $P(f)$
называется
\AddIndex{пассивным преобразованием многообразия базисов}
{passive transformation of basis}
#2.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis}{#3}
\ShowEq{passive transformation of basis def}{#3}
для обозначения образа базиса $\Basis e$ при пассивном преобразовании $#3$.
Пассивное преобразование базиса имеет вид
\DrawEq[#3]{passive transformation}{#1}
\end{theorem}
}

\AddEq[1]{proof: passive transformation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#1},
активное преобразование действует на координаты
базиса слева.
Равенство
\eqRef{passive transformation}{diagram of representations}
следует из теорем
\RefTheorem{shift is automorphism of representation},
\RefTheorem{two representations of group},
\RefTheorem{twin representations of group, automorphism},
согласно которым
пассивное преобразование действует на координаты
базиса справа.
\end{proof}
}

\AddEq{definition: side representation of group}
{
\begin{definition}
\labelDefinition{\SideNS-side representation of group} 
Пусть
\ShowEq{End O2}{A_2}{}
- мультипликативная $\Omega$\Hyph группа с произведением\,\footnote{
Очень часто произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
совпадает с суперпозицией эндоморфизмов
\ShowEq{Act=circ}
Однако, как мы увидим в примере
\RefExample{left shift Lie algebra},
произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
может отличаться от суперпозиции эндоморфизмов.
Согласно определению
\RefDefinition{biring},
мы можем рассматривать две операции произведения
в универсальной алгебре $A$.
}
\ShowEq{(fg)->fg}
Пусть эндоморфизм $f$ действует на $A_2$\Hyph число $a$ с\SideRu ва.
Мы будем пользоваться записью
\ShowEq{f(a)=o \SideNS}
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа с произведением
\ShowEq{(ab)->ab}
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideRu восторонним представлением}{\SideNS-side representation}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{\SideRu восторонним $A_1$\Hyph представлением}{\SideNS-side A representation}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{\SideNS-side representation of group}{def}
Мы будем отождествлять
$A_1$\Hyph число $a_1$ с его образом $f(a_1)$
и записывать \SideRu востороннее преобразование,
порождённое $A_1$\Hyph числом $a_1$,
в форме
\ShowEq{\SideNS-side representation}
В этом случае равенство
\eqRef{\SideNS-side representation of group}{def}
принимает вид
\DrawEq{* \SideNS-side representation of group}{def}
Отображение
\ShowEq{A12->A2 1 \SideNS}
порождённое \SideRu восторонним представлением $f$, называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
$A_2$\Hyph числа $a_2$ на $A_1$\Hyph число $a_1$.
\qed
\end{definition}
}

\DefDefinition{reduced morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть
\ShowEq{id:A1->A1 A2->B2}
морфизм представлений.
В этом случае мы можем отождествить морфизм
\ShowEq{map r,R}{\id}{r_2}{}
представлений $\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $r_2$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $r_2$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $r_2$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of universal algebra}
Мы будем также пользоваться диаграммой
\ShowEq{morphism id,R of representations 2}
вместо диаграммы
\EqRef{morphism id,R of representations}.
}

\DefDefinition{action of rational integers in Abelian group}
{
Мы определим действие кольца целых чисел $Z$
в абелевой группе $G$
согласно правилу
\ShowEq{action of rational integers in Abelian group}
}

\DefTheorem{action of ring of rational integers in Abelian group}
{
Действие кольца целых чисел $Z$
в абелевой группе $G$,
рассмотренное в определении
\RefDefinition{action of rational integers in Abelian group},
является представлением.
Верны следующие равенства
\ShowEq{representation of Z in G}
}

\DefProof{action of ring of rational integers in Abelian group}
{
Равенство
\EqRef{1a=a}
является следствием равенства
\EqRef{0g=0}
и равенства
\EqRef{(n+1)g=},
когда $n=0$.

\ShowEq{step of proof: action in Abelian group}{(m+n)a=ma+na}

Равенство
\ShowEq{(k+n)a-na=ka}
является следствием равенства
\EqRef{(m+n)a=ma+na}.
Равенство
\EqRef{(m-n)a=ma-na}
является следствием равенства
\EqRef{(k+n)a-na=ka},
если мы положим
$m=k+n$, $k=m-n$.

\ShowEq{step of proof: action in Abelian group}{(nm)a=n(ma)}

\ShowEq{step of proof: action in Abelian group}{n(a+b)=na+nb}

Из равенства
\EqRef{n(a+b)=na+nb}
следует, что отображение
\ShowEq{phi(n):G->G}
является эндоморфизмом абелевой группы $G$.
Из равенств
\EqRef{(m+n)a=ma+na},
\EqRef{(nm)a=n(ma)}
следует, что отображение
\ShowEq{phi:Z->End(G)}
является гомоморфизмом кольца $Z$.
Согласно определению
\RefDefinition[\RefRepresentation]{representation of algebra},
отображение $\varphi$ является представлением
кольца целых чисел $Z$
в абелевой группе $G$.
}

\DefEq
{
\begin{definition}
\labelDefinition{tensor product of representations}
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{a1n}An{}
- $\Omega_2$\Hyph алгебры.\,\footnote{
Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
Пусть для любого
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $A_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм
\ShowEq{r1->r2}
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений
\ShowEq{a1n}An.
\qed
\end{definition}
}
{definition: tensor product of representations}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{theorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{theorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{theorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{theorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinition{free representation of algebra}
{
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnote{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Смотри также теорему
\RefTheorem{free representation of group}.
\fi
}
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что
\ShowEq{a=b}.
}

\DefDefinition{continuous map, Omega group}
{
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
}

\DefTheorem{image of interval is interval, real field}
{
Пусть
\ShowEq{f:A->B}fRR
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
}

\DefEq
{
\begin{definition}
\labelDefinition{norm of operation}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
\qed
\end{definition}
}
{definition: norm of operation}
%\DefEq

\DefTheorem{|fx|<|f||x|1n}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{definition}
\labelDefinition{norm of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление\
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
Смотри определение
\EqParm{ref definition: left-side representation of algebra}{=z}
представления универсальной алгебры.
Согласно определению
\xRef[1211.6965]{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
\fi
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{definition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{definition}
\labelDefinition{open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\,\footnote{
В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\EqParm{a in U}{=z}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{definition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\,\footnote{
Смотри также определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{definition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
}

\AddEq{definition: limit of sequence}
{
\begin{definition}
\labelDefinition{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
$\Module$\Hyph число $a$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
\qed
\end{definition}
}

\AddEq{theorem: limit of sequence}
{
\begin{theorem}
\labelTheorem{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
$\Module$\Hyph число $a$ является 
пределом последовательности
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
\end{theorem}
}

\DefProof{limit of sequence}
{
Следствие определений
\RefDefinition{open ball},
\RefDefinition{limit of sequence, normed \Algebrac}.
}

\AddEq{definition: fundamental sequence}
{
\begin{definition}
\labelDefinition{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
\qed
\end{definition}
}

\AddEq{theorem: fundamental sequence}
{
\begin{theorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
является фундаментальной последовательностью,
тогда и только тогда, когда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{theorem}
}

\DefProof{fundamental sequence}
{
Следствие определений
\RefDefinition{open ball},
\RefDefinition{fundamental sequence, normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
}

\DefTheorem{lim a=lim b}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
}

\DefEq
{
\begin{definition}
\labelDefinition{complete Omega group}
Нормированная $\Omega$\Hyph группа $A$ называется 
\AddIndex{полной}{complete Omega group}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph группы $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph группе.
\qed
\end{definition}
}
{definition: complete Omega group}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{definition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{definition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{sequence converges uniformly, fn-fm}
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
\end{theorem}
}
{theorem: sequence converges uniformly, fn-fm}
%\DefEq

\DefTheorem{h=f+g, converges uniformly}
{
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\EqParm{M(X,A)}{=.}
Однако мы можем определить сходимость последовательности в
\EqParm{M(X,A)}{=.c}
следовательно, мы можем определить топологию в
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
}

\DefDefinition{open ball}
{
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $r_2$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f$.
}

\AddEq{convention: Einstein summation}
{
\begin{convention}
Мы будем пользоваться соглашением Эйнштейна о сумме.
Это означает, что, когда индекс присутствует в
выражении дважды (один вверху и один внизу) и множество индексов известно,
это выражение подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}av
Я буду явно указывать множество
индексов, если это необходимо.
\qed
\end{convention}
}

\DefTheorem{structure of Abelian group}
{
Пусть $G$ - абелевая группа.
Множество $G$\Hyph чисел, порождённое множеством
\ShowEq{S=si},
имеет вид
\ShowEq{J(S)=gi si}
где множество
\ShowEq{|gi ne 0|}
конечно.
}

\DefProof{structure of Abelian group}
{
Мы докажем теорему по индукции, опираясь на теоремы
\citeBib{Cohn: Universal Algebra}\Hyph 5.1, страница 94, и
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного $s_k\in S$,
положим
\ShowEq{gi=dik}
Тогда
\ShowEq{sk=sum si}
\ShowEq{sk in JS}
следует из
\EqRef{J(S)=gi si},
\EqRef{sk=sum si}.

Пусть
\ShowEq{w12 in Jv}gS
Так как $G$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv}gS
Согласно равенству
\EqRef{J(S)=gi si},
существуют $Z$\Hyph числа
\ShowEq{gi12}g
такие, что
\DrawEq[g]{w12= }{group}
где множества
\DrawEq[g]{|ci12 ne 0|}{group}
конечны.
Из равенства
\eqRef{w12= }{group}
следует, что
\DrawEq[g]{w1+w2= }{group}
Равенство
\DrawEq[g]{w1+w2= 1 }{group}
является следствием равенств
\EqRef{(m+n)a=ma+na},
\eqRef{w1+w2= }{group}.
Из равенства
\eqRef{|ci12 ne 0|}{group}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}g
конечно.
Из равенства
\eqRef{w1+w2= 1 }{group}
следует, что
\ShowEq{w1+w2 in Jv}gS
}

\AddEq [1]{step of proof: action in Abelian group}
{
Из равенства
\EqRef{0g=0}
следует, что равенство
\EqRef{#1}
верно, когда $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempB{#1}
\begin{itemize}
\item
Пусть равенство
\EqRef{#1}
верно, когда $n=k\ge 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k+1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n+1)g=},
\EqRef{(m+n)a=ma+na}.
\else
равенства
\EqRef{(n+1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k+1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\ge 0$.
\item
Пусть равенство
\EqRef{(m+n)a=ma+na}
верно, когда $n=k\le 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k-1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n-1)g=},
\EqRef{(m-n)a=ma-na}.
\else
равенства
\EqRef{(n-1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k-1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\le 0$.
\item
Следовательно, равенство
\EqRef{#1}
верно для любого $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{A1(mA2) symb}
представлений}
{category of representations}
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
}

\DefProof{rcstar transpose}
{
Цепочка равенств
\ShowEq{rcstar transpose, 1}
следует из \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} и
\EqRef{cr-product of matrices}.
Равенство \eqRef{rcstar transpose}{Theorem} следует из
\EqRef{rcstar transpose, 1}.
}

\AddEq{matrix operations}
{
Произведение матриц связано с произведением гомоморфизмов
векторных пространств над полем. Согласно традиции произведение
матриц $a$ и $b$ определено как произведение
строк матрицы $a$ и столбцов матрицы $b$.

\ShowExample{matrix in right vector space}

\ShowExample{matrix in left vector space}

Из примеров
\RefExample{matrix in right vector space},
\RefExample{matrix in left vector space}
следует, что
мы не можем ограничиться традиционным произведением матриц
и нам нужно определить два вида произведения матриц.
Чтобы различать эти произведения, мы вводим
новые обозначения.
Для совместимости
обозначений с существующими мы будем иметь
в виду \RC произведение, когда
нет явных обозначений.

\ShowDefinition{row over column product}

\ShowDefinition{column over row product}

Мы так же определим следующие операции на множестве матриц.

\ShowDefinition{transpose of matrix}

\ShowDefinition{sum of matrices}
}

\DefExample{matrix in left vector space}
{
Пусть $\Basis e$ - базис
левого векторного пространства $V$
над $D$\Hyph алгеброй $A$
(смотри определение
\RefDefinition{left vector space over algebra}
и теорему
\RefTheorem{division algebra, left basis}).
Мы представим базис $\Basis e$
как строку матрицы
\ShowEq{a=(a1.n row)}en
Мы можем представить координаты вектора $v$
как вектор столбец
\ShowEq{a=(a1.n col)}vn
Однако мы не можем представить вектор
\[v=\aU vi\aD ei\]
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
Линейный гомоморфизм
левого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=vf}
Равенство
\EqRef{v'=vf}
не может быть выражено как традиционное произведение матриц $v$ и $f$.
}

\DefExample{matrix in right vector space}
{
Пусть $\Basis e$ - базис
правого векторного пространства $V$
над $D$\Hyph алгеброй $A$
(смотри определение
\RefDefinition{right vector space over algebra}
и теорему
\RefTheorem{division algebra, right basis}).
Мы представим базис $\Basis e$
как строку матрицы
\ShowEq{a=(a1.n row)}en
Мы можем представить координаты вектора $v$
как вектор столбец
\ShowEq{a=(a1.n col)}vn
Поэтому мы можем представить вектор $v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
Линейный гомоморфизм
правого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=fv}
Равенство
\EqRef{v'=fv}
выражает традиционное произведение матриц $f$ и $v$.
}

\DefDefinition{row over column product}
{
Пусть число столбцов матрицы $a$ равно числу строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$ имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
и может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.\,\footnote{
Мы будем пользоваться символом \RC\  в последующей терминологии
и обозначениях. Мы будем читать символ
$\RCstar$ как $rc$\hyph произведение
или произведение строки на столбец.
Символ произведения строки на столбец
сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
Например, если произведение $A$\Hyph чисел имеет вид
$a\circ b$,
то \RC произведение
матриц $a$ и $b$ имеет вид
$a\RCcirc b$.
}
}

\DefDefinition{column over row product}
{
Пусть число строк матрицы $a$ равно числу столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$ имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
и может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.\,\footnote{
Мы будем пользоваться символом \CR\  в последующей терминологии
и обозначениях. Мы будем читать символ
$\CRstar$ как $cr$\hyph произведение
или произведение столбца на строку.
Символ произведение столбца на строку
сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
Например, если произведение $A$\Hyph чисел имеет вид
$a\circ b$,
то \CR произведение
матриц $a$ и $b$ имеет вид
$a\CRcirc b$.
}
}

\DefDefinition{transpose of matrix}
{
Транспонирование $a^T$ матрицы $a$
меняет местами строки и столбцы
\ShowEq{transpose of matrix, 1}
}

\DefDefinition{sum of matrices}
{
Сумма матриц $a$ и $b$ определена равенством
\ShowEq{(a+b)=}
}

\DefEq
{
\begin{remark}
\labelRemark{pronunciation of product}
Мы будем пользоваться символом \RC\  или \CR\  в имени свойств
каждого произведения и в обозначениях.
Мы можем читать символы
$\RCstar$ и $\CRstar$ как $rc$\hyph произведение и $cr$\hyph произведение.
Это правило мы распространим на последующую терминологию.
\qed
\end{remark}
}
{remark: pronunciation of product}
%\DefEq

\DefDefinition{biring}
{
\AddIndex{Бикольцо}{biring} $\mathcal A$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal A$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal A$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\DrawEq{rcstar transpose}{}
\item транспозиция единицы есть единица
\ShowEq{transpose of identity}
\item двойная транспозиция есть исходный элемент
\ShowEq{double transpose}
\end{itemize}
}

\DefEq
{
\begin{theorem}[принцип двойственности для бикольца]
\AddIndex{}{duality principle for biring}
\labelTheorem{duality principle for biring}
Пусть $\mathcal{A}$ - истинное утверждение о
бикольце $A$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in A$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{theorem}[принцип двойственности для бикольца матриц]
\AddIndex{}{duality principle for biring of matrices}
\labelTheorem{duality principle for biring of matrices}
Пусть $A$ является бикольцом матриц.
Пусть $\mathcal{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item строки и столбцы всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
Если произведение в $\Omega$\Hyph кольце коммутативно, то
\ShowEq{reducibility of products}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
Поэтому в приводимом бикольце достаточно рассматривать только
\RC произведение. Однако в тех случаях, когда
порядок сомножителей существенен,
мы будем пользоваться также \CR произведением.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Так как левостороннее представление и правостороннее представление
опирается на гомоморфизм $\Omega$\Hyph группы,
то верно следующее утверждение.

\begin{theorem}[принцип двойственности для представления мультипликативной $\Omega$\Hyph группы]
\labelTheorem{duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$,
будет справедливо для правостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$, если
мы будем пользоваться правосторонним произведением на $A_1$\Hyph число $a_1$ вместо
левостороннего произведения на $A_1$\Hyph число $a_1$.
\qed
\end{theorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefTheorem{left right shift}
{
Произведение
\ShowEq{(ab)->ab}
в мультипликативной $\Omega$\Hyph группе $A$
определяет два различных представления.
\begin{itemize}
\EqParm{associative shift}{=left}
\EqParm{associative shift}{=right}
\end{itemize}
}

\AddEq{non associative shift}
{
\item
\SideRuC вый сдвиг
\ShowEq{\SideWS shift}
является представлением
$\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебре $A$.
}

\AddEq{associative shift}
{
\item
\AddIndex{\SideRuC вый сдвиг}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$
\ShowEq{\SideWS shift, product}
}

\DefEq
{
Если мультипликативная $\Omega$\Hyph группа $A_1$ - абелевая,
то нет разницы между левосторонним и правосторонним представлениями.

\begin{definition}
\labelDefinition{representation of Abelian group} 
Пусть $A_1$ - абелевая мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{представлением}{representation of algebra}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{left-side representation of group}{Abelian}
\qed
\end{definition}

Обычно мы отождествляем представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и левостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
Однако, если это необходимо нам,
мы можем отождествить представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и правостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefDefinition{algebra of sets}
{
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, страница 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\,\footnote{
Смотри определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:A->B}fXY
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:A->B}fXA
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:A->B}fXA
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
}

\DefTheorem{measurable simple map}
{
Пусть отображение
\ShowEq{f:A->B}fXA
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\DrawEq{Fn=}{}
$\mu$\Hyph измеримы.\,\footnote{
Смотри аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
}

\DefDefinition{measure}
{
Пусть \(\mathcal C_m\) - полукольцо множеств.\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{f:A->B}f{\mathcal C_m}R
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
}

\DefDefinition{sigma-additive measure}
{
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\,\footnote{
Смотри аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\,\footnote{
Другими словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\,\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{f:A->B}{f_n}XA
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\).
}

\DefDefinition{integrable map}
{
Для простого отображения
\ShowEq{f:A->B}fXA
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Пусть
\ShowEq{f:A->B}fXA
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Пусть
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {B}{0}%
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate representation}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
   {O}{0}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {орбита \Ts{G}представления группы}%
   {orbit of representation of group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate representation}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex

